Measurements of top-quark pair differential cross-sections in the lepton+jets channel in $pp$ collisions at $\sqrt{s}$=13 TeV using the ATLAS detector

Measurements of differential cross-sections of top-quark pair production in fiducial phase-spaces are presented as a function of top-quark and $t\bar{t}$ system kinematic observables in proton-proton collisions at a centre-of-mass energy of $\sqrt{s}$=13 TeV. The data set corresponds to an integrated luminosity of $3.2$ fb${}^{-1}$, recorded in 2015 with the ATLAS detector at the CERN Large Hadron Collider. Events with exactly one electron or muon and at least two jets in the final state are used for the measurement. Two separate selections are applied that each focus on different top-quark momentum regions, referred to as resolved and boosted topologies of the $t\bar{t}$ final state. The measured spectra are corrected for detector effects and are compared to several Monte Carlo simulations by means of calculated $\chi^2$ and $p$-values.

==> tables/EventYield_boosted.tex <==
\begin{tabular}{l|r|r|r} 
\hline 
\hline 
Process & Events & Stat & Syst \\ 
\hline 
$t\bar{t}$ & 6746.51 & 17.1 & 1107.32 \\ 
$W$+jets & 476.66 & 20.67 & 268.53 \\ 
$Z$+jets & 63.39 & 8.81 & 37.7 \\ 
Diboson & 62.61 & 2.17 & 11.53 \\ 
Single top & 447.53 & 3.58 & 82.08 \\ 
$t\bar{t}V$ & 66.65 & 0.2 & 12.17 \\ 
Multijets & 272.81 & 25.6 & 78.78 \\ 
\hline 
Total prediction & 8136.16 & 38.34 & 1308.34 \\ 
\hline 
Data & 7368 & & \\ 
\hline 
Data/Pred & 0.91 & & \\ 
\hline 
\end{tabular}

==> tables/EventYield_boosted_el.tex <==
\begin{tabular}{l|r|r|r} 
\hline 
\hline 
Process & Events & Stat & Syst \\ 
\hline 
$t\bar{t}$ & 3577.91 & 17.95 & 571.91 \\ 
$W$+jets & 254.49 & 13.31 & 181.22 \\ 
$Z$+jets & 25.88 & 4.65 & 17.89 \\ 
Diboson & 32.3 & 1.46 & 5.97 \\ 
Single top & 242.1 & 2.68 & 43.24 \\ 
Multijets & 251.57 & 22.62 & 79.01 \\ 
$t\bar{t}V$ & 37.99 & 0.16 & 7.83 \\ 
\hline 
Total prediction & 4422.24 & 32.28 & 685.87 \\ 
\hline 
Data & 4007 & & \\ 
\hline 
Data/Pred & 0.91 & & \\ 
\hline 
\end{tabular}

==> tables/EventYield_boosted_mu.tex <==
\begin{tabular}{l|r|r|r} 
\hline 
\hline 
Process & Events & Stat & Syst \\ 
\hline 
$t\bar{t}$ & 3168.6 & 16.21 & 538.36 \\ 
$W$+jets & 222.32 & 15.81 & 116.83 \\ 
$Z$+jets & 37.62 & 7.48 & 21.91 \\ 
Diboson & 30.31 & 1.61 & 5.81 \\ 
Single top & 205.43 & 2.37 & 38.8 \\ 
Multijets & 21.24 & 11.97 & 22.47 \\ 
$t\bar{t}V$ & 33.63 & 0.14 & 7.58 \\ 
\hline 
Total prediction & 3719.14 & 26.84 & 633.76 \\ 
\hline 
Data & 3361 & & \\ 
\hline 
Data/Pred & 0.9 & & \\ 
\hline 
\end{tabular}

==> tables/EventYield_combinedBoostedResolved.tex <==
\begin{table}[t]
\centering
 \begin{tabular}{lrr}
\hline\hline 
Process & \multicolumn{2}{c}{\ \ \ Expected events\ \ \ } \\ 
\hline
& \hbox{Resolved} & \hbox{Boosted} \\ 
 \hline
$t\bar{t}$ & 123800  $\pm$ 10600 & 7000 $\pm$ 1100 \\
 Single top & 6300  $\pm$ 800 & 500 $\pm$ 80 \\
Multijets & 5700  $\pm$ 3000 & 300 $\pm$ 80 \\ 
$W$+jets & 3600 ${}^{+2000}_{-2400}$ & $500 \pm 200$ \\
$Z$+jets & 1300  $\pm$    700 & 60 $\pm$ 40 \\ 
$t\bar{t}V$ & 400  $\pm$ 100 & 70 $\pm$ 10 \\ 
Diboson & 300  $\pm$    200 & 60 $\pm$ 10 \\
\hline
\\[-1.1em]
Total prediction & 142000 ${}^{+11000}_{-12000}$  & 8300  $\pm$ 1300 \\[2.3pt]
\hline 
 Data & 155593 & 7368  \\ 
\hline 
\hline
\end{tabular}
\caption{Event yields 
after the resolved and boosted selections. The signal model, denoted $t\bar{t}$ in the table, is generated using \PowHeg{}+\PythiaSix{}, normalised to NNLO calculations.  The uncertainties include the combined statistical and systematic uncertainties, excluding the systematic uncertainties related to the modelling of the \ttbar{} system, as described in Section~\ref{sec:Uncertainties}.
}
\label{tab:yields}
\end{table}



==> tables/Yields_co.tex <==
$t\bar{t}$ & $120543^{+11721.5}_{-11673.6}$\\
$W$+jets & $3339.18^{+1885.11}_{-3580.96}$\\
$Z$+jets & $1335.48^{+704.854}_{-688.943}$\\
Singletop & 6169  $\pm$    794  \\
Diboson & $348.208^{+174.978}_{-174.842}$\\
$t\bar{t}V$ & $428.215^{+68.7149}_{-68.2792}$\\
Multijet & $5694.22^{+2988.45}_{-3042.01}$\\
TotalPrediction & $137857^{+12852.3}_{-14921.6}$\\
\hline
Data & 155593  $\pm$ 394 (stat) \\
\hline 



==> tables/Yields_el.tex <==
$t\bar{t}$ & $62402.3^{+6132.87}_{-6084.75}$\\
$W$+jets & $1784.46^{+1187.64}_{-2237.42}$\\
$Z$+jets & $941.515^{+504.093}_{-492.039}$\\
Singletop &  3200  $\pm$   418  \\
Diboson & $185.848^{+93.61}_{-93.0659}$\\
$t\bar{t}V$ & $227.745^{+36.64}_{-36.4026}$\\
Multijet & $4199.84^{+2256.86}_{-2321.76}$\\
TotalPrediction & $72941.4^{+6941.88}_{-8410.89}$\\
\hline
Data & 81722 $\pm$ 286 (stat) \\
\hline



==> tables/Yields_mu.tex <==
$t\bar{t}$ & $58140.5^{+5630.66}_{-5631.18}$\\
$W$+jets & $1554.72^{+722.617}_{-1541.41}$\\
$Z$+jets & $393.965^{+206.233}_{-202.076}$\\
Singletop  &2970  $\pm$    379  \\
Diboson & $162.36^{+81.5245}_{-81.9947}$\\
$t\bar{t}V$ & $200.47^{+32.1778}_{-31.981}$\\
Multijet & $1494.38^{+774.662}_{-776.789}$\\
TotalPrediction &$ 64916^{+5792.26}_{-6435.52}$\\
\hline
Data & 73871  $\pm$ 272 (stat) \\
\hline 




==> tables/correlations/boosted/absXs_correlation_topH_absrap_boosted.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrr}
bin  &  0.0-0.2  &  0.2-0.4  &  0.4-0.6  &  0.6-0.8  &  0.8-1.0  &  1.0-1.2  &  1.2-1.4  &  1.4-1.6  &  1.6-1.8  &  1.8-2.0   \\ \hline
 0.0-0.2  & \textbf{1.00} & 0.94  & 0.95  & 0.93  & 0.93  & 0.94  & 0.85  & 0.88  & 0.88  & 0.88  \\ 
 0.2-0.4  & 0.94  & \textbf{1.00} & 0.93  & 0.92  & 0.93  & 0.93  & 0.82  & 0.87  & 0.88  & 0.88  \\ 
 0.4-0.6  & 0.95  & 0.93  & \textbf{1.00} & 0.90  & 0.93  & 0.92  & 0.83  & 0.85  & 0.87  & 0.87  \\ 
 0.6-0.8  & 0.93  & 0.92  & 0.90  & \textbf{1.00} & 0.90  & 0.92  & 0.86  & 0.89  & 0.89  & 0.87  \\ 
 0.8-1.0  & 0.93  & 0.93  & 0.93  & 0.90  & \textbf{1.00} & 0.92  & 0.85  & 0.88  & 0.89  & 0.88  \\ 
 1.0-1.2  & 0.94  & 0.93  & 0.92  & 0.92  & 0.92  & \textbf{1.00} & 0.85  & 0.90  & 0.89  & 0.88  \\ 
 1.2-1.4  & 0.85  & 0.82  & 0.83  & 0.86  & 0.85  & 0.85  & \textbf{1.00} & 0.85  & 0.83  & 0.82  \\ 
 1.4-1.6  & 0.88  & 0.87  & 0.85  & 0.89  & 0.88  & 0.90  & 0.85  & \textbf{1.00} & 0.87  & 0.86  \\ 
 1.6-1.8  & 0.88  & 0.88  & 0.87  & 0.89  & 0.89  & 0.89  & 0.83  & 0.87  & \textbf{1.00} & 0.84  \\ 
 1.8-2.0  & 0.88  & 0.88  & 0.87  & 0.87  & 0.88  & 0.88  & 0.82  & 0.86  & 0.84  & \textbf{1.00} \\ 
\end{tabular} 



==> tables/correlations/boosted/absXs_correlation_topH_pt_boosted.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrr}
bin $[{\textrm GeV}]$  &  300-350  &  350-400  &  400-450  &  450-500  &  500-550  &  550-650  &  650-750  &  750-1500   \\ \hline
 300-350  & \textbf{1.00} & 0.91  & 0.85  & 0.81  & 0.69  & 0.66  & 0.62  & 0.55  \\ 
 350-400  & 0.91  & \textbf{1.00} & 0.91  & 0.88  & 0.79  & 0.79  & 0.71  & 0.71  \\ 
 400-450  & 0.85  & 0.91  & \textbf{1.00} & 0.92  & 0.84  & 0.85  & 0.76  & 0.75  \\ 
 450-500  & 0.81  & 0.88  & 0.92  & \textbf{1.00} & 0.89  & 0.85  & 0.78  & 0.78  \\ 
 500-550  & 0.69  & 0.79  & 0.84  & 0.89  & \textbf{1.00} & 0.86  & 0.73  & 0.79  \\ 
 550-650  & 0.66  & 0.79  & 0.85  & 0.85  & 0.86  & \textbf{1.00} & 0.71  & 0.78  \\ 
 650-750  & 0.62  & 0.71  & 0.76  & 0.78  & 0.73  & 0.71  & \textbf{1.00} & 0.63  \\ 
 750-1500  & 0.55  & 0.71  & 0.75  & 0.78  & 0.79  & 0.78  & 0.63  & \textbf{1.00} \\ 
\end{tabular} 



==> tables/correlations/boosted/absXs_covariance_topH_absrap_boosted.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrr}
bin  &  0.0-0.2  &  0.2-0.4  &  0.4-0.6  &  0.6-0.8  &  0.8-1.0  &  1.0-1.2  &  1.2-1.4  &  1.4-1.6  &  1.6-1.8  &  1.8-2.0   \\ \hline
 0.0-0.2  & 1.65e-01  & 1.48e-01  & 1.44e-01  & 1.28e-01  & 1.11e-01  & 1.09e-01  & 8.73e-02  & 6.73e-02  & 4.94e-02  & 3.21e-02  \\ 
 0.2-0.4  & 1.48e-01  & 1.49e-01  & 1.35e-01  & 1.21e-01  & 1.06e-01  & 1.02e-01  & 8.00e-02  & 6.32e-02  & 4.69e-02  & 3.03e-02  \\ 
 0.4-0.6  & 1.44e-01  & 1.35e-01  & 1.40e-01  & 1.14e-01  & 1.02e-01  & 9.83e-02  & 7.87e-02  & 5.96e-02  & 4.47e-02  & 2.91e-02  \\ 
 0.6-0.8  & 1.28e-01  & 1.21e-01  & 1.14e-01  & 1.15e-01  & 9.00e-02  & 8.92e-02  & 7.43e-02  & 5.70e-02  & 4.15e-02  & 2.66e-02  \\ 
 0.8-1.0  & 1.11e-01  & 1.06e-01  & 1.02e-01  & 9.00e-02  & 8.66e-02  & 7.71e-02  & 6.31e-02  & 4.85e-02  & 3.60e-02  & 2.33e-02  \\ 
 1.0-1.2  & 1.09e-01  & 1.02e-01  & 9.83e-02  & 8.92e-02  & 7.71e-02  & 8.16e-02  & 6.15e-02  & 4.81e-02  & 3.48e-02  & 2.26e-02  \\ 
 1.2-1.4  & 8.73e-02  & 8.00e-02  & 7.87e-02  & 7.43e-02  & 6.31e-02  & 6.15e-02  & 6.42e-02  & 4.04e-02  & 2.89e-02  & 1.86e-02  \\ 
 1.4-1.6  & 6.73e-02  & 6.32e-02  & 5.96e-02  & 5.70e-02  & 4.85e-02  & 4.81e-02  & 4.04e-02  & 3.54e-02  & 2.24e-02  & 1.44e-02  \\ 
 1.6-1.8  & 4.94e-02  & 4.69e-02  & 4.47e-02  & 4.15e-02  & 3.60e-02  & 3.48e-02  & 2.89e-02  & 2.24e-02  & 1.89e-02  & 1.03e-02  \\ 
 1.8-2.0  & 3.21e-02  & 3.03e-02  & 2.91e-02  & 2.66e-02  & 2.33e-02  & 2.26e-02  & 1.86e-02  & 1.44e-02  & 1.03e-02  & 8.03e-03  \\ 
\end{tabular} 



==> tables/correlations/boosted/absXs_covariance_topH_pt_boosted.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrr}
Bin $[{\textrm GeV}]$  &  300-350  &  350-400  &  400-450  &  450-500  &  500-550  &  550-650  &  650-750  &  750-1500   \\ \hline
 300-350  & 1.49e-05  & 8.83e-06  & 4.86e-06  & 3.12e-06  & 2.04e-06  & 1.25e-06  & 4.46e-07  & 7.02e-08  \\ 
 350-400  & 8.83e-06  & 6.27e-06  & 3.34e-06  & 2.21e-06  & 1.52e-06  & 9.70e-07  & 3.29e-07  & 5.88e-08  \\ 
 400-450  & 4.86e-06  & 3.34e-06  & 2.18e-06  & 1.36e-06  & 9.56e-07  & 6.15e-07  & 2.08e-07  & 3.65e-08  \\ 
 450-500  & 3.12e-06  & 2.21e-06  & 1.36e-06  & 1.00e-06  & 6.79e-07  & 4.20e-07  & 1.45e-07  & 2.57e-08  \\ 
 500-550  & 2.04e-06  & 1.52e-06  & 9.56e-07  & 6.79e-07  & 5.89e-07  & 3.25e-07  & 1.04e-07  & 1.99e-08  \\ 
 550-650  & 1.25e-06  & 9.70e-07  & 6.15e-07  & 4.20e-07  & 3.25e-07  & 2.42e-07  & 6.42e-08  & 1.27e-08  \\ 
 650-750  & 4.46e-07  & 3.29e-07  & 2.08e-07  & 1.45e-07  & 1.04e-07  & 6.42e-08  & 3.41e-08  & 3.84e-09  \\ 
 750-1500  & 7.02e-08  & 5.88e-08  & 3.65e-08  & 2.57e-08  & 1.99e-08  & 1.27e-08  & 3.84e-09  & 1.08e-09  \\ 
\end{tabular} 



==> tables/correlations/boosted/relXs_correlation_topH_absrap_boosted.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrr}
bin  &  0.0-0.2  &  0.2-0.4  &  0.4-0.6  &  0.6-0.8  &  0.8-1.0  &  1.0-1.2  &  1.2-1.4  &  1.4-1.6  &  1.6-1.8  &  1.8-2.0   \\ \hline
 0.0-0.2  & \textbf{1.00} & 0.09  & 0.32  & 0.02  & 0.09  & 0.08  & 0.07  & 0.02  & -0.11  & 0.12  \\ 
 0.2-0.4  & 0.09  & \textbf{1.00} & 0.11  & -0.00  & -0.04  & -0.01  & -0.01  & -0.05  & -0.23  & -0.05  \\ 
 0.4-0.6  & 0.32  & 0.11  & \textbf{1.00} & 0.06  & 0.29  & 0.11  & 0.40  & 0.25  & 0.03  & 0.24  \\ 
 0.6-0.8  & 0.02  & -0.00  & 0.06  & \textbf{1.00} & 0.05  & -0.05  & 0.20  & 0.07  & 0.07  & 0.16  \\ 
 0.8-1.0  & 0.09  & -0.04  & 0.29  & 0.05  & \textbf{1.00} & -0.01  & 0.39  & 0.19  & 0.15  & 0.28  \\ 
 1.0-1.2  & 0.08  & -0.01  & 0.11  & -0.05  & -0.01  & \textbf{1.00} & 0.07  & 0.12  & -0.06  & 0.16  \\ 
 1.2-1.4  & 0.07  & -0.01  & 0.40  & 0.20  & 0.39  & 0.07  & \textbf{1.00} & 0.38  & 0.27  & 0.32  \\ 
 1.4-1.6  & 0.02  & -0.05  & 0.25  & 0.07  & 0.19  & 0.12  & 0.38  & \textbf{1.00} & 0.12  & 0.21  \\ 
 1.6-1.8  & -0.11  & -0.23  & 0.03  & 0.07  & 0.15  & -0.06  & 0.27  & 0.12  & \textbf{1.00} & 0.11  \\ 
 1.8-2.0  & 0.12  & -0.05  & 0.24  & 0.16  & 0.28  & 0.16  & 0.32  & 0.21  & 0.11  & \textbf{1.00} \\ 
\end{tabular} 



==> tables/correlations/boosted/relXs_correlation_topH_pt_boosted.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrr}
Bin \GeV{}  &  300--350  &  350--400  &  400--450  &  450--500  &  500--550  &  550--650  &  650--750  &  750--1500   \\ \hline
 300--350  & \textbf{1.00} & 0.36  & $-$0.42  & $-$0.57  & $-$0.46  & $-$0.47  & $-$0.53  & $-$0.52  \\ 
 350--400  & 0.36  & \textbf{1.00} & $-$0.01  & $-$0.22  & $-$0.03  & 0.04  & $-$0.23  & $-$0.11  \\ 
 400--450  & $-$0.42  & $-$0.01  & \textbf{1.00} & 0.34  & 0.30  & 0.50  & 0.27  & 0.37  \\ 
 450--500  & $-$0.57  & $-$0.22  & 0.34  & \textbf{1.00} & 0.51  & 0.45  & 0.48  & 0.49  \\ 
 500--550  & $-$0.46  & $-$0.03  & 0.30  & 0.51  & \textbf{1.00} & 0.59  & 0.44  & 0.51  \\ 
 550--650  & $-$0.47  & 0.04  & 0.50  & 0.45  & 0.59  & \textbf{1.00} & 0.43  & 0.54  \\ 
 650--750  & $-$0.53  & $-$0.23  & 0.27  & 0.48  & 0.44  & 0.43  & \textbf{1.00} & 0.44  \\ 
 750--1500  & $-$0.52  & $-$0.11  & 0.37  & 0.49  & 0.51  & 0.54  & 0.44  & \textbf{1.00} \\ 
\end{tabular} 



==> tables/correlations/boosted/relXs_covariance_topH_absrap_boosted.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrr}
bin  &  0.0-0.2  &  0.2-0.4  &  0.4-0.6  &  0.6-0.8  &  0.8-1.0  &  1.0-1.2  &  1.2-1.4  &  1.4-1.6  &  1.6-1.8  &  1.8-2.0   \\ \hline
 0.0-0.2  & 1.71e-03  & 1.60e-04  & 6.31e-04  & 3.77e-05  & 1.46e-04  & 1.06e-04  & 1.24e-04  & 2.52e-05  & -1.17e-04  & 8.75e-05  \\ 
 0.2-0.4  & 1.60e-04  & 1.82e-03  & 2.26e-04  & -7.75e-06  & -7.06e-05  & -2.11e-05  & -1.32e-05  & -6.38e-05  & -2.47e-04  & -3.52e-05  \\ 
 0.4-0.6  & 6.31e-04  & 2.26e-04  & 2.32e-03  & 1.08e-04  & 5.74e-04  & 1.72e-04  & 8.59e-04  & 3.71e-04  & 4.06e-05  & 2.02e-04  \\ 
 0.6-0.8  & 3.77e-05  & -7.75e-06  & 1.08e-04  & 1.40e-03  & 7.38e-05  & -6.42e-05  & 3.30e-04  & 8.43e-05  & 6.23e-05  & 1.01e-04  \\ 
 0.8-1.0  & 1.46e-04  & -7.06e-05  & 5.74e-04  & 7.38e-05  & 1.73e-03  & -1.40e-05  & 7.26e-04  & 2.41e-04  & 1.54e-04  & 2.02e-04  \\ 
 1.0-1.2  & 1.06e-04  & -2.11e-05  & 1.72e-04  & -6.42e-05  & -1.40e-05  & 1.09e-03  & 9.89e-05  & 1.22e-04  & -4.75e-05  & 9.35e-05  \\ 
 1.2-1.4  & 1.24e-04  & -1.32e-05  & 8.59e-04  & 3.30e-04  & 7.26e-04  & 9.89e-05  & 2.03e-03  & 5.30e-04  & 2.96e-04  & 2.52e-04  \\ 
 1.4-1.6  & 2.52e-05  & -6.38e-05  & 3.71e-04  & 8.43e-05  & 2.41e-04  & 1.22e-04  & 5.30e-04  & 9.45e-04  & 9.27e-05  & 1.10e-04  \\ 
 1.6-1.8  & -1.17e-04  & -2.47e-04  & 4.06e-05  & 6.23e-05  & 1.54e-04  & -4.75e-05  & 2.96e-04  & 9.27e-05  & 6.05e-04  & 4.88e-05  \\ 
 1.8-2.0  & 8.75e-05  & -3.52e-05  & 2.02e-04  & 1.01e-04  & 2.02e-04  & 9.35e-05  & 2.52e-04  & 1.10e-04  & 4.88e-05  & 3.00e-04  \\ 
\end{tabular} 



==> tables/correlations/boosted/relXs_covariance_topH_pt_boosted.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrr}
Bin $[{\textrm GeV}]$  &  300-350  &  350-400  &  400-450  &  450-500  &  500-550  &  550-650  &  650-750  &  750-1500   \\ \hline
 300-350  & 3.59e-07  & 6.24e-08  & -4.84e-08  & -5.53e-08  & -4.82e-08  & -3.43e-08  & -1.79e-08  & -3.44e-09  \\ 
 350-400  & 6.24e-08  & 8.14e-08  & -7.38e-10  & -1.03e-08  & -1.62e-09  & 1.28e-09  & -3.70e-09  & -3.52e-10  \\ 
 400-450  & -4.84e-08  & -7.38e-10  & 3.70e-08  & 1.07e-08  & 1.01e-08  & 1.15e-08  & 2.98e-09  & 7.79e-10  \\ 
 450-500  & -5.53e-08  & -1.03e-08  & 1.07e-08  & 2.61e-08  & 1.44e-08  & 8.77e-09  & 4.37e-09  & 8.65e-10  \\ 
 500-550  & -4.82e-08  & -1.62e-09  & 1.01e-08  & 1.44e-08  & 3.10e-08  & 1.24e-08  & 4.36e-09  & 9.80e-10  \\ 
 550-650  & -3.43e-08  & 1.28e-09  & 1.15e-08  & 8.77e-09  & 1.24e-08  & 1.45e-08  & 2.93e-09  & 7.11e-10  \\ 
 650-750  & -1.79e-08  & -3.70e-09  & 2.98e-09  & 4.37e-09  & 4.36e-09  & 2.93e-09  & 3.20e-09  & 2.72e-10  \\ 
 750-1500  & -3.44e-09  & -3.52e-10  & 7.79e-10  & 8.65e-10  & 9.80e-10  & 7.11e-10  & 2.72e-10  & 1.19e-10  \\ 
\end{tabular} 



==> tables/correlations/boosted/topH_absrap.covariance_mc.AbsoluteDiffXsAbsoluteDiffXscorrSumModel.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrr}
bin  &  0.0-0.2  &  0.2-0.4  &  0.4-0.6  &  0.6-0.8  &  0.8-1.0  &  1.0-1.2  &  1.2-1.4  &  1.4-1.6  &  1.6-1.8  &  1.8-2.0   \\ \hline
 0.0-0.2  & \textbf{1.00} & 0.91  & 0.88  & 1.00  & 0.88  & 0.95  & 0.62  & 0.97  & 0.83  & 0.91  \\ 
 0.2-0.4  & 0.91  & \textbf{1.00} & 0.97  & 0.92  & 0.99  & 0.98  & 0.75  & 0.95  & 0.85  & 0.81  \\ 
 0.4-0.6  & 0.88  & 0.97  & \textbf{1.00} & 0.89  & 1.00  & 0.99  & 0.87  & 0.96  & 0.93  & 0.87  \\ 
 0.6-0.8  & 1.00  & 0.92  & 0.89  & \textbf{1.00} & 0.89  & 0.95  & 0.62  & 0.97  & 0.83  & 0.90  \\ 
 0.8-1.0  & 0.88  & 0.99  & 1.00  & 0.89  & \textbf{1.00} & 0.99  & 0.84  & 0.95  & 0.90  & 0.85  \\ 
 1.0-1.2  & 0.95  & 0.98  & 0.99  & 0.95  & 0.99  & \textbf{1.00} & 0.80  & 0.99  & 0.92  & 0.90  \\ 
 1.2-1.4  & 0.62  & 0.75  & 0.87  & 0.62  & 0.84  & 0.80  & \textbf{1.00} & 0.78  & 0.94  & 0.81  \\ 
 1.4-1.6  & 0.97  & 0.95  & 0.96  & 0.97  & 0.95  & 0.99  & 0.78  & \textbf{1.00} & 0.93  & 0.94  \\ 
 1.6-1.8  & 0.83  & 0.85  & 0.93  & 0.83  & 0.90  & 0.92  & 0.94  & 0.93  & \textbf{1.00} & 0.96  \\ 
 1.8-2.0  & 0.91  & 0.81  & 0.87  & 0.90  & 0.85  & 0.90  & 0.81  & 0.94  & 0.96  & \textbf{1.00} \\ 
\end{tabular} 



==> tables/correlations/boosted/topH_absrap.covariance_mc.AbsoluteDiffXsAbsoluteDiffXscovSumModel.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrr}
bin  &  0.0-0.2  &  0.2-0.4  &  0.4-0.6  &  0.6-0.8  &  0.8-1.0  &  1.0-1.2  &  1.2-1.4  &  1.4-1.6  &  1.6-1.8  &  1.8-2.0   \\ \hline
 0.0-0.2  & 2.60e-02  & 3.41e-02  & 2.73e-02  & 3.00e-02  & 1.87e-02  & 2.24e-02  & 1.12e-02  & 1.18e-02  & 4.89e-03  & 5.99e-03  \\ 
 0.2-0.4  & 3.41e-02  & 5.36e-02  & 4.32e-02  & 3.98e-02  & 3.01e-02  & 3.35e-02  & 1.93e-02  & 1.65e-02  & 7.16e-03  & 7.69e-03  \\ 
 0.4-0.6  & 2.73e-02  & 4.32e-02  & 3.67e-02  & 3.18e-02  & 2.52e-02  & 2.78e-02  & 1.88e-02  & 1.39e-02  & 6.54e-03  & 6.84e-03  \\ 
 0.6-0.8  & 3.00e-02  & 3.98e-02  & 3.18e-02  & 3.47e-02  & 2.19e-02  & 2.61e-02  & 1.30e-02  & 1.36e-02  & 5.65e-03  & 6.87e-03  \\ 
 0.8-1.0  & 1.87e-02  & 3.01e-02  & 2.52e-02  & 2.19e-02  & 1.74e-02  & 1.91e-02  & 1.24e-02  & 9.45e-03  & 4.36e-03  & 4.55e-03  \\ 
 1.0-1.2  & 2.24e-02  & 3.35e-02  & 2.78e-02  & 2.61e-02  & 1.91e-02  & 2.16e-02  & 1.32e-02  & 1.09e-02  & 4.93e-03  & 5.43e-03  \\ 
 1.2-1.4  & 1.12e-02  & 1.93e-02  & 1.88e-02  & 1.30e-02  & 1.24e-02  & 1.32e-02  & 1.26e-02  & 6.61e-03  & 3.85e-03  & 3.69e-03  \\ 
 1.4-1.6  & 1.18e-02  & 1.65e-02  & 1.39e-02  & 1.36e-02  & 9.45e-03  & 1.09e-02  & 6.61e-03  & 5.67e-03  & 2.56e-03  & 2.89e-03  \\ 
 1.6-1.8  & 4.89e-03  & 7.16e-03  & 6.54e-03  & 5.65e-03  & 4.36e-03  & 4.93e-03  & 3.85e-03  & 2.56e-03  & 1.34e-03  & 1.43e-03  \\ 
 1.8-2.0  & 5.99e-03  & 7.69e-03  & 6.84e-03  & 6.87e-03  & 4.55e-03  & 5.43e-03  & 3.69e-03  & 2.89e-03  & 1.43e-03  & 1.67e-03  \\ 
\end{tabular} 



==> tables/correlations/boosted/topH_absrap.covariance_mc.RelativeDiffXsRelativeDiffXscorrSumModel.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrr}
bin  &  0.0-0.2  &  0.2-0.4  &  0.4-0.6  &  0.6-0.8  &  0.8-1.0  &  1.0-1.2  &  1.2-1.4  &  1.4-1.6  &  1.6-1.8  &  1.8-2.0   \\ \hline
 0.0-0.2  & \textbf{1.00} & 0.85  & 0.98  & 0.95  & 0.84  & 0.97  & 0.98  & 0.97  & 0.62  & 0.81  \\ 
 0.2-0.4  & 0.85  & \textbf{1.00} & 0.72  & 0.96  & 0.62  & 0.86  & 0.92  & 0.79  & 0.93  & 0.65  \\ 
 0.4-0.6  & 0.98  & 0.72  & \textbf{1.00} & 0.86  & 0.88  & 0.93  & 0.93  & 0.97  & 0.44  & 0.78  \\ 
 0.6-0.8  & 0.95  & 0.96  & 0.86  & \textbf{1.00} & 0.67  & 0.97  & 0.96  & 0.87  & 0.81  & 0.83  \\ 
 0.8-1.0  & 0.84  & 0.62  & 0.88  & 0.67  & \textbf{1.00} & 0.69  & 0.85  & 0.93  & 0.36  & 0.40  \\ 
 1.0-1.2  & 0.97  & 0.86  & 0.93  & 0.97  & 0.69  & \textbf{1.00} & 0.93  & 0.89  & 0.65  & 0.91  \\ 
 1.2-1.4  & 0.98  & 0.92  & 0.93  & 0.96  & 0.85  & 0.93  & \textbf{1.00} & 0.96  & 0.73  & 0.71  \\ 
 1.4-1.6  & 0.97  & 0.79  & 0.97  & 0.87  & 0.93  & 0.89  & 0.96  & \textbf{1.00} & 0.53  & 0.68  \\ 
 1.6-1.8  & 0.62  & 0.93  & 0.44  & 0.81  & 0.36  & 0.65  & 0.73  & 0.53  & \textbf{1.00} & 0.47  \\ 
 1.8-2.0  & 0.81  & 0.65  & 0.78  & 0.83  & 0.40  & 0.91  & 0.71  & 0.68  & 0.47  & \textbf{1.00} \\ 
\end{tabular} 



==> tables/correlations/boosted/topH_absrap.covariance_mc.RelativeDiffXsRelativeDiffXscovSumModel.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrr}
bin  &  0.0-0.2  &  0.2-0.4  &  0.4-0.6  &  0.6-0.8  &  0.8-1.0  &  1.0-1.2  &  1.2-1.4  &  1.4-1.6  &  1.6-1.8  &  1.8-2.0   \\ \hline
 0.0-0.2  & 5.22e-04  & 5.24e-04  & 6.40e-04  & 3.98e-04  & 6.50e-04  & 3.70e-04  & 7.57e-04  & 3.69e-04  & 1.53e-04  & 1.43e-04  \\ 
 0.2-0.4  & 5.24e-04  & 7.23e-04  & 5.56e-04  & 4.71e-04  & 5.64e-04  & 3.84e-04  & 8.35e-04  & 3.54e-04  & 2.71e-04  & 1.36e-04  \\ 
 0.4-0.6  & 6.40e-04  & 5.56e-04  & 8.23e-04  & 4.53e-04  & 8.56e-04  & 4.43e-04  & 9.00e-04  & 4.64e-04  & 1.36e-04  & 1.74e-04  \\ 
 0.6-0.8  & 3.98e-04  & 4.71e-04  & 4.53e-04  & 3.35e-04  & 4.18e-04  & 2.96e-04  & 5.93e-04  & 2.67e-04  & 1.59e-04  & 1.17e-04  \\ 
 0.8-1.0  & 6.50e-04  & 5.64e-04  & 8.56e-04  & 4.18e-04  & 1.15e-03  & 3.89e-04  & 9.80e-04  & 5.30e-04  & 1.33e-04  & 1.06e-04  \\ 
 1.0-1.2  & 3.70e-04  & 3.84e-04  & 4.43e-04  & 2.96e-04  & 3.89e-04  & 2.78e-04  & 5.26e-04  & 2.49e-04  & 1.16e-04  & 1.17e-04  \\ 
 1.2-1.4  & 7.57e-04  & 8.35e-04  & 9.00e-04  & 5.93e-04  & 9.80e-04  & 5.26e-04  & 1.14e-03  & 5.43e-04  & 2.66e-04  & 1.86e-04  \\ 
 1.4-1.6  & 3.69e-04  & 3.54e-04  & 4.64e-04  & 2.67e-04  & 5.30e-04  & 2.49e-04  & 5.43e-04  & 2.79e-04  & 9.58e-05  & 8.75e-05  \\ 
 1.6-1.8  & 1.53e-04  & 2.71e-04  & 1.36e-04  & 1.59e-04  & 1.33e-04  & 1.16e-04  & 2.66e-04  & 9.58e-05  & 1.16e-04  & 3.89e-05  \\ 
 1.8-2.0  & 1.43e-04  & 1.36e-04  & 1.74e-04  & 1.17e-04  & 1.06e-04  & 1.17e-04  & 1.86e-04  & 8.75e-05  & 3.89e-05  & 5.98e-05  \\ 
\end{tabular} 



==> tables/correlations/boosted/topH_pt.covariance_mc.AbsoluteDiffXsAbsoluteDiffXscorrSumModel.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrr}
bin $[{\textrm GeV}]$  &  300-350  &  350-400  &  400-450  &  450-500  &  500-550  &  550-650  &  650-750  &  750-1500   \\ \hline
 300-350  & \textbf{1.00} & 0.92  & 0.87  & 0.96  & 1.00  & 0.86  & 0.70  & 0.53  \\ 
 350-400  & 0.92  & \textbf{1.00} & 0.80  & 0.94  & 0.90  & 0.98  & 0.65  & 0.80  \\ 
 400-450  & 0.87  & 0.80  & \textbf{1.00} & 0.95  & 0.84  & 0.84  & 0.93  & 0.59  \\ 
 450-500  & 0.96  & 0.94  & 0.95  & \textbf{1.00} & 0.94  & 0.95  & 0.83  & 0.69  \\ 
 500-550  & 1.00  & 0.90  & 0.84  & 0.94  & \textbf{1.00} & 0.83  & 0.66  & 0.48  \\ 
 550-650  & 0.86  & 0.98  & 0.84  & 0.95  & 0.83  & \textbf{1.00} & 0.73  & 0.88  \\ 
 650-750  & 0.70  & 0.65  & 0.93  & 0.83  & 0.66  & 0.73  & \textbf{1.00} & 0.56  \\ 
 750-1500  & 0.53  & 0.80  & 0.59  & 0.69  & 0.48  & 0.88  & 0.56  & \textbf{1.00} \\ 
\end{tabular} 



==> tables/correlations/boosted/topH_pt.covariance_mc.AbsoluteDiffXsAbsoluteDiffXscovSumModel.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrr}
bin $[{\textrm GeV}]$  &  300-350  &  350-400  &  400-450  &  450-500  &  500-550  &  550-650  &  650-750  &  750-1500   \\ \hline
 300-350  & 4.63e-06  & 2.71e-06  & 6.24e-07  & 7.15e-07  & 5.88e-07  & 3.32e-07  & 3.24e-08  & 1.03e-08  \\ 
 350-400  & 2.71e-06  & 1.88e-06  & 3.63e-07  & 4.47e-07  & 3.39e-07  & 2.39e-07  & 1.92e-08  & 9.96e-09  \\ 
 400-450  & 6.24e-07  & 3.63e-07  & 1.11e-07  & 1.09e-07  & 7.64e-08  & 5.03e-08  & 6.67e-09  & 1.78e-09  \\ 
 450-500  & 7.15e-07  & 4.47e-07  & 1.09e-07  & 1.20e-07  & 8.89e-08  & 5.85e-08  & 6.15e-09  & 2.17e-09  \\ 
 500-550  & 5.88e-07  & 3.39e-07  & 7.64e-08  & 8.89e-08  & 7.51e-08  & 4.08e-08  & 3.90e-09  & 1.20e-09  \\ 
 550-650  & 3.32e-07  & 2.39e-07  & 5.03e-08  & 5.85e-08  & 4.08e-08  & 3.20e-08  & 2.82e-09  & 1.43e-09  \\ 
 650-750  & 3.24e-08  & 1.92e-08  & 6.67e-09  & 6.15e-09  & 3.90e-09  & 2.82e-09  & 4.61e-10  & 1.09e-10  \\ 
 750-1500  & 1.03e-08  & 9.96e-09  & 1.78e-09  & 2.17e-09  & 1.20e-09  & 1.43e-09  & 1.09e-10  & 8.20e-11  \\ 
\end{tabular} 



==> tables/correlations/boosted/topH_pt.covariance_mc.RelativeDiffXsRelativeDiffXscorrSumModel.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrr}
bin $[{\textrm GeV}]$  &  300-350  &  350-400  &  400-450  &  450-500  &  500-550  &  550-650  &  650-750  &  750-1500   \\ \hline
 300-350  & \textbf{1.00} & 0.76  & 0.98  & 0.67  & 0.81  & 0.52  & 0.97  & 0.52  \\ 
 350-400  & 0.76  & \textbf{1.00} & 0.60  & 0.56  & 0.90  & 0.94  & 0.74  & 0.95  \\ 
 400-450  & 0.98  & 0.60  & \textbf{1.00} & 0.63  & 0.69  & 0.33  & 0.94  & 0.32  \\ 
 450-500  & 0.67  & 0.56  & 0.63  & \textbf{1.00} & 0.86  & 0.57  & 0.80  & 0.38  \\ 
 500-550  & 0.81  & 0.90  & 0.69  & 0.86  & \textbf{1.00} & 0.87  & 0.86  & 0.78  \\ 
 550-650  & 0.52  & 0.94  & 0.33  & 0.57  & 0.87  & \textbf{1.00} & 0.55  & 0.97  \\ 
 650-750  & 0.97  & 0.74  & 0.94  & 0.80  & 0.86  & 0.55  & \textbf{1.00} & 0.51  \\ 
 750-1500  & 0.52  & 0.95  & 0.32  & 0.38  & 0.78  & 0.97  & 0.51  & \textbf{1.00} \\ 
\end{tabular} 


==> tables/correlations/boosted/topH_pt.covariance_mc.RelativeDiffXsRelativeDiffXscovSumModel.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrr}
bin $[{\textrm GeV}]$  &  300-350  &  350-400  &  400-450  &  450-500  &  500-550  &  550-650  &  650-750  &  750-1500   \\ \hline
 300-350  & 3.79e-08  & 2.53e-08  & 2.99e-08  & 5.56e-09  & 4.18e-09  & 5.59e-09  & 2.46e-09  & 2.70e-10  \\ 
 350-400  & 2.53e-08  & 2.95e-08  & 1.61e-08  & 4.08e-09  & 4.11e-09  & 8.82e-09  & 1.66e-09  & 4.37e-10  \\ 
 400-450  & 2.99e-08  & 1.61e-08  & 2.47e-08  & 4.19e-09  & 2.87e-09  & 2.81e-09  & 1.93e-09  & 1.35e-10  \\ 
 450-500  & 5.56e-09  & 4.08e-09  & 4.19e-09  & 1.80e-09  & 9.71e-10  & 1.32e-09  & 4.44e-10  & 4.35e-11  \\ 
 500-550  & 4.18e-09  & 4.11e-09  & 2.87e-09  & 9.71e-10  & 7.04e-10  & 1.26e-09  & 3.00e-10  & 5.54e-11  \\ 
 550-650  & 5.59e-09  & 8.82e-09  & 2.81e-09  & 1.32e-09  & 1.26e-09  & 3.01e-09  & 3.97e-10  & 1.42e-10  \\ 
 650-750  & 2.46e-09  & 1.66e-09  & 1.93e-09  & 4.44e-10  & 3.00e-10  & 3.97e-10  & 1.71e-10  & 1.78e-11  \\ 
 750-1500  & 2.70e-10  & 4.37e-10  & 1.35e-10  & 4.35e-11  & 5.54e-11  & 1.42e-10  & 1.78e-11  & 7.19e-12  \\ 
\end{tabular} 



==> tables/correlations/correlations.tex <==

\begin{landscape}
\begin{table}
\input{tables/correlations/resolved/absXs_correlation_topH_pt_co.res_13TeV} 
\caption{Correlation matrix of the absolute cross-section as function of the top quark \pt{}, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cor_topH_pt_abs_resol}
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}
\input{tables/correlations/resolved/relXs_correlation_topH_pt_co.res_13TeV} 
\caption{Correlation matrix of the relative cross-section as function of the top quark \pt{}, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cor_topH_pt_rel_resol}
\end{table}
\end{landscape}


\begin{table}[!hp]
\input{tables/correlations/boosted/absXs_correlation_topH_pt_boosted}
\caption{Correlation matrix for the absolute cross-section as function of the hadronic top-quark top quark \pt{}, accounting for the statistic and systematic uncertainties in the boosted topology.}
\label{tab:cor_topH_pt_abs_boosted}
\end{table}


\begin{table}[!hp]
\input{tables/correlations/boosted/relXs_correlation_topH_pt_boosted}
\caption{Correlation matrix for the relative cross-section as function of the hadronic top-quark top quark \pt{}, accounting for the statistic and systematic uncertainties in the boosted topology.}
\label{tab:cor_topH_pt_rel_boosted}
\end{table}


\begin{landscape}
\begin{table}
\input{tables/correlations/resolved/absXs_correlation_topH_absrap_co.res_13TeV} 
\caption{Correlation matrix of the absolute cross-section as function of the absolute value of the rapidity of the top quark, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cor_topH_pt_abs_resol}
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}
\input{tables/correlations/resolved/relXs_correlation_topH_absrap_co.res_13TeV} 
\caption{Correlation matrix of the relative cross-section as function of the absolute value of the rapidity of the top quark, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cor_topH_pt_rel_resol}
\end{table}
\end{landscape}


\begin{table}[!hp]
\input{tables/correlations/boosted/absXs_correlation_topH_absrap_boosted}
\caption{Correlation matrix for the absolute cross-section as function of the hadronic top-quark top quark \pt{}, accounting for the statistic and systematic uncertainties in the boosted topology.}
\label{tab:cor_topH_pt_abs_boosted}
\end{table}


\begin{table}[!hp]
\input{tables/correlations/boosted/relXs_correlation_topH_absrap_boosted}
\caption{Correlation matrix for the relative cross-section as function of the hadronic top-quark top quark \pt{}, accounting for the statistic and systematic uncertainties in the boosted topology.}
\label{tab:cor_topH_pt_rel_boosted}
\end{table}

\begin{landscape}
\begin{table}
\input{tables/correlations/resolved/absXs_correlation_tt_m_co.res_13TeV} 
\caption{Correlation matrix of the absolute cross-section as function of the mass of the $\ttbar$ system, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cor_tt_m_abs_resol}
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}
\input{tables/correlations/resolved/relXs_correlation_tt_m_co.res_13TeV} 
\caption{Correlation matrix of the relative cross-section as function of the mass of the $\ttbar$ system, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cor_tt_m_rel_resol}
\end{table}
\end{landscape}


\begin{landscape}
\begin{table}
\input{tables/correlations/resolved/absXs_correlation_tt_pt_co.res_13TeV} 
\caption{Correlation matrix of the absolute cross-section as function of the $\ttbar$ system \pt{}, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cor_tt_pt_abs_resol}
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}
\input{tables/correlations/resolved/relXs_correlation_tt_pt_co.res_13TeV} 
\caption{Correlation matrix of the relative cross-section as function of the $\ttbar$ system \pt{}, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cor_tt_pt_rel_resol}
\end{table}
\end{landscape}


\begin{landscape}
\begin{table}
\input{tables/correlations/resolved/absXs_correlation_tt_absrap_co.res_13TeV} 
\caption{Correlation matrix of the absolute cross-section as function of the absolute value of the rapidity of the $\ttbar$ system, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cor_tt_absrap_abs_resol}
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}
\input{tables/correlations/resolved/relXs_correlation_tt_absrap_co.res_13TeV} 
\caption{Correlation matrix of the relative cross-section as function of the absolute value of the rapidity of the $\ttbar$ system, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cor_tt_absrap_rel_resol}
\end{table}
\end{landscape}



==> tables/correlations/correlations_pTt.tex <==

\clearpage

\begin{table}[!p]
\input{tables/correlations/resolved/relXs_correlation_topH_pt_co.res_13TeV} 
\caption{Correlation matrix of the relative cross-section as a function of the hadronic top-quark \pt{}, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cor_topH_pt_rel_resol}
\end{table}
\begin{table}[!p]
\input{tables/correlations/boosted/relXs_correlation_topH_pt_boosted}
\caption{Correlation matrix for the relative cross-section as a function of the hadronic top-quark \pt{}, accounting for the statistical and systematic uncertainties in the boosted topology.}
\label{tab:cor_topH_pt_rel_boosted}
\end{table}



==> tables/correlations/covariances.tex <==
\begin{landscape}
\begin{table}
\resizebox{1.35\textwidth}{!}{
\input{tables/correlations/resolved/absXs_covariance_topH_pt_co.res_13TeV} 
}
\caption{Covariance matrix of the absolute cross-section as function of the top quark \pt{}, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cov_topH_pt_abs_resol}
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}
\resizebox{1.35\textwidth}{!}{
\input{tables/correlations/resolved/relXs_covariance_topH_pt_co.res_13TeV} 
}
\caption{Covariance matrix of the relative cross-section as function of the top quark \pt{}, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cov_topH_pt_rel_resol}
\end{table}
\end{landscape}


\begin{table}[!hp]
\input{tables/correlations/boosted/absXs_covariance_topH_pt_boosted}
\caption{Covariance matrix for the absolute cross-section as function of the hadronic top-quark top quark \pt{}, accounting for the statistic and systematic uncertainties in the boosted topology.}
\label{tab:cov_topH_pt_abs_boosted}
\end{table}


\begin{table}[!hp]
\input{tables/correlations/boosted/relXs_covariance_topH_pt_boosted}
\caption{Covariance matrix for the relative cross-section as function of the hadronic top-quark top quark \pt{}, accounting for the statistic and systematic uncertainties in the boosted topology.}
\label{tab:cov_topH_pt_rel_boosted}
\end{table}

\begin{landscape}
\begin{table}
\resizebox{1.35\textwidth}{!}{
\input{tables/correlations/resolved/absXs_covariance_topH_absrap_co.res_13TeV}
 }
\caption{Covariance matrix of the absolute cross-section as function of the absolute value of the rapidity of the top quark, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cov_topH_pt_abs_resol}
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}
\resizebox{1.35\textwidth}{!}{
\input{tables/correlations/resolved/relXs_covariance_topH_absrap_co.res_13TeV}
 }
\caption{Covariance matrix of the relative cross-section as function of the absolute value of the rapidity of the top quark, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cov_topH_pt_rel_resol}
\end{table}
\end{landscape}


\begin{table}[!hp]
\input{tables/correlations/boosted/absXs_covariance_topH_absrap_boosted}
\caption{Covariance matrix for the absolute cross-section as function of the absolute value of the rapidity of the top quark, accounting for the statistic and systematic uncertainties in the boosted topology.}
\label{tab:cov_topH_pt_abs_boosted}
\end{table}


\begin{table}[!hp]
\input{tables/correlations/boosted/relXs_covariance_topH_absrap_boosted}
\caption{Covariance matrix for the relative cross-section as function of the absolute value of the rapidity of the top quark, accounting for the statistic and systematic uncertainties in the boosted topology.}
\label{tab:cov_topH_pt_rel_boosted}
\end{table}

\begin{landscape}
\begin{table}
\resizebox{1.35\textwidth}{!}{
\input{tables/correlations/resolved/absXs_covariance_tt_m_co.res_13TeV} 
}
\caption{Covariance matrix of the absolute cross-section as function of the mass of the $\ttbar$ system, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cov_tt_m_abs_resol}
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}
\resizebox{1.35\textwidth}{!}{
\input{tables/correlations/resolved/relXs_covariance_tt_m_co.res_13TeV} 
}
\caption{Covariance matrix of the relative cross-section as function of the mass of the $\ttbar$ system, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cov_tt_m_rel_resol}
\end{table}
\end{landscape}

\begin{table}
\input{tables/correlations/resolved/absXs_covariance_tt_pt_co.res_13TeV} 
\caption{Covariance matrix of the absolute cross-section as function of the $\ttbar$ system \pt{}, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cov_tt_pt_abs_resol}
\end{table}

\begin{table}
\input{tables/correlations/resolved/relXs_covariance_tt_pt_co.res_13TeV} 
\caption{Covariance matrix of the relative cross-section as function of the $\ttbar$ system \pt{}, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cov_tt_pt_rel_resol}
\end{table}

\begin{landscape}
\begin{table}
\resizebox{1.35\textwidth}{!}{
\input{tables/correlations/resolved/absXs_covariance_tt_absrap_co.res_13TeV} 
}
\caption{Covariance matrix of the absolute cross-section as function of the absolute value of the rapidity of the $\ttbar$ system, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cov_tt_absrap_abs_resol}
\end{table}
\end{landscape}

\begin{landscape}
\begin{table}
\resizebox{1.35\textwidth}{!}{
\input{tables/correlations/resolved/relXs_covariance_tt_absrap_co.res_13TeV} 
}
\caption{Covariance matrix of the relative cross-section as function of the absolute value of the rapidity of the $\ttbar$ system, accounting for the statistical and systematic uncertainties in the resolved topology.}
\label{tab:cov_tt_absrap_rel_resol}
\end{table}
\end{landscape}


==> tables/correlations/resolved/absXs_correlation_topH_absrap_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrrrrrrrrrr}
bin  &  0.0-0.1  &  0.1-0.2  &  0.2-0.3  &  0.3-0.4  &  0.4-0.5  &  0.5-0.6  &  0.6-0.7  &  0.7-0.8  &  0.8-0.9  &  0.9-1.0  &  1.0-1.1  &  1.1-1.2  &  1.2-1.3  &  1.3-1.4  &  1.4-1.5  &  1.5-1.7  &  1.7-1.9  &  1.9-2.5   \\ \hline
 0.0-0.1  & \textbf{1.00} & 0.97  & 0.97  & 0.96  & 0.95  & 0.98  & 0.97  & 0.97  & 0.96  & 0.96  & 0.95  & 0.96  & 0.95  & 0.93  & 0.94  & 0.95  & 0.92  & 0.86  \\ 
 0.1-0.2  & 0.97  & \textbf{1.00} & 0.98  & 0.96  & 0.95  & 0.97  & 0.97  & 0.97  & 0.96  & 0.97  & 0.95  & 0.96  & 0.95  & 0.94  & 0.94  & 0.95  & 0.93  & 0.87  \\ 
 0.2-0.3  & 0.97  & 0.98  & \textbf{1.00} & 0.96  & 0.95  & 0.98  & 0.98  & 0.97  & 0.96  & 0.97  & 0.96  & 0.95  & 0.96  & 0.93  & 0.94  & 0.94  & 0.91  & 0.88  \\ 
 0.3-0.4  & 0.96  & 0.96  & 0.96  & \textbf{1.00} & 0.92  & 0.96  & 0.97  & 0.95  & 0.97  & 0.97  & 0.93  & 0.95  & 0.94  & 0.94  & 0.94  & 0.94  & 0.91  & 0.86  \\ 
 0.4-0.5  & 0.95  & 0.95  & 0.95  & 0.92  & \textbf{1.00} & 0.95  & 0.95  & 0.94  & 0.92  & 0.93  & 0.96  & 0.93  & 0.95  & 0.90  & 0.92  & 0.92  & 0.90  & 0.90  \\ 
 0.5-0.6  & 0.98  & 0.97  & 0.98  & 0.96  & 0.95  & \textbf{1.00} & 0.97  & 0.97  & 0.96  & 0.96  & 0.96  & 0.96  & 0.96  & 0.94  & 0.94  & 0.95  & 0.92  & 0.89  \\ 
 0.6-0.7  & 0.97  & 0.97  & 0.98  & 0.97  & 0.95  & 0.97  & \textbf{1.00} & 0.97  & 0.97  & 0.97  & 0.96  & 0.96  & 0.96  & 0.95  & 0.95  & 0.96  & 0.93  & 0.90  \\ 
 0.7-0.8  & 0.97  & 0.97  & 0.97  & 0.95  & 0.94  & 0.97  & 0.97  & \textbf{1.00} & 0.95  & 0.96  & 0.95  & 0.96  & 0.95  & 0.94  & 0.94  & 0.95  & 0.92  & 0.87  \\ 
 0.8-0.9  & 0.96  & 0.96  & 0.96  & 0.97  & 0.92  & 0.96  & 0.97  & 0.95  & \textbf{1.00} & 0.97  & 0.94  & 0.96  & 0.96  & 0.95  & 0.95  & 0.96  & 0.93  & 0.90  \\ 
 0.9-1.0  & 0.96  & 0.97  & 0.97  & 0.97  & 0.93  & 0.96  & 0.97  & 0.96  & 0.97  & \textbf{1.00} & 0.94  & 0.96  & 0.96  & 0.95  & 0.95  & 0.96  & 0.94  & 0.89  \\ 
 1.0-1.1  & 0.95  & 0.95  & 0.96  & 0.93  & 0.96  & 0.96  & 0.96  & 0.95  & 0.94  & 0.94  & \textbf{1.00} & 0.94  & 0.96  & 0.93  & 0.95  & 0.94  & 0.92  & 0.93  \\ 
 1.1-1.2  & 0.96  & 0.96  & 0.95  & 0.95  & 0.93  & 0.96  & 0.96  & 0.96  & 0.96  & 0.96  & 0.94  & \textbf{1.00} & 0.95  & 0.95  & 0.95  & 0.96  & 0.95  & 0.89  \\ 
 1.2-1.3  & 0.95  & 0.95  & 0.96  & 0.94  & 0.95  & 0.96  & 0.96  & 0.95  & 0.96  & 0.96  & 0.96  & 0.95  & \textbf{1.00} & 0.94  & 0.95  & 0.95  & 0.93  & 0.92  \\ 
 1.3-1.4  & 0.93  & 0.94  & 0.93  & 0.94  & 0.90  & 0.94  & 0.95  & 0.94  & 0.95  & 0.95  & 0.93  & 0.95  & 0.94  & \textbf{1.00} & 0.93  & 0.96  & 0.95  & 0.89  \\ 
 1.4-1.5  & 0.94  & 0.94  & 0.94  & 0.94  & 0.92  & 0.94  & 0.95  & 0.94  & 0.95  & 0.95  & 0.95  & 0.95  & 0.95  & 0.93  & \textbf{1.00} & 0.94  & 0.92  & 0.91  \\ 
 1.5-1.7  & 0.95  & 0.95  & 0.94  & 0.94  & 0.92  & 0.95  & 0.96  & 0.95  & 0.96  & 0.96  & 0.94  & 0.96  & 0.95  & 0.96  & 0.94  & \textbf{1.00} & 0.95  & 0.89  \\ 
 1.7-1.9  & 0.92  & 0.93  & 0.91  & 0.91  & 0.90  & 0.92  & 0.93  & 0.92  & 0.93  & 0.94  & 0.92  & 0.95  & 0.93  & 0.95  & 0.92  & 0.95  & \textbf{1.00} & 0.88  \\ 
 1.9-2.5  & 0.86  & 0.87  & 0.88  & 0.86  & 0.90  & 0.89  & 0.90  & 0.87  & 0.90  & 0.89  & 0.93  & 0.89  & 0.92  & 0.89  & 0.91  & 0.89  & 0.88  & \textbf{1.00} \\ 
\end{tabular} 



==> tables/correlations/resolved/absXs_correlation_topH_pt_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrrrrrrr}
bin $[{\textrm GeV}]$  &  0-25  &  25-50  &  50-75  &  75-105  &  105-135  &  135-165  &  165-195  &  195-230  &  230-265  &  265-300  &  300-350  &  350-400  &  400-450  &  450-500  &  500-1000   \\ \hline
 0-25  & \textbf{1.00} & 0.97  & 0.97  & 0.97  & 0.95  & 0.93  & 0.90  & 0.85  & 0.80  & 0.71  & 0.71  & 0.57  & 0.59  & 0.42  & 0.47  \\ 
 25-50  & 0.97  & \textbf{1.00} & 0.99  & 0.98  & 0.95  & 0.93  & 0.90  & 0.83  & 0.78  & 0.68  & 0.69  & 0.54  & 0.56  & 0.37  & 0.46  \\ 
 50-75  & 0.97  & 0.99  & \textbf{1.00} & 0.98  & 0.96  & 0.94  & 0.91  & 0.85  & 0.80  & 0.70  & 0.71  & 0.55  & 0.57  & 0.38  & 0.45  \\ 
 75-105  & 0.97  & 0.98  & 0.98  & \textbf{1.00} & 0.98  & 0.96  & 0.93  & 0.87  & 0.82  & 0.70  & 0.73  & 0.60  & 0.59  & 0.39  & 0.49  \\ 
 105-135  & 0.95  & 0.95  & 0.96  & 0.98  & \textbf{1.00} & 0.98  & 0.96  & 0.91  & 0.87  & 0.74  & 0.76  & 0.64  & 0.62  & 0.41  & 0.50  \\ 
 135-165  & 0.93  & 0.93  & 0.94  & 0.96  & 0.98  & \textbf{1.00} & 0.97  & 0.92  & 0.90  & 0.78  & 0.80  & 0.69  & 0.66  & 0.45  & 0.54  \\ 
 165-195  & 0.90  & 0.90  & 0.91  & 0.93  & 0.96  & 0.97  & \textbf{1.00} & 0.93  & 0.91  & 0.80  & 0.83  & 0.71  & 0.68  & 0.46  & 0.56  \\ 
 195-230  & 0.85  & 0.83  & 0.85  & 0.87  & 0.91  & 0.92  & 0.93  & \textbf{1.00} & 0.93  & 0.89  & 0.89  & 0.78  & 0.76  & 0.66  & 0.63  \\ 
 230-265  & 0.80  & 0.78  & 0.80  & 0.82  & 0.87  & 0.90  & 0.91  & 0.93  & \textbf{1.00} & 0.86  & 0.88  & 0.82  & 0.78  & 0.60  & 0.67  \\ 
 265-300  & 0.71  & 0.68  & 0.70  & 0.70  & 0.74  & 0.78  & 0.80  & 0.89  & 0.86  & \textbf{1.00} & 0.90  & 0.76  & 0.81  & 0.77  & 0.67  \\ 
 300-350  & 0.71  & 0.69  & 0.71  & 0.73  & 0.76  & 0.80  & 0.83  & 0.89  & 0.88  & 0.90  & \textbf{1.00} & 0.82  & 0.81  & 0.70  & 0.74  \\ 
 350-400  & 0.57  & 0.54  & 0.55  & 0.60  & 0.64  & 0.69  & 0.71  & 0.78  & 0.82  & 0.76  & 0.82  & \textbf{1.00} & 0.75  & 0.65  & 0.77  \\ 
 400-450  & 0.59  & 0.56  & 0.57  & 0.59  & 0.62  & 0.66  & 0.68  & 0.76  & 0.78  & 0.81  & 0.81  & 0.75  & \textbf{1.00} & 0.66  & 0.70  \\ 
 450-500  & 0.42  & 0.37  & 0.38  & 0.39  & 0.41  & 0.45  & 0.46  & 0.66  & 0.60  & 0.77  & 0.70  & 0.65  & 0.66  & \textbf{1.00} & 0.59  \\ 
 500-1000  & 0.47  & 0.46  & 0.45  & 0.49  & 0.50  & 0.54  & 0.56  & 0.63  & 0.67  & 0.67  & 0.74  & 0.77  & 0.70  & 0.59  & \textbf{1.00} \\ 
\end{tabular} 



==> tables/correlations/resolved/absXs_correlation_tt_absrap_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrrrrrrrrrr}
bin  &  0.0-0.1  &  0.1-0.2  &  0.2-0.3  &  0.3-0.4  &  0.4-0.5  &  0.5-0.6  &  0.6-0.7  &  0.7-0.8  &  0.8-0.9  &  0.9-1.0  &  1.0-1.1  &  1.1-1.2  &  1.2-1.3  &  1.3-1.4  &  1.4-1.5  &  1.5-1.6  &  1.6-1.8  &  1.8-2.5   \\ \hline
 0.0-0.1  & \textbf{1.00} & 0.97  & 0.98  & 0.98  & 0.97  & 0.96  & 0.97  & 0.97  & 0.97  & 0.97  & 0.97  & 0.95  & 0.94  & 0.91  & 0.87  & 0.88  & 0.87  & 0.71  \\ 
 0.1-0.2  & 0.97  & \textbf{1.00} & 0.97  & 0.97  & 0.98  & 0.98  & 0.98  & 0.98  & 0.97  & 0.97  & 0.97  & 0.96  & 0.94  & 0.92  & 0.89  & 0.89  & 0.87  & 0.74  \\ 
 0.2-0.3  & 0.98  & 0.97  & \textbf{1.00} & 0.97  & 0.98  & 0.98  & 0.97  & 0.98  & 0.97  & 0.98  & 0.97  & 0.96  & 0.94  & 0.92  & 0.91  & 0.89  & 0.89  & 0.77  \\ 
 0.3-0.4  & 0.98  & 0.97  & 0.97  & \textbf{1.00} & 0.98  & 0.96  & 0.98  & 0.97  & 0.98  & 0.97  & 0.97  & 0.96  & 0.94  & 0.92  & 0.87  & 0.90  & 0.87  & 0.72  \\ 
 0.4-0.5  & 0.97  & 0.98  & 0.98  & 0.98  & \textbf{1.00} & 0.98  & 0.97  & 0.98  & 0.98  & 0.98  & 0.97  & 0.97  & 0.95  & 0.93  & 0.90  & 0.90  & 0.90  & 0.77  \\ 
 0.5-0.6  & 0.96  & 0.98  & 0.98  & 0.96  & 0.98  & \textbf{1.00} & 0.97  & 0.97  & 0.96  & 0.97  & 0.96  & 0.97  & 0.94  & 0.92  & 0.92  & 0.89  & 0.89  & 0.79  \\ 
 0.6-0.7  & 0.97  & 0.98  & 0.97  & 0.98  & 0.97  & 0.97  & \textbf{1.00} & 0.97  & 0.96  & 0.97  & 0.97  & 0.96  & 0.94  & 0.92  & 0.87  & 0.90  & 0.87  & 0.72  \\ 
 0.7-0.8  & 0.97  & 0.98  & 0.98  & 0.97  & 0.98  & 0.97  & 0.97  & \textbf{1.00} & 0.97  & 0.97  & 0.97  & 0.97  & 0.95  & 0.93  & 0.92  & 0.90  & 0.91  & 0.79  \\ 
 0.8-0.9  & 0.97  & 0.97  & 0.97  & 0.98  & 0.98  & 0.96  & 0.96  & 0.97  & \textbf{1.00} & 0.98  & 0.96  & 0.96  & 0.96  & 0.94  & 0.88  & 0.91  & 0.90  & 0.76  \\ 
 0.9-1.0  & 0.97  & 0.97  & 0.98  & 0.97  & 0.98  & 0.97  & 0.97  & 0.97  & 0.98  & \textbf{1.00} & 0.98  & 0.96  & 0.95  & 0.94  & 0.89  & 0.91  & 0.90  & 0.76  \\ 
 1.0-1.1  & 0.97  & 0.97  & 0.97  & 0.97  & 0.97  & 0.96  & 0.97  & 0.97  & 0.96  & 0.98  & \textbf{1.00} & 0.96  & 0.93  & 0.93  & 0.89  & 0.90  & 0.89  & 0.74  \\ 
 1.1-1.2  & 0.95  & 0.96  & 0.96  & 0.96  & 0.97  & 0.97  & 0.96  & 0.97  & 0.96  & 0.96  & 0.96  & \textbf{1.00} & 0.94  & 0.92  & 0.91  & 0.90  & 0.90  & 0.78  \\ 
 1.2-1.3  & 0.94  & 0.94  & 0.94  & 0.94  & 0.95  & 0.94  & 0.94  & 0.95  & 0.96  & 0.95  & 0.93  & 0.94  & \textbf{1.00} & 0.95  & 0.86  & 0.90  & 0.90  & 0.75  \\ 
 1.3-1.4  & 0.91  & 0.92  & 0.92  & 0.92  & 0.93  & 0.92  & 0.92  & 0.93  & 0.94  & 0.94  & 0.93  & 0.92  & 0.95  & \textbf{1.00} & 0.88  & 0.89  & 0.90  & 0.78  \\ 
 1.4-1.5  & 0.87  & 0.89  & 0.91  & 0.87  & 0.90  & 0.92  & 0.87  & 0.92  & 0.88  & 0.89  & 0.89  & 0.91  & 0.86  & 0.88  & \textbf{1.00} & 0.86  & 0.87  & 0.82  \\ 
 1.5-1.6  & 0.88  & 0.89  & 0.89  & 0.90  & 0.90  & 0.89  & 0.90  & 0.90  & 0.91  & 0.91  & 0.90  & 0.90  & 0.90  & 0.89  & 0.86  & \textbf{1.00} & 0.86  & 0.72  \\ 
 1.6-1.8  & 0.87  & 0.87  & 0.89  & 0.87  & 0.90  & 0.89  & 0.87  & 0.91  & 0.90  & 0.90  & 0.89  & 0.90  & 0.90  & 0.90  & 0.87  & 0.86  & \textbf{1.00} & 0.79  \\ 
 1.8-2.5  & 0.71  & 0.74  & 0.77  & 0.72  & 0.77  & 0.79  & 0.72  & 0.79  & 0.76  & 0.76  & 0.74  & 0.78  & 0.75  & 0.78  & 0.82  & 0.72  & 0.79  & \textbf{1.00} \\ 
\end{tabular} 



==> tables/correlations/resolved/absXs_correlation_tt_m_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrrr}
bin $[{\textrm GeV}]$  &  225-345  &  345-420  &  420-500  &  500-590  &  590-685  &  685-790  &  790-910  &  910-1040  &  1040-1175  &  1175-1320  &  1320-3000   \\ \hline
 225-345  & \textbf{1.00} & 0.71  & 0.42  & 0.34  & 0.37  & 0.35  & 0.43  & 0.39  & 0.41  & 0.41  & 0.47  \\ 
 345-420  & 0.71  & \textbf{1.00} & 0.88  & 0.83  & 0.80  & 0.73  & 0.72  & 0.62  & 0.58  & 0.56  & 0.38  \\ 
 420-500  & 0.42  & 0.88  & \textbf{1.00} & 0.98  & 0.95  & 0.88  & 0.81  & 0.71  & 0.64  & 0.63  & 0.36  \\ 
 500-590  & 0.34  & 0.83  & 0.98  & \textbf{1.00} & 0.97  & 0.93  & 0.85  & 0.77  & 0.70  & 0.67  & 0.39  \\ 
 590-685  & 0.37  & 0.80  & 0.95  & 0.97  & \textbf{1.00} & 0.96  & 0.90  & 0.85  & 0.79  & 0.76  & 0.52  \\ 
 685-790  & 0.35  & 0.73  & 0.88  & 0.93  & 0.96  & \textbf{1.00} & 0.93  & 0.90  & 0.84  & 0.80  & 0.60  \\ 
 790-910  & 0.43  & 0.72  & 0.81  & 0.85  & 0.90  & 0.93  & \textbf{1.00} & 0.94  & 0.91  & 0.86  & 0.76  \\ 
 910-1040  & 0.39  & 0.62  & 0.71  & 0.77  & 0.85  & 0.90  & 0.94  & \textbf{1.00} & 0.93  & 0.86  & 0.80  \\ 
 1040-1175  & 0.41  & 0.58  & 0.64  & 0.70  & 0.79  & 0.84  & 0.91  & 0.93  & \textbf{1.00} & 0.88  & 0.84  \\ 
 1175-1320  & 0.41  & 0.56  & 0.63  & 0.67  & 0.76  & 0.80  & 0.86  & 0.86  & 0.88  & \textbf{1.00} & 0.79  \\ 
 1320-3000  & 0.47  & 0.38  & 0.36  & 0.39  & 0.52  & 0.60  & 0.76  & 0.80  & 0.84  & 0.79  & \textbf{1.00} \\ 
\end{tabular} 



==> tables/correlations/resolved/absXs_correlation_tt_pt_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrr}
bin $[{\textrm GeV}]$  &  0-35  &  35-75  &  75-125  &  125-170  &  170-225  &  225-800   \\ \hline
 0-35  & \textbf{1.00} & 0.38  & 0.35  & 0.25  & 0.24  & 0.41  \\ 
 35-75  & 0.38  & \textbf{1.00} & 0.94  & 0.93  & 0.95  & 0.93  \\ 
 75-125  & 0.35  & 0.94  & \textbf{1.00} & 0.94  & 0.94  & 0.91  \\ 
 125-170  & 0.25  & 0.93  & 0.94  & \textbf{1.00} & 0.98  & 0.92  \\ 
 170-225  & 0.24  & 0.95  & 0.94  & 0.98  & \textbf{1.00} & 0.93  \\ 
 225-800  & 0.41  & 0.93  & 0.91  & 0.92  & 0.93  & \textbf{1.00} \\ 
\end{tabular} 



==> tables/correlations/resolved/absXs_covariance_topH_absrap_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrrrrrrrrrr}
bin  &  0.0-0.1  &  0.1-0.2  &  0.2-0.3  &  0.3-0.4  &  0.4-0.5  &  0.5-0.6  &  0.6-0.7  &  0.7-0.8  &  0.8-0.9  &  0.9-1.0  &  1.0-1.1  &  1.1-1.2  &  1.2-1.3  &  1.3-1.4  &  1.4-1.5  &  1.5-1.7  &  1.7-1.9  &  1.9-2.5   \\ \hline
 0.0-0.1  & 7.55e+01  & 7.08e+01  & 6.88e+01  & 6.61e+01  & 7.15e+01  & 6.46e+01  & 6.22e+01  & 5.70e+01  & 5.74e+01  & 5.09e+01  & 4.52e+01  & 4.29e+01  & 3.83e+01  & 3.34e+01  & 2.78e+01  & 2.25e+01  & 1.43e+01  & 3.00e+00  \\ 
 0.1-0.2  & 7.08e+01  & 7.01e+01  & 6.63e+01  & 6.37e+01  & 6.91e+01  & 6.21e+01  & 6.00e+01  & 5.50e+01  & 5.56e+01  & 4.93e+01  & 4.38e+01  & 4.16e+01  & 3.70e+01  & 3.25e+01  & 2.70e+01  & 2.17e+01  & 1.38e+01  & 2.93e+00  \\ 
 0.2-0.3  & 6.88e+01  & 6.63e+01  & 6.60e+01  & 6.17e+01  & 6.72e+01  & 6.03e+01  & 5.83e+01  & 5.32e+01  & 5.39e+01  & 4.76e+01  & 4.26e+01  & 4.01e+01  & 3.60e+01  & 3.12e+01  & 2.61e+01  & 2.09e+01  & 1.32e+01  & 2.86e+00  \\ 
 0.3-0.4  & 6.61e+01  & 6.37e+01  & 6.17e+01  & 6.24e+01  & 6.29e+01  & 5.76e+01  & 5.62e+01  & 5.07e+01  & 5.29e+01  & 4.63e+01  & 4.04e+01  & 3.88e+01  & 3.45e+01  & 3.05e+01  & 2.53e+01  & 2.03e+01  & 1.28e+01  & 2.72e+00  \\ 
 0.4-0.5  & 7.15e+01  & 6.91e+01  & 6.72e+01  & 6.29e+01  & 7.55e+01  & 6.28e+01  & 6.05e+01  & 5.50e+01  & 5.55e+01  & 4.90e+01  & 4.58e+01  & 4.19e+01  & 3.81e+01  & 3.22e+01  & 2.74e+01  & 2.17e+01  & 1.39e+01  & 3.14e+00  \\ 
 0.5-0.6  & 6.46e+01  & 6.21e+01  & 6.03e+01  & 5.76e+01  & 6.28e+01  & 5.79e+01  & 5.44e+01  & 4.97e+01  & 5.06e+01  & 4.46e+01  & 4.00e+01  & 3.76e+01  & 3.38e+01  & 2.94e+01  & 2.45e+01  & 1.97e+01  & 1.25e+01  & 2.70e+00  \\ 
 0.6-0.7  & 6.22e+01  & 6.00e+01  & 5.83e+01  & 5.62e+01  & 6.05e+01  & 5.44e+01  & 5.41e+01  & 4.81e+01  & 4.92e+01  & 4.34e+01  & 3.88e+01  & 3.66e+01  & 3.29e+01  & 2.88e+01  & 2.40e+01  & 1.92e+01  & 1.22e+01  & 2.64e+00  \\ 
 0.7-0.8  & 5.70e+01  & 5.50e+01  & 5.32e+01  & 5.07e+01  & 5.50e+01  & 4.97e+01  & 4.81e+01  & 4.56e+01  & 4.43e+01  & 3.95e+01  & 3.52e+01  & 3.33e+01  & 2.99e+01  & 2.61e+01  & 2.17e+01  & 1.75e+01  & 1.10e+01  & 2.35e+00  \\ 
 0.8-0.9  & 5.74e+01  & 5.56e+01  & 5.39e+01  & 5.29e+01  & 5.55e+01  & 5.06e+01  & 4.92e+01  & 4.43e+01  & 4.78e+01  & 4.06e+01  & 3.58e+01  & 3.42e+01  & 3.07e+01  & 2.72e+01  & 2.24e+01  & 1.80e+01  & 1.14e+01  & 2.48e+00  \\ 
 0.9-1.0  & 5.09e+01  & 4.93e+01  & 4.76e+01  & 4.63e+01  & 4.90e+01  & 4.46e+01  & 4.34e+01  & 3.95e+01  & 4.06e+01  & 3.69e+01  & 3.14e+01  & 3.02e+01  & 2.70e+01  & 2.39e+01  & 1.97e+01  & 1.59e+01  & 1.01e+01  & 2.15e+00  \\ 
 1.0-1.1  & 4.52e+01  & 4.38e+01  & 4.26e+01  & 4.04e+01  & 4.58e+01  & 4.00e+01  & 3.88e+01  & 3.52e+01  & 3.58e+01  & 3.14e+01  & 3.01e+01  & 2.67e+01  & 2.44e+01  & 2.11e+01  & 1.77e+01  & 1.41e+01  & 9.00e+00  & 2.04e+00  \\ 
 1.1-1.2  & 4.29e+01  & 4.16e+01  & 4.01e+01  & 3.88e+01  & 4.19e+01  & 3.76e+01  & 3.66e+01  & 3.33e+01  & 3.42e+01  & 3.02e+01  & 2.67e+01  & 2.67e+01  & 2.28e+01  & 2.02e+01  & 1.67e+01  & 1.35e+01  & 8.73e+00  & 1.84e+00  \\ 
 1.2-1.3  & 3.83e+01  & 3.70e+01  & 3.60e+01  & 3.45e+01  & 3.81e+01  & 3.38e+01  & 3.29e+01  & 2.99e+01  & 3.07e+01  & 2.70e+01  & 2.44e+01  & 2.28e+01  & 2.15e+01  & 1.79e+01  & 1.50e+01  & 1.20e+01  & 7.65e+00  & 1.71e+00  \\ 
 1.3-1.4  & 3.34e+01  & 3.25e+01  & 3.12e+01  & 3.05e+01  & 3.22e+01  & 2.94e+01  & 2.88e+01  & 2.61e+01  & 2.72e+01  & 2.39e+01  & 2.11e+01  & 2.02e+01  & 1.79e+01  & 1.70e+01  & 1.31e+01  & 1.07e+01  & 6.96e+00  & 1.46e+00  \\ 
 1.4-1.5  & 2.78e+01  & 2.70e+01  & 2.61e+01  & 2.53e+01  & 2.74e+01  & 2.45e+01  & 2.40e+01  & 2.17e+01  & 2.24e+01  & 1.97e+01  & 1.77e+01  & 1.67e+01  & 1.50e+01  & 1.31e+01  & 1.17e+01  & 8.77e+00  & 5.62e+00  & 1.25e+00  \\ 
 1.5-1.7  & 2.25e+01  & 2.17e+01  & 2.09e+01  & 2.03e+01  & 2.17e+01  & 1.97e+01  & 1.92e+01  & 1.75e+01  & 1.80e+01  & 1.59e+01  & 1.41e+01  & 1.35e+01  & 1.20e+01  & 1.07e+01  & 8.77e+00  & 7.43e+00  & 4.63e+00  & 9.76e-01  \\ 
 1.7-1.9  & 1.43e+01  & 1.38e+01  & 1.32e+01  & 1.28e+01  & 1.39e+01  & 1.25e+01  & 1.22e+01  & 1.10e+01  & 1.14e+01  & 1.01e+01  & 9.00e+00  & 8.73e+00  & 7.65e+00  & 6.96e+00  & 5.62e+00  & 4.63e+00  & 3.18e+00  & 6.24e-01  \\ 
 1.9-2.5  & 3.00e+00  & 2.93e+00  & 2.86e+00  & 2.72e+00  & 3.14e+00  & 2.70e+00  & 2.64e+00  & 2.35e+00  & 2.48e+00  & 2.15e+00  & 2.04e+00  & 1.84e+00  & 1.71e+00  & 1.46e+00  & 1.25e+00  & 9.76e-01  & 6.24e-01  & 1.60e-01  \\ 
\end{tabular} 



==> tables/correlations/resolved/absXs_covariance_topH_pt_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrrrrrrr}
bin $[{\textrm GeV}]$  &  0-25  &  25-50  &  50-75  &  75-105  &  105-135  &  135-165  &  165-195  &  195-230  &  230-265  &  265-300  &  300-350  &  350-400  &  400-450  &  450-500  &  500-1000   \\ \hline
 0-25  & 3.05e-04  & 8.25e-04  & 1.17e-03  & 1.22e-03  & 1.04e-03  & 6.95e-04  & 4.26e-04  & 2.74e-04  & 1.49e-04  & 9.81e-05  & 5.13e-05  & 2.62e-05  & 1.47e-05  & 8.74e-06  & 1.17e-06  \\ 
 25-50  & 8.25e-04  & 2.38e-03  & 3.33e-03  & 3.46e-03  & 2.91e-03  & 1.94e-03  & 1.18e-03  & 7.47e-04  & 4.05e-04  & 2.64e-04  & 1.40e-04  & 6.87e-05  & 3.94e-05  & 2.18e-05  & 3.17e-06  \\ 
 50-75  & 1.17e-03  & 3.33e-03  & 4.79e-03  & 4.94e-03  & 4.18e-03  & 2.79e-03  & 1.71e-03  & 1.09e-03  & 5.87e-04  & 3.83e-04  & 2.03e-04  & 9.94e-05  & 5.63e-05  & 3.15e-05  & 4.42e-06  \\ 
 75-105  & 1.22e-03  & 3.46e-03  & 4.94e-03  & 5.25e-03  & 4.43e-03  & 2.98e-03  & 1.83e-03  & 1.16e-03  & 6.35e-04  & 4.05e-04  & 2.19e-04  & 1.14e-04  & 6.08e-05  & 3.41e-05  & 5.02e-06  \\ 
 105-135  & 1.04e-03  & 2.91e-03  & 4.18e-03  & 4.43e-03  & 3.92e-03  & 2.63e-03  & 1.64e-03  & 1.05e-03  & 5.77e-04  & 3.68e-04  & 1.98e-04  & 1.05e-04  & 5.55e-05  & 3.10e-05  & 4.42e-06  \\ 
 135-165  & 6.95e-04  & 1.94e-03  & 2.79e-03  & 2.98e-03  & 2.63e-03  & 1.83e-03  & 1.13e-03  & 7.29e-04  & 4.12e-04  & 2.64e-04  & 1.43e-04  & 7.80e-05  & 4.04e-05  & 2.33e-05  & 3.29e-06  \\ 
 165-195  & 4.26e-04  & 1.18e-03  & 1.71e-03  & 1.83e-03  & 1.64e-03  & 1.13e-03  & 7.35e-04  & 4.64e-04  & 2.63e-04  & 1.72e-04  & 9.31e-05  & 5.04e-05  & 2.65e-05  & 1.49e-05  & 2.13e-06  \\ 
 195-230  & 2.74e-04  & 7.47e-04  & 1.09e-03  & 1.16e-03  & 1.05e-03  & 7.29e-04  & 4.64e-04  & 3.40e-04  & 1.82e-04  & 1.31e-04  & 6.80e-05  & 3.78e-05  & 2.01e-05  & 1.47e-05  & 1.64e-06  \\ 
 230-265  & 1.49e-04  & 4.05e-04  & 5.87e-04  & 6.35e-04  & 5.77e-04  & 4.12e-04  & 2.63e-04  & 1.82e-04  & 1.13e-04  & 7.31e-05  & 3.91e-05  & 2.29e-05  & 1.19e-05  & 7.65e-06  & 1.01e-06  \\ 
 265-300  & 9.81e-05  & 2.64e-04  & 3.83e-04  & 4.05e-04  & 3.68e-04  & 2.64e-04  & 1.72e-04  & 1.31e-04  & 7.31e-05  & 6.33e-05  & 2.97e-05  & 1.60e-05  & 9.20e-06  & 7.41e-06  & 7.48e-07  \\ 
 300-350  & 5.13e-05  & 1.40e-04  & 2.03e-04  & 2.19e-04  & 1.98e-04  & 1.43e-04  & 9.31e-05  & 6.80e-05  & 3.91e-05  & 2.97e-05  & 1.73e-05  & 9.03e-06  & 4.81e-06  & 3.51e-06  & 4.36e-07  \\ 
 350-400  & 2.62e-05  & 6.87e-05  & 9.94e-05  & 1.14e-04  & 1.05e-04  & 7.80e-05  & 5.04e-05  & 3.78e-05  & 2.29e-05  & 1.60e-05  & 9.03e-06  & 6.91e-06  & 2.81e-06  & 2.04e-06  & 2.87e-07  \\ 
 400-450  & 1.47e-05  & 3.94e-05  & 5.63e-05  & 6.08e-05  & 5.55e-05  & 4.04e-05  & 2.65e-05  & 2.01e-05  & 1.19e-05  & 9.20e-06  & 4.81e-06  & 2.81e-06  & 2.05e-06  & 1.13e-06  & 1.42e-07  \\ 
 450-500  & 8.74e-06  & 2.18e-05  & 3.15e-05  & 3.41e-05  & 3.10e-05  & 2.33e-05  & 1.49e-05  & 1.47e-05  & 7.65e-06  & 7.41e-06  & 3.51e-06  & 2.04e-06  & 1.13e-06  & 1.45e-06  & 9.93e-08  \\ 
 500-1000  & 1.17e-06  & 3.17e-06  & 4.42e-06  & 5.02e-06  & 4.42e-06  & 3.29e-06  & 2.13e-06  & 1.64e-06  & 1.01e-06  & 7.48e-07  & 4.36e-07  & 2.87e-07  & 1.42e-07  & 9.93e-08  & 1.99e-08  \\ 
\end{tabular} 



==> tables/correlations/resolved/absXs_covariance_tt_absrap_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrrrrrrrrrr}
bin  &  0.0-0.1  &  0.1-0.2  &  0.2-0.3  &  0.3-0.4  &  0.4-0.5  &  0.5-0.6  &  0.6-0.7  &  0.7-0.8  &  0.8-0.9  &  0.9-1.0  &  1.0-1.1  &  1.1-1.2  &  1.2-1.3  &  1.3-1.4  &  1.4-1.5  &  1.5-1.6  &  1.6-1.8  &  1.8-2.5   \\ \hline
 0.0-0.1  & 1.25e+02  & 1.19e+02  & 1.23e+02  & 1.15e+02  & 1.12e+02  & 9.68e+01  & 8.65e+01  & 8.21e+01  & 7.25e+01  & 6.08e+01  & 4.90e+01  & 3.90e+01  & 3.31e+01  & 2.58e+01  & 1.84e+01  & 1.26e+01  & 7.24e+00  & 7.20e-01  \\ 
 0.1-0.2  & 1.19e+02  & 1.19e+02  & 1.21e+02  & 1.12e+02  & 1.10e+02  & 9.60e+01  & 8.50e+01  & 8.11e+01  & 7.10e+01  & 5.91e+01  & 4.77e+01  & 3.85e+01  & 3.23e+01  & 2.55e+01  & 1.84e+01  & 1.25e+01  & 7.12e+00  & 7.37e-01  \\ 
 0.2-0.3  & 1.23e+02  & 1.21e+02  & 1.28e+02  & 1.16e+02  & 1.14e+02  & 9.95e+01  & 8.71e+01  & 8.42e+01  & 7.36e+01  & 6.19e+01  & 4.98e+01  & 4.00e+01  & 3.36e+01  & 2.66e+01  & 1.94e+01  & 1.28e+01  & 7.59e+00  & 7.88e-01  \\ 
 0.3-0.4  & 1.15e+02  & 1.12e+02  & 1.16e+02  & 1.11e+02  & 1.06e+02  & 9.11e+01  & 8.23e+01  & 7.75e+01  & 6.91e+01  & 5.74e+01  & 4.61e+01  & 3.70e+01  & 3.13e+01  & 2.47e+01  & 1.73e+01  & 1.21e+01  & 6.90e+00  & 6.86e-01  \\ 
 0.4-0.5  & 1.12e+02  & 1.10e+02  & 1.14e+02  & 1.06e+02  & 1.06e+02  & 9.12e+01  & 7.97e+01  & 7.68e+01  & 6.77e+01  & 5.63e+01  & 4.51e+01  & 3.66e+01  & 3.09e+01  & 2.44e+01  & 1.76e+01  & 1.19e+01  & 6.94e+00  & 7.19e-01  \\ 
 0.5-0.6  & 9.68e+01  & 9.60e+01  & 9.95e+01  & 9.11e+01  & 9.12e+01  & 8.11e+01  & 6.93e+01  & 6.67e+01  & 5.81e+01  & 4.87e+01  & 3.91e+01  & 3.19e+01  & 2.66e+01  & 2.11e+01  & 1.57e+01  & 1.03e+01  & 6.03e+00  & 6.47e-01  \\ 
 0.6-0.7  & 8.65e+01  & 8.50e+01  & 8.71e+01  & 8.23e+01  & 7.97e+01  & 6.93e+01  & 6.33e+01  & 5.86e+01  & 5.15e+01  & 4.32e+01  & 3.48e+01  & 2.80e+01  & 2.36e+01  & 1.86e+01  & 1.32e+01  & 9.16e+00  & 5.17e+00  & 5.18e-01  \\ 
 0.7-0.8  & 8.21e+01  & 8.11e+01  & 8.42e+01  & 7.75e+01  & 7.68e+01  & 6.67e+01  & 5.86e+01  & 5.79e+01  & 4.97e+01  & 4.12e+01  & 3.32e+01  & 2.71e+01  & 2.28e+01  & 1.80e+01  & 1.32e+01  & 8.77e+00  & 5.17e+00  & 5.43e-01  \\ 
 0.8-0.9  & 7.25e+01  & 7.10e+01  & 7.36e+01  & 6.91e+01  & 6.77e+01  & 5.81e+01  & 5.15e+01  & 4.97e+01  & 4.51e+01  & 3.67e+01  & 2.92e+01  & 2.36e+01  & 2.04e+01  & 1.61e+01  & 1.12e+01  & 7.83e+00  & 4.55e+00  & 4.61e-01  \\ 
 0.9-1.0  & 6.08e+01  & 5.91e+01  & 6.19e+01  & 5.74e+01  & 5.63e+01  & 4.87e+01  & 4.32e+01  & 4.12e+01  & 3.67e+01  & 3.14e+01  & 2.47e+01  & 1.96e+01  & 1.68e+01  & 1.34e+01  & 9.49e+00  & 6.51e+00  & 3.78e+00  & 3.84e-01  \\ 
 1.0-1.1  & 4.90e+01  & 4.77e+01  & 4.98e+01  & 4.61e+01  & 4.51e+01  & 3.91e+01  & 3.48e+01  & 3.32e+01  & 2.92e+01  & 2.47e+01  & 2.04e+01  & 1.59e+01  & 1.33e+01  & 1.07e+01  & 7.63e+00  & 5.18e+00  & 3.02e+00  & 3.05e-01  \\ 
 1.1-1.2  & 3.90e+01  & 3.85e+01  & 4.00e+01  & 3.70e+01  & 3.66e+01  & 3.19e+01  & 2.80e+01  & 2.71e+01  & 2.36e+01  & 1.96e+01  & 1.59e+01  & 1.35e+01  & 1.09e+01  & 8.57e+00  & 6.32e+00  & 4.24e+00  & 2.48e+00  & 2.59e-01  \\ 
 1.2-1.3  & 3.31e+01  & 3.23e+01  & 3.36e+01  & 3.13e+01  & 3.09e+01  & 2.66e+01  & 2.36e+01  & 2.28e+01  & 2.04e+01  & 1.68e+01  & 1.33e+01  & 1.09e+01  & 9.98e+00  & 7.60e+00  & 5.13e+00  & 3.65e+00  & 2.14e+00  & 2.16e-01  \\ 
 1.3-1.4  & 2.58e+01  & 2.55e+01  & 2.66e+01  & 2.47e+01  & 2.44e+01  & 2.11e+01  & 1.86e+01  & 1.80e+01  & 1.61e+01  & 1.34e+01  & 1.07e+01  & 8.57e+00  & 7.60e+00  & 6.48e+00  & 4.26e+00  & 2.91e+00  & 1.71e+00  & 1.80e-01  \\ 
 1.4-1.5  & 1.84e+01  & 1.84e+01  & 1.94e+01  & 1.73e+01  & 1.76e+01  & 1.57e+01  & 1.32e+01  & 1.32e+01  & 1.12e+01  & 9.49e+00  & 7.63e+00  & 6.32e+00  & 5.13e+00  & 4.26e+00  & 3.59e+00  & 2.08e+00  & 1.24e+00  & 1.42e-01  \\ 
 1.5-1.6  & 1.26e+01  & 1.25e+01  & 1.28e+01  & 1.21e+01  & 1.19e+01  & 1.03e+01  & 9.16e+00  & 8.77e+00  & 7.83e+00  & 6.51e+00  & 5.18e+00  & 4.24e+00  & 3.65e+00  & 2.91e+00  & 2.08e+00  & 1.63e+00  & 8.20e-01  & 8.39e-02  \\ 
 1.6-1.8  & 7.24e+00  & 7.12e+00  & 7.59e+00  & 6.90e+00  & 6.94e+00  & 6.03e+00  & 5.17e+00  & 5.17e+00  & 4.55e+00  & 3.78e+00  & 3.02e+00  & 2.48e+00  & 2.14e+00  & 1.71e+00  & 1.24e+00  & 8.20e-01  & 5.62e-01  & 5.35e-02  \\ 
 1.8-2.5  & 7.20e-01  & 7.37e-01  & 7.88e-01  & 6.86e-01  & 7.19e-01  & 6.47e-01  & 5.18e-01  & 5.43e-01  & 4.61e-01  & 3.84e-01  & 3.05e-01  & 2.59e-01  & 2.16e-01  & 1.80e-01  & 1.42e-01  & 8.39e-02  & 5.35e-02  & 8.25e-03  \\ 
\end{tabular} 



==> tables/correlations/resolved/absXs_covariance_tt_m_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrrr}
bin $[{\textrm GeV}]$  &  225-345  &  345-420  &  420-500  &  500-590  &  590-685  &  685-790  &  790-910  &  910-1040  &  1040-1175  &  1175-1320  &  1320-3000   \\ \hline
 225-345  & 6.45e-05  & 1.87e-04  & 1.16e-04  & 6.61e-05  & 4.10e-05  & 2.19e-05  & 1.53e-05  & 8.10e-06  & 5.03e-06  & 2.72e-06  & 5.52e-07  \\ 
 345-420  & 1.87e-04  & 1.07e-03  & 9.92e-04  & 6.54e-04  & 3.65e-04  & 1.87e-04  & 1.04e-04  & 5.31e-05  & 2.87e-05  & 1.52e-05  & 1.83e-06  \\ 
 420-500  & 1.16e-04  & 9.92e-04  & 1.17e-03  & 8.06e-04  & 4.51e-04  & 2.35e-04  & 1.23e-04  & 6.32e-05  & 3.34e-05  & 1.79e-05  & 1.79e-06  \\ 
 500-590  & 6.61e-05  & 6.54e-04  & 8.06e-04  & 5.79e-04  & 3.26e-04  & 1.74e-04  & 9.05e-05  & 4.84e-05  & 2.53e-05  & 1.32e-05  & 1.38e-06  \\ 
 590-685  & 4.10e-05  & 3.65e-04  & 4.51e-04  & 3.26e-04  & 1.93e-04  & 1.04e-04  & 5.58e-05  & 3.09e-05  & 1.66e-05  & 8.75e-06  & 1.07e-06  \\ 
 685-790  & 2.19e-05  & 1.87e-04  & 2.35e-04  & 1.74e-04  & 1.04e-04  & 6.07e-05  & 3.21e-05  & 1.83e-05  & 9.94e-06  & 5.15e-06  & 6.84e-07  \\ 
 790-910  & 1.53e-05  & 1.04e-04  & 1.23e-04  & 9.05e-05  & 5.58e-05  & 3.21e-05  & 1.97e-05  & 1.09e-05  & 6.11e-06  & 3.17e-06  & 4.95e-07  \\ 
 910-1040  & 8.10e-06  & 5.31e-05  & 6.32e-05  & 4.84e-05  & 3.09e-05  & 1.83e-05  & 1.09e-05  & 6.80e-06  & 3.67e-06  & 1.86e-06  & 3.05e-07  \\ 
 1040-1175  & 5.03e-06  & 2.87e-05  & 3.34e-05  & 2.53e-05  & 1.66e-05  & 9.94e-06  & 6.11e-06  & 3.67e-06  & 2.28e-06  & 1.09e-06  & 1.87e-07  \\ 
 1175-1320  & 2.72e-06  & 1.52e-05  & 1.79e-05  & 1.32e-05  & 8.75e-06  & 5.15e-06  & 3.17e-06  & 1.86e-06  & 1.09e-06  & 6.81e-07  & 9.56e-08  \\ 
 1320-3000  & 5.52e-07  & 1.83e-06  & 1.79e-06  & 1.38e-06  & 1.07e-06  & 6.84e-07  & 4.95e-07  & 3.05e-07  & 1.87e-07  & 9.56e-08  & 2.16e-08  \\ 
\end{tabular} 



==> tables/correlations/resolved/absXs_covariance_tt_pt_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrr}
bin $[{\textrm GeV}]$  &  0-35  &  35-75  &  75-125  &  125-170  &  170-225  &  225-800   \\ \hline
 0-35  & 1.33e-02  & 4.50e-03  & 2.42e-03  & 7.19e-04  & 3.14e-04  & 4.66e-05  \\ 
 35-75  & 4.50e-03  & 1.03e-02  & 5.73e-03  & 2.36e-03  & 1.07e-03  & 9.25e-05  \\ 
 75-125  & 2.42e-03  & 5.73e-03  & 3.62e-03  & 1.42e-03  & 6.26e-04  & 5.36e-05  \\ 
 125-170  & 7.19e-04  & 2.36e-03  & 1.42e-03  & 6.29e-04  & 2.72e-04  & 2.26e-05  \\ 
 170-225  & 3.14e-04  & 1.07e-03  & 6.26e-04  & 2.72e-04  & 1.24e-04  & 1.02e-05  \\ 
 225-800  & 4.66e-05  & 9.25e-05  & 5.36e-05  & 2.26e-05  & 1.02e-05  & 9.55e-07  \\ 
\end{tabular} 



==> tables/correlations/resolved/relXs_correlation_topH_absrap_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrrrrrrrrrr}
bin  &  0.0-0.1  &  0.1-0.2  &  0.2-0.3  &  0.3-0.4  &  0.4-0.5  &  0.5-0.6  &  0.6-0.7  &  0.7-0.8  &  0.8-0.9  &  0.9-1.0  &  1.0-1.1  &  1.1-1.2  &  1.2-1.3  &  1.3-1.4  &  1.4-1.5  &  1.5-1.7  &  1.7-1.9  &  1.9-2.5   \\ \hline
 0.0-0.1  & \textbf{1.00} & 0.18  & 0.41  & 0.06  & 0.24  & 0.45  & 0.13  & 0.24  & 0.15  & 0.07  & 0.16  & -0.06  & 0.05  & -0.18  & 0.03  & -0.09  & -0.12  & -0.04  \\ 
 0.1-0.2  & 0.18  & \textbf{1.00} & 0.33  & 0.18  & 0.53  & 0.27  & 0.41  & 0.37  & 0.05  & 0.01  & 0.36  & -0.11  & 0.29  & -0.10  & 0.05  & -0.07  & -0.08  & 0.22  \\ 
 0.2-0.3  & 0.41  & 0.33  & \textbf{1.00} & 0.21  & 0.24  & 0.39  & 0.28  & 0.30  & 0.17  & 0.09  & 0.25  & -0.09  & 0.13  & -0.13  & 0.04  & -0.15  & -0.19  & 0.06  \\ 
 0.3-0.4  & 0.06  & 0.18  & 0.21  & \textbf{1.00} & 0.07  & 0.06  & 0.31  & -0.03  & 0.34  & 0.09  & 0.09  & -0.14  & 0.14  & -0.00  & 0.09  & -0.14  & -0.17  & 0.14  \\ 
 0.4-0.5  & 0.24  & 0.53  & 0.24  & 0.07  & \textbf{1.00} & 0.29  & 0.49  & 0.53  & -0.03  & -0.00  & 0.53  & 0.03  & 0.55  & -0.02  & 0.19  & 0.15  & 0.12  & 0.44  \\ 
 0.5-0.6  & 0.45  & 0.27  & 0.39  & 0.06  & 0.29  & \textbf{1.00} & 0.14  & 0.17  & 0.15  & 0.03  & 0.23  & -0.04  & 0.17  & -0.10  & 0.05  & -0.01  & -0.06  & 0.10  \\ 
 0.6-0.7  & 0.13  & 0.41  & 0.28  & 0.31  & 0.49  & 0.14  & \textbf{1.00} & 0.28  & 0.16  & 0.15  & 0.43  & 0.01  & 0.47  & 0.08  & 0.24  & 0.14  & 0.06  & 0.41  \\ 
 0.7-0.8  & 0.24  & 0.37  & 0.30  & -0.03  & 0.53  & 0.17  & 0.28  & \textbf{1.00} & -0.09  & 0.00  & 0.35  & 0.06  & 0.32  & -0.08  & 0.10  & 0.00  & -0.00  & 0.21  \\ 
 0.8-0.9  & 0.15  & 0.05  & 0.17  & 0.34  & -0.03  & 0.15  & 0.16  & -0.09  & \textbf{1.00} & 0.26  & 0.11  & 0.17  & 0.21  & 0.28  & 0.27  & 0.17  & 0.14  & 0.28  \\ 
 0.9-1.0  & 0.07  & 0.01  & 0.09  & 0.09  & -0.00  & 0.03  & 0.15  & 0.00  & 0.26  & \textbf{1.00} & 0.02  & 0.11  & 0.16  & 0.14  & 0.21  & 0.12  & 0.10  & 0.17  \\ 
 1.0-1.1  & 0.16  & 0.36  & 0.25  & 0.09  & 0.53  & 0.23  & 0.43  & 0.35  & 0.11  & 0.02  & \textbf{1.00} & 0.05  & 0.48  & 0.23  & 0.31  & 0.28  & 0.31  & 0.56  \\ 
 1.1-1.2  & -0.06  & -0.11  & -0.09  & -0.14  & 0.03  & -0.04  & 0.01  & 0.06  & 0.17  & 0.11  & 0.05  & \textbf{1.00} & 0.15  & 0.15  & 0.25  & 0.22  & 0.30  & 0.24  \\ 
 1.2-1.3  & 0.05  & 0.29  & 0.13  & 0.14  & 0.55  & 0.17  & 0.47  & 0.32  & 0.21  & 0.16  & 0.48  & 0.15  & \textbf{1.00} & 0.17  & 0.31  & 0.37  & 0.30  & 0.61  \\ 
 1.3-1.4  & -0.18  & -0.10  & -0.13  & -0.00  & -0.02  & -0.10  & 0.08  & -0.08  & 0.28  & 0.14  & 0.23  & 0.15  & 0.17  & \textbf{1.00} & 0.18  & 0.29  & 0.43  & 0.38  \\ 
 1.4-1.5  & 0.03  & 0.05  & 0.04  & 0.09  & 0.19  & 0.05  & 0.24  & 0.10  & 0.27  & 0.21  & 0.31  & 0.25  & 0.31  & 0.18  & \textbf{1.00} & 0.26  & 0.37  & 0.46  \\ 
 1.5-1.7  & -0.09  & -0.07  & -0.15  & -0.14  & 0.15  & -0.01  & 0.14  & 0.00  & 0.17  & 0.12  & 0.28  & 0.22  & 0.37  & 0.29  & 0.26  & \textbf{1.00} & 0.41  & 0.50  \\ 
 1.7-1.9  & -0.12  & -0.08  & -0.19  & -0.17  & 0.12  & -0.06  & 0.06  & -0.00  & 0.14  & 0.10  & 0.31  & 0.30  & 0.30  & 0.43  & 0.37  & 0.41  & \textbf{1.00} & 0.50  \\ 
 1.9-2.5  & -0.04  & 0.22  & 0.06  & 0.14  & 0.44  & 0.10  & 0.41  & 0.21  & 0.28  & 0.17  & 0.56  & 0.24  & 0.61  & 0.38  & 0.46  & 0.50  & 0.50  & \textbf{1.00} \\ 
\end{tabular} 



==> tables/correlations/resolved/relXs_correlation_topH_pt_co.res_13TeV.tex <==
\centering 
\resizebox*{\textwidth}{!}{
\begin{tabular}{r|rrrrrrrrrrrrrrr}
Bin \GeV{}  &  0--25  &  25--50  &  50--75  &  75--105  &  105--135  &  135--165  &  165--195  &  195--230  &  230--265  &  265--300  &  300--350  &  350--400  &  400--450  &450--500&500--1000\\ \hline
 0--25  & \textbf{1.00} & 0.70  & 0.61  & 0.59  & 0.08  & $-$0.23  & $-$0.49  & $-$0.30  & $-$0.52  & $-$0.22  & $-$0.39  & $-$0.42  & $-$0.23  & 0.07  & $-$0.17  \\ 
 25--50  & 0.70  & \textbf{1.00} & 0.77  & 0.69  & $-$0.01  & $-$0.39  & $-$0.65  & $-$0.45  & $-$0.66  & $-$0.35  & $-$0.50  & $-$0.53  & $-$0.31  & $-$0.01  & $-$0.21  \\ 
 50--75  & 0.61  & 0.77  & \textbf{1.00} & 0.67  & $-$0.01  & $-$0.40  & $-$0.58  & $-$0.46  & $-$0.70  & $-$0.49  & $-$0.60  & $-$0.56  & $-$0.41  & $-$0.12  & $-$0.28  \\ 
 75--105  & 0.59  & 0.69  & 0.67  & \textbf{1.00} & 0.06  & $-$0.21  & $-$0.53  & $-$0.38  & $-$0.56  & $-$0.35  & $-$0.50  & $-$0.52  & $-$0.37  & $-$0.08  & $-$0.32  \\ 
 105--135  & 0.08  & $-$0.01  & $-$0.01  & 0.06  & \textbf{1.00} & 0.35  & 0.09  & 0.15  & $-$0.12  & 0.05  & $-$0.12  & $-$0.16  & $-$0.19  & 0.11  & $-$0.27  \\ 
 135--165  & $-$0.23  & $-$0.39  & $-$0.40  & $-$0.21  & 0.35  & \textbf{1.00} & 0.57  & 0.54  & 0.50  & 0.47  & 0.40  & 0.37  & 0.25  & 0.35  & 0.12  \\ 
 165--195  & $-$0.49  & $-$0.65  & $-$0.58  & $-$0.53  & 0.09  & 0.57  & \textbf{1.00} & 0.66  & 0.64  & 0.50  & 0.53  & 0.61  & 0.38  & 0.33  & 0.29  \\ 
 195--230  & $-$0.30  & $-$0.45  & $-$0.46  & $-$0.38  & 0.15  & 0.54  & 0.66  & \textbf{1.00} & 0.67  & 0.76  & 0.71  & 0.62  & 0.56  & 0.66  & 0.39  \\ 
 230--265  & $-$0.52  & $-$0.66  & $-$0.70  & $-$0.56  & $-$0.12  & 0.50  & 0.64  & 0.67  & \textbf{1.00} & 0.68  & 0.73  & 0.73  & 0.58  & 0.42  & 0.45  \\ 
 265--300  & $-$0.22  & $-$0.35  & $-$0.49  & $-$0.35  & 0.05  & 0.47  & 0.50  & 0.76  & 0.68  & \textbf{1.00} & 0.77  & 0.60  & 0.65  & 0.71  & 0.45  \\ 
 300--350  & $-$0.39  & $-$0.50  & $-$0.60  & $-$0.50  & $-$0.12  & 0.40  & 0.53  & 0.71  & 0.73  & 0.77  & \textbf{1.00} & 0.71  & 0.66  & 0.59  & 0.57  \\ 
 350--400  & $-$0.42  & $-$0.53  & $-$0.56  & $-$0.52  & $-$0.16  & 0.37  & 0.61  & 0.62  & 0.73  & 0.60  & 0.71  & \textbf{1.00} & 0.59  & 0.49  & 0.62  \\ 
 400--450  & $-$0.23  & $-$0.31  & $-$0.41  & $-$0.37  & $-$0.19  & 0.25  & 0.38  & 0.56  & 0.58  & 0.65  & 0.66  & 0.59  & \textbf{1.00} & 0.54  & 0.57  \\ 
 450--500  & 0.07  & $-$0.01  & $-$0.12  & $-$0.08  & 0.11  & 0.35  & 0.33  & 0.66  & 0.42  & 0.71  & 0.59  & 0.49  & 0.54  & \textbf{1.00} & 0.46  \\ 
 500--1000  & $-$0.17  & $-$0.21  & $-$0.28  & $-$0.32  & $-$0.27  & 0.12  & 0.29  & 0.39  & 0.45  & 0.45  & 0.57  & 0.62  & 0.57  & 0.46  & \textbf{1.00} \\ 
\end{tabular}}



==> tables/correlations/resolved/relXs_correlation_tt_absrap_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrrrrrrrrrr}
bin  &  0.0-0.1  &  0.1-0.2  &  0.2-0.3  &  0.3-0.4  &  0.4-0.5  &  0.5-0.6  &  0.6-0.7  &  0.7-0.8  &  0.8-0.9  &  0.9-1.0  &  1.0-1.1  &  1.1-1.2  &  1.2-1.3  &  1.3-1.4  &  1.4-1.5  &  1.5-1.6  &  1.6-1.8  &  1.8-2.5   \\ \hline
 0.0-0.1  & \textbf{1.00} & 0.35  & 0.38  & 0.05  & 0.34  & 0.40  & 0.15  & 0.20  & -0.17  & 0.13  & 0.07  & 0.07  & -0.01  & -0.11  & 0.10  & -0.12  & -0.01  & 0.08  \\ 
 0.1-0.2  & 0.35  & \textbf{1.00} & 0.59  & 0.06  & 0.36  & 0.36  & 0.26  & 0.17  & -0.14  & 0.14  & 0.18  & 0.14  & -0.09  & 0.03  & 0.09  & -0.02  & -0.04  & 0.06  \\ 
 0.2-0.3  & 0.38  & 0.59  & \textbf{1.00} & 0.11  & 0.43  & 0.46  & 0.18  & 0.38  & -0.03  & 0.32  & 0.27  & 0.25  & 0.15  & 0.25  & 0.27  & 0.06  & 0.20  & 0.28  \\ 
 0.3-0.4  & 0.05  & 0.06  & 0.11  & \textbf{1.00} & 0.28  & 0.12  & 0.28  & 0.22  & 0.03  & 0.05  & -0.10  & 0.07  & -0.17  & -0.18  & 0.07  & -0.05  & 0.08  & 0.09  \\ 
 0.4-0.5  & 0.34  & 0.36  & 0.43  & 0.28  & \textbf{1.00} & 0.41  & 0.05  & 0.37  & 0.14  & 0.28  & 0.10  & 0.23  & 0.16  & 0.14  & 0.22  & 0.05  & 0.26  & 0.24  \\ 
 0.5-0.6  & 0.40  & 0.36  & 0.46  & 0.12  & 0.41  & \textbf{1.00} & 0.43  & 0.48  & -0.17  & 0.40  & 0.11  & 0.32  & 0.08  & 0.03  & 0.48  & 0.02  & 0.27  & 0.40  \\ 
 0.6-0.7  & 0.15  & 0.26  & 0.18  & 0.28  & 0.05  & 0.43  & \textbf{1.00} & 0.29  & -0.32  & 0.13  & 0.06  & 0.24  & -0.14  & -0.11  & 0.23  & 0.04  & 0.06  & 0.12  \\ 
 0.7-0.8  & 0.20  & 0.17  & 0.38  & 0.22  & 0.37  & 0.48  & 0.29  & \textbf{1.00} & 0.13  & 0.38  & 0.04  & 0.36  & 0.32  & 0.17  & 0.59  & 0.09  & 0.53  & 0.55  \\ 
 0.8-0.9  & -0.17  & -0.14  & -0.03  & 0.03  & 0.14  & -0.17  & -0.32  & 0.13  & \textbf{1.00} & 0.15  & -0.18  & -0.01  & 0.30  & 0.23  & -0.00  & 0.15  & 0.27  & 0.13  \\ 
 0.9-1.0  & 0.13  & 0.14  & 0.32  & 0.05  & 0.28  & 0.40  & 0.13  & 0.38  & 0.15  & \textbf{1.00} & 0.24  & 0.18  & 0.27  & 0.30  & 0.45  & 0.20  & 0.44  & 0.43  \\ 
 1.0-1.1  & 0.07  & 0.18  & 0.27  & -0.10  & 0.10  & 0.11  & 0.06  & 0.04  & -0.18  & 0.24  & \textbf{1.00} & 0.26  & -0.05  & 0.24  & 0.15  & 0.14  & 0.14  & 0.12  \\ 
 1.1-1.2  & 0.07  & 0.14  & 0.25  & 0.07  & 0.23  & 0.32  & 0.24  & 0.36  & -0.01  & 0.18  & 0.26  & \textbf{1.00} & 0.26  & 0.17  & 0.33  & 0.24  & 0.32  & 0.31  \\ 
 1.2-1.3  & -0.01  & -0.09  & 0.15  & -0.17  & 0.16  & 0.08  & -0.14  & 0.32  & 0.30  & 0.27  & -0.05  & 0.26  & \textbf{1.00} & 0.44  & 0.19  & 0.22  & 0.48  & 0.33  \\ 
 1.3-1.4  & -0.11  & 0.03  & 0.25  & -0.18  & 0.14  & 0.03  & -0.11  & 0.17  & 0.23  & 0.30  & 0.24  & 0.17  & 0.44  & \textbf{1.00} & 0.28  & 0.29  & 0.37  & 0.31  \\ 
 1.4-1.5  & 0.10  & 0.09  & 0.27  & 0.07  & 0.22  & 0.48  & 0.23  & 0.59  & -0.00  & 0.45  & 0.15  & 0.33  & 0.19  & 0.28  & \textbf{1.00} & 0.22  & 0.43  & 0.52  \\ 
 1.5-1.6  & -0.12  & -0.02  & 0.06  & -0.05  & 0.05  & 0.02  & 0.04  & 0.09  & 0.15  & 0.20  & 0.14  & 0.24  & 0.22  & 0.29  & 0.22  & \textbf{1.00} & 0.21  & 0.13  \\ 
 1.6-1.8  & -0.01  & -0.04  & 0.20  & 0.08  & 0.26  & 0.27  & 0.06  & 0.53  & 0.27  & 0.44  & 0.14  & 0.32  & 0.48  & 0.37  & 0.43  & 0.21  & \textbf{1.00} & 0.46  \\ 
 1.8-2.5  & 0.08  & 0.06  & 0.28  & 0.09  & 0.24  & 0.40  & 0.12  & 0.55  & 0.13  & 0.43  & 0.12  & 0.31  & 0.33  & 0.31  & 0.52  & 0.13  & 0.46  & \textbf{1.00} \\ 
\end{tabular} 



==> tables/correlations/resolved/relXs_correlation_tt_m_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrrr}
bin $[{\textrm GeV}]$  &  225-345  &  345-420  &  420-500  &  500-590  &  590-685  &  685-790  &  790-910  &  910-1040  &  1040-1175  &  1175-1320  &  1320-3000   \\ \hline
 225-345  & \textbf{1.00} & 0.60  & -0.53  & -0.83  & -0.67  & -0.38  & -0.06  & -0.07  & 0.02  & 0.07  & 0.31  \\ 
 345-420  & 0.60  & \textbf{1.00} & 0.20  & -0.38  & -0.59  & -0.55  & -0.27  & -0.38  & -0.32  & -0.20  & -0.08  \\ 
 420-500  & -0.53  & 0.20  & \textbf{1.00} & 0.66  & 0.18  & -0.13  & -0.34  & -0.39  & -0.44  & -0.40  & -0.52  \\ 
 500-590  & -0.83  & -0.38  & 0.66  & \textbf{1.00} & 0.65  & 0.39  & 0.09  & 0.07  & -0.04  & -0.12  & -0.27  \\ 
 590-685  & -0.67  & -0.59  & 0.18  & 0.65  & \textbf{1.00} & 0.74  & 0.53  & 0.59  & 0.46  & 0.37  & 0.27  \\ 
 685-790  & -0.38  & -0.55  & -0.13  & 0.39  & 0.74  & \textbf{1.00} & 0.73  & 0.74  & 0.62  & 0.58  & 0.47  \\ 
 790-910  & -0.06  & -0.27  & -0.34  & 0.09  & 0.53  & 0.73  & \textbf{1.00} & 0.85  & 0.80  & 0.69  & 0.75  \\ 
 910-1040  & -0.07  & -0.38  & -0.39  & 0.07  & 0.59  & 0.74  & 0.85  & \textbf{1.00} & 0.84  & 0.71  & 0.79  \\ 
 1040-1175  & 0.02  & -0.32  & -0.44  & -0.04  & 0.46  & 0.62  & 0.80  & 0.84  & \textbf{1.00} & 0.71  & 0.82  \\ 
 1175-1320  & 0.07  & -0.20  & -0.40  & -0.12  & 0.37  & 0.58  & 0.69  & 0.71  & 0.71  & \textbf{1.00} & 0.71  \\ 
 1320-3000  & 0.31  & -0.08  & -0.52  & -0.27  & 0.27  & 0.47  & 0.75  & 0.79  & 0.82  & 0.71  & \textbf{1.00} \\ 
\end{tabular} 



==> tables/correlations/resolved/relXs_correlation_tt_pt_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrr}
bin $[{\textrm GeV}]$  &  0-35  &  35-75  &  75-125  &  125-170  &  170-225  &  225-800   \\ \hline
 0-35  & \textbf{1.00} & -0.10  & -0.28  & -0.45  & -0.32  & -0.15  \\ 
 35-75  & -0.10  & \textbf{1.00} & 0.92  & 0.59  & 0.67  & 0.23  \\ 
 75-125  & -0.28  & 0.92  & \textbf{1.00} & 0.77  & 0.82  & 0.39  \\ 
 125-170  & -0.45  & 0.59  & 0.77  & \textbf{1.00} & 0.88  & 0.51  \\ 
 170-225  & -0.32  & 0.67  & 0.82  & 0.88  & \textbf{1.00} & 0.54  \\ 
 225-800  & -0.15  & 0.23  & 0.39  & 0.51  & 0.54  & \textbf{1.00} \\ 
\end{tabular} 



==> tables/correlations/resolved/relXs_covariance_topH_absrap_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrrrrrrrrrr}
bin  &  0.0-0.1  &  0.1-0.2  &  0.2-0.3  &  0.3-0.4  &  0.4-0.5  &  0.5-0.6  &  0.6-0.7  &  0.7-0.8  &  0.8-0.9  &  0.9-1.0  &  1.0-1.1  &  1.1-1.2  &  1.2-1.3  &  1.3-1.4  &  1.4-1.5  &  1.5-1.7  &  1.7-1.9  &  1.9-2.5   \\ \hline
 0.0-0.1  & 3.30e-04  & 5.03e-05  & 1.24e-04  & 1.86e-05  & 1.14e-04  & 1.14e-04  & 3.47e-05  & 5.96e-05  & 4.40e-05  & 1.43e-05  & 4.21e-05  & -1.23e-05  & 1.13e-05  & -3.44e-05  & 5.27e-06  & -9.81e-06  & -1.22e-05  & -1.32e-06  \\ 
 0.1-0.2  & 5.03e-05  & 2.38e-04  & 8.47e-05  & 5.18e-05  & 2.12e-04  & 5.90e-05  & 9.29e-05  & 7.89e-05  & 1.28e-05  & 1.93e-06  & 8.02e-05  & -1.80e-05  & 5.99e-05  & -1.75e-05  & 8.05e-06  & -6.33e-06  & -7.28e-06  & 5.93e-06  \\ 
 0.2-0.3  & 1.24e-04  & 8.47e-05  & 2.80e-04  & 6.62e-05  & 1.07e-04  & 9.16e-05  & 6.94e-05  & 6.95e-05  & 4.63e-05  & 1.62e-05  & 6.10e-05  & -1.67e-05  & 2.88e-05  & -2.34e-05  & 7.14e-06  & -1.51e-05  & -1.75e-05  & 1.77e-06  \\ 
 0.3-0.4  & 1.86e-05  & 5.18e-05  & 6.62e-05  & 3.42e-04  & 3.14e-05  & 1.60e-05  & 8.51e-05  & -6.78e-06  & 1.01e-04  & 1.85e-05  & 2.44e-05  & -2.81e-05  & 3.54e-05  & -5.56e-07  & 1.65e-05  & -1.59e-05  & -1.70e-05  & 4.47e-06  \\ 
 0.4-0.5  & 1.14e-04  & 2.12e-04  & 1.07e-04  & 3.14e-05  & 6.78e-04  & 1.05e-04  & 1.87e-04  & 1.93e-04  & -1.21e-05  & -6.40e-07  & 1.99e-04  & 7.97e-06  & 1.90e-04  & -5.03e-06  & 4.59e-05  & 2.47e-05  & 1.79e-05  & 2.03e-05  \\ 
 0.5-0.6  & 1.14e-04  & 5.90e-05  & 9.16e-05  & 1.60e-05  & 1.05e-04  & 1.98e-04  & 2.89e-05  & 3.26e-05  & 3.38e-05  & 4.58e-06  & 4.60e-05  & -5.25e-06  & 3.17e-05  & -1.45e-05  & 7.30e-06  & -1.29e-06  & -4.42e-06  & 2.60e-06  \\ 
 0.6-0.7  & 3.47e-05  & 9.29e-05  & 6.94e-05  & 8.51e-05  & 1.87e-04  & 2.89e-05  & 2.15e-04  & 5.65e-05  & 3.73e-05  & 2.39e-05  & 9.20e-05  & 1.91e-06  & 9.16e-05  & 1.20e-05  & 3.29e-05  & 1.31e-05  & 4.52e-06  & 1.07e-05  \\ 
 0.7-0.8  & 5.96e-05  & 7.89e-05  & 6.95e-05  & -6.78e-06  & 1.93e-04  & 3.26e-05  & 5.65e-05  & 1.93e-04  & -2.07e-05  & 6.21e-07  & 6.95e-05  & 8.83e-06  & 5.87e-05  & -1.26e-05  & 1.34e-05  & 2.89e-07  & -1.92e-07  & 5.08e-06  \\ 
 0.8-0.9  & 4.40e-05  & 1.28e-05  & 4.63e-05  & 1.01e-04  & -1.21e-05  & 3.38e-05  & 3.73e-05  & -2.07e-05  & 2.56e-04  & 4.61e-05  & 2.45e-05  & 2.80e-05  & 4.43e-05  & 4.81e-05  & 4.11e-05  & 1.71e-05  & 1.25e-05  & 7.94e-06  \\ 
 0.9-1.0  & 1.43e-05  & 1.93e-06  & 1.62e-05  & 1.85e-05  & -6.40e-07  & 4.58e-06  & 2.39e-05  & 6.21e-07  & 4.61e-05  & 1.25e-04  & 3.97e-06  & 1.30e-05  & 2.40e-05  & 1.74e-05  & 2.20e-05  & 8.02e-06  & 6.18e-06  & 3.34e-06  \\ 
 1.0-1.1  & 4.21e-05  & 8.02e-05  & 6.10e-05  & 2.44e-05  & 1.99e-04  & 4.60e-05  & 9.20e-05  & 6.95e-05  & 2.45e-05  & 3.97e-06  & 2.10e-04  & 7.44e-06  & 9.26e-05  & 3.59e-05  & 4.33e-05  & 2.55e-05  & 2.49e-05  & 1.44e-05  \\ 
 1.1-1.2  & -1.23e-05  & -1.80e-05  & -1.67e-05  & -2.81e-05  & 7.97e-06  & -5.25e-06  & 1.91e-06  & 8.83e-06  & 2.80e-05  & 1.30e-05  & 7.44e-06  & 1.12e-04  & 2.03e-05  & 1.71e-05  & 2.55e-05  & 1.47e-05  & 1.76e-05  & 4.53e-06  \\ 
 1.2-1.3  & 1.13e-05  & 5.99e-05  & 2.88e-05  & 3.54e-05  & 1.90e-04  & 3.17e-05  & 9.16e-05  & 5.87e-05  & 4.43e-05  & 2.40e-05  & 9.26e-05  & 2.03e-05  & 1.75e-04  & 2.45e-05  & 3.91e-05  & 3.01e-05  & 2.17e-05  & 1.42e-05  \\ 
 1.3-1.4  & -3.44e-05  & -1.75e-05  & -2.34e-05  & -5.56e-07  & -5.03e-06  & -1.45e-05  & 1.20e-05  & -1.26e-05  & 4.81e-05  & 1.74e-05  & 3.59e-05  & 1.71e-05  & 2.45e-05  & 1.17e-04  & 1.89e-05  & 1.96e-05  & 2.59e-05  & 7.31e-06  \\ 
 1.4-1.5  & 5.27e-06  & 8.05e-06  & 7.14e-06  & 1.65e-05  & 4.59e-05  & 7.30e-06  & 3.29e-05  & 1.34e-05  & 4.11e-05  & 2.20e-05  & 4.33e-05  & 2.55e-05  & 3.91e-05  & 1.89e-05  & 9.03e-05  & 1.55e-05  & 1.96e-05  & 7.72e-06  \\ 
 1.5-1.7  & -9.81e-06  & -6.33e-06  & -1.51e-05  & -1.59e-05  & 2.47e-05  & -1.29e-06  & 1.31e-05  & 2.89e-07  & 1.71e-05  & 8.02e-06  & 2.55e-05  & 1.47e-05  & 3.01e-05  & 1.96e-05  & 1.55e-05  & 3.85e-05  & 1.42e-05  & 5.54e-06  \\ 
 1.7-1.9  & -1.22e-05  & -7.28e-06  & -1.75e-05  & -1.70e-05  & 1.79e-05  & -4.42e-06  & 4.52e-06  & -1.92e-07  & 1.25e-05  & 6.18e-06  & 2.49e-05  & 1.76e-05  & 2.17e-05  & 2.59e-05  & 1.96e-05  & 1.42e-05  & 3.11e-05  & 4.91e-06  \\ 
 1.9-2.5  & -1.32e-06  & 5.93e-06  & 1.77e-06  & 4.47e-06  & 2.03e-05  & 2.60e-06  & 1.07e-05  & 5.08e-06  & 7.94e-06  & 3.34e-06  & 1.44e-05  & 4.53e-06  & 1.42e-05  & 7.31e-06  & 7.72e-06  & 5.54e-06  & 4.91e-06  & 3.13e-06  \\ 
\end{tabular} 



==> tables/correlations/resolved/relXs_covariance_topH_pt_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrrrrrrr}
Bin $[{\textrm GeV}]$  &  0-25  &  25-50  &  50-75  &  75-105  &  105-135  &  135-165  &  165-195  &  195-230  &  230-265  &  265-300  &  300-350  &  350-400  &  400-450  &  450-500  &  500-1000   \\ \hline
 0-25  & 3.25e-09  & 5.52e-09  & 5.68e-09  & 3.97e-09  & 3.79e-10  & -1.18e-09  & -2.21e-09  & -1.29e-09  & -1.67e-09  & -6.67e-10  & -5.91e-10  & -4.89e-10  & -1.38e-10  & 4.26e-11  & -1.11e-11  \\ 
 25-50  & 5.52e-09  & 1.90e-08  & 1.72e-08  & 1.12e-08  & -1.28e-10  & -4.83e-09  & -7.02e-09  & -4.66e-09  & -5.13e-09  & -2.59e-09  & -1.87e-09  & -1.51e-09  & -4.57e-10  & -1.30e-11  & -3.32e-11  \\ 
 50-75  & 5.68e-09  & 1.72e-08  & 2.62e-08  & 1.28e-08  & -1.45e-10  & -5.84e-09  & -7.42e-09  & -5.62e-09  & -6.38e-09  & -4.20e-09  & -2.61e-09  & -1.85e-09  & -7.18e-10  & -2.02e-10  & -5.22e-11  \\ 
 75-105  & 3.97e-09  & 1.12e-08  & 1.28e-08  & 1.39e-08  & 6.17e-10  & -2.21e-09  & -4.95e-09  & -3.40e-09  & -3.76e-09  & -2.17e-09  & -1.59e-09  & -1.27e-09  & -4.72e-10  & -9.56e-11  & -4.43e-11  \\ 
 105-135  & 3.79e-10  & -1.28e-10  & -1.45e-10  & 6.17e-10  & 7.57e-09  & 2.77e-09  & 6.11e-10  & 9.98e-10  & -6.14e-10  & 2.15e-10  & -2.74e-10  & -2.95e-10  & -1.78e-10  & 1.00e-10  & -2.77e-11  \\ 
 135-165  & -1.18e-09  & -4.83e-09  & -5.84e-09  & -2.21e-09  & 2.77e-09  & 8.28e-09  & 4.05e-09  & 3.73e-09  & 2.57e-09  & 2.27e-09  & 9.70e-10  & 6.91e-10  & 2.40e-10  & 3.37e-10  & 1.31e-11  \\ 
 165-195  & -2.21e-09  & -7.02e-09  & -7.42e-09  & -4.95e-09  & 6.11e-10  & 4.05e-09  & 6.19e-09  & 3.93e-09  & 2.86e-09  & 2.08e-09  & 1.12e-09  & 9.91e-10  & 3.22e-10  & 2.74e-10  & 2.68e-11  \\ 
 195-230  & -1.29e-09  & -4.66e-09  & -5.62e-09  & -3.40e-09  & 9.98e-10  & 3.73e-09  & 3.93e-09  & 5.71e-09  & 2.88e-09  & 3.04e-09  & 1.44e-09  & 9.67e-10  & 4.52e-10  & 5.21e-10  & 3.45e-11  \\ 
 230-265  & -1.67e-09  & -5.13e-09  & -6.38e-09  & -3.76e-09  & -6.14e-10  & 2.57e-09  & 2.86e-09  & 2.88e-09  & 3.20e-09  & 2.04e-09  & 1.11e-09  & 8.55e-10  & 3.50e-10  & 2.46e-10  & 2.94e-11  \\ 
 265-300  & -6.67e-10  & -2.59e-09  & -4.20e-09  & -2.17e-09  & 2.15e-10  & 2.27e-09  & 2.08e-09  & 3.04e-09  & 2.04e-09  & 2.80e-09  & 1.10e-09  & 6.58e-10  & 3.70e-10  & 3.94e-10  & 2.79e-11  \\ 
 300-350  & -5.91e-10  & -1.87e-09  & -2.61e-09  & -1.59e-09  & -2.74e-10  & 9.70e-10  & 1.12e-09  & 1.44e-09  & 1.11e-09  & 1.10e-09  & 7.25e-10  & 3.92e-10  & 1.91e-10  & 1.66e-10  & 1.79e-11  \\ 
 350-400  & -4.89e-10  & -1.51e-09  & -1.85e-09  & -1.27e-09  & -2.95e-10  & 6.91e-10  & 9.91e-10  & 9.67e-10  & 8.55e-10  & 6.58e-10  & 3.92e-10  & 4.23e-10  & 1.31e-10  & 1.06e-10  & 1.49e-11  \\ 
 400-450  & -1.38e-10  & -4.57e-10  & -7.18e-10  & -4.72e-10  & -1.78e-10  & 2.40e-10  & 3.22e-10  & 4.52e-10  & 3.50e-10  & 3.70e-10  & 1.91e-10  & 1.31e-10  & 1.15e-10  & 6.03e-11  & 7.12e-12  \\ 
 450-500  & 4.26e-11  & -1.30e-11  & -2.02e-10  & -9.56e-11  & 1.00e-10  & 3.37e-10  & 2.74e-10  & 5.21e-10  & 2.46e-10  & 3.94e-10  & 1.66e-10  & 1.06e-10  & 6.03e-11  & 1.10e-10  & 5.59e-12  \\ 
 500-1000  & -1.11e-11  & -3.32e-11  & -5.22e-11  & -4.43e-11  & -2.77e-11  & 1.31e-11  & 2.68e-11  & 3.45e-11  & 2.94e-11  & 2.79e-11  & 1.79e-11  & 1.49e-11  & 7.12e-12  & 5.59e-12  & 1.35e-12  \\ 
\end{tabular} 



==> tables/correlations/resolved/relXs_covariance_tt_absrap_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrrrrrrrrrr}
bin  &  0.0-0.1  &  0.1-0.2  &  0.2-0.3  &  0.3-0.4  &  0.4-0.5  &  0.5-0.6  &  0.6-0.7  &  0.7-0.8  &  0.8-0.9  &  0.9-1.0  &  1.0-1.1  &  1.1-1.2  &  1.2-1.3  &  1.3-1.4  &  1.4-1.5  &  1.5-1.6  &  1.6-1.8  &  1.8-2.5   \\ \hline
 0.0-0.1  & 3.19e-04  & 1.06e-04  & 1.51e-04  & 1.26e-05  & 9.64e-05  & 1.26e-04  & 3.84e-05  & 6.55e-05  & -3.43e-05  & 2.38e-05  & 1.11e-05  & 1.09e-05  & -1.12e-06  & -1.75e-05  & 1.44e-05  & -1.15e-05  & -9.25e-07  & 8.06e-07  \\ 
 0.1-0.2  & 1.06e-04  & 2.79e-04  & 2.23e-04  & 1.55e-05  & 9.46e-05  & 1.07e-04  & 5.95e-05  & 5.13e-05  & -2.71e-05  & 2.47e-05  & 2.55e-05  & 2.08e-05  & -1.40e-05  & 4.40e-06  & 1.21e-05  & -1.90e-06  & -2.19e-06  & 5.60e-07  \\ 
 0.2-0.3  & 1.51e-04  & 2.23e-04  & 5.08e-04  & 3.93e-05  & 1.53e-04  & 1.83e-04  & 5.57e-05  & 1.54e-04  & -6.71e-06  & 7.50e-05  & 5.20e-05  & 5.18e-05  & 2.98e-05  & 5.16e-05  & 4.93e-05  & 7.44e-06  & 1.62e-05  & 3.63e-06  \\ 
 0.3-0.4  & 1.26e-05  & 1.55e-05  & 3.93e-05  & 2.37e-04  & 6.82e-05  & 3.34e-05  & 6.03e-05  & 6.19e-05  & 5.92e-06  & 8.42e-06  & -1.39e-05  & 9.98e-06  & -2.33e-05  & -2.47e-05  & 9.08e-06  & -3.76e-06  & 4.42e-06  & 7.72e-07  \\ 
 0.4-0.5  & 9.64e-05  & 9.46e-05  & 1.53e-04  & 6.82e-05  & 2.53e-04  & 1.16e-04  & 1.19e-05  & 1.05e-04  & 2.56e-05  & 4.61e-05  & 1.41e-05  & 3.25e-05  & 2.29e-05  & 1.93e-05  & 2.80e-05  & 4.17e-06  & 1.48e-05  & 2.20e-06  \\ 
 0.5-0.6  & 1.26e-04  & 1.07e-04  & 1.83e-04  & 3.34e-05  & 1.16e-04  & 3.16e-04  & 1.08e-04  & 1.54e-04  & -3.33e-05  & 7.26e-05  & 1.72e-05  & 5.21e-05  & 1.26e-05  & 4.47e-06  & 7.00e-05  & 2.16e-06  & 1.73e-05  & 4.10e-06  \\ 
 0.6-0.7  & 3.84e-05  & 5.95e-05  & 5.57e-05  & 6.03e-05  & 1.19e-05  & 1.08e-04  & 1.96e-04  & 7.15e-05  & -4.99e-05  & 1.87e-05  & 6.98e-06  & 3.01e-05  & -1.71e-05  & -1.37e-05  & 2.65e-05  & 3.24e-06  & 2.81e-06  & 9.41e-07  \\ 
 0.7-0.8  & 6.55e-05  & 5.13e-05  & 1.54e-04  & 6.19e-05  & 1.05e-04  & 1.54e-04  & 7.15e-05  & 3.21e-04  & 2.55e-05  & 6.98e-05  & 5.83e-06  & 5.85e-05  & 5.13e-05  & 2.74e-05  & 8.63e-05  & 8.52e-06  & 3.38e-05  & 5.74e-06  \\ 
 0.8-0.9  & -3.43e-05  & -2.71e-05  & -6.71e-06  & 5.92e-06  & 2.56e-05  & -3.33e-05  & -4.99e-05  & 2.55e-05  & 1.28e-04  & 1.81e-05  & -1.71e-05  & -1.00e-06  & 3.01e-05  & 2.30e-05  & -3.10e-07  & 8.83e-06  & 1.10e-05  & 8.27e-07  \\ 
 0.9-1.0  & 2.38e-05  & 2.47e-05  & 7.50e-05  & 8.42e-06  & 4.61e-05  & 7.26e-05  & 1.87e-05  & 6.98e-05  & 1.81e-05  & 1.07e-04  & 2.18e-05  & 1.69e-05  & 2.53e-05  & 2.75e-05  & 3.76e-05  & 1.07e-05  & 1.60e-05  & 2.58e-06  \\ 
 1.0-1.1  & 1.11e-05  & 2.55e-05  & 5.20e-05  & -1.39e-05  & 1.41e-05  & 1.72e-05  & 6.98e-06  & 5.83e-06  & -1.71e-05  & 2.18e-05  & 7.42e-05  & 2.01e-05  & -4.08e-06  & 1.86e-05  & 1.06e-05  & 6.35e-06  & 4.17e-06  & 6.09e-07  \\ 
 1.1-1.2  & 1.09e-05  & 2.08e-05  & 5.18e-05  & 9.98e-06  & 3.25e-05  & 5.21e-05  & 3.01e-05  & 5.85e-05  & -1.00e-06  & 1.69e-05  & 2.01e-05  & 8.17e-05  & 2.14e-05  & 1.34e-05  & 2.40e-05  & 1.12e-05  & 1.04e-05  & 1.61e-06  \\ 
 1.2-1.3  & -1.12e-06  & -1.40e-05  & 2.98e-05  & -2.33e-05  & 2.29e-05  & 1.26e-05  & -1.71e-05  & 5.13e-05  & 3.01e-05  & 2.53e-05  & -4.08e-06  & 2.14e-05  & 8.14e-05  & 3.57e-05  & 1.41e-05  & 1.05e-05  & 1.54e-05  & 1.76e-06  \\ 
 1.3-1.4  & -1.75e-05  & 4.40e-06  & 5.16e-05  & -2.47e-05  & 1.93e-05  & 4.47e-06  & -1.37e-05  & 2.74e-05  & 2.30e-05  & 2.75e-05  & 1.86e-05  & 1.34e-05  & 3.57e-05  & 8.07e-05  & 2.03e-05  & 1.35e-05  & 1.18e-05  & 1.62e-06  \\ 
 1.4-1.5  & 1.44e-05  & 1.21e-05  & 4.93e-05  & 9.08e-06  & 2.80e-05  & 7.00e-05  & 2.65e-05  & 8.63e-05  & -3.10e-07  & 3.76e-05  & 1.06e-05  & 2.40e-05  & 1.41e-05  & 2.03e-05  & 6.64e-05  & 9.29e-06  & 1.24e-05  & 2.44e-06  \\ 
 1.5-1.6  & -1.15e-05  & -1.90e-06  & 7.44e-06  & -3.76e-06  & 4.17e-06  & 2.16e-06  & 3.24e-06  & 8.52e-06  & 8.83e-06  & 1.07e-05  & 6.35e-06  & 1.12e-05  & 1.05e-05  & 1.35e-05  & 9.29e-06  & 2.71e-05  & 3.94e-06  & 4.07e-07  \\ 
 1.6-1.8  & -9.25e-07  & -2.19e-06  & 1.62e-05  & 4.42e-06  & 1.48e-05  & 1.73e-05  & 2.81e-06  & 3.38e-05  & 1.10e-05  & 1.60e-05  & 4.17e-06  & 1.04e-05  & 1.54e-05  & 1.18e-05  & 1.24e-05  & 3.94e-06  & 1.25e-05  & 9.47e-07  \\ 
 1.8-2.5  & 8.06e-07  & 5.60e-07  & 3.63e-06  & 7.72e-07  & 2.20e-06  & 4.10e-06  & 9.41e-07  & 5.74e-06  & 8.27e-07  & 2.58e-06  & 6.09e-07  & 1.61e-06  & 1.76e-06  & 1.62e-06  & 2.44e-06  & 4.07e-07  & 9.47e-07  & 3.39e-07  \\ 
\end{tabular} 



==> tables/correlations/resolved/relXs_covariance_tt_m_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrrrrrrr}
bin $[{\textrm GeV}]$  &  225-345  &  345-420  &  420-500  &  500-590  &  590-685  &  685-790  &  790-910  &  910-1040  &  1040-1175  &  1175-1320  &  1320-3000   \\ \hline
 225-345  & 4.41e-09  & 5.25e-09  & -2.89e-09  & -3.55e-09  & -1.69e-09  & -8.63e-10  & -9.50e-11  & -7.97e-11  & 1.40e-11  & 2.58e-11  & 2.57e-11  \\ 
 345-420  & 5.25e-09  & 1.73e-08  & 2.21e-09  & -3.26e-09  & -2.98e-09  & -2.47e-09  & -8.18e-10  & -8.11e-10  & -4.22e-10  & -1.58e-10  & -1.25e-11  \\ 
 420-500  & -2.89e-09  & 2.21e-09  & 6.88e-09  & 3.55e-09  & 5.65e-10  & -3.53e-10  & -6.43e-10  & -5.21e-10  & -3.69e-10  & -1.94e-10  & -5.39e-11  \\ 
 500-590  & -3.55e-09  & -3.26e-09  & 3.55e-09  & 4.15e-09  & 1.60e-09  & 8.52e-10  & 1.39e-10  & 7.45e-11  & -2.53e-11  & -4.56e-11  & -2.22e-11  \\ 
 590-685  & -1.69e-09  & -2.98e-09  & 5.65e-10  & 1.60e-09  & 1.45e-09  & 9.60e-10  & 4.70e-10  & 3.66e-10  & 1.78e-10  & 8.28e-11  & 1.28e-11  \\ 
 685-790  & -8.63e-10  & -2.47e-09  & -3.53e-10  & 8.52e-10  & 9.60e-10  & 1.15e-09  & 5.71e-10  & 4.05e-10  & 2.13e-10  & 1.16e-10  & 2.00e-11  \\ 
 790-910  & -9.50e-11  & -8.18e-10  & -6.43e-10  & 1.39e-10  & 4.70e-10  & 5.71e-10  & 5.31e-10  & 3.18e-10  & 1.86e-10  & 9.36e-11  & 2.19e-11  \\ 
 910-1040  & -7.97e-11  & -8.11e-10  & -5.21e-10  & 7.45e-11  & 3.66e-10  & 4.05e-10  & 3.18e-10  & 2.61e-10  & 1.38e-10  & 6.76e-11  & 1.61e-11  \\ 
 1040-1175  & 1.40e-11  & -4.22e-10  & -3.69e-10  & -2.53e-11  & 1.78e-10  & 2.13e-10  & 1.86e-10  & 1.38e-10  & 1.03e-10  & 4.27e-11  & 1.04e-11  \\ 
 1175-1320  & 2.58e-11  & -1.58e-10  & -1.94e-10  & -4.56e-11  & 8.28e-11  & 1.16e-10  & 9.36e-11  & 6.76e-11  & 4.27e-11  & 3.49e-11  & 5.28e-12  \\ 
 1320-3000  & 2.57e-11  & -1.25e-11  & -5.39e-11  & -2.22e-11  & 1.28e-11  & 2.00e-11  & 2.19e-11  & 1.61e-11  & 1.04e-11  & 5.28e-12  & 1.59e-12  \\ 
\end{tabular} 



==> tables/correlations/resolved/relXs_covariance_tt_pt_co.res_13TeV.tex <==

\footnotesize 
\centering 
\begin{tabular}{r|rrrrrr}
bin $[{\textrm GeV}]$  &  0-35  &  35-75  &  75-125  &  125-170  &  170-225  &  225-800   \\ \hline
 0-35  & 1.10e-06  & -3.36e-08  & -1.04e-07  & -5.63e-08  & -1.61e-08  & -5.22e-10  \\ 
 35-75  & -3.36e-08  & 1.00e-07  & 1.06e-07  & 2.23e-08  & 1.00e-08  & 2.32e-10  \\ 
 75-125  & -1.04e-07  & 1.06e-07  & 1.30e-07  & 3.30e-08  & 1.39e-08  & 4.62e-10  \\ 
 125-170  & -5.63e-08  & 2.23e-08  & 3.30e-08  & 1.41e-08  & 4.95e-09  & 1.97e-10  \\ 
 170-225  & -1.61e-08  & 1.00e-08  & 1.39e-08  & 4.95e-09  & 2.24e-09  & 8.37e-11  \\ 
 225-800  & -5.22e-10  & 2.32e-10  & 4.62e-10  & 1.97e-10  & 8.37e-11  & 1.06e-11  \\ 
\end{tabular} 



==> tables/rivet/boosted/table_chi2_particle_abs.tex <==
\footnotesize
\centering
\noindent\makebox[\textwidth]{
\begin{tabular}{l | r @{/} l r  | r @{/} l r  }
\hline
  & \multicolumn{3}{c|}{$ p_{\text{T}}^{t,\text{had}}$} & \multicolumn{3}{|c}{$ |y^{t,\text{had}}|$} \\
& \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-val  & \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-val  \\
\hline
\hline
\Powheg{}+\PythiaSix{}&
  {\ } 14.7 & 8 & 0.06 & {\ } 11.0 & 10 & 0.36   \\
\Powheg{}+\PythiaSix{} (radHi)&
 {\ } 19.5 & 8 & 0.01 & {\ } 12.3 & 10 & 0.27   \\
\Powheg{}+\PythiaSix{} (radLo)&
 {\ } 15.0 & 8 & 0.06 & {\ } 10.0 & 10 & 0.44   \\
\mgamcatnlo{}+\herwigpp{} &
 {\ } 17.9 & 8 & 0.02 & {\ } 12.8 & 10 & 0.24   \\
\Powheg{}+\herwigpp{} &
 {\ } 14.1 & 8 & 0.08 & {\ } 8.0 & 10 & 0.63  \\

\mgamcatnlo{}+\PythiaEight{} &
 {\ } 12.8 & 8 & 0.12  & {\ } 20.4 & 10 & 0.03   \\

\Powheg{}+\PythiaEight{} &
 {\ } 16.7 & 8 & 0.03  & {\ } 18.4 & 10 & 0.05   \\

\Powheg{}+\HerwigSeven{} &
 {\ } 11.9 & 8 & 0.15 & {\ } 11.7 & 10 & 0.30    \\

\hline
\end{tabular}}


==> tables/rivet/boosted/table_chi2_particle_rel.tex <==
\footnotesize
\centering
\noindent\makebox[\textwidth]{
\begin{tabular}{l | r @{/} l r  | r @{/} l r }
\hline
  & \multicolumn{3}{c|}{$p_{\text{T}}^{t,\text{had}} $} & \multicolumn{3}{|c}{$ |y^{t,\text{had}}|$} \\
& \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-val  & \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-val  \\
\hline
\hline
\Powheg{}+\PythiaSix{}&
 {\ } 10.2 & 7 & 0.18 & {\ } 2.9 & 9 & 0.97    \\
\Powheg{}+\PythiaSix{} (radHi)&
 {\ } 11.3 & 7 & 0.12 & {\ } 2.9 & 9 & 0.97    \\
\Powheg{}+\PythiaSix{} (radLo)&
 {\ } 11.5 & 7 & 0.12 & {\ } 2.8 & 9 & 0.97   \\
\mgamcatnlo{}+\herwigpp{} &
 {\ } 11.1 & 7 & 0.13 & {\ } 4.6 & 9 & 0.87   \\
\Powheg{}+\herwigpp{} &
 {\ } 10.7 & 7 & 0.15 & {\ } 2.5 & 9 & 0.98   \\
\mgamcatnlo{}+\PythiaEight{}  &
 {\ } 10.9 & 7 & 0.14 & {\ } 7.2 & 9 & 0.62   \\

\Powheg{}+\PythiaEight{} &
 {\ } 11.3 & 7 & 0.13 & {\ } 4.3 & 9 & 0.89   \\
 
\Powheg{}+\HerwigSeven{}&
 {\ } 9.9 & 7 & 0.20 & {\ } 3.6 & 9 & 0.94   \\
\hline
\end{tabular}}


==> tables/rivet/resolved/table_chi2_particle_abs.tex <==
\footnotesize
\centering
\noindent\makebox[\textwidth]{
\begin{tabular}{l | r @{/} l r  | r @{/} l r  | r @{/} l r  | r @{/} l r  | r @{/} l r }
\hline
& \multicolumn{3}{c|}{$p_{\textrm{T}}^{t,\textrm{had}}$} & \multicolumn{3}{|c|}{$  |y^{t,\textrm{had}}|$} & \multicolumn{3}{|c|}{$        m^{t\bar{t}}$}& \multicolumn{3}{|c|}{$p_{\textrm{T}}^{t\bar{t}}$} & \multicolumn{3}{|c}{$      |y^{t\bar{t}}|$} \\
& \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-val  & \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-val  & \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-val  & \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-val  & \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-val  \\
\hline
\hline
\Powheg{}+\PythiaSix{}&
{\ }  19.0 & 15 & 0.22  & {\ } 7.8 & 18 & 0.98  &  {\ } 9.8 & 11 & 0.55  & {\ } 14.9 & 6 & 0.02  &  {\ } 20.0 & 18 & 0.33 \\
\Powheg{}+\PythiaSix{} (radHi)&
{\ } 20.9 & 15 & 0.14  & {\ } 8.5 & 18 & 0.97  &  {\ } 8.7 & 11 & 0.65  & {\ } 56.1 & 6 & $<$0.01  &  {\ } 17.3 & 18 & 0.51 \\
\Powheg{}+\PythiaSix{} (radLo)&
{\ } 20.8 & 15 & 0.14  & {\ } 7.4 & 18 & 0.99  &  {\ } 12.7 & 11 & 0.32  &  {\ } 22.1 & 6 & $<$0.01  &  {\ } 25.5 & 18 & 0.11 \\
\mgamcatnlo{}+\herwigpp{}&
{\ } 23.5 & 15 & 0.07  &   {\ } 10.7 & 18 & 0.91  &  {\ } 32.4 & 11 & $<$0.01& {\ } 16.4 & 6 & 0.01  &  {\ } 28.1 & 18 & 0.06 \\
\Powheg{}+\herwigpp{}&
{\ } 30.3 & 15 & 0.01  & {\ } 7.9 & 18 & 0.98  &  {\ } 34.8 & 11 & $<$0.01  & {\ } 28.0 & 6 & $<$0.01  &  {\ } 30.4 & 18 & 0.03 \\
\mgamcatnlo{}+\PythiaEight{} &
{\ } 19.1 & 15 & 0.21  & {\ } 8.4 & 18 & 0.97  &  {\ }  7.6 & 11 & 0.75  &{\ } 19.0 & 6 & $<$0.01  &  {\ } 16.1 & 18 & 0.59 \\

\Powheg{}+\PythiaEight{} &
{\ } 18.4 & 15 & 0.24  & {\ } 10.5 & 18 & 0.92  &  {\ } 7.7 & 11 & 0.74  & {\ } 11.7 & 6 & 0.07  &  {\ } 12.3 & 18 & 0.83 \\

\Powheg{}+\HerwigSeven{}&
{\ } 13.8 & 15 & 0.54  & {\ } 10.9 & 18 & 0.90  &  {\ }  7.0 & 11 & 0.80  & {\ } 11.6 & 6 & 0.07  &  {\ } 12.8 & 18 & 0.80 \\
\hline
\end{tabular}}


==> tables/rivet/resolved/table_chi2_particle_rel.tex <==
\footnotesize
\centering
\noindent\makebox[\textwidth]{
\begin{tabular}{l | r @{/} l r  | r @{/} l r  | r @{/} l r  | r @{/} l r  | r @{/} l r  }
\hline
Observable  & \multicolumn{3}{c|}{$p_{\textrm{T}}^{t,\textrm{had}}$} & \multicolumn{3}{|c|}{$  |y^{t,\textrm{had}}|$} & \multicolumn{3}{|c|}{$        m^{t\bar{t}}$} & \multicolumn{3}{c|}{$p_{\textrm{T}}^{t\bar{t}}$} & \multicolumn{3}{|c}{$      |y^{t\bar{t}}|$} \\
& \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-val  & \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-val  & \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-val  & \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-val  & \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-val  \\
\hline
\hline
\Powheg{}+\PythiaSix{}&
{\ } 23.0 & 14 & 0.06 &  {\ } 8.1 & 17 & 0.96  &  {\ }  6.3 & 10 & 0.79  & {\ } 7.7 & 5 & 0.17  &  {\ } 22.5 & 17 & 0.17 \\
\Powheg{}+\PythiaSix{} (radHi)&
{\ } 23.8 & 14 & 0.05  & {\ } 8.5 & 17 & 0.95  &  {\ } 7.7 & 10 & 0.66  & {\ } 5.1 & 5 & 0.41  &  {\ } 19.3 & 17 & 0.31 \\
\Powheg{}+\PythiaSix{} (radLo)&
{\ } 25.9 & 14 & 0.03  &{\ } 7.5 & 17 & 0.98  &  {\ } 8.2 & 10 & 0.61  &  {\ } 20.4 & 5 & $<$0.01  &  {\ } 28.0 & 17 & 0.04 \\
\mgamcatnlo{}+\herwigpp{} &
{\ } 24.4 & 14 & 0.04  & {\ } 10.8 & 17 & 0.87  &  {\ } 23.6 & 10 & $<$0.01  & {\ } 2.6 & 5 & 0.76  &  {\ } 30.0 & 17 & 0.03 \\
\Powheg{}+\herwigpp{}&
{\ }24.0 & 14 & 0.05  &   {\ } 7.4 & 17 & 0.98  &  {\ } 37.9 & 10 & $<$0.01  & {\ } 25.0 & 5 & $<$0.01  &  {\ } 32.8 & 17 & 0.01 \\

\mgamcatnlo{}+\PythiaEight{}  &
{\ } 21.8 & 14 & 0.08  &{\ } 7.8 & 17 & 0.97  &  {\ } 6.8 & 10 & 0.75  &  {\ } 3.3 & 5 & 0.66  &  {\ } 18.0 & 17 & 0.39 \\

\Powheg{}+\PythiaEight{} &
{\ } 21.5 & 14 & 0.09  &{\ } 9.6 & 17 & 0.92  &  {\ } 6.5 & 10 & 0.77  &   {\ } 1.1 & 5 & 0.96  &  {\ } 14.0 & 17 & 0.67 \\

\Powheg{}+\HerwigSeven{}&
{\ }15.4 & 14 & 0.35  &  {\ } 9.3 & 17 & 0.93  &  {\ }  6.7 & 10 & 0.76  & {\ } 5.4 & 5 & 0.37  &  {\ } 15.1 & 17 & 0.59 \\
\hline
\end{tabular}}


==> tables/systematics/boosted/table_syst_particle_topH_absrap_AbsoluteDiffXs.tex <==
\resizebox*{!}{\textheight}{
\begin{tabular}{l c c c c c c c c c c}
\hline
Bins  [ Unit $|y^{t}|$ ]
 & 0--0.20   & 0.20--0.40   & 0.40--0.60   & 0.60--0.80   & 0.80--1   & 1--1.20   & 1.20--1.40   & 1.40--1.60   & 1.60--1.80   & 1.80--2  \\
\hline
\hline
d$\sigma$ / d$|y^{t}|$ [pb/ Unit $|y^{t}|$ ]	&	$1.90 \cdot 10^{0}$ &	$1.94 \cdot 10^{0}$ &	$1.71 \cdot 10^{0}$ &	$1.60 \cdot 10^{0}$ &	$1.41 \cdot 10^{0}$ &	$1.29 \cdot 10^{0}$ &	$1.05 \cdot 10^{0}$ &	$8.63 \cdot 10^{-1}$ &	$5.56 \cdot 10^{-1}$ &	$3.58 \cdot 10^{-1}$ \\
\hline
\rowcolor{Gray}
Total uncertainty [\%]	
&	$^{+22.3}_{-20.0}$ &	$\pm$19.6 &	$^{+20.8}_{-21.8}$ &	$^{+21.0}_{-20.6}$ &	$^{+19.9}_{-20.8}$ &	$^{+22.5}_{-21.0}$ &	$^{+23.1}_{-22.2}$ &	$^{+22.4}_{-21.4}$ &	$^{+22.1}_{-25.3}$ &	$^{+25.6}_{-25.3}$ \\
Statistical uncertainty [\%]	
&	$\pm4.0$ &	$\pm4.2$ &	$\pm4.6$ &	$\pm4.7$ &	$\pm4.9$ &	$\pm5.0$ &	$\pm5.6$ &	$\pm6.1$ &	$\pm7.8$ &	$\pm8.6$ \\
\rowcolor{Gray}
Systematic uncertainty [\%]	
&	$^{+21.9}_{-19.6}$ &	$\pm$19.1 &	$^{+20.2}_{-21.3}$ &	$^{+20.3}_{-20.0}$ &	$^{+19.2}_{-20.2}$ &	$^{+21.9}_{-20.3}$ &	$^{+22.3}_{-21.4}$ &	$^{+21.5}_{-20.4}$ &	$^{+20.5}_{-23.9}$ &	$^{+24.0}_{-23.6}$ \\
\hline
\hline
Large-$R$ jet Baseline (JES) [\%]	
&	$^{+10.9}_{-9.53}$ &	$^{+9.63}_{-9.52}$ &	$^{+9.83}_{-9.48}$ &	$^{+10.0}_{-9.26}$ &	$^{+9.48}_{-9.10}$ &	$^{+11.1}_{-9.39}$ &	$^{+10.0}_{-9.87}$ &	$^{+10.5}_{-9.76}$ &	$^{+10.3}_{-11.1}$ &	$^{+11.4}_{-10.4}$ \\
\rowcolor{Gray}
Large-$R$ jet Tracking (JES) [\%]	
&	$^{+13.4}_{-13.1}$ &	$^{+11.8}_{-12.6}$ &	$^{+12.3}_{-12.7}$ &	$^{+12.1}_{-13.5}$ &	$^{+12.6}_{-13.0}$ &	$^{+14.1}_{-12.7}$ &	$\pm$13.0 &	$^{+13.0}_{-13.6}$ &	$^{+12.5}_{-16.0}$ &	{$^{+17.6}_{-15.6}$} \\
Large-$R$ jet Modelling (JES) [\%]	
&	$^{+6.85}_{-6.09}$ &	$^{+5.99}_{-6.20}$ &	$^{+6.22}_{-6.40}$ &	$^{+6.29}_{-5.89}$ &	$^{+5.68}_{-6.21}$ &	$^{+6.79}_{-6.18}$ &	$^{+6.29}_{-6.25}$ &	$^{+6.87}_{-6.13}$ &	$^{+6.56}_{-7.17}$ &	$^{+6.26}_{-6.76}$ \\
\rowcolor{Gray}
Large-$R$ jet CrossCalib $\tau$32 (JES) [\%]	
&	$^{-1.31}_{+0.58}$ &	$^{-1.30}_{+0.74}$ &	$^{-1.51}_{+0.86}$ &	{$^{-1.67}_{+1.16}$} &	$^{-2.10}_{+1.30}$ &	$^{-1.77}_{+1.49}$ &	$^{-3.27}_{+1.90}$ &	$^{-2.40}_{+1.75}$ &	$^{-3.00}_{+1.68}$ &	$^{-1.88}_{+2.06}$ \\
Large-$R$ jet Run1 $\tau$32 (JES) [\%]	
&	$^{-3.79}_{+1.88}$ &	{$^{-3.54}_{+2.49}$} &	$^{-4.90}_{+2.46}$ &	{$^{-5.51}_{+3.26}$} &	$^{-6.73}_{+3.95}$ &	$^{-6.83}_{+5.09}$ &	$^{-9.06}_{+5.59}$ &	$^{-8.11}_{+5.98}$ &	$^{-8.19}_{+5.95}$ &	$^{-7.70}_{+6.06}$ \\
\rowcolor{Gray}
Large-$R$ jet JMR [\%]	
&	$\mp$0.53 &	$\mp$0.45 &	{$\mp$0.61} &	{$\mp$0.40} &	$\mp$0.44 &	{$\mp$1.01} &	$\mp$0.82 &	{$\pm$0.21} &	{$\mp$0.60} &	{$\mp$1.16} \\
$b$-Tagged jet energy scale (JES) [\%]	
&	\textrm - &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{+0.20}$} &	{\textrm -} &	\textrm - &	{\textrm -} &	{$^{+0.19}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	\textrm - &	$^{+0.26}_{-0.10}$ \\
\rowcolor{Gray}
Effective detector NP set 1 (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.74}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.65}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.59}$ &	$^{-0.91}_{\textrm{ \phantom{ai}-}}$ &	$^{\textrm{ \phantom{ai}-}}_{-1.09}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.46}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.29}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.92}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.62}$ &	$^{+0.23}_{-0.77}$ \\
Effective detector NP set 2 (JES) [\%]	
&	$^{+0.36}_{-0.54}$ &	$^{+0.33}_{-0.53}$ &	$^{+0.40}_{-0.33}$ &	$^{+0.50}_{-0.71}$ &	{$^{+0.35}_{-0.50}$} &	{$^{+0.59}_{-0.45}$} &	{$^{+0.44}_{-0.71}$} &	{$^{+0.17}_{-0.40}$} &	{$^{+0.38}_{-0.44}$} &	{$^{+0.51}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Effective detector NP set 3 (JES) [\%]	
&	$^{-0.23}_{+0.20}$ &	{$^{-0.22}_{+0.13}$} &	{$^{-0.26}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.23}_{+0.14}$} &	{$^{-0.25}_{\textrm{ \phantom{ai}-}}$} &	\textrm - &	$^{-0.43}_{\textrm{ \phantom{ai}-}}$ &	{$^{-0.35}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.22}_{+0.13}$} &	{$^{+0.61}_{\textrm{ \phantom{ai}-}}$} \\
Effective detector NP set 4 (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.18}$ &	\textrm - &	$^{+0.20}_{-0.19}$ &	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.20}$ &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Effective detector NP set 5 (JES) [\%]	
&	\textrm - &	{\textrm -} &	{$^{+0.25}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Effective detector NP set 6 restTerm (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
$\eta$ intercalibration model (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.62}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.47}$ &	$^{-0.38}_{\textrm{ \phantom{ai}-}}$ &	$^{-0.53}_{+0.10}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.29}$ &	$^{-0.19}_{+0.17}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.26}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.36}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.32}$ &	{$^{+0.85}_{-0.30}$} \\
$\eta$ intercalibration total stat (JES) [\%]	
&	$^{-0.44}_{+0.28}$ &	$^{-0.24}_{+0.33}$ &	$^{-0.34}_{+0.31}$ &	$^{-0.46}_{+0.27}$ &	{$^{-0.24}_{+0.12}$} &	{$^{-0.30}_{+0.55}$} &	{$^{-0.60}_{+0.21}$} &	{$^{-0.32}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.39}_{+0.36}$} &	{$^{+0.48}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Flavour composition (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.66}$ &	$^{-0.59}_{\textrm{ \phantom{ai}-}}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.48}$ &	$^{-0.75}_{+0.24}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.51}$ &	$^{-0.43}_{+0.24}$ &	$^{-0.63}_{+0.22}$ &	$^{\textrm{ \phantom{ai}-}}_{-1.02}$ &	$^{-0.87}_{\textrm{ \phantom{ai}-}}$ &	$^{+0.31}_{\textrm{ \phantom{ai}-}}$ \\
Flavour response (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.54}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.40}$ &	$^{+0.20}_{-0.51}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.79}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.42}$ &	$^{+0.23}_{-0.36}$ &	{$^{+0.11}_{-0.51}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.85}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.22}$ &	{$^{+0.44}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Pile-up offset $\mu$ (JES) [\%]	
&	$^{+0.10}_{-0.26}$ &	{$^{+0.15}_{-0.17}$} &	$^{+0.12}_{-0.25}$ &	$^{+0.14}_{-0.25}$ &	$^{+0.12}_{-0.19}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.13}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.35}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.21}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.20}$ &	{$^{-0.11}_{+0.78}$} \\
Pile-up offset $N_{\textrm PV}$ (JES) [\%]	
&	$^{+0.15}_{\textrm{ \phantom{ai}-}}$ &	{$^{+0.24}_{\textrm{ \phantom{ai}-}}$} &	$^{+0.19}_{-0.15}$ &	$\pm$0.15 &	$^{+0.16}_{\textrm{ \phantom{ai}-}}$ &	$^{+0.20}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{$^{+0.18}_{-0.22}$} &	\textrm - &	{$^{+0.79}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Pile-up offset $p_{\textrm T}$ (JES) [\%]	
&	$^{-0.10}_{+0.12}$ &	\textrm - &	{$^{-0.11}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	$^{-0.50}_{+0.10}$ \\
Pile-up offset $\rho$ topology (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.71}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.62}$ &	$^{-0.70}_{\textrm{ \phantom{ai}-}}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.87}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.61}$ &	$^{-0.53}_{\textrm{ \phantom{ai}-}}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.57}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.73}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.95}$ &	$^{+0.17}_{-0.31}$ \\
\rowcolor{Gray}
Punch-through (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Single particle high-$p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Jet energy resolution [\%]	
&	$\mp$1.88 &	{$\mp$1.11} &	{$\mp$2.13} &	{$\mp$1.02} &	{$\mp$0.72} &	{$\mp$1.77} &	{$\mp$1.00} &	{$\mp$1.46} &	$\mp$1.34 &	{$\mp$2.06} \\
Jet vertex fraction [\%]	
&	$^{+0.76}_{-0.70}$ &	{$^{+0.56}_{-0.52}$} &	{$^{+0.27}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.43}_{-0.34}$} &	$^{+0.48}_{-0.47}$ &	{$\pm$0.65} &	$^{+0.70}_{-0.63}$ &	{$^{+0.42}_{-0.39}$} &	$^{+0.52}_{-0.48}$ &	$^{+0.44}_{-0.35}$ \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-0.97}_{+0.94}$ &	$^{-0.84}_{+0.80}$ &	$^{-0.88}_{+0.85}$ &	$^{-0.96}_{+0.92}$ &	$^{-0.92}_{+0.88}$ &	$^{-0.91}_{+0.88}$ &	$^{-1.08}_{+1.04}$ &	$^{-1.06}_{+1.03}$ &	$^{-1.03}_{+1.01}$ &	$^{-1.10}_{+1.06}$ \\
$b$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$^{-1.15}_{+1.06}$ &	$^{-1.09}_{+1.01}$ &	$^{-1.14}_{+1.07}$ &	$^{-1.22}_{+1.15}$ &	$^{-1.13}_{+1.04}$ &	$^{-1.14}_{+1.07}$ &	$^{-1.16}_{+1.03}$ &	$^{-1.27}_{+1.22}$ &	$^{-1.13}_{+1.05}$ &	$^{-1.37}_{+1.33}$ \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	{$\mp$0.11} &	$\mp$0.11 &	\textrm - &	\textrm - &	{\textrm -} &	{$\mp$0.15} &	{\textrm -} &	{$\mp$0.15} \\
$b$-Quark tagging efficiency (eigenvector 3) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.21}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.36}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.33}$ &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.33}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.30}$ &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
$c$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-0.53}_{+0.15}$ &	{$^{-0.65}_{+0.30}$} &	$^{-0.62}_{+0.31}$ &	$^{-0.62}_{+0.30}$ &	{$^{-0.50}_{+0.16}$} &	$^{-0.45}_{+0.14}$ &	{$^{-0.69}_{+0.42}$} &	{$^{-0.49}_{+0.18}$} &	$^{-0.48}_{+0.15}$ &	{$^{-0.66}_{+0.27}$} \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	{$\mp$0.18} &	$\mp$0.17 &	$\mp$0.20 &	{\textrm -} &	{$\mp$0.16} &	{\textrm -} &	{$\mp$0.10} &	$\mp$0.13 &	{$\mp$0.24} \\
$c$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 0) [\%]	
&	$^{-1.02}_{+0.99}$ &	{$^{-0.54}_{+0.60}$} &	{$^{-0.83}_{+0.87}$} &	{$^{-1.40}_{+1.44}$} &	{$^{-0.93}_{+0.95}$} &	{$^{-0.56}_{+0.55}$} &	{$^{-1.23}_{+1.22}$} &	{$^{-1.89}_{+2.19}$} &	$^{-2.51}_{+2.47}$ &	{$^{-1.24}_{+1.26}$} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 1) [\%]	
&	$\pm$0.21 &	{$\pm$0.10} &	{$\pm$0.14} &	{\textrm -} &	{$\pm$0.14} &	\textrm - &	\textrm - &	{\textrm -} &	{$\mp$0.22} &	{$\mp$0.14} \\
Light-jet tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\mp$0.20} &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - \\
Light-jet tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 5) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 6) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 7) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - \\
Light-jet tagging efficiency (eigenvector 8) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 9) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 10) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 11) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$b$-Quark tagging  extrapolation  [\%]	
&	$^{+0.95}_{-0.98}$ &	$^{+0.88}_{-0.92}$ &	$^{+0.97}_{-1.00}$ &	$^{+0.91}_{-0.94}$ &	$^{+0.76}_{-0.80}$ &	$^{+0.98}_{-1.02}$ &	$^{+0.86}_{-0.88}$ &	$^{+0.99}_{-1.02}$ &	{$^{+0.70}_{-0.72}$} &	{$^{+1.19}_{-1.22}$} \\
\rowcolor{Gray}
$b$-Quark tagging extrapolation from $c$-Quark [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} \\
Electron energy resolution [\%]	
&	$^{-0.23}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	\textrm - &	$^{-0.32}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.36}$ &	$^{\textrm{ \phantom{ai}-}}_{+0.17}$ &	\textrm - &	$^{-0.20}_{\textrm{ \phantom{ai}-}}$ \\
\rowcolor{Gray}
Electron energy scale [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	$^{-0.21}_{\textrm{ \phantom{ai}-}}$ \\
Electron trigger efficiency [\%]	
&	$\pm$0.31 &	$\pm$0.31 &	$\pm$0.31 &	$\pm$0.32 &	$\pm$0.32 &	$\pm$0.31 &	$\pm$0.32 &	$\pm$0.34 &	$\pm$0.35 &	$\pm$0.34 \\
\rowcolor{Gray}
Electron reconstruction efficiency [\%]	
&	$\pm$0.24 &	$\pm$0.25 &	$\pm$0.25 &	$\pm$0.25 &	$\pm$0.25 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.26 &	$\pm$0.26 &	$\pm$0.25 \\
Electron identification efficiency [\%]	
&	$\pm$0.70 &	$\pm$0.71 &	$\pm$0.70 &	$\pm$0.71 &	$\pm$0.71 &	$\pm$0.69 &	$\pm$0.69 &	$\pm$0.74 &	$\pm$0.71 &	$\pm$0.70 \\
\rowcolor{Gray}
Electron isolation efficiency [\%]	
&	$\pm$0.41 &	$\pm$0.41 &	$\pm$0.41 &	$\pm$0.42 &	$\pm$0.42 &	$\pm$0.40 &	$\pm$0.40 &	$\pm$0.43 &	$\pm$0.40 &	$\pm$0.39 \\
Muon energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon (MS) momentum resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - \\
Muon (ID) momentum resolution [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Muon trigger efficiency stat [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
Muon trigger efficiency syst [\%]	
&	$\pm$0.26 &	$\pm$0.26 &	$\pm$0.26 &	$\pm$0.26 &	$\pm$0.26 &	$\pm$0.25 &	$^{+0.28}_{-0.27}$ &	$\pm$0.25 &	$\pm$0.26 &	$\pm$0.25 \\
\rowcolor{Gray}
Muon identification stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon identification syst [\%]	
&	$\pm$0.33 &	$^{+0.33}_{-0.32}$ &	$\pm$0.33 &	$\pm$0.33 &	$\pm$0.33 &	$\pm$0.32 &	$\pm$0.35 &	$\pm$0.31 &	$\pm$0.37 &	$\pm$0.32 \\
\rowcolor{Gray}
Muon isolation efficiency stat [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
Muon isolation efficiency syst [\%]	
&	$\pm$0.12 &	$\pm$0.12 &	$\pm$0.12 &	$\pm$0.12 &	$\pm$0.12 &	$\pm$0.11 &	$\pm$0.12 &	$\pm$0.11 &	$\pm$0.12 &	$\pm$0.11 \\
\rowcolor{Gray}
Muon TTVA efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon TTVA efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution para [\%]	
&	$\pm$0.12 &	{\textrm -} &	\textrm - &	\textrm - &	{$\mp$0.27} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.13} \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution perp [\%]	
&	$\mp$0.48 &	{$\mp$0.31} &	{$\mp$0.52} &	{$\mp$0.34} &	{$\mp$0.49} &	$\mp$0.43 &	{$\mp$0.30} &	{$\mp$0.18} &	$\mp$0.22 &	{$\mp$0.40} \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet scale [\%]	
&	$^{-0.22}_{+0.10}$ &	{$^{-0.22}_{+0.14}$} &	$^{-0.20}_{\textrm{ \phantom{ai}-}}$ &	$^{-0.26}_{\textrm{ \phantom{ai}-}}$ &	{$^{-0.36}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.35}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.17}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.31}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.24}$ \\
Luminosity [\%]	
&	$\mp$2.05 &	$\mp$2.05 &	$\mp$2.05 &	$\mp$2.05 &	$\mp$2.05 &	$\mp$2.05 &	$\mp$2.05 &	$\mp$2.05 &	$\mp$2.05 &	$\mp$2.05 \\
\rowcolor{Gray}
$W$+jets $CA_{3ex}$ stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
$W$+jets $CA_{2ex}$ stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$W$+jets $CA_{4incl}$ stat error [\%]	
&	$\pm$0.18 &	$\pm$0.17 &	$\pm$0.19 &	$\pm$0.23 &	{$\pm$0.16} &	$\pm$0.17 &	$\pm$0.21 &	$\pm$0.22 &	$\pm$0.24 &	$\pm$0.20 \\
$W$+jets Fcc stat error [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.13}$ &	{$^{+0.10}_{-0.18}$} &	{$^{+0.16}_{-0.27}$} &	{$^{-0.12}_{+0.20}$} &	{\textrm -} &	{$^{+0.19}_{-0.33}$} &	{$^{-0.52}_{+0.87}$} &	{$^{-0.12}_{+0.21}$} &	$^{-0.11}_{+0.20}$ &	$^{-0.14}_{+0.24}$ \\
\rowcolor{Gray}
$W$+jets Flight stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$W$+jets Fc  error [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{$^{+0.10}_{-0.11}$} &	{\textrm -} &	{$^{-0.11}_{+0.12}$} &	$^{+0.12}_{-0.13}$ \\
\rowcolor{Gray}
QCD norm. impact on $W$+jets [\%]	
&	$^{+0.94}_{-1.04}$ &	{$^{+0.70}_{-0.77}$} &	{$^{+1.04}_{-1.15}$} &	$^{+0.80}_{-0.87}$ &	{$^{+0.61}_{-0.66}$} &	{$^{+0.91}_{-1.00}$} &	{$^{+0.40}_{-0.44}$} &	{$^{+0.97}_{-1.08}$} &	{$^{+1.37}_{-1.50}$} &	{$^{+0.63}_{-0.73}$} \\
Single top cross-section [\%]	
&	$\pm$0.37 &	$\pm$0.35 &	$\pm$0.36 &	$\pm$0.33 &	$\pm$0.35 &	$\pm$0.33 &	$\pm$0.31 &	$\pm$0.32 &	$\pm$0.33 &	$\pm$0.31 \\
\rowcolor{Gray}
$Z$+jets cross-section [\%]	
&	$\pm$0.20 &	{$\pm$0.33} &	{$\pm$0.18} &	{$\pm$0.51} &	$\pm$0.52 &	{$\pm$0.17} &	{$\pm$0.43} &	$\pm$0.47 &	{$\pm$0.78} &	{$\pm$0.11} \\
Diboson cross-section [\%]	
&	$\pm$0.30 &	$\pm$0.29 &	$\pm$0.28 &	$\pm$0.29 &	$\pm$0.34 &	$\pm$0.32 &	$\pm$0.26 &	{$\pm$0.40} &	$\pm$0.33 &	$\pm$0.34 \\
\rowcolor{Gray}
$t\bar{t}V$ cross-section [\%]	
&	$\pm$0.15 &	$\pm$0.14 &	$\pm$0.14 &	$\pm$0.14 &	$\pm$0.14 &	$\pm$0.14 &	$\pm$0.14 &	$\pm$0.14 &	$\pm$0.13 &	$\pm$0.12 \\
Monte Carlo sample statistics [\%]	
&	$\pm$1.09 &	$\pm$1.14 &	$\pm$1.26 &	{$\pm$1.69} &	$\pm$1.39 &	$\pm$1.40 &	{$\pm$2.41} &	$\pm$1.92 &	{$\pm$3.10} &	$\pm$2.79 \\
\rowcolor{Gray}
ISR/FSR + scale [\%]	
&	$^{-0.62}_{+8.00}$ &	{$^{-0.68}_{+5.43}$} &	{$^{-4.90}_{+3.03}$} &	{$^{-3.60}_{+8.49}$} &	{$^{-1.86}_{+3.36}$} &	{$^{-4.58}_{+4.84}$} &	{$^{+9.95}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.74}_{+8.30}$} &	{$^{-2.48}_{+5.06}$} &	{$^{-6.78}_{+0.46}$} \\
Alternate hard-scattering model [\%]	
&	$\pm$2.75 &	{$\pm$1.55} &	{$\pm$4.30} &	{$\pm$0.31} &	{$\mp$3.43} &	{$\pm$1.79} &	{$\pm$5.90} &	{$\mp$0.11} &	{$\mp$0.98} &	{$\mp$2.12} \\
\rowcolor{Gray}
Alternate parton-shower model [\%]	
&	$\mp$6.30 &	$\mp$6.75 &	$\mp$8.35 &	{$\mp$5.20} &	$\mp$6.09 &	$\mp$5.82 &	{$\mp$0.47} &	{$\mp$1.66} &	{$\mp$4.72} &	$\mp$4.88 \\
Inter PDF [\%]	
&	$\pm$0.32 &	{\textrm -} &	{$\pm$0.20} &	{$\pm$0.39} &	{$\pm$0.22} &	{\textrm -} &	{$\pm$0.36} &	{$\pm$0.82} &	{$\pm$0.24} &	{\textrm -} \\
\rowcolor{Gray}
Intra PDF [\%]	
&	$\pm$0.22 &	$\pm$0.26 &	{$\pm$0.15} &	{$\pm$0.29} &	{$\pm$0.21} &	{$\pm$0.29} &	$\pm$0.35 &	$\pm$0.38 &	{$\pm$0.71} &	{$\pm$1.10} \\
Real lepton efficiency stat [\%]	
&	$^{+0.34}_{-0.48}$ &	$^{+0.36}_{-0.52}$ &	$^{+0.32}_{-0.48}$ &	$^{+0.35}_{-0.55}$ &	$^{+0.34}_{-0.49}$ &	$^{+0.31}_{-0.40}$ &	$^{+0.29}_{-0.38}$ &	$^{+0.34}_{-0.48}$ &	$^{+0.27}_{-0.34}$ &	{$^{+0.51}_{-0.91}$} \\
\rowcolor{Gray}
Fake lepton efficiency MC scale [\%]	
&	$^{-0.62}_{+0.53}$ &	$^{-0.78}_{+0.68}$ &	$^{-1.03}_{+0.84}$ &	$^{-1.01}_{+0.86}$ &	$^{-0.80}_{+0.76}$ &	{$^{-0.36}_{+0.24}$} &	{$^{-1.78}_{+1.56}$} &	{$^{-0.88}_{+0.84}$} &	$^{-1.19}_{+0.97}$ &	{$^{+0.16}_{-0.14}$} \\
Fake lepton efficiency alternate CR [\%]	
&	$\pm$0.17 &	$\mp$0.21 &	{$\pm$0.29} &	{$\mp$0.17} &	$\pm$0.18 &	$\pm$0.16 &	{$\pm$0.62} &	{$\pm$0.41} &	{$\pm$0.23} &	{$\pm$1.02} \\
\rowcolor{Gray}
Poor MTW Modelling in QCD [\%]	
&	$\mp$0.31 &	$\mp$0.28 &	{$\mp$1.13} &	{$\mp$0.46} &	{$\mp$0.64} &	{$\mp$0.30} &	{$\mp$0.87} &	{$\mp$0.40} &	{$\mp$2.03} &	{$\mp$0.44} \\
\hline
\end{tabular}}


==> tables/systematics/boosted/table_syst_particle_topH_absrap_RelativeDiffXs.tex <==
\resizebox*{!}{\textheight}{
\begin{tabular}{l c c c c c c c c c c}
\hline
Bins  [ Unit $|y^{t}|$ ]
 & 0--0.20   & 0.20--0.40   & 0.40--0.60   & 0.60--0.80   & 0.80--1   & 1--1.20   & 1.20--1.40   & 1.40--1.60   & 1.60--1.80   & 1.80--2  \\
\hline
\hline
1/$\sigma$ $\cdot$ d$\sigma$ / d$|y^{t}|$	&	$7.50 \cdot 10^{-1}$ &	$7.64 \cdot 10^{-1}$ &	$6.76 \cdot 10^{-1}$ &	$6.31 \cdot 10^{-1}$ &	$5.56 \cdot 10^{-1}$ &	$5.09 \cdot 10^{-1}$ &	$4.14 \cdot 10^{-1}$ &	$3.40 \cdot 10^{-1}$ &	$2.19 \cdot 10^{-1}$ &	$1.41 \cdot 10^{-1}$ \\
\hline
\rowcolor{Gray}
Total uncertainty [\%]	
&	$^{+5.35}_{-4.62}$ &	$^{+5.37}_{-4.75}$ &	$^{+6.34}_{-6.94}$ &	$^{+5.59}_{-5.67}$ &	$^{+7.01}_{-7.56}$ &	$^{+6.00}_{-5.77}$ &	$^{+10.2}_{-10.1}$ &	$^{+8.69}_{-8.28}$ &	$^{+9.27}_{-10.3}$ &	$^{+11.5}_{-11.8}$ \\
Statistical uncertainty [\%]	
&	$\pm3.7$ &	$\pm4.0$ &	$\pm4.3$ &	$\pm4.5$ &	$\pm4.7$ &	$\pm4.8$ &	$\pm5.4$ &	$\pm5.9$ &	$\pm7.7$ &	$\pm8.5$ \\
\rowcolor{Gray}
Systematic uncertainty [\%]	
&	$^{+3.68}_{-2.50}$ &	$^{+3.39}_{-2.29}$ &	$^{+4.42}_{-5.24}$ &	$^{+2.90}_{-3.05}$ &	$^{+5.02}_{-5.76}$ &	$^{+3.32}_{-2.89}$ &	$^{+8.31}_{-8.25}$ &	$^{+6.00}_{-5.38}$ &	$^{+4.13}_{-6.20}$ &	$^{+7.28}_{-7.67}$ \\
\hline
\hline
Large-$R$ jet Baseline (JES) [\%]	
&	$^{+0.67}_{\textrm{ \phantom{ai}-}}$ &	$^{-0.52}_{\textrm{ \phantom{ai}-}}$ &	{$^{-0.34}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.14}_{+0.33}$} &	{$^{-0.65}_{+0.51}$} &	{$^{+0.86}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.33}$} &	$^{+0.28}_{-0.22}$ &	{$^{\textrm{ \phantom{ai}-}}_{-1.73}$} &	{$^{+1.13}_{-0.94}$} \\
\rowcolor{Gray}
Large-$R$ jet Tracking (JES) [\%]	
&	$^{+0.55}_{\textrm{ \phantom{ai}-}}$ &	{$^{-0.87}_{+0.65}$} &	$^{-0.45}_{+0.54}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.61}$ &	$^{-0.20}_{+0.24}$ &	{$^{+1.10}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	$^{+0.15}_{-0.48}$ &	$^{\textrm{ \phantom{ai}-}}_{-3.23}$ &	{$^{+4.26}_{-2.73}$} \\
Large-$R$ jet Modelling (JES) [\%]	
&	$^{+0.47}_{\textrm{ \phantom{ai}-}}$ &	{$^{-0.33}_{\textrm{ \phantom{ai}-}}$} &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{+0.36}$} &	{$^{-0.63}_{\textrm{ \phantom{ai}-}}$} &	$^{+0.41}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{$^{+0.49}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.19}_{-1.00}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.57}$ \\
\rowcolor{Gray}
Large-$R$ jet CrossCalib $\tau$32 (JES) [\%]	
&	$^{+0.54}_{-0.57}$ &	$^{+0.55}_{-0.41}$ &	{$^{+0.33}_{-0.29}$} &	{\textrm -} &	$^{-0.26}_{+0.14}$ &	$^{+0.32}_{\textrm{ \phantom{ai}-}}$ &	{$^{-1.45}_{+0.73}$} &	$^{-0.57}_{+0.58}$ &	$^{-1.18}_{+0.51}$ &	{$^{\textrm{ \phantom{ai}-}}_{+0.88}$} \\
Large-$R$ jet Run1 $\tau$32 (JES) [\%]	
&	$^{+2.10}_{-1.69}$ &	$^{+2.36}_{-1.10}$ &	{$^{+0.92}_{-1.13}$} &	{$^{+0.27}_{-0.36}$} &	$^{-1.01}_{+0.30}$ &	{$^{-1.13}_{+1.40}$} &	{$^{-3.48}_{+1.88}$} &	$^{-2.48}_{+2.26}$ &	$^{-2.57}_{+2.23}$ &	$^{-2.05}_{+2.34}$ \\
\rowcolor{Gray}
Large-$R$ jet JMR [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{$\pm$0.14} &	{\textrm -} &	{$\mp$0.46} &	{$\mp$0.28} &	{$\pm$0.76} &	{\textrm -} &	{$\mp$0.61} \\
$b$-Tagged jet energy scale (JES) [\%]	
&	\textrm - &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{+0.19}$} &	{\textrm -} &	\textrm - &	\textrm - &	$^{+0.16}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{\textrm -} &	$^{+0.24}_{-0.11}$ \\
\rowcolor{Gray}
Effective detector NP set 1 (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.22}$ &	$^{-0.12}_{+0.11}$ &	{$^{+0.14}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.38}_{+0.54}$} &	$^{+0.29}_{-0.57}$ &	$^{+0.23}_{\textrm{ \phantom{ai}-}}$ &	$^{+0.29}_{\textrm{ \phantom{ai}-}}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.39}$ &	\textrm - &	{$^{+0.76}_{-0.25}$} \\
Effective detector NP set 2 (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{-0.21}$} &	\textrm - &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{-0.20}$} &	$^{-0.22}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{$^{+0.91}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Effective detector NP set 3 (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.20}$ &	\textrm - &	\textrm - &	{$^{+0.84}_{\textrm{ \phantom{ai}-}}$} \\
Effective detector NP set 4 (JES) [\%]	
&	\textrm - &	{\textrm -} &	{$^{+0.21}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{\textrm -} &	{$^{-0.13}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Effective detector NP set 5 (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Effective detector NP set 6 restTerm (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$^{+0.14}_{-0.10}$} \\
\rowcolor{Gray}
$\eta$ intercalibration model (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.25}$ &	\textrm - &	{\textrm -} &	$^{-0.16}_{+0.14}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.14}$ &	{$^{+0.21}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.28}$ &	{$^{+0.31}_{-0.27}$} &	{$^{+1.23}_{-0.26}$} \\
$\eta$ intercalibration total stat (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	$^{+0.10}_{-0.16}$ &	{$^{+0.26}_{\textrm{ \phantom{ai}-}}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.25}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.21}$ &	\textrm - &	{$^{+0.83}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Flavour composition (JES) [\%]	
&	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.23}$ &	{$^{-0.17}_{+0.31}$} &	{$^{+0.28}_{-0.45}$} &	$^{+0.31}_{\textrm{ \phantom{ai}-}}$ &	{$^{\textrm{ \phantom{ai}-}}_{+0.28}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.43}$ &	$^{-0.29}_{+0.10}$ &	{$^{+0.90}_{\textrm{ \phantom{ai}-}}$} \\
Flavour response (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.30}$} &	$^{-0.18}_{\textrm{ \phantom{ai}-}}$ &	$^{+0.20}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.35}$ &	$^{\textrm{ \phantom{ai}-}}_{+0.27}$ &	{$^{+0.95}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Pile-up offset $\mu$ (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$^{-0.21}_{+0.99}$} \\
Pile-up offset $N_{\textrm PV}$ (JES) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{$^{+0.88}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Pile-up offset $p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.24}$ &	\textrm - &	\textrm - &	$^{-0.41}_{\textrm{ \phantom{ai}-}}$ \\
Pile-up offset $\rho$ topology (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{$^{-0.20}_{+0.12}$} &	\textrm - &	{$^{+0.21}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.24}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.29}$ &	{$^{+0.85}_{-0.15}$} \\
\rowcolor{Gray}
Punch-through (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
Single particle high-$p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Jet energy resolution [\%]	
&	$\mp$0.45 &	{$\pm$0.31} &	{$\mp$0.72} &	{$\pm$0.41} &	{$\pm$0.71} &	{$\mp$0.35} &	$\pm$0.42 &	{\textrm -} &	{\textrm -} &	{$\mp$0.64} \\
Jet vertex fraction [\%]	
&	$^{+0.22}_{-0.25}$ &	{\textrm -} &	{$^{-0.25}_{+0.48}$} &	{$\mp$0.10} &	{\textrm -} &	$^{+0.11}_{-0.20}$ &	{$\pm$0.17} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 0) [\%]	
&	\textrm - &	{$\pm$0.10} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{$\mp$0.13} &	$\mp$0.11 &	\textrm - &	{$\mp$0.15} \\
$b$-Quark tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{$^{-0.11}_{+0.13}$} &	{\textrm -} &	{$^{-0.21}_{+0.24}$} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} \\
$b$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{$^{+0.33}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	\textrm - &	$^{+0.19}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$c$-Quark tagging efficiency (eigenvector 0) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{$^{+0.11}_{-0.10}$} &	{$^{-0.11}_{+0.17}$} &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{$\pm$0.10} &	{\textrm -} &	\textrm - &	$\mp$0.10 \\
$c$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 0) [\%]	
&	\textrm - &	{$^{+0.52}_{-0.49}$} &	{$^{+0.24}_{-0.22}$} &	{$^{-0.33}_{+0.34}$} &	{$^{+0.13}_{-0.14}$} &	{$^{+0.50}_{-0.54}$} &	{$^{-0.17}_{+0.12}$} &	{$^{-0.83}_{+1.08}$} &	$^{-1.45}_{+1.36}$ &	{$^{-0.17}_{+0.16}$} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 1) [\%]	
&	$\pm$0.14 &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\mp$0.16} &	{$\mp$0.30} &	{$\mp$0.22} \\
Light-jet tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	$\mp$0.15 &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 5) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 6) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 7) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 8) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 9) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 10) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 11) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$b$-Quark tagging  extrapolation  [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	$^{-0.14}_{+0.13}$ &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$^{-0.21}_{+0.22}$} &	{$^{+0.28}_{-0.27}$} \\
\rowcolor{Gray}
$b$-Quark tagging extrapolation from $c$-Quark [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Electron energy resolution [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.21}$ &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Electron energy scale [\%]	
&	\textrm - &	\textrm - &	$^{+0.21}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{+0.21}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{$^{-0.17}_{\textrm{ \phantom{ai}-}}$} \\
Electron trigger efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Electron reconstruction efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Electron identification efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Electron isolation efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - \\
Muon energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon (MS) momentum resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - \\
Muon (ID) momentum resolution [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon trigger efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon trigger efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon identification stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon identification syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
Muon isolation efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon isolation efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon TTVA efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon TTVA efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution para [\%]	
&	$\pm$0.14 &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\mp$0.25} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	$\pm$0.15 \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution perp [\%]	
&	\textrm - &	\textrm - &	{$\mp$0.12} &	{\textrm -} &	{$\mp$0.10} &	{\textrm -} &	{\textrm -} &	{$\pm$0.21} &	{$\pm$0.16} &	\textrm - \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet scale [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Luminosity [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$W$+jets $CA_{3ex}$ stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} \\
$W$+jets $CA_{2ex}$ stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$W$+jets $CA_{4incl}$ stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
$W$+jets Fcc stat error [\%]	
&	\textrm - &	{$^{+0.10}_{-0.17}$} &	{$^{+0.15}_{-0.26}$} &	$^{-0.12}_{+0.21}$ &	{\textrm -} &	{$^{+0.19}_{-0.33}$} &	{$^{-0.52}_{+0.88}$} &	{$^{-0.13}_{+0.22}$} &	$^{-0.12}_{+0.20}$ &	$^{-0.15}_{+0.25}$ \\
\rowcolor{Gray}
$W$+jets Flight stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$W$+jets Fc  error [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{$^{+0.10}_{-0.11}$} &	{\textrm -} &	{$^{-0.11}_{+0.12}$} &	$^{+0.12}_{-0.14}$ \\
\rowcolor{Gray}
QCD norm. impact on $W$+jets [\%]	
&	$^{+0.10}_{-0.12}$ &	$^{-0.12}_{+0.14}$ &	{$^{+0.20}_{-0.23}$} &	{\textrm -} &	{$^{-0.21}_{+0.25}$} &	{\textrm -} &	{$^{-0.42}_{+0.47}$} &	{$^{+0.13}_{-0.16}$} &	{$^{+0.53}_{-0.59}$} &	{$^{-0.19}_{+0.18}$} \\
Single top cross-section [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$Z$+jets cross-section [\%]	
&	$\mp$0.15 &	{\textrm -} &	{$\mp$0.17} &	$\pm$0.15 &	$\pm$0.16 &	$\mp$0.18 &	{\textrm -} &	{$\pm$0.11} &	{$\pm$0.42} &	{$\mp$0.24} \\
Diboson cross-section [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$t\bar{t}V$ cross-section [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Monte Carlo sample statistics [\%]	
&	$\pm$1.04 &	$\pm$1.10 &	$\pm$1.21 &	$\pm$1.57 &	$\pm$1.34 &	$\pm$1.38 &	{$\pm$2.28} &	$\pm$1.88 &	{$\pm$3.00} &	$\pm$2.78 \\
\rowcolor{Gray}
ISR/FSR + scale [\%]	
&	$^{+1.88}_{\textrm{ \phantom{ai}-}}$ &	$^{+1.65}_{-0.54}$ &	{$^{\textrm{ \phantom{ai}-}}_{-2.80}$} &	$^{-1.33}_{+2.33}$ &	$^{+0.45}_{-2.49}$ &	{$^{\textrm{ \phantom{ai}-}}_{-2.33}$} &	{$^{+3.72}_{\textrm{ \phantom{ai}-}}$} &	{$^{+2.16}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.89}$} &	$^{\textrm{ \phantom{ai}-}}_{-5.23}$ \\
Alternate hard-scattering model [\%]	
&	$\pm$1.27 &	{\textrm -} &	{$\pm$2.80} &	{$\mp$1.12} &	{$\mp$4.81} &	{$\pm$0.32} &	{$\pm$4.38} &	{$\mp$1.54} &	{$\mp$2.40} &	{$\mp$3.53} \\
\rowcolor{Gray}
Alternate parton-shower model [\%]	
&	$\mp$0.77 &	{$\mp$1.26} &	{$\mp$2.95} &	{$\pm$0.39} &	{$\mp$0.56} &	{$\mp$0.26} &	{$\pm$5.39} &	{$\pm$4.13} &	{$\pm$0.89} &	$\pm$0.72 \\
Inter PDF [\%]	
&	\textrm - &	{$\mp$0.17} &	{\textrm -} &	{$\pm$0.12} &	{\textrm -} &	{$\mp$0.19} &	{\textrm -} &	{$\pm$0.55} &	{\textrm -} &	{$\mp$0.31} \\
\rowcolor{Gray}
Intra PDF [\%]	
&	\textrm - &	{\textrm -} &	{$\mp$0.14} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{$\pm$0.41} &	{$\pm$0.80} \\
Real lepton efficiency stat [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$^{+0.17}_{-0.42}$} \\
\rowcolor{Gray}
Fake lepton efficiency MC scale [\%]	
&	$^{+0.24}_{-0.21}$ &	{\textrm -} &	{$^{-0.15}_{\textrm{ \phantom{ai}-}}$} &	$^{-0.14}_{+0.10}$ &	\textrm - &	{$^{+0.51}_{-0.50}$} &	{$^{-0.92}_{+0.80}$} &	{\textrm -} &	{$^{-0.32}_{+0.22}$} &	{$^{+1.04}_{-0.89}$} \\
Fake lepton efficiency alternate CR [\%]	
&	\textrm - &	{$\mp$0.37} &	{$\pm$0.12} &	{$\mp$0.33} &	{\textrm -} &	\textrm - &	{$\pm$0.46} &	{$\pm$0.25} &	{\textrm -} &	{$\pm$0.85} \\
\rowcolor{Gray}
Poor MTW Modelling in QCD [\%]	
&	$\pm$0.30 &	$\pm$0.33 &	{$\mp$0.51} &	{$\pm$0.15} &	{\textrm -} &	{$\pm$0.32} &	$\mp$0.25 &	$\pm$0.21 &	{$\mp$1.42} &	{$\pm$0.17} \\
\hline
\end{tabular}}


==> tables/systematics/boosted/table_syst_particle_topH_pt_AbsoluteDiffXs.tex <==
\resizebox*{!}{\textheight}{
\begin{tabular}{l c c c c c c c c}
\hline
Bins  [GeV]
 & 300--350   & 350--400   & 400--450   & 450--500   & 500--550   & 550--650   & 650--750   & 750--1500  \\
\hline
\hline
d$\sigma$ / d$p_{\textrm T}^{t}$ [pb/GeV]	&	$1.91 \cdot 10^{-2}$ &	$1.22 \cdot 10^{-2}$ &	$6.92 \cdot 10^{-3}$ &	$3.97 \cdot 10^{-3}$ &	$2.79 \cdot 10^{-3}$ &	$1.75 \cdot 10^{-3}$ &	$4.19 \cdot 10^{-4}$ &	$5.72 \cdot 10^{-5}$ \\
\hline
\rowcolor{Gray}
Total uncertainty [\%]	
&	$^{+20.5}_{-20.0}$ &	$^{+20.6}_{-19.9}$ &	$^{+19.6}_{-21.5}$ &	$^{+23.9}_{-23.6}$ &	$^{+27.8}_{-23.8}$ &	$^{+28.0}_{-26.4}$ &	$\pm$38.1 &	$^{+51.8}_{-47.5}$ \\
Statistical uncertainty [\%]	
&	$\pm2.5$ &	$\pm3.3$ &	$\pm4.7$ &	$\pm6.6$ &	$\pm8.5$ &	$\pm8.1$ &	$\pm21.$ &	$\pm22.$ \\
\rowcolor{Gray}
Systematic uncertainty [\%]	
&	$^{+20.3}_{-19.8}$ &	$^{+20.3}_{-19.6}$ &	$^{+18.9}_{-20.9}$ &	$^{+22.9}_{-22.6}$ &	$^{+26.4}_{-22.1}$ &	$^{+26.7}_{-25.0}$ &	$\pm$31.1 &	$^{+45.5}_{-40.5}$ \\
\hline
\hline
Large-$R$ jet Baseline (JES) [\%]	
&	$^{+13.0}_{-12.0}$ &	$^{+10.4}_{-9.53}$ &	{$^{+7.76}_{-7.91}$} &	$^{+7.30}_{-7.52}$ &	$^{+7.06}_{-4.88}$ &	{$^{+4.61}_{-5.01}$} &	{$^{+3.35}_{-6.78}$} &	{$^{+8.47}_{-6.43}$} \\
\rowcolor{Gray}
Large-$R$ jet Tracking (JES) [\%]	
&	$^{+8.70}_{-10.3}$ &	{$^{+12.5}_{-11.7}$} &	$^{+12.8}_{-15.2}$ &	{$^{+18.1}_{-16.9}$} &	$^{+22.4}_{-18.5}$ &	$^{+20.6}_{-20.1}$ &	$^{+23.9}_{-24.8}$ &	{$^{+36.3}_{-29.7}$} \\
Large-$R$ jet Modelling (JES) [\%]	
&	$^{+7.90}_{-7.63}$ &	$^{+6.53}_{-6.47}$ &	$^{+5.32}_{-5.12}$ &	$^{+4.70}_{-5.35}$ &	$^{+3.88}_{-2.46}$ &	{$^{+2.95}_{-3.98}$} &	$^{+3.03}_{-3.76}$ &	$^{+3.74}_{-2.90}$ \\
\rowcolor{Gray}
Large-$R$ jet CrossCalib $\tau$32 (JES) [\%]	
&	$^{-1.17}_{+0.38}$ &	{$^{-1.50}_{+1.14}$} &	{$^{-2.75}_{+1.62}$} &	$^{-2.71}_{+1.89}$ &	$^{-2.62}_{+1.82}$ &	{$^{-3.13}_{+2.73}$} &	{$^{-2.94}_{+3.82}$} &	$^{-4.67}_{+4.06}$ \\
Large-$R$ jet Run1 $\tau$32 (JES) [\%]	
&	$^{-3.69}_{+1.02}$ &	{$^{-5.53}_{+3.24}$} &	{$^{-7.55}_{+5.16}$} &	$^{-7.93}_{+6.25}$ &	$^{-8.65}_{+7.58}$ &	$^{-9.53}_{+9.20}$ &	{$^{-8.04}_{+12.7}$} &	$^{-13.5}_{+11.6}$ \\
\rowcolor{Gray}
Large-$R$ jet JMR [\%]	
&	$\mp$0.28 &	{$\mp$0.81} &	$\mp$1.01 &	{$\mp$0.33} &	{$\mp$0.24} &	$\mp$0.24 &	{$\mp$0.44} &	{$\mp$0.98} \\
$b$-Tagged jet energy scale (JES) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{+0.19}$} &	{$^{-0.14}_{+0.31}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.41}$ \\
\rowcolor{Gray}
Effective detector NP set 1 (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.67}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.92}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.86}$ &	$^{\textrm{ \phantom{ai}-}}_{-1.08}$ &	$^{\textrm{ \phantom{ai}-}}_{-1.26}$ &	$^{\textrm{ \phantom{ai}-}}_{-1.51}$ &	$^{-0.15}_{+0.38}$ &	{$^{-4.83}_{+1.66}$} \\
Effective detector NP set 2 (JES) [\%]	
&	$^{+0.32}_{-0.22}$ &	$^{+0.28}_{-0.57}$ &	{$^{+0.58}_{-0.74}$} &	$^{+0.46}_{-0.61}$ &	{$^{+0.74}_{-0.62}$} &	{$^{+0.39}_{-0.85}$} &	{$^{+1.04}_{-0.93}$} &	{$^{+0.71}_{-1.50}$} \\
\rowcolor{Gray}
Effective detector NP set 3 (JES) [\%]	
&	$\mp$0.10 &	$^{-0.35}_{+0.12}$ &	$^{-0.25}_{+0.10}$ &	{$\mp$0.14} &	$^{-0.27}_{+0.12}$ &	$^{-0.36}_{+0.14}$ &	{$^{-0.41}_{+0.33}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.33}$ \\
Effective detector NP set 4 (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.14}$ &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.24}$ &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.50}$ \\
\rowcolor{Gray}
Effective detector NP set 5 (JES) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{$^{+0.34}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.19}$} \\
Effective detector NP set 6 restTerm (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{$^{+0.21}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} \\
\rowcolor{Gray}
$\eta$ intercalibration model (JES) [\%]	
&	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.34}$ &	$^{-0.63}_{+0.13}$ &	{$^{-0.57}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.57}_{+0.52}$} &	{$^{-0.84}_{\textrm{ \phantom{ai}-}}$} &	$^{+0.67}_{-0.23}$ &	{$^{-2.60}_{+1.40}$} \\
$\eta$ intercalibration total stat (JES) [\%]	
&	$\mp$0.12 &	{$^{-0.39}_{+0.23}$} &	{$^{-0.55}_{+0.45}$} &	{$^{-0.38}_{+0.33}$} &	{$^{-0.37}_{+0.59}$} &	$^{-0.78}_{+0.65}$ &	{$^{-0.82}_{+1.02}$} &	$^{-0.94}_{+0.96}$ \\
\rowcolor{Gray}
Flavour composition (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.26}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.53}$ &	$^{-0.97}_{+0.16}$ &	{$^{-0.95}_{+0.29}$} &	{$^{-1.33}_{+0.48}$} &	$^{\textrm{ \phantom{ai}-}}_{-1.20}$ &	{$^{+0.63}_{\textrm{ \phantom{ai}-}}$} &	{$^{-4.16}_{+3.81}$} \\
Flavour response (JES) [\%]	
&	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.42}$ &	{$^{+0.13}_{-0.89}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.78}$ &	{$^{+0.39}_{-0.77}$} &	{$^{\textrm{ \phantom{ai}-}}_{-1.20}$} &	{$^{+0.39}_{\textrm{ \phantom{ai}-}}$} &	{$^{+1.21}_{-2.39}$} \\
\rowcolor{Gray}
Pile-up offset $\mu$ (JES) [\%]	
&	\textrm - &	{$^{+0.15}_{-0.24}$} &	$^{+0.16}_{-0.28}$ &	$^{+0.14}_{-0.30}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.30}$ &	$^{+0.13}_{-0.45}$ &	{$^{+0.59}_{-0.31}$} &	{$^{+0.24}_{-0.48}$} \\
Pile-up offset $N_{\textrm PV}$ (JES) [\%]	
&	\textrm - &	{$^{+0.16}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.22}_{-0.10}$} &	$^{+0.27}_{-0.11}$ &	{$\pm$0.14} &	{$^{+0.24}_{-0.15}$} &	{$^{+0.74}_{-0.13}$} &	{$^{+0.31}_{-0.74}$} \\
\rowcolor{Gray}
Pile-up offset $p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{+0.12}$ &	{\textrm -} &	{\textrm -} &	{$^{-0.29}_{+0.19}$} &	$^{\textrm{ \phantom{ai}-}}_{+0.21}$ &	{$^{-0.32}_{+0.12}$} \\
Pile-up offset $\rho$ topology (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.28}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.66}$ &	$^{\textrm{ \phantom{ai}-}}_{-1.05}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.90}$ &	$^{-0.88}_{\textrm{ \phantom{ai}-}}$ &	$^{\textrm{ \phantom{ai}-}}_{-1.58}$ &	$^{-0.36}_{+0.19}$ &	{$^{-2.48}_{+0.95}$} \\
\rowcolor{Gray}
Punch-through (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$^{+0.21}_{\textrm{ \phantom{ai}-}}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.21}$ \\
Single particle high-$p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Jet energy resolution [\%]	
&	$\mp$0.82 &	{$\mp$1.24} &	{$\mp$1.74} &	$\mp$2.23 &	$\mp$2.41 &	$\mp$2.80 &	{$\mp$2.02} &	{$\mp$5.32} \\
Jet vertex fraction [\%]	
&	$^{+0.58}_{-0.54}$ &	$^{+0.55}_{-0.42}$ &	{$^{+0.28}_{-0.20}$} &	{$^{+0.75}_{-0.71}$} &	$^{+0.92}_{-0.82}$ &	{$^{+0.24}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.44}_{-0.49}$} &	$^{+0.45}_{-0.31}$ \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-0.94}_{+0.91}$ &	$^{-0.94}_{+0.90}$ &	$^{-0.97}_{+0.94}$ &	$^{-0.98}_{+0.94}$ &	$^{-0.86}_{+0.82}$ &	$^{-0.99}_{+0.95}$ &	$^{-1.04}_{+1.01}$ &	$^{-0.90}_{+0.86}$ \\
$b$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$^{-1.07}_{+1.01}$ &	$^{-1.19}_{+1.08}$ &	$^{-1.20}_{+1.12}$ &	$^{-1.22}_{+1.09}$ &	$^{-1.17}_{+1.12}$ &	$^{-1.35}_{+1.27}$ &	$^{-1.31}_{+1.22}$ &	$^{-1.48}_{+1.36}$ \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	{$\mp$0.12} &	$\mp$0.14 &	$^{-0.13}_{+0.12}$ &	{$\mp$0.18} &	$^{-0.22}_{+0.21}$ &	{$^{-0.15}_{+0.14}$} &	{$\mp$0.20} \\
$b$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.33}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.22}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.28}$ &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.43}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.57}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.99}$ \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
$c$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-0.52}_{+0.32}$ &	$^{-0.70}_{+0.36}$ &	{$^{-0.55}_{+0.10}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.43}$ &	$^{-0.57}_{+0.17}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.43}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.43}$ &	{$^{-1.20}_{+0.59}$} \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$\mp$0.12 &	$\mp$0.15 &	{$\mp$0.20} &	{\textrm -} &	$\mp$0.10 &	$\mp$0.10 &	{$\mp$0.23} &	$^{-0.23}_{+0.22}$ \\
$c$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 0) [\%]	
&	$^{-0.88}_{+0.91}$ &	{$^{-0.59}_{+0.62}$} &	{$^{-1.90}_{+1.95}$} &	{$^{-1.10}_{+1.09}$} &	$^{-1.26}_{+1.22}$ &	{$^{-0.74}_{+0.75}$} &	{$^{-1.45}_{+1.99}$} &	{$^{-7.21}_{+7.14}$} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	{\textrm -} &	{$\pm$0.11} &	$\pm$0.10 &	{\textrm -} &	{$^{+0.12}_{-0.13}$} &	{\textrm -} &	{$\pm$0.61} \\
Light-jet tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	{\textrm -} &	{$\mp$0.11} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\mp$0.25} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{$\mp$0.35} \\
Light-jet tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\mp$0.38} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 5) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{$\mp$0.50} \\
Light-jet tagging efficiency (eigenvector 6) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\pm$0.19} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 7) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\pm$0.26} \\
Light-jet tagging efficiency (eigenvector 8) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 9) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 10) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 11) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$b$-Quark tagging  extrapolation  [\%]	
&	$^{+0.61}_{-0.62}$ &	{$^{+0.88}_{-0.91}$} &	$^{+1.13}_{-1.16}$ &	$^{+1.12}_{-1.17}$ &	$^{+1.24}_{-1.29}$ &	$^{+1.34}_{-1.44}$ &	{$^{+1.00}_{-1.09}$} &	{$^{+3.71}_{-3.98}$} \\
\rowcolor{Gray}
$b$-Quark tagging extrapolation from $c$-Quark [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	$\pm$0.14 \\
Electron energy resolution [\%]	
&	\textrm - &	\textrm - &	$^{-0.24}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	$^{-0.28}_{\textrm{ \phantom{ai}-}}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.44}$ &	$^{-0.16}_{+0.14}$ &	$^{\textrm{ \phantom{ai}-}}_{-1.75}$ \\
\rowcolor{Gray}
Electron energy scale [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	$^{-0.30}_{\textrm{ \phantom{ai}-}}$ &	{$^{-0.37}_{+0.42}$} &	$^{\textrm{ \phantom{ai}-}}_{-1.29}$ \\
Electron trigger efficiency [\%]	
&	$\pm$0.30 &	$\pm$0.31 &	$\pm$0.33 &	$\pm$0.34 &	$\pm$0.35 &	$\pm$0.35 &	$\pm$0.35 &	$\pm$0.39 \\
\rowcolor{Gray}
Electron reconstruction efficiency [\%]	
&	$\pm$0.23 &	$\pm$0.24 &	$\pm$0.26 &	$\pm$0.27 &	$\pm$0.28 &	$\pm$0.29 &	$\pm$0.30 &	$\pm$0.35 \\
Electron identification efficiency [\%]	
&	$\pm$0.61 &	$\pm$0.68 &	$\pm$0.76 &	$\pm$0.80 &	$\pm$0.88 &	$\pm$0.92 &	$\pm$1.00 &	$\pm$1.18 \\
\rowcolor{Gray}
Electron isolation efficiency [\%]	
&	$\pm$0.31 &	$\pm$0.39 &	$\pm$0.47 &	$\pm$0.51 &	$\pm$0.57 &	$\pm$0.61 &	$\pm$0.70 &	$\pm$0.84 \\
Muon energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon (MS) momentum resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} \\
Muon (ID) momentum resolution [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Muon trigger efficiency stat [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon trigger efficiency syst [\%]	
&	$\pm$0.26 &	$\pm$0.26 &	$\pm$0.26 &	$^{+0.26}_{-0.25}$ &	$\pm$0.25 &	$\pm$0.25 &	$\pm$0.27 &	$\pm$0.26 \\
\rowcolor{Gray}
Muon identification stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon identification syst [\%]	
&	$\pm$0.28 &	$\pm$0.33 &	$\pm$0.36 &	$\pm$0.39 &	$\pm$0.38 &	$\pm$0.41 &	$\pm$0.47 &	$^{+0.48}_{-0.47}$ \\
\rowcolor{Gray}
Muon isolation efficiency stat [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon isolation efficiency syst [\%]	
&	$\pm$0.11 &	$\pm$0.11 &	$\pm$0.12 &	$\pm$0.11 &	$\pm$0.12 &	$\pm$0.14 &	{$\pm$0.23} &	$\pm$0.25 \\
\rowcolor{Gray}
Muon TTVA efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon TTVA efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution para [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.13} &	{$\pm$0.41} &	{$\mp$2.23} \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution perp [\%]	
&	$\mp$0.37 &	$\mp$0.42 &	{$\mp$0.32} &	$\mp$0.28 &	$\mp$0.32 &	{$\mp$0.63} &	$\mp$0.79 &	$\mp$0.85 \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet scale [\%]	
&	$^{-0.29}_{\textrm{ \phantom{ai}-}}$ &	{$^{-0.23}_{+0.10}$} &	{\textrm -} &	{\textrm -} &	{$^{-0.13}_{\textrm{ \phantom{ai}-}}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.35}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.53}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.98}$ \\
Luminosity [\%]	
&	$\mp$2.05 &	$\mp$2.05 &	$\mp$2.05 &	$\mp$2.05 &	$\mp$2.05 &	$\mp$2.05 &	$\mp$2.05 &	$\mp$2.05 \\
\rowcolor{Gray}
$W$+jets $CA_{3ex}$ stat error [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - \\
$W$+jets $CA_{2ex}$ stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$W$+jets $CA_{4incl}$ stat error [\%]	
&	$\pm$0.17 &	$\pm$0.16 &	$\pm$0.20 &	$\pm$0.20 &	$\pm$0.26 &	$\pm$0.23 &	{$\pm$0.30} &	{$\pm$0.90} \\
$W$+jets Fcc stat error [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.16}$} &	{\textrm -} &	{$^{+0.50}_{-0.85}$} &	$^{+0.47}_{-0.79}$ &	{$^{-1.70}_{+2.88}$} \\
\rowcolor{Gray}
$W$+jets Flight stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$W$+jets Fc  error [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{$^{-0.11}_{+0.12}$} &	{\textrm -} &	{$^{-0.48}_{+0.53}$} \\
\rowcolor{Gray}
QCD norm. impact on $W$+jets [\%]	
&	$^{+0.56}_{-0.61}$ &	$^{+0.71}_{-0.78}$ &	{$^{+1.13}_{-1.24}$} &	$^{+0.97}_{-1.07}$ &	$^{+1.04}_{-1.14}$ &	{$^{+1.90}_{-2.09}$} &	$^{+1.72}_{-1.87}$ &	$^{+1.48}_{-1.55}$ \\
Single top cross-section [\%]	
&	$\pm$0.32 &	$\pm$0.33 &	$\pm$0.33 &	$\pm$0.36 &	$\pm$0.37 &	$\pm$0.45 &	$\pm$0.49 &	$\pm$0.63 \\
\rowcolor{Gray}
$Z$+jets cross-section [\%]	
&	$\pm$0.23 &	$\pm$0.29 &	{$\pm$0.61} &	$\pm$0.50 &	{$\pm$0.12} &	{$\pm$0.23} &	{$\pm$1.23} &	$\pm$1.51 \\
Diboson cross-section [\%]	
&	$\pm$0.25 &	$\pm$0.28 &	$\pm$0.29 &	$\pm$0.32 &	{$\pm$0.49} &	$\pm$0.50 &	$\pm$0.64 &	{$\pm$1.16} \\
\rowcolor{Gray}
$t\bar{t}V$ cross-section [\%]	
&	$\pm$0.10 &	$\pm$0.13 &	$\pm$0.15 &	$\pm$0.18 &	$\pm$0.22 &	$\pm$0.26 &	$\pm$0.31 &	$\pm$0.40 \\
Monte Carlo sample statistics [\%]	
&	$\pm$0.81 &	{$\pm$1.06} &	{$\pm$1.61} &	$\pm$1.65 &	{$\pm$2.26} &	$\pm$2.23 &	{$\pm$4.37} &	{$\pm$9.25} \\
\rowcolor{Gray}
ISR/FSR + scale [\%]	
&	$^{-2.27}_{+6.31}$ &	{$^{-1.80}_{+3.98}$} &	{$^{-1.18}_{+5.81}$} &	$^{-3.80}_{+5.29}$ &	{$^{+6.27}_{\textrm{ \phantom{ai}-}}$} &	{$^{+8.89}_{\textrm{ \phantom{ai}-}}$} &	{$^{-4.61}_{+2.86}$} &	{$^{-1.43}_{+7.92}$} \\
Alternate hard-scattering model [\%]	
&	$\pm$0.17 &	{$\pm$4.92} &	{$\mp$0.99} &	{$\pm$2.70} &	$\mp$2.24 &	{$\mp$6.00} &	{$\pm$0.53} &	{$\pm$16.6} \\
\rowcolor{Gray}
Alternate parton-shower model [\%]	
&	$\mp$7.25 &	$\mp$6.24 &	{$\mp$4.40} &	$\mp$4.56 &	{$\pm$0.44} &	{$\mp$0.84} &	{$\mp$11.9} &	{$\pm$0.70} \\
Inter PDF [\%]	
&	\textrm - &	{\textrm -} &	{$\mp$0.14} &	{$\pm$0.20} &	{$\pm$0.15} &	$\pm$0.12 &	{$\pm$1.54} &	{$\mp$0.61} \\
\rowcolor{Gray}
Intra PDF [\%]	
&	$\pm$0.10 &	$\pm$0.12 &	{$\pm$0.43} &	$\pm$0.47 &	{$\pm$0.16} &	{$\pm$0.68} &	$\pm$0.66 &	$\pm$0.65 \\
Real lepton efficiency stat [\%]	
&	$^{+0.24}_{-0.29}$ &	$^{+0.28}_{-0.35}$ &	{$^{+0.40}_{-0.66}$} &	$^{+0.31}_{-0.45}$ &	{$^{+0.53}_{-0.83}$} &	{$^{+0.78}_{-1.42}$} &	$^{+0.73}_{-1.38}$ &	$^{+0.93}_{-1.80}$ \\
\rowcolor{Gray}
Fake lepton efficiency MC scale [\%]	
&	$^{-0.63}_{+0.53}$ &	{$^{-0.87}_{+0.72}$} &	{$^{-1.22}_{+1.01}$} &	$^{-1.14}_{+1.02}$ &	$^{-0.99}_{+0.98}$ &	$^{-0.95}_{+0.82}$ &	{$^{-1.29}_{+1.24}$} &	$^{-1.03}_{+1.05}$ \\
Fake lepton efficiency alternate CR [\%]	
&	\textrm - &	$\pm$0.24 &	{\textrm -} &	{$\pm$0.39} &	$\pm$0.44 &	{$\pm$1.01} &	{$\mp$0.19} &	{$\pm$1.09} \\
\rowcolor{Gray}
Poor MTW Modelling in QCD [\%]	
&	$\mp$0.46 &	$\mp$0.39 &	$\mp$0.40 &	{$\mp$0.86} &	$\mp$1.01 &	$\mp$1.15 &	{$\mp$3.74} &	$\mp$4.24 \\
\hline
\end{tabular}}


==> tables/systematics/boosted/table_syst_particle_topH_pt_AbsoluteDiffXs_PLTagging.tex <==
\resizebox*{!}{\textheight}{
\begin{tabular}{l c c c c c c c c}
\hline
Bins  [GeV]
 & 300--350   & 350--400   & 400--450   & 450--500   & 500--550   & 550--650   & 650--750   & 750--1500  \\
\hline
\hline
d$\sigma$ / d$p_{\textrm T}^{t}$ [pb/GeV]	&	$3.30 \cdot 10^{-2}$ &	$1.84 \cdot 10^{-2}$ &	$1.05 \cdot 10^{-2}$ &	$6.15 \cdot 10^{-3}$ &	$3.68 \cdot 10^{-3}$ &	$1.88 \cdot 10^{-3}$ &	$7.95 \cdot 10^{-4}$ &	$9.50 \cdot 10^{-5}$ \\
\hline
\rowcolor{Gray}
Total uncertainty [\%]	
&	$^{+13.8}_{-16.7}$ &	$^{+16.5}_{-19.0}$ &	$^{+20.1}_{-20.6}$ &	$^{+22.2}_{-24.9}$ &	$^{+27.9}_{-22.9}$ &	$^{+28.9}_{-29.0}$ &	$^{+32.1}_{-30.9}$ &	$^{+39.2}_{-36.7}$ \\
Statistical uncertainty [\%]	
&	$\pm2.4$ &	$\pm3.4$ &	$\pm4.8$ &	$\pm6.5$ &	$\pm8.6$ &	$\pm8.2$ &	$\pm18.$ &	$\pm22.$ \\
\rowcolor{Gray}
Systematic uncertainty [\%]	
&	$^{+13.5}_{-16.5}$ &	$^{+16.1}_{-18.7}$ &	$^{+19.4}_{-20.0}$ &	$^{+21.2}_{-24.0}$ &	$^{+26.4}_{-21.1}$ &	$\pm$27.7 &	$^{+25.7}_{-24.1}$ &	$^{+31.8}_{-28.6}$ \\
\hline
\hline
Large-$R$ jet Run1 mass (JES) [\%]	
&	$^{+1.98}_{-2.26}$ &	$^{+1.62}_{-2.55}$ &	$^{+1.62}_{-2.49}$ &	$^{+1.86}_{-2.42}$ &	$^{+1.49}_{-1.71}$ &	$^{+1.75}_{-1.88}$ &	$^{+1.93}_{-2.47}$ &	{$^{+2.57}_{-1.93}$} \\
\rowcolor{Gray}
Large-$R$ jet Run1 $p_{\textrm T}$ (JES) [\%]	
&	$^{+6.80}_{-7.71}$ &	{$^{+10.6}_{-10.1}$} &	$^{+12.3}_{-11.5}$ &	$^{+13.7}_{-13.3}$ &	{$^{+18.9}_{-14.3}$} &	$^{+16.1}_{-17.4}$ &	{$^{+24.0}_{-20.7}$} &	$^{+28.3}_{-23.0}$ \\
Large-$R$ jet Run1 $\tau$32 (JES) [\%]	
&	$^{-3.38}_{+4.46}$ &	{$^{-3.61}_{+2.45}$} &	{$^{-2.56}_{+4.71}$} &	{$^{-5.19}_{+3.20}$} &	{$^{-0.38}_{+5.24}$} &	{$^{+7.89}_{\textrm{ \phantom{ai}-}}$} &	{$^{-1.44}_{+1.20}$} &	{$^{-3.05}_{+3.04}$} \\
\rowcolor{Gray}
Large-$R$ jet CrossCalib mass (JES) [\%]	
&	$^{+2.05}_{-2.46}$ &	{$^{+1.48}_{-2.46}$} &	$^{+1.41}_{-2.15}$ &	{$^{+1.06}_{-1.18}$} &	{$^{+0.48}_{-0.42}$} &	$\pm$0.58 &	{$^{+0.31}_{-0.60}$} &	{$^{+1.16}_{-0.49}$} \\
Large-$R$ jet CrossCalib $p_{\textrm T}$ (JES) [\%]	
&	$^{+6.39}_{-6.68}$ &	{$^{+9.60}_{-9.53}$} &	$^{+12.4}_{-11.5}$ &	$^{+13.3}_{-13.4}$ &	$^{+14.6}_{-8.11}$ &	{$^{+8.12}_{-8.17}$} &	$^{+7.20}_{-7.79}$ &	{$^{+9.77}_{-7.56}$} \\
\rowcolor{Gray}
Large-$R$ jet CrossCalib $\tau$32 (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$b$-Tagged jet energy scale (JES) [\%]	
&	$^{+0.18}_{-0.17}$ &	$^{+0.17}_{-0.25}$ &	{\textrm -} &	{\textrm -} &	{$^{+0.12}_{-0.21}$} &	{$\pm$0.18} &	{$^{\textrm{ \phantom{ai}-}}_{-0.26}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.22}$ \\
\rowcolor{Gray}
Effective detector NP set 1 (JES) [\%]	
&	$^{+0.70}_{-0.75}$ &	{$^{+0.39}_{-0.52}$} &	{$^{+0.14}_{-0.12}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.25}$ &	$^{+0.28}_{-0.55}$ &	{\textrm -} &	{$^{+0.59}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{+0.23}$} \\
Effective detector NP set 2 (JES) [\%]	
&	\textrm - &	{\textrm -} &	{$^{+0.17}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.28}_{\textrm{ \phantom{ai}-}}$} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
Effective detector NP set 3 (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.28}$ \\
Effective detector NP set 4 (JES) [\%]	
&	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{+0.12}$ &	\textrm - &	{\textrm -} &	{$\mp$0.10} &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
Effective detector NP set 5 (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.20}$ \\
Effective detector NP set 6 restTerm (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
$\eta$ intercalibration total stat (JES) [\%]	
&	$^{+0.18}_{-0.14}$ &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.17}$} &	\textrm - &	{$^{+0.10}_{-0.15}$} &	$^{-0.15}_{+0.12}$ \\
Flavour composition (JES) [\%]	
&	$^{+0.26}_{-0.32}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.18}$} &	{\textrm -} &	{$^{-0.29}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Flavour response (JES) [\%]	
&	$^{-0.17}_{+0.20}$ &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{$^{+0.23}_{\textrm{ \phantom{ai}-}}$} \\
Grouped NP set 1 (JES) [\%]	
&	$^{+0.17}_{-0.27}$ &	{\textrm -} &	{\textrm -} &	\textrm - &	$^{-0.12}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	{$^{+0.40}_{-0.31}$} &	{$^{-0.13}_{+0.38}$} \\
\rowcolor{Gray}
Pile-up offset $\mu$ (JES) [\%]	
&	$^{-0.35}_{+0.33}$ &	{$^{-0.31}_{\textrm{ \phantom{ai}-}}$} &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.25}$ &	$^{-0.32}_{+0.16}$ &	{$^{+0.13}_{\textrm{ \phantom{ai}-}}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.27}$ &	$^{+0.23}_{\textrm{ \phantom{ai}-}}$ \\
Pile-up offset $N_{\textrm PV}$ (JES) [\%]	
&	$^{-0.19}_{+0.27}$ &	{\textrm -} &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.22}$ &	$^{-0.20}_{+0.16}$ &	{\textrm -} &	{$\mp$0.20} &	\textrm - \\
\rowcolor{Gray}
Pile-up offset $p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Pile-up offset $\rho$ topology (JES) [\%]	
&	$^{+0.27}_{-0.18}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.16}$} &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.21}$ &	$^{+0.29}_{-0.28}$ &	{$^{\textrm{ \phantom{ai}-}}_{+0.13}$} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Punch-through (JES) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Single particle high-$p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Jet energy resolution [\%]	
&	$\pm$0.31 &	$\mp$0.33 &	{$\mp$0.21} &	{$\mp$0.12} &	$\mp$0.13 &	{$\mp$0.24} &	{$\pm$0.74} &	{\textrm -} \\
$b$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-0.93}_{+0.90}$ &	$^{-0.91}_{+0.88}$ &	$^{-0.90}_{+0.86}$ &	$^{-0.85}_{+0.82}$ &	$^{-0.79}_{+0.75}$ &	$^{-0.88}_{+0.84}$ &	$^{-0.99}_{+0.97}$ &	{$^{-0.73}_{+0.71}$} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$^{-0.96}_{+0.93}$ &	$^{-1.07}_{+1.02}$ &	$^{-1.04}_{+0.99}$ &	$^{-1.00}_{+0.94}$ &	$^{-0.98}_{+0.92}$ &	$^{-1.15}_{+1.08}$ &	$^{-1.08}_{+1.04}$ &	$^{-1.03}_{+0.98}$ \\
$b$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	$\mp$0.10 &	\textrm - &	\textrm - &	{$^{-0.15}_{+0.14}$} &	$\mp$0.15 &	{$^{-0.12}_{+0.11}$} &	$\mp$0.13 \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$\mp$0.13} &	{\textrm -} &	\textrm - &	\textrm - \\
$b$-Quark tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-0.16}_{+0.15}$ &	{$\mp$0.24} &	{$\mp$0.14} &	$^{-0.13}_{+0.12}$ &	{$^{-0.21}_{+0.20}$} &	{\textrm -} &	{\textrm -} &	{$^{-0.31}_{+0.33}$} \\
$c$-Quark tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{$\pm$0.19} \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$\pm$0.16} \\
$c$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 0) [\%]	
&	$^{-0.17}_{+0.19}$ &	\textrm - &	{$\mp$0.37} &	$^{-0.36}_{+0.37}$ &	{$^{-0.20}_{+0.19}$} &	{\textrm -} &	{$\mp$0.28} &	{$^{-0.65}_{+0.59}$} \\
Light-jet tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.16} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - \\
Light-jet tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 5) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 6) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 7) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 8) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 9) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 10) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 11) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 12) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 13) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$b$-Quark tagging  extrapolation  [\%]	
&	$^{+0.51}_{-0.52}$ &	{$^{+0.73}_{-0.76}$} &	$^{+0.81}_{-0.84}$ &	$^{+0.79}_{-0.84}$ &	$^{+0.98}_{-1.02}$ &	$^{+0.85}_{-0.94}$ &	$^{+0.78}_{-0.86}$ &	{$^{+1.11}_{-1.35}$} \\
$b$-Quark tagging extrapolation from $c$-Quark [\%]	
&	$^{+0.51}_{-0.52}$ &	{$^{+0.73}_{-0.76}$} &	$^{+0.81}_{-0.84}$ &	$^{+0.79}_{-0.84}$ &	$^{+0.98}_{-1.02}$ &	$^{+0.85}_{-0.94}$ &	$^{+0.78}_{-0.86}$ &	{$^{+1.11}_{-1.35}$} \\
\rowcolor{Gray}
Electron energy resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Electron energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Electron trigger efficiency [\%]	
&	$\pm$0.26 &	$\pm$0.27 &	$\pm$0.28 &	$\pm$0.29 &	$\pm$0.29 &	$\pm$0.28 &	$\pm$0.26 &	$\pm$0.29 \\
Electron reconstruction efficiency [\%]	
&	$\pm$0.20 &	$\pm$0.21 &	$\pm$0.22 &	$\pm$0.23 &	$\pm$0.23 &	$\pm$0.24 &	$\pm$0.22 &	$\pm$0.26 \\
\rowcolor{Gray}
Electron identification efficiency [\%]	
&	$\pm$0.55 &	$\pm$0.56 &	$\pm$0.59 &	$\pm$0.60 &	$\pm$0.62 &	$\pm$0.62 &	$\pm$0.58 &	$\pm$0.67 \\
Electron isolation efficiency [\%]	
&	$\pm$0.35 &	$\pm$0.42 &	$\pm$0.49 &	$\pm$0.54 &	$\pm$0.59 &	$\pm$0.60 &	$\pm$0.62 &	$\pm$0.70 \\
\rowcolor{Gray}
Muon energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon (MS) momentum resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.50}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.17}$ \\
\rowcolor{Gray}
Muon (ID) momentum resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - \\
Muon trigger efficiency stat [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-2.86}$ &	{$^{\textrm{ \phantom{ai}-}}_{-2.88}$} &	$^{\textrm{ \phantom{ai}-}}_{-2.92}$ &	$^{\textrm{ \phantom{ai}-}}_{-3.08}$ &	{$^{\textrm{ \phantom{ai}-}}_{-3.09}$} &	$^{\textrm{ \phantom{ai}-}}_{-3.60}$ &	$^{\textrm{ \phantom{ai}-}}_{-2.31}$ &	$^{\textrm{ \phantom{ai}-}}_{-3.44}$ \\
\rowcolor{Gray}
Muon trigger efficiency syst [\%]	
&	$^{+0.23}_{-4.05}$ &	$^{+0.23}_{-3.52}$ &	$^{+0.22}_{-4.19}$ &	$^{+0.22}_{-3.79}$ &	$^{+0.21}_{-3.91}$ &	$^{+0.21}_{-4.52}$ &	$^{+0.22}_{-4.15}$ &	$^{+0.18}_{-4.62}$ \\
Muon identification stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon identification syst [\%]	
&	$^{+0.24}_{-6.16}$ &	$^{+0.28}_{-5.69}$ &	$^{+0.30}_{-6.22}$ &	$^{+0.32}_{-7.01}$ &	$^{+0.32}_{-6.88}$ &	$^{+0.34}_{-6.80}$ &	$^{+0.39}_{-4.58}$ &	$^{+0.31}_{-8.30}$ \\
Muon isolation efficiency stat [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-2.86}$ &	{$^{\textrm{ \phantom{ai}-}}_{-2.88}$} &	$^{\textrm{ \phantom{ai}-}}_{-2.92}$ &	$^{\textrm{ \phantom{ai}-}}_{-3.08}$ &	{$^{\textrm{ \phantom{ai}-}}_{-3.09}$} &	$^{\textrm{ \phantom{ai}-}}_{-3.60}$ &	$^{\textrm{ \phantom{ai}-}}_{-2.31}$ &	$^{\textrm{ \phantom{ai}-}}_{-3.44}$ \\
\rowcolor{Gray}
Muon isolation efficiency syst [\%]	
&	$^{+0.11}_{-2.09}$ &	$^{+0.12}_{-2.28}$ &	$^{+0.13}_{-2.24}$ &	$^{+0.14}_{-2.06}$ &	$^{+0.15}_{-2.55}$ &	$^{+0.17}_{-2.24}$ &	{$^{+0.23}_{-2.24}$} &	$^{+0.21}_{-2.14}$ \\
Muon TTVA efficiency stat [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-2.49}$ &	$^{\textrm{ \phantom{ai}-}}_{-2.73}$ &	$^{\textrm{ \phantom{ai}-}}_{-2.56}$ &	$^{\textrm{ \phantom{ai}-}}_{-2.90}$ &	$^{\textrm{ \phantom{ai}-}}_{-2.50}$ &	$^{\textrm{ \phantom{ai}-}}_{-2.92}$ &	$^{\textrm{ \phantom{ai}-}}_{-2.62}$ &	$^{\textrm{ \phantom{ai}-}}_{-2.26}$ \\
\rowcolor{Gray}
Muon TTVA efficiency syst [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-2.00}$ &	$^{\textrm{ \phantom{ai}-}}_{-2.17}$ &	$^{\textrm{ \phantom{ai}-}}_{-2.13}$ &	$^{\textrm{ \phantom{ai}-}}_{-1.94}$ &	$^{\textrm{ \phantom{ai}-}}_{-2.42}$ &	$^{\textrm{ \phantom{ai}-}}_{-2.09}$ &	$^{\textrm{ \phantom{ai}-}}_{-2.03}$ &	{$^{\textrm{ \phantom{ai}-}}_{-1.94}$} \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution para [\%]	
&	\textrm - &	{$\mp$0.33} &	{\textrm -} &	\textrm - &	\textrm - &	$\mp$0.23 &	{$\pm$0.17} &	$\mp$0.14 \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution perp [\%]	
&	$\mp$0.20 &	{$\mp$0.14} &	{$\mp$0.10} &	\textrm - &	\textrm - &	{$\mp$0.19} &	\textrm - &	{$\mp$0.43} \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet scale [\%]	
&	$\mp$0.21 &	{$^{-0.20}_{+0.10}$} &	$^{-0.11}_{+0.10}$ &	{$^{-0.11}_{+0.21}$} &	{$^{\textrm{ \phantom{ai}-}}_{+0.15}$} &	{\textrm -} &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.30}$ \\
\rowcolor{Gray}
Monte Carlo sample statistics [\%]	
&	$\pm$0.63 &	{$\pm$0.86} &	$\pm$1.11 &	{$\pm$1.48} &	{$\pm$2.00} &	$\pm$2.14 &	{$\pm$3.60} &	$\pm$3.76 \\
ISR/FSR + scale [\%]	
&	$^{-3.38}_{+4.46}$ &	{$^{-3.61}_{+2.45}$} &	{$^{-2.56}_{+4.71}$} &	{$^{-5.19}_{+3.20}$} &	{$^{-0.38}_{+5.24}$} &	{$^{+7.89}_{\textrm{ \phantom{ai}-}}$} &	{$^{-1.44}_{+1.20}$} &	{$^{-3.05}_{+3.04}$} \\
\rowcolor{Gray}
Alternate hard-scattering model [\%]	
&	$\pm$0.14 &	{$\mp$3.81} &	{$\mp$2.56} &	$\mp$3.21 &	{$\pm$0.17} &	{$\pm$6.02} &	{$\mp$2.01} &	{$\mp$8.35} \\
Alternate parton-shower model [\%]	
&	$\pm$6.68 &	{$\pm$4.29} &	$\pm$3.43 &	{$\pm$6.64} &	$\pm$8.14 &	{$\pm$15.5} &	{$\pm$2.97} &	{$\mp$1.73} \\
\hline
\end{tabular}}


==> tables/systematics/boosted/table_syst_particle_topH_pt_RelativeDiffXs.tex <==
\resizebox*{!}{\textheight}{
\begin{tabular}{l c c c c c c c c}
\hline
Bins  [GeV]
 & 300--350   & 350--400   & 400--450   & 450--500   & 500--550   & 550--650   & 650--750   & 750--1500  \\
\hline
\hline
1/$\sigma$ $\cdot$ d$\sigma$ / d$p_{\textrm T}^{t}$	&	$7.60 \cdot 10^{-3}$ &	$4.86 \cdot 10^{-3}$ &	$2.76 \cdot 10^{-3}$ &	$1.58 \cdot 10^{-3}$ &	$1.12 \cdot 10^{-3}$ &	$6.98 \cdot 10^{-4}$ &	$1.67 \cdot 10^{-4}$ &	$2.28 \cdot 10^{-5}$ \\
\hline
\rowcolor{Gray}
Total uncertainty [\%]	
&	$^{+7.15}_{-7.40}$ &	$^{+5.88}_{-5.76}$ &	$^{+5.97}_{-6.45}$ &	$^{+8.50}_{-8.75}$ &	$^{+15.3}_{-13.1}$ &	$^{+16.1}_{-15.7}$ &	$^{+26.6}_{-27.6}$ &	$^{+38.2}_{-37.7}$ \\
Statistical uncertainty [\%]	
&	$\pm2.2$ &	$\pm3.2$ &	$\pm4.5$ &	$\pm6.3$ &	$\pm8.2$ &	$\pm7.8$ &	$\pm21.$ &	$\pm22.$ \\
\rowcolor{Gray}
Systematic uncertainty [\%]	
&	$^{+6.73}_{-6.99}$ &	$^{+4.83}_{-4.67}$ &	$^{+3.50}_{-4.26}$ &	$^{+5.40}_{-5.79}$ &	$^{+12.7}_{-9.97}$ &	$^{+13.9}_{-13.4}$ &	$^{+15.4}_{-17.0}$ &	$^{+29.3}_{-28.7}$ \\
\hline
\hline
Large-$R$ jet Baseline (JES) [\%]	
&	$^{+2.89}_{-3.05}$ &	{$^{+0.58}_{-0.30}$} &	{$^{-1.88}_{+1.47}$} &	$^{-2.30}_{+1.90}$ &	{$^{-2.52}_{+4.81}$} &	$^{-4.75}_{+4.67}$ &	{$^{-5.90}_{+2.72}$} &	$^{-1.24}_{+3.10}$ \\
\rowcolor{Gray}
Large-$R$ jet Tracking (JES) [\%]	
&	$^{-4.48}_{+4.26}$ &	{$^{-1.12}_{+2.70}$} &	{$^{\textrm{ \phantom{ai}-}}_{-1.45}$} &	{$^{+3.83}_{-3.43}$} &	{$^{+7.58}_{-5.31}$} &	$^{+6.03}_{-7.10}$ &	{$^{+8.89}_{-12.5}$} &	{$^{+19.8}_{-18.3}$} \\
Large-$R$ jet Modelling (JES) [\%]	
&	$^{+1.69}_{-1.72}$ &	{$^{+0.40}_{-0.48}$} &	{$^{-0.73}_{+0.94}$} &	{$^{-1.32}_{+0.70}$} &	{$^{-2.09}_{+3.77}$} &	{$^{-2.97}_{+2.16}$} &	$^{-2.90}_{+2.39}$ &	{$^{-2.22}_{+3.30}$} \\
\rowcolor{Gray}
Large-$R$ jet CrossCalib $\tau$32 (JES) [\%]	
&	$^{+0.82}_{-0.91}$ &	{$^{+0.48}_{-0.16}$} &	{$^{-0.79}_{+0.31}$} &	{$^{-0.75}_{+0.57}$} &	$^{-0.65}_{+0.50}$ &	{$^{-1.17}_{+1.40}$} &	{$^{-0.97}_{+2.47}$} &	$^{-2.75}_{+2.72}$ \\
Large-$R$ jet Run1 $\tau$32 (JES) [\%]	
&	$^{+2.59}_{-3.00}$ &	{$^{+0.63}_{-0.87}$} &	$^{-1.51}_{+0.97}$ &	{$^{-1.91}_{+2.01}$} &	{$^{-2.68}_{+3.29}$} &	{$^{-3.62}_{+4.84}$} &	{$^{-2.03}_{+8.24}$} &	$^{-7.85}_{+7.23}$ \\
\rowcolor{Gray}
Large-$R$ jet JMR [\%]	
&	$\pm$0.25 &	$\mp$0.28 &	{$\mp$0.47} &	{$\pm$0.20} &	{$\pm$0.29} &	$\pm$0.29 &	{$\pm$0.10} &	{$\mp$0.44} \\
$b$-Tagged jet energy scale (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{+0.18}$} &	{$^{-0.16}_{+0.30}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.42}$ \\
\rowcolor{Gray}
Effective detector NP set 1 (JES) [\%]	
&	$^{+0.56}_{-0.21}$ &	{$^{+0.29}_{-0.47}$} &	{$^{-0.22}_{+0.37}$} &	$^{-0.44}_{+0.39}$ &	$^{-0.63}_{+0.36}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.87}$ &	{$^{+0.84}_{\textrm{ \phantom{ai}-}}$} &	{$^{-4.22}_{+2.12}$} \\
Effective detector NP set 2 (JES) [\%]	
&	$^{-0.10}_{+0.31}$ &	{\textrm -} &	$^{+0.16}_{-0.20}$ &	{\textrm -} &	{$^{+0.31}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.32}$} &	{$^{+0.62}_{-0.40}$} &	{$^{+0.28}_{-0.97}$} \\
\rowcolor{Gray}
Effective detector NP set 3 (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{$^{-0.18}_{+0.21}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.23}$ \\
Effective detector NP set 4 (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{$^{-0.49}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Effective detector NP set 5 (JES) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$^{+0.26}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.26}$} \\
Effective detector NP set 6 restTerm (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{$^{+0.24}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} \\
\rowcolor{Gray}
$\eta$ intercalibration model (JES) [\%]	
&	$^{+0.28}_{-0.18}$ &	{\textrm -} &	$^{-0.23}_{+0.14}$ &	{\textrm -} &	{$^{-0.16}_{+0.53}$} &	{$^{-0.44}_{\textrm{ \phantom{ai}-}}$} &	{$^{+1.08}_{-0.22}$} &	{$^{-2.20}_{+1.41}$} \\
$\eta$ intercalibration total stat (JES) [\%]	
&	$^{+0.24}_{-0.20}$ &	\textrm - &	{$^{-0.17}_{+0.12}$} &	\textrm - &	{$^{+0.26}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.41}_{+0.32}$} &	{$^{-0.45}_{+0.70}$} &	$^{-0.57}_{+0.63}$ \\
\rowcolor{Gray}
Flavour composition (JES) [\%]	
&	$^{+0.51}_{-0.29}$ &	{$^{+0.12}_{-0.31}$} &	$^{-0.30}_{+0.14}$ &	{$^{-0.29}_{+0.26}$} &	{$^{-0.67}_{+0.45}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.54}$ &	{$^{+1.06}_{\textrm{ \phantom{ai}-}}$} &	{$^{-3.52}_{+3.78}$} \\
Flavour response (JES) [\%]	
&	$^{-0.14}_{+0.35}$ &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.35}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.24}$ &	{$^{+0.34}_{-0.22}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.66}$} &	{$^{+0.93}_{\textrm{ \phantom{ai}-}}$} &	$^{+1.17}_{-1.85}$ \\
\rowcolor{Gray}
Pile-up offset $\mu$ (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{+0.15}$ &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.23}$ &	{$^{+0.48}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.13}_{-0.26}$} \\
Pile-up offset $N_{\textrm PV}$ (JES) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$^{+0.55}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.12}_{-0.64}$} \\
\rowcolor{Gray}
Pile-up offset $p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$^{-0.20}_{+0.11}$} &	\textrm - &	$^{-0.23}_{\textrm{ \phantom{ai}-}}$ \\
Pile-up offset $\rho$ topology (JES) [\%]	
&	$^{+0.44}_{-0.14}$ &	{\textrm -} &	$^{-0.32}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	$^{-0.16}_{+0.19}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.86}$ &	{$^{+0.36}_{\textrm{ \phantom{ai}-}}$} &	{$^{-1.76}_{+1.08}$} \\
\rowcolor{Gray}
Punch-through (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{$^{+0.21}_{\textrm{ \phantom{ai}-}}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.20}$ \\
Single particle high-$p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Jet energy resolution [\%]	
&	$\pm$0.74 &	{$\pm$0.32} &	{$\mp$0.18} &	{$\mp$0.68} &	$\mp$0.86 &	{$\mp$1.26} &	{$\mp$0.47} &	{$\mp$3.81} \\
Jet vertex fraction [\%]	
&	\textrm - &	{\textrm -} &	$^{-0.24}_{+0.23}$ &	$^{+0.22}_{-0.27}$ &	{$^{+0.39}_{-0.38}$} &	{$^{-0.48}_{+0.68}$} &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{+0.13}$} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 0) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
$b$-Quark tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$^{-0.17}_{+0.18}$} &	{$^{-0.14}_{+0.12}$} &	{$^{-0.31}_{+0.26}$} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\mp$0.11} &	{\textrm -} &	{$\mp$0.10} \\
$b$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$^{+0.26}_{\textrm{ \phantom{ai}-}}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.20}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.34}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.76}$ \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$c$-Quark tagging efficiency (eigenvector 0) [\%]	
&	\textrm - &	$^{-0.12}_{+0.13}$ &	\textrm - &	{$^{+0.14}_{-0.27}$} &	\textrm - &	$^{+0.13}_{-0.23}$ &	$^{+0.14}_{-0.41}$ &	$^{-0.62}_{+0.36}$ \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - \\
$c$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 0) [\%]	
&	$\pm$0.30 &	{$^{+0.59}_{-0.58}$} &	$^{-0.73}_{+0.72}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.12}$} &	\textrm - &	{$^{+0.44}_{-0.45}$} &	{$^{-0.27}_{+0.77}$} &	{$^{-6.10}_{+5.85}$} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{$\pm$0.52} \\
Light-jet tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\mp$0.19} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{$\mp$0.36} \\
Light-jet tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\mp$0.38} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 5) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\mp$0.48} \\
Light-jet tagging efficiency (eigenvector 6) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\pm$0.19} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 7) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$\pm$0.26 \\
Light-jet tagging efficiency (eigenvector 8) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 9) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 10) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 11) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$b$-Quark tagging  extrapolation  [\%]	
&	$^{-0.36}_{+0.39}$ &	{\textrm -} &	{$\pm$0.15} &	$^{+0.14}_{-0.16}$ &	{$^{+0.26}_{-0.27}$} &	{$^{+0.36}_{-0.43}$} &	{\textrm -} &	{$^{+2.71}_{-2.99}$} \\
\rowcolor{Gray}
$b$-Quark tagging extrapolation from $c$-Quark [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{$\pm$0.10} \\
Electron energy resolution [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.25}$ &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-1.56}$ \\
\rowcolor{Gray}
Electron energy scale [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.25}$ &	{$^{-0.32}_{+0.40}$} &	$^{\textrm{ \phantom{ai}-}}_{-1.32}$ \\
Electron trigger efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Electron reconstruction efficiency [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
Electron identification efficiency [\%]	
&	$^{-0.11}_{+0.12}$ &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.15} &	$\pm$0.19 &	{$\pm$0.27} &	{$\pm$0.45} \\
\rowcolor{Gray}
Electron isolation efficiency [\%]	
&	$\mp$0.11 &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.14} &	$\pm$0.18 &	{$^{+0.26}_{-0.27}$} &	{$^{+0.40}_{-0.41}$} \\
Muon energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon (MS) momentum resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
Muon (ID) momentum resolution [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon trigger efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - \\
Muon trigger efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon identification stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon identification syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{$\pm$0.13} &	$^{+0.14}_{-0.13}$ \\
\rowcolor{Gray}
Muon isolation efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - \\
Muon isolation efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\pm$0.10} &	$\pm$0.12 \\
\rowcolor{Gray}
Muon TTVA efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon TTVA efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution para [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$\pm$0.18 &	{$\pm$0.45} &	{$\mp$2.19} \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution perp [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{$\pm$0.12} &	{\textrm -} &	{$\mp$0.22} &	{$\mp$0.38} &	$\mp$0.45 \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet scale [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.26}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.71}$ \\
Luminosity [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$W$+jets $CA_{3ex}$ stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$W$+jets $CA_{2ex}$ stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$W$+jets $CA_{4incl}$ stat error [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{$\pm$0.69} \\
$W$+jets Fcc stat error [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	$^{+0.10}_{-0.17}$ &	{\textrm -} &	{$^{+0.51}_{-0.86}$} &	$^{+0.48}_{-0.81}$ &	{$^{-1.69}_{+2.86}$} \\
\rowcolor{Gray}
$W$+jets Flight stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$W$+jets Fc  error [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{$^{-0.10}_{+0.11}$} &	{\textrm -} &	{$^{-0.47}_{+0.51}$} \\
\rowcolor{Gray}
QCD norm. impact on $W$+jets [\%]	
&	$^{-0.32}_{+0.36}$ &	{$^{-0.17}_{+0.19}$} &	{$^{+0.23}_{-0.27}$} &	{\textrm -} &	{$^{+0.15}_{-0.16}$} &	{$^{+1.00}_{-1.13}$} &	$^{+0.82}_{-0.90}$ &	{$^{+0.59}_{-0.58}$} \\
Single top cross-section [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{$\pm$0.13} &	{$\pm$0.27} \\
\rowcolor{Gray}
$Z$+jets cross-section [\%]	
&	$\mp$0.15 &	{\textrm -} &	{$\pm$0.23} &	{$\pm$0.12} &	{$\mp$0.25} &	{$\mp$0.15} &	{$\pm$0.84} &	{$\pm$1.12} \\
Diboson cross-section [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{$\pm$0.15} &	$\pm$0.17 &	{$\pm$0.30} &	{$\pm$0.82} \\
\rowcolor{Gray}
$t\bar{t}V$ cross-section [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{$\pm$0.11} &	{$\pm$0.15} &	{$\pm$0.24} \\
Monte Carlo sample statistics [\%]	
&	$\pm$0.75 &	{$\pm$1.02} &	{$\pm$1.50} &	$\pm$1.61 &	{$\pm$2.22} &	$\pm$2.20 &	{$\pm$4.34} &	{$\pm$9.04} \\
\rowcolor{Gray}
ISR/FSR + scale [\%]	
&	$^{-0.43}_{+0.57}$ &	$^{\textrm{ \phantom{ai}-}}_{-1.63}$ &	{$^{+0.68}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-1.99}$} &	{$^{+1.90}_{\textrm{ \phantom{ai}-}}$} &	{$^{+3.01}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-2.81}$} &	{$^{+2.10}_{\textrm{ \phantom{ai}-}}$} \\
Alternate hard-scattering model [\%]	
&	$\mp$1.06 &	{$\pm$3.62} &	{$\mp$2.22} &	{$\pm$1.43} &	{$\mp$3.45} &	{$\mp$7.17} &	{$\mp$0.71} &	{$\pm$15.1} \\
\rowcolor{Gray}
Alternate parton-shower model [\%]	
&	$\mp$1.95 &	{$\mp$0.88} &	$\pm$1.05 &	$\pm$0.88 &	{$\pm$6.18} &	$\pm$4.81 &	{$\mp$6.89} &	$\pm$6.45 \\
Inter PDF [\%]	
&	\textrm - &	{\textrm -} &	{$\mp$0.21} &	{$\pm$0.13} &	{\textrm -} &	{\textrm -} &	{$\pm$1.47} &	{$\mp$0.67} \\
\rowcolor{Gray}
Intra PDF [\%]	
&	$\mp$0.15 &	$\mp$0.13 &	{$\pm$0.17} &	$\pm$0.20 &	{\textrm -} &	{$\pm$0.42} &	$\pm$0.39 &	$\pm$0.39 \\
Real lepton efficiency stat [\%]	
&	$^{-0.12}_{+0.26}$ &	{$^{\textrm{ \phantom{ai}-}}_{+0.19}$} &	{\textrm -} &	\textrm - &	{$^{+0.16}_{-0.29}$} &	{$^{+0.41}_{-0.88}$} &	$^{+0.36}_{-0.83}$ &	{$^{+0.56}_{-1.26}$} \\
\rowcolor{Gray}
Fake lepton efficiency MC scale [\%]	
&	$^{+0.26}_{-0.23}$ &	{\textrm -} &	{$^{-0.33}_{+0.23}$} &	$^{-0.25}_{+0.24}$ &	$^{\textrm{ \phantom{ai}-}}_{+0.20}$ &	{\textrm -} &	{$^{-0.40}_{+0.46}$} &	{$^{-0.13}_{+0.27}$} \\
Fake lepton efficiency alternate CR [\%]	
&	$\mp$0.20 &	{\textrm -} &	{$\mp$0.22} &	$\pm$0.18 &	{$\pm$0.24} &	{$\pm$0.80} &	{$\mp$0.39} &	{$\pm$0.89} \\
\rowcolor{Gray}
Poor MTW Modelling in QCD [\%]	
&	$\pm$0.27 &	$\pm$0.35 &	$\pm$0.33 &	{$\mp$0.12} &	{$\mp$0.27} &	{$\mp$0.42} &	{$\mp$3.03} &	$\mp$3.52 \\
\hline
\end{tabular}}


==> tables/systematics/boosted/table_syst_particle_topH_pt_RelativeDiffXs_PLTagging.tex <==
\resizebox*{!}{\textheight}{
\begin{tabular}{l c c c c c c c c}
\hline
Bins  [GeV]
 & 300--350   & 350--400   & 400--450   & 450--500   & 500--550   & 550--650   & 650--750   & 750--1500  \\
\hline
\hline
1/$\sigma$ $\cdot$ d$\sigma$ / d$p_{\textrm T}^{t}$	&	$8.40 \cdot 10^{-3}$ &	$4.70 \cdot 10^{-3}$ &	$2.68 \cdot 10^{-3}$ &	$1.56 \cdot 10^{-3}$ &	$9.36 \cdot 10^{-4}$ &	$4.78 \cdot 10^{-4}$ &	$2.02 \cdot 10^{-4}$ &	$2.40 \cdot 10^{-5}$ \\
\hline
\rowcolor{Gray}
Total uncertainty [\%]	
&	$^{+4.79}_{-5.12}$ &	$^{+4.59}_{-5.29}$ &	$^{+6.60}_{-6.45}$ &	$^{+8.45}_{-9.89}$ &	$^{+13.4}_{-10.1}$ &	$^{+17.8}_{-16.4}$ &	$^{+23.1}_{-22.9}$ &	$^{+29.9}_{-28.8}$ \\
Statistical uncertainty [\%]	
&	$\pm1.9$ &	$\pm3.2$ &	$\pm4.6$ &	$\pm6.3$ &	$\pm8.5$ &	$\pm8.0$ &	$\pm18.$ &	$\pm22.$ \\
\rowcolor{Gray}
Systematic uncertainty [\%]	
&	$^{+4.34}_{-4.70}$ &	$^{+3.16}_{-4.11}$ &	$^{+4.54}_{-4.32}$ &	$^{+5.37}_{-7.44}$ &	$^{+10.2}_{-5.17}$ &	$^{+15.7}_{-14.2}$ &	$^{+13.0}_{-12.5}$ &	$^{+19.3}_{-17.5}$ \\
\hline
\hline
Large-$R$ jet Run1 mass (JES) [\%]	
&	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.23}$ &	\textrm - &	\textrm - &	{$^{-0.31}_{+0.62}$} &	{$^{\textrm{ \phantom{ai}-}}_{+0.45}$} &	{$^{+0.11}_{-0.14}$} &	{$^{+0.73}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Large-$R$ jet Run1 $p_{\textrm T}$ (JES) [\%]	
&	$^{-3.55}_{+3.18}$ &	{$^{\textrm{ \phantom{ai}-}}_{+0.41}$} &	{$^{+1.42}_{-1.06}$} &	{$^{+2.69}_{-3.09}$} &	{$^{+7.37}_{-4.19}$} &	{$^{+4.85}_{-7.71}$} &	{$^{+12.0}_{-11.3}$} &	{$^{+15.8}_{-13.9}$} \\
Large-$R$ jet Run1 $\tau$32 (JES) [\%]	
&	$^{-0.37}_{+0.41}$ &	$^{\textrm{ \phantom{ai}-}}_{-1.52}$ &	{$^{+0.65}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-2.24}$} &	{$^{+2.71}_{\textrm{ \phantom{ai}-}}$} &	{$^{+5.36}_{\textrm{ \phantom{ai}-}}$} &	{$^{+1.61}_{-2.72}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.95}$} \\
\rowcolor{Gray}
Large-$R$ jet CrossCalib mass (JES) [\%]	
&	$^{+0.48}_{-0.40}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.40}$} &	\textrm - &	{$^{-0.49}_{+0.89}$} &	{$^{-1.06}_{+1.67}$} &	$^{-0.96}_{+1.50}$ &	$^{-1.23}_{+1.48}$ &	$^{-0.38}_{+1.60}$ \\
Large-$R$ jet CrossCalib $p_{\textrm T}$ (JES) [\%]	
&	$^{-2.43}_{+2.22}$ &	{$^{+0.50}_{-0.90}$} &	{$\pm$3.14} &	$^{+3.92}_{-5.14}$ &	{$^{+5.11}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.84}_{+0.59}$} &	{$^{-1.69}_{+1.00}$} &	{$^{+1.26}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Large-$R$ jet CrossCalib $\tau$32 (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$b$-Tagged jet energy scale (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	$\mp$0.11 &	{\textrm -} &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.22}$ \\
\rowcolor{Gray}
Effective detector NP set 1 (JES) [\%]	
&	$^{+0.28}_{-0.25}$ &	\textrm - &	{$^{-0.28}_{+0.37}$} &	{$^{-0.61}_{+0.25}$} &	{\textrm -} &	{$^{-0.29}_{+0.46}$} &	{$^{+0.49}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.46}_{+0.73}$} \\
Effective detector NP set 2 (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	$^{-0.23}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Effective detector NP set 3 (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.29}$ \\
Effective detector NP set 4 (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{$^{+0.14}_{\textrm{ \phantom{ai}-}}$} &	\textrm - \\
\rowcolor{Gray}
Effective detector NP set 5 (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - \\
Effective detector NP set 6 restTerm (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
$\eta$ intercalibration total stat (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$^{-0.16}_{+0.18}$} &	{\textrm -} &	{$\mp$0.24} \\
Flavour composition (JES) [\%]	
&	$\pm$0.14 &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{+0.15}$} &	{$^{-0.42}_{+0.22}$} &	{$^{\textrm{ \phantom{ai}-}}_{+0.14}$} &	{\textrm -} &	{$^{-0.11}_{+0.24}$} &	{$^{-0.13}_{+0.36}$} \\
\rowcolor{Gray}
Flavour response (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.27}$ &	$^{+0.21}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	{\textrm -} &	{$^{+0.33}_{\textrm{ \phantom{ai}-}}$} \\
Grouped NP set 1 (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.13}$ &	\textrm - &	{\textrm -} &	$^{-0.20}_{+0.10}$ &	{$^{-0.21}_{+0.23}$} &	$^{+0.22}_{\textrm{ \phantom{ai}-}}$ &	{$^{+0.31}_{-0.17}$} &	{$^{-0.22}_{+0.52}$} \\
\rowcolor{Gray}
Pile-up offset $\mu$ (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{+0.15}$ &	{\textrm -} &	$^{+0.26}_{\textrm{ \phantom{ai}-}}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.25}$ &	\textrm - &	{$^{+0.39}_{-0.25}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.22}$} &	{$^{+0.32}_{\textrm{ \phantom{ai}-}}$} \\
Pile-up offset $N_{\textrm PV}$ (JES) [\%]	
&	\textrm - &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.13}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.36}$ &	\textrm - &	{\textrm -} &	{\textrm -} &	{$^{+0.24}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Pile-up offset $p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Pile-up offset $\rho$ topology (JES) [\%]	
&	\textrm - &	\textrm - &	{$^{-0.11}_{+0.10}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.22}$ &	$^{+0.14}_{-0.13}$ &	{$^{-0.22}_{+0.27}$} &	{$^{-0.17}_{+0.15}$} &	{$^{\textrm{ \phantom{ai}-}}_{+0.23}$} \\
\rowcolor{Gray}
Punch-through (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
Single particle high-$p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Jet energy resolution [\%]	
&	$\pm$0.30 &	$\mp$0.34 &	{$\mp$0.22} &	{$\mp$0.13} &	$\mp$0.14 &	{$\mp$0.25} &	{$\pm$0.73} &	{\textrm -} \\
$b$-Quark tagging efficiency (eigenvector 0) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\pm$0.11} &	{\textrm -} &	{\textrm -} &	{$^{+0.17}_{-0.16}$} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{$^{-0.13}_{+0.11}$} &	{\textrm -} &	\textrm - \\
$b$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} \\
$b$-Quark tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 0) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{$\pm$0.17} &	{$^{+0.24}_{-0.26}$} &	{$^{-0.14}_{+0.17}$} \\
$c$-Quark tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	$\pm$0.21 \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{+0.15}_{-0.14}$ \\
$c$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 0) [\%]	
&	\textrm - &	$\pm$0.17 &	$\mp$0.19 &	$\mp$0.18 &	{\textrm -} &	{$\pm$0.24} &	{$\mp$0.10} &	{$^{-0.48}_{+0.41}$} \\
Light-jet tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	$\pm$0.12 \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 5) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 6) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 7) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 8) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 9) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 10) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 11) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 12) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 13) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$b$-Quark tagging  extrapolation  [\%]	
&	$^{-0.16}_{+0.19}$ &	{\textrm -} &	{$\pm$0.13} &	$^{+0.11}_{-0.13}$ &	{$^{+0.29}_{-0.31}$} &	{$^{+0.16}_{-0.23}$} &	{$^{+0.10}_{-0.15}$} &	{$^{+0.42}_{-0.64}$} \\
$b$-Quark tagging extrapolation from $c$-Quark [\%]	
&	$^{-0.16}_{+0.19}$ &	{\textrm -} &	{$\pm$0.13} &	$^{+0.11}_{-0.13}$ &	{$^{+0.29}_{-0.31}$} &	{$^{+0.16}_{-0.23}$} &	{$^{+0.10}_{-0.15}$} &	{$^{+0.42}_{-0.64}$} \\
\rowcolor{Gray}
Electron energy resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Electron energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Electron trigger efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - \\
Electron reconstruction efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Electron identification efficiency [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - \\
Electron isolation efficiency [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{$\pm$0.10} &	{$\pm$0.15} &	$\pm$0.16 &	$\pm$0.18 &	{$\pm$0.26} \\
\rowcolor{Gray}
Muon energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon (MS) momentum resolution [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.48}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.16}$ \\
\rowcolor{Gray}
Muon (ID) momentum resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - \\
Muon trigger efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.68}$ &	{$^{+0.64}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.52}$} \\
\rowcolor{Gray}
Muon trigger efficiency syst [\%]	
&	\textrm - &	{$^{+0.45}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.24}$} &	\textrm - &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.59}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.20}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.69}$ \\
Muon identification stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon identification syst [\%]	
&	\textrm - &	{$^{+0.54}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.87}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.73}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.64}$} &	{$^{+1.72}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-2.24}$} \\
Muon isolation efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.68}$ &	{$^{+0.64}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.52}$} \\
\rowcolor{Gray}
Muon isolation efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{-0.37}$} &	{\textrm -} &	{\textrm -} &	\textrm - \\
Muon TTVA efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.30}$ &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.32}$ &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{+0.35}$} \\
\rowcolor{Gray}
Muon TTVA efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.35}$ &	\textrm - &	{\textrm -} &	{\textrm -} \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution para [\%]	
&	\textrm - &	{$\mp$0.20} &	{\textrm -} &	{$\pm$0.13} &	$\pm$0.12 &	$\mp$0.10 &	{$\pm$0.30} &	{\textrm -} \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution perp [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{$\pm$0.16} &	{$\mp$0.27} \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{$^{+0.22}_{\textrm{ \phantom{ai}-}}$} &	\textrm - \\
\rowcolor{Gray}
Monte Carlo sample statistics [\%]	
&	$\pm$0.51 &	{$\pm$0.80} &	{$\pm$1.07} &	{$\pm$1.44} &	{$\pm$1.97} &	$\pm$2.10 &	{$\pm$3.57} &	$\pm$3.72 \\
ISR/FSR + scale [\%]	
&	$^{-0.37}_{+0.41}$ &	$^{\textrm{ \phantom{ai}-}}_{-1.52}$ &	{$^{+0.65}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-2.24}$} &	{$^{+2.71}_{\textrm{ \phantom{ai}-}}$} &	{$^{+5.36}_{\textrm{ \phantom{ai}-}}$} &	{$^{+1.61}_{-2.72}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.95}$} \\
\rowcolor{Gray}
Alternate hard-scattering model [\%]	
&	$\pm$1.48 &	{$\mp$2.52} &	{$\mp$1.25} &	{$\mp$1.90} &	$\pm$1.52 &	{$\pm$7.45} &	{$\mp$0.69} &	{$\mp$7.12} \\
Alternate parton-shower model [\%]	
&	$\pm$0.69 &	{$\mp$1.56} &	{$\mp$2.37} &	{$\pm$0.65} &	{$\pm$2.07} &	{$\pm$9.10} &	{$\mp$2.81} &	{$\mp$7.25} \\
\hline
\end{tabular}}


==> tables/systematics/resolved/table_syst_particle_topH_absrap_AbsoluteDiffXs.tex <==
\resizebox*{\textwidth}{!}{
\begin{tabular}{l c c c c c c c c c c c c c c c c c c}
\hline
Bins  [ Unit $|y^{t}|$ ]
 & 0--0.10   & 0.10--0.20   & 0.20--0.30   & 0.30--0.40   & 0.40--0.50   & 0.50--0.60   & 0.60--0.70   & 0.70--0.80   & 0.80--0.90   & 0.90--1   & 1--1.10   & 1.10--1.20   & 1.20--1.30   & 1.30--1.40   & 1.40--1.50   & 1.50--1.70   & 1.70--1.90   & 1.90--2.50  \\
\hline
\hline
d$\sigma$ / d$|y^{t}|$ [pb/ Unit $|y^{t}|$ ]	&	$8.13 \cdot 10^{1}$ &	$7.87 \cdot 10^{1}$ &	$7.88 \cdot 10^{1}$ &	$7.73 \cdot 10^{1}$ &	$7.43 \cdot 10^{1}$ &	$7.22 \cdot 10^{1}$ &	$6.75 \cdot 10^{1}$ &	$6.31 \cdot 10^{1}$ &	$6.29 \cdot 10^{1}$ &	$5.55 \cdot 10^{1}$ &	$5.06 \cdot 10^{1}$ &	$4.76 \cdot 10^{1}$ &	$4.24 \cdot 10^{1}$ &	$3.74 \cdot 10^{1}$ &	$3.21 \cdot 10^{1}$ &	$2.45 \cdot 10^{1}$ &	$1.58 \cdot 10^{1}$ &	$3.59 \cdot 10^{0}$ \\
\hline
\rowcolor{Gray}
Total uncertainty [\%]	
&	$^{+10.0}_{-11.9}$ &	$^{+10.5}_{-11.1}$ &	$^{+10.4}_{-10.6}$ &	$^{+10.0}_{-10.8}$ &	$^{+11.2}_{-12.5}$ &	$^{+10.3}_{-11.2}$ &	$^{+10.5}_{-11.6}$ &	$^{+10.3}_{-11.4}$ &	$^{+11.3}_{-11.1}$ &	$^{+10.5}_{-11.7}$ &	$^{+10.6}_{-11.3}$ &	$^{+10.2}_{-11.9}$ &	$^{+10.5}_{-11.7}$ &	$\pm$11.2 &	$^{+10.3}_{-11.3}$ &	$^{+11.0}_{-11.5}$ &	$^{+11.2}_{-11.7}$ &	$\pm$11.3 \\
Statistical uncertainty [\%]	
&	$\pm1.1$ &	$\pm1.2$ &	$\pm1.2$ &	$\pm1.2$ &	$\pm1.3$ &	$\pm1.3$ &	$\pm1.3$ &	$\pm1.4$ &	$\pm1.4$ &	$\pm1.5$ &	$\pm1.6$ &	$\pm1.6$ &	$\pm1.7$ &	$\pm1.9$ &	$\pm2.1$ &	$\pm1.5$ &	$\pm1.9$ &	$\pm2.2$ \\
\rowcolor{Gray}
Systematic uncertainty [\%]	
&	$^{+9.93}_{-11.8}$ &	$^{+10.4}_{-11.0}$ &	$^{+10.3}_{-10.5}$ &	$^{+9.95}_{-10.7}$ &	$^{+11.1}_{-12.4}$ &	$^{+10.2}_{-11.1}$ &	$^{+10.4}_{-11.5}$ &	$^{+10.2}_{-11.3}$ &	$^{+11.2}_{-11.0}$ &	$^{+10.4}_{-11.6}$ &	$^{+10.4}_{-11.2}$ &	$^{+10.1}_{-11.8}$ &	$^{+10.3}_{-11.6}$ &	$\pm$11.0 &	$^{+10.0}_{-11.1}$ &	$^{+10.9}_{-11.4}$ &	$^{+11.0}_{-11.5}$ &	$\pm$11.0 \\
\hline
\hline
$b$-Tagged jet energy scale (JES) [\%]	
&	$^{+0.51}_{-0.60}$ &	$^{+0.53}_{-0.40}$ &	{$^{+0.37}_{-0.60}$} &	{$^{+0.69}_{-0.52}$} &	$^{+0.56}_{-0.51}$ &	$^{+0.48}_{-0.42}$ &	$\pm$0.59 &	$^{+0.54}_{-0.48}$ &	$^{+0.53}_{-0.51}$ &	$^{+0.56}_{-0.61}$ &	$^{+0.58}_{-0.45}$ &	{$^{+0.29}_{-0.70}$} &	{$^{+0.59}_{-0.42}$} &	$^{+0.53}_{-0.32}$ &	$^{+0.59}_{-0.56}$ &	$^{+0.73}_{-0.55}$ &	{$^{+0.41}_{-0.45}$} &	$^{+0.42}_{-0.37}$ \\
\rowcolor{Gray}
Effective detector NP set 1 (JES) [\%]	
&	$^{+4.53}_{-5.73}$ &	$^{+4.86}_{-5.33}$ &	$^{+4.62}_{-5.19}$ &	$^{+4.57}_{-5.57}$ &	$^{+4.64}_{-5.93}$ &	$^{+4.36}_{-5.68}$ &	$^{+4.78}_{-5.85}$ &	$^{+4.72}_{-5.46}$ &	$^{+5.51}_{-5.85}$ &	$^{+4.99}_{-5.68}$ &	$^{+4.69}_{-5.04}$ &	$^{+4.53}_{-5.99}$ &	$^{+4.44}_{-5.76}$ &	$^{+5.54}_{-5.49}$ &	$^{+4.75}_{-5.78}$ &	$^{+5.14}_{-5.66}$ &	$^{+5.14}_{-5.54}$ &	$^{+4.84}_{-5.03}$ \\
Effective detector NP set 2 (JES) [\%]	
&	$^{-0.88}_{+0.42}$ &	{$^{-0.74}_{+0.63}$} &	$^{-0.47}_{+0.59}$ &	$^{-0.84}_{+0.75}$ &	$^{-0.74}_{+0.87}$ &	$^{-0.89}_{+0.73}$ &	$^{-0.52}_{+0.64}$ &	{$^{-0.77}_{+0.44}$} &	{$^{-0.92}_{+0.85}$} &	$^{-0.68}_{+0.84}$ &	$^{-0.69}_{+0.80}$ &	$^{-1.05}_{+0.64}$ &	$^{-0.91}_{+0.55}$ &	{$^{-0.76}_{+1.25}$} &	{$^{-0.65}_{+0.62}$} &	{$^{-0.72}_{+0.88}$} &	$^{-0.74}_{+0.83}$ &	{$^{-0.67}_{+0.47}$} \\
\rowcolor{Gray}
Effective detector NP set 3 (JES) [\%]	
&	$^{+0.10}_{-0.20}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.19}$} &	{$^{+0.15}_{-0.13}$} &	{$^{+0.10}_{-0.26}$} &	{$^{+0.24}_{-0.17}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.19}$} &	{$^{+0.20}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.30}$} &	{$^{+0.19}_{-0.30}$} &	{\textrm -} &	{$^{+0.17}_{-0.15}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.28}$} &	{$^{+0.12}_{-0.10}$} &	{$^{+0.35}_{-0.21}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.21}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.15}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.17}$ &	\textrm - \\
Effective detector NP set 4 (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{$^{-0.16}_{+0.11}$} &	$^{-0.12}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	\textrm - &	$^{-0.14}_{\textrm{ \phantom{ai}-}}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.24}$ &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$^{-0.11}_{+0.15}$} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Effective detector NP set 5 (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
Effective detector NP set 6 restTerm (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$\eta$ intercalibration model (JES) [\%]	
&	$^{+0.37}_{-1.04}$ &	{$^{+0.66}_{-1.02}$} &	$^{+0.68}_{-0.89}$ &	{$^{+0.38}_{-0.78}$} &	{$^{+0.69}_{-1.23}$} &	$^{+0.79}_{-1.24}$ &	{$^{+1.08}_{-1.57}$} &	$^{+0.89}_{-1.50}$ &	{$^{+1.58}_{-1.75}$} &	$^{+1.61}_{-1.98}$ &	$^{+1.70}_{-1.83}$ &	$^{+1.87}_{-2.73}$ &	$^{+1.97}_{-2.33}$ &	{$^{+2.65}_{-2.13}$} &	{$^{+1.99}_{-2.81}$} &	{$^{+2.86}_{-3.15}$} &	$^{+3.23}_{-3.12}$ &	$^{+3.37}_{-3.27}$ \\
$\eta$ intercalibration total stat (JES) [\%]	
&	$^{+0.27}_{-0.66}$ &	{$^{+0.60}_{-0.70}$} &	$^{+0.50}_{-0.32}$ &	$^{+0.58}_{-0.61}$ &	$^{+0.67}_{-0.49}$ &	$^{+0.58}_{-0.78}$ &	$\pm$0.58 &	{$^{+0.39}_{-0.73}$} &	{$^{+0.89}_{-0.73}$} &	$^{+0.74}_{-0.79}$ &	$^{+0.74}_{-0.71}$ &	$^{+0.60}_{-0.96}$ &	$^{+0.77}_{-0.86}$ &	{$^{+1.14}_{-0.80}$} &	{$\pm$0.63} &	{$^{+0.87}_{-0.67}$} &	$^{+1.02}_{-0.96}$ &	$\pm$0.92 \\
\rowcolor{Gray}
Flavour composition (JES) [\%]	
&	$^{+2.78}_{-3.84}$ &	$^{+3.41}_{-3.72}$ &	$^{+2.77}_{-3.37}$ &	$^{+3.25}_{-3.61}$ &	$^{+2.96}_{-4.40}$ &	$^{+2.48}_{-3.84}$ &	{$^{+3.39}_{-4.09}$} &	$^{+3.17}_{-4.02}$ &	$^{+3.89}_{-3.59}$ &	$^{+3.47}_{-4.26}$ &	$^{+3.27}_{-3.66}$ &	$^{+3.02}_{-4.13}$ &	$^{+3.23}_{-4.46}$ &	$^{+4.03}_{-4.15}$ &	{$^{+2.98}_{-4.15}$} &	$^{+3.41}_{-4.20}$ &	$^{+3.78}_{-4.13}$ &	$^{+3.63}_{-3.87}$ \\
Flavour response (JES) [\%]	
&	$^{-1.34}_{+0.18}$ &	{$^{-0.99}_{+0.72}$} &	$^{-0.85}_{+0.56}$ &	$^{-0.82}_{+0.62}$ &	$^{-1.15}_{+0.57}$ &	{$^{-1.31}_{+0.78}$} &	{$^{-0.92}_{+0.44}$} &	$^{-0.91}_{+0.51}$ &	{$^{-1.14}_{+1.13}$} &	{$^{-1.37}_{+0.56}$} &	{$^{-0.81}_{+0.83}$} &	$^{-1.51}_{+0.77}$ &	$^{-1.50}_{+0.77}$ &	{$^{-0.95}_{+1.63}$} &	{$^{-0.95}_{+0.40}$} &	{$^{-1.07}_{+0.60}$} &	{$^{-1.32}_{+1.40}$} &	{$^{-1.36}_{+1.05}$} \\
\rowcolor{Gray}
Pile-up offset $\mu$ (JES) [\%]	
&	\textrm - &	{$^{-0.20}_{+0.18}$} &	{\textrm -} &	{$^{-0.20}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{$^{-0.22}_{+0.20}$} &	$^{-0.10}_{+0.21}$ &	{\textrm -} &	{$^{-0.28}_{+0.20}$} &	{$^{-0.29}_{+0.15}$} &	{$^{-0.24}_{+0.26}$} &	{$^{-0.26}_{+0.13}$} &	$^{-0.26}_{+0.16}$ &	{$^{-0.24}_{+0.29}$} &	{$^{-0.13}_{+0.20}$} &	$^{-0.31}_{+0.19}$ &	{$^{-0.32}_{+0.39}$} &	$^{-0.43}_{+0.31}$ \\
Pile-up offset $N_{\textrm PV}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{+0.25}$} &	\textrm - &	{\textrm -} &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.17}$} \\
\rowcolor{Gray}
Pile-up offset $p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	{\textrm -} &	{$^{-0.13}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	$^{-0.10}_{+0.13}$ &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	$^{-0.12}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} \\
Pile-up offset $\rho$ topology (JES) [\%]	
&	$^{+0.96}_{-2.22}$ &	$^{+1.20}_{-1.78}$ &	$^{+1.27}_{-1.68}$ &	$^{+1.25}_{-1.99}$ &	$^{+1.32}_{-2.00}$ &	$^{+1.33}_{-1.94}$ &	$^{+1.27}_{-1.78}$ &	$^{+1.12}_{-1.91}$ &	{$^{+1.75}_{-2.10}$} &	{$^{+1.18}_{-1.98}$} &	$^{+1.37}_{-1.70}$ &	$^{+1.37}_{-2.24}$ &	$^{+1.18}_{-2.26}$ &	{$^{+2.26}_{-1.63}$} &	{$^{+1.03}_{-1.87}$} &	{$^{+1.42}_{-1.67}$} &	$^{+1.64}_{-1.77}$ &	$^{+1.47}_{-1.74}$ \\
\rowcolor{Gray}
Punch-through (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Single particle high-$p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Jet energy resolution [\%]	
&	$\mp$2.13 &	$\mp$1.84 &	$\mp$1.65 &	{$\mp$0.11} &	{$\mp$2.89} &	{$\mp$1.89} &	{$\mp$1.39} &	{$\mp$2.19} &	{$\mp$0.32} &	{$\mp$1.03} &	{$\mp$2.14} &	{$\mp$1.39} &	$\mp$1.58 &	{$\mp$1.11} &	$\mp$1.03 &	{$\mp$1.71} &	$\mp$1.75 &	{$\mp$1.19} \\
Jet vertex fraction [\%]	
&	$^{+3.40}_{-3.33}$ &	$^{+3.48}_{-3.41}$ &	$^{+3.42}_{-3.37}$ &	$^{+3.46}_{-3.40}$ &	$^{+3.47}_{-3.39}$ &	$^{+3.52}_{-3.46}$ &	$^{+3.61}_{-3.53}$ &	$^{+3.49}_{-3.41}$ &	$^{+3.50}_{-3.45}$ &	$^{+3.52}_{-3.44}$ &	$^{+3.60}_{-3.53}$ &	$^{+3.57}_{-3.50}$ &	$^{+3.58}_{-3.49}$ &	$^{+3.56}_{-3.48}$ &	$^{+3.54}_{-3.47}$ &	$^{+3.45}_{-3.39}$ &	$^{+3.37}_{-3.31}$ &	$^{+3.04}_{-3.00}$ \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-4.06}_{+4.13}$ &	$^{-4.06}_{+4.13}$ &	$^{-4.09}_{+4.16}$ &	$^{-4.06}_{+4.13}$ &	$^{-4.08}_{+4.15}$ &	$^{-4.11}_{+4.18}$ &	$^{-4.08}_{+4.15}$ &	$^{-4.05}_{+4.12}$ &	$^{-4.05}_{+4.12}$ &	$^{-4.13}_{+4.20}$ &	$^{-4.04}_{+4.11}$ &	$^{-4.04}_{+4.11}$ &	$^{-4.04}_{+4.11}$ &	$^{-4.04}_{+4.11}$ &	$^{-4.11}_{+4.19}$ &	$^{-4.01}_{+4.08}$ &	$^{-4.00}_{+4.07}$ &	$^{-3.99}_{+4.06}$ \\
$b$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$^{-1.65}_{+1.66}$ &	$^{-1.65}_{+1.66}$ &	$^{-1.65}_{+1.67}$ &	$^{-1.67}_{+1.69}$ &	$^{-1.66}_{+1.67}$ &	$^{-1.65}_{+1.66}$ &	$^{-1.65}_{+1.67}$ &	$^{-1.63}_{+1.64}$ &	$^{-1.65}_{+1.66}$ &	$^{-1.66}_{+1.68}$ &	$^{-1.65}_{+1.66}$ &	$^{-1.64}_{+1.66}$ &	$^{-1.64}_{+1.65}$ &	$^{-1.63}_{+1.65}$ &	$^{-1.65}_{+1.66}$ &	$^{-1.65}_{+1.66}$ &	$^{-1.67}_{+1.68}$ &	$^{-1.75}_{+1.76}$ \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 2) [\%]	
&	$^{+1.07}_{-1.06}$ &	$^{+1.07}_{-1.06}$ &	$^{+1.09}_{-1.08}$ &	$\pm$1.06 &	$^{+1.08}_{-1.07}$ &	$^{+1.08}_{-1.07}$ &	$\pm$1.07 &	$^{+1.08}_{-1.07}$ &	$^{+1.08}_{-1.07}$ &	$^{+1.09}_{-1.08}$ &	$^{+1.09}_{-1.08}$ &	$\pm$1.08 &	$^{+1.10}_{-1.09}$ &	$^{+1.10}_{-1.09}$ &	$\pm$1.11 &	$^{+1.10}_{-1.09}$ &	$^{+1.09}_{-1.08}$ &	$^{+1.06}_{-1.05}$ \\
$b$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$\pm$0.10 \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$c$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-1.61}_{+1.62}$ &	$^{-1.56}_{+1.58}$ &	$^{-1.54}_{+1.55}$ &	$^{-1.52}_{+1.53}$ &	$^{-1.52}_{+1.53}$ &	$^{-1.57}_{+1.58}$ &	$^{-1.53}_{+1.54}$ &	$^{-1.56}_{+1.57}$ &	$\mp$1.43 &	$\mp$1.43 &	$\mp$1.42 &	$\mp$1.42 &	$^{-1.44}_{+1.45}$ &	$^{-1.31}_{+1.32}$ &	$\mp$1.35 &	$^{-1.38}_{+1.39}$ &	$\mp$1.27 &	$\mp$1.15 \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$\pm$0.17 &	$\pm$0.16 &	$\pm$0.14 &	$\pm$0.16 &	$\pm$0.15 &	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.15 &	$\pm$0.14 &	$\pm$0.15 &	$\pm$0.15 &	$\pm$0.14 &	$\pm$0.15 &	$\pm$0.14 &	$\pm$0.13 &	$\pm$0.14 &	$\pm$0.15 &	{\textrm -} \\
$c$-Quark tagging efficiency (eigenvector 2) [\%]	
&	$\pm$0.19 &	$\pm$0.19 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.16 &	$\pm$0.17 &	$\pm$0.18 &	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.16 &	$\pm$0.15 &	$\pm$0.13 \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 0) [\%]	
&	$\mp$1.38 &	{$^{-1.72}_{+1.87}$} &	{$^{-1.31}_{+1.33}$} &	$^{-1.39}_{+1.47}$ &	$^{-1.62}_{+1.74}$ &	{$^{-1.27}_{+1.28}$} &	$^{-1.54}_{+1.65}$ &	$^{-1.47}_{+1.53}$ &	$^{-1.27}_{+1.26}$ &	$^{-1.54}_{+1.63}$ &	$^{-1.69}_{+1.82}$ &	$^{-1.57}_{+1.77}$ &	{$^{-1.35}_{+1.33}$} &	$^{-1.60}_{+1.69}$ &	$^{-1.68}_{+1.66}$ &	$^{-1.49}_{+1.51}$ &	{$^{-2.15}_{+2.42}$} &	$^{-2.08}_{+2.07}$ \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	{\textrm -} &	{$^{+0.11}_{-0.10}$} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{$\mp$0.12} &	{$\mp$0.20} \\
Light-jet tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	{$\pm$0.12} &	{\textrm -} &	\textrm - &	$\pm$0.11 &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{$\pm$0.11} &	{\textrm -} &	{\textrm -} &	\textrm - &	{$\pm$0.10} &	{\textrm -} &	{$\pm$0.11} &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 5) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 6) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 7) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 8) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 9) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 10) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 11) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$b$-Quark tagging  extrapolation  [\%]	
&	$^{+0.32}_{-0.33}$ &	$\pm$0.31 &	$^{+0.32}_{-0.31}$ &	$\pm$0.33 &	$^{+0.32}_{-0.31}$ &	$^{+0.32}_{-0.31}$ &	$\pm$0.32 &	$^{+0.30}_{-0.31}$ &	$\pm$0.31 &	$\pm$0.30 &	$\pm$0.31 &	$\pm$0.29 &	$\pm$0.28 &	$\pm$0.28 &	$\pm$0.27 &	$\pm$0.27 &	$\pm$0.26 &	$\pm$0.28 \\
\rowcolor{Gray}
$b$-Quark tagging extrapolation from $c$-Quark [\%]	
&	$^{+0.10}_{-0.12}$ &	$\pm$0.12 &	$^{+0.11}_{-0.10}$ &	$^{+0.12}_{-0.13}$ &	$\pm$0.12 &	\textrm - &	$\pm$0.11 &	$^{+0.11}_{-0.12}$ &	\textrm - &	$\pm$0.10 &	$^{+0.12}_{-0.13}$ &	{\textrm -} &	$\pm$0.10 &	{\textrm -} &	{\textrm -} &	$\pm$0.10 &	{\textrm -} &	\textrm - \\
Electron energy resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{+0.15}$} &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Electron energy scale [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
Electron trigger efficiency [\%]	
&	$\pm$0.26 &	$\pm$0.25 &	$\pm$0.26 &	$\pm$0.26 &	$\pm$0.26 &	$\pm$0.26 &	$\pm$0.26 &	$\pm$0.26 &	$\pm$0.25 &	$\pm$0.27 &	$\pm$0.26 &	$\pm$0.26 &	$\pm$0.26 &	$\pm$0.26 &	$\pm$0.27 &	$\pm$0.26 &	$\pm$0.27 &	$\pm$0.27 \\
\rowcolor{Gray}
Electron reconstruction efficiency [\%]	
&	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 \\
Electron identification efficiency [\%]	
&	$\pm$0.44 &	$\pm$0.43 &	$\pm$0.44 &	$\pm$0.44 &	$\pm$0.44 &	$\pm$0.44 &	$\pm$0.44 &	$\pm$0.45 &	$\pm$0.43 &	$\pm$0.45 &	$\pm$0.44 &	$\pm$0.44 &	$\pm$0.43 &	$\pm$0.43 &	$\pm$0.45 &	$\pm$0.43 &	$\pm$0.44 &	$\pm$0.43 \\
\rowcolor{Gray}
Electron isolation efficiency [\%]	
&	$\pm$0.17 &	$\pm$0.16 &	$\pm$0.17 &	$\pm$0.16 &	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.17 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.17 &	$\pm$0.16 \\
Muon energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon (MS) momentum resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon (ID) momentum resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$^{-0.18}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon trigger efficiency stat [\%]	
&	$^{+0.57}_{-0.58}$ &	$^{+0.58}_{-0.59}$ &	$^{+0.57}_{-0.58}$ &	$^{+0.58}_{-0.60}$ &	$^{+0.57}_{-0.59}$ &	$^{+0.56}_{-0.58}$ &	$^{+0.57}_{-0.59}$ &	$^{+0.56}_{-0.58}$ &	$^{+0.56}_{-0.58}$ &	$^{+0.58}_{-0.59}$ &	$^{+0.56}_{-0.58}$ &	$^{+0.56}_{-0.57}$ &	$^{+0.56}_{-0.58}$ &	$^{+0.56}_{-0.57}$ &	$^{+0.56}_{-0.58}$ &	$^{+0.56}_{-0.57}$ &	$^{+0.55}_{-0.57}$ &	$^{+0.55}_{-0.57}$ \\
Muon trigger efficiency syst [\%]	
&	$^{+0.25}_{-0.24}$ &	$\pm$0.25 &	$^{+0.25}_{-0.24}$ &	$\pm$0.25 &	$^{+0.25}_{-0.24}$ &	$\pm$0.24 &	$^{+0.25}_{-0.24}$ &	$\pm$0.24 &	$\pm$0.24 &	$^{+0.25}_{-0.24}$ &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.24 &	$^{+0.24}_{-0.23}$ \\
\rowcolor{Gray}
Muon identification stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon identification syst [\%]	
&	$\pm$0.18 &	$\pm$0.18 &	$^{+0.18}_{-0.17}$ &	$\pm$0.18 &	$\pm$0.18 &	$^{+0.18}_{-0.17}$ &	$\pm$0.18 &	$^{+0.18}_{-0.17}$ &	$\pm$0.17 &	$\pm$0.18 &	$\pm$0.18 &	$^{+0.18}_{-0.17}$ &	$\pm$0.18 &	$\pm$0.18 &	$^{+0.18}_{-0.17}$ &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 \\
\rowcolor{Gray}
Muon isolation efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon isolation efficiency syst [\%]	
&	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 \\
\rowcolor{Gray}
Muon TTVA efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon TTVA efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution para [\%]	
&	$\pm$0.10 &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution perp [\%]	
&	$\mp$0.10 &	$\mp$0.10 &	$\mp$0.10 &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\mp$0.12} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Luminosity [\%]	
&	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 \\
\rowcolor{Gray}
Single top cross-section [\%]	
&	$\pm$0.28 &	$\pm$0.28 &	$\pm$0.29 &	$\pm$0.29 &	$\pm$0.27 &	$\pm$0.27 &	$\pm$0.27 &	$\pm$0.26 &	$\pm$0.26 &	$\pm$0.25 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.23 &	$\pm$0.23 &	$\pm$0.22 &	$\pm$0.20 &	$\pm$0.21 \\
$Z$+jets cross-section [\%]	
&	$\pm$0.66 &	$\pm$0.61 &	$\pm$0.66 &	$\pm$0.55 &	$\pm$0.67 &	$\pm$0.56 &	$\pm$0.57 &	$\pm$0.58 &	$\pm$0.50 &	{$\pm$0.82} &	{$\pm$0.60} &	$\pm$0.53 &	$\pm$0.47 &	{$\pm$0.36} &	{$\pm$0.74} &	{$\pm$0.35} &	{$\pm$0.62} &	{$\pm$0.40} \\
\rowcolor{Gray}
Diboson cross-section [\%]	
&	$\pm$0.14 &	$\pm$0.14 &	$\pm$0.15 &	$\pm$0.14 &	$\pm$0.14 &	$\pm$0.15 &	$\pm$0.14 &	$\pm$0.12 &	$\pm$0.14 &	$\pm$0.15 &	$\pm$0.13 &	$\pm$0.13 &	$\pm$0.16 &	{$\pm$0.12} &	$\pm$0.14 &	$\pm$0.13 &	$\pm$0.12 &	$\pm$0.11 \\
$t\bar{t}V$ cross-section [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Monte Carlo sample statistics [\%]	
&	$\pm$0.45 &	$\pm$0.52 &	$\pm$0.50 &	$\pm$0.53 &	$\pm$0.55 &	$\pm$0.49 &	$\pm$0.54 &	$\pm$0.59 &	$\pm$0.52 &	$\pm$0.64 &	$\pm$0.64 &	$\pm$0.66 &	$\pm$0.65 &	$\pm$0.67 &	$\pm$0.76 &	{$\pm$0.54} &	{$\pm$0.80} &	$\pm$0.83 \\
ISR/FSR + scale [\%]	
&	$^{-4.16}_{+1.31}$ &	{$^{-2.52}_{+1.77}$} &	{$^{-1.85}_{+3.04}$} &	{$^{-2.52}_{+2.12}$} &	$^{-2.75}_{+1.66}$ &	{$^{-2.08}_{+3.06}$} &	$^{-3.46}_{+2.42}$ &	$^{-3.19}_{+2.08}$ &	{$^{-2.17}_{+3.61}$} &	{$^{-3.53}_{+1.53}$} &	$^{-3.76}_{+1.93}$ &	$^{-2.49}_{+1.61}$ &	{$^{-2.65}_{+2.84}$} &	{$^{-3.45}_{+1.93}$} &	$^{-1.91}_{+2.47}$ &	$^{-2.53}_{+2.71}$ &	{$^{-3.11}_{+1.50}$} &	{$^{-1.65}_{+2.71}$} \\
\rowcolor{Gray}
Alternate hard-scattering model [\%]	
&	$\pm$0.44 &	$\mp$0.56 &	{$\pm$1.05} &	{$\mp$0.36} &	{$\pm$3.21} &	{$\pm$0.95} &	$\mp$1.00 &	{$\mp$0.39} &	{$\pm$0.88} &	{$\pm$0.36} &	{$\pm$2.31} &	{$\pm$0.47} &	{$\mp$1.75} &	{$\pm$0.13} &	{$\pm$1.36} &	{$\mp$0.17} &	{\textrm -} &	{$\pm$3.74} \\
Alternate parton-shower model [\%]	
&	$\mp$2.11 &	$\mp$2.07 &	$\mp$1.86 &	$\mp$1.97 &	{$\mp$2.99} &	{$\mp$1.77} &	$\mp$1.89 &	{$\mp$1.37} &	{$\mp$1.82} &	$\mp$1.87 &	$\mp$1.74 &	{$\mp$2.51} &	{$\mp$1.55} &	$\mp$1.84 &	{$\mp$1.26} &	{$\mp$2.27} &	{$\mp$3.06} &	{$\mp$0.92} \\
\rowcolor{Gray}
Inter PDF [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\pm$0.12} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.15} &	{\textrm -} &	{$\pm$0.13} &	\textrm - &	$\pm$0.19 \\
Intra PDF [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.19} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{$\pm$0.11} &	$\pm$0.13 &	{$\pm$0.17} &	{$\pm$0.25} \\
\rowcolor{Gray}
Real lepton efficiency stat [\%]	
&	$^{-0.17}_{+0.15}$ &	$^{-0.16}_{+0.15}$ &	$^{-0.16}_{+0.15}$ &	$^{-0.18}_{+0.16}$ &	$^{-0.16}_{+0.15}$ &	$^{-0.18}_{+0.16}$ &	$^{-0.16}_{+0.15}$ &	$^{-0.16}_{+0.15}$ &	$^{-0.17}_{+0.16}$ &	$^{-0.17}_{+0.15}$ &	$^{-0.17}_{+0.15}$ &	$^{-0.17}_{+0.15}$ &	$^{-0.16}_{+0.15}$ &	$^{-0.17}_{+0.15}$ &	$^{-0.16}_{+0.15}$ &	$^{-0.17}_{+0.15}$ &	$^{-0.17}_{+0.15}$ &	$^{-0.18}_{+0.16}$ \\
Fake lepton efficiency MC scale [\%]	
&	$^{+0.58}_{-0.74}$ &	{$^{+0.77}_{-0.92}$} &	{$^{+0.59}_{-0.76}$} &	$^{+0.69}_{-0.84}$ &	$^{+0.72}_{-0.84}$ &	$^{+0.69}_{-0.80}$ &	$^{+0.59}_{-0.76}$ &	$^{+0.55}_{-0.66}$ &	$^{+0.63}_{-0.87}$ &	$^{+0.65}_{-0.70}$ &	{$^{+0.41}_{-0.69}$} &	{$^{+0.54}_{-0.72}$} &	$^{+0.46}_{-0.56}$ &	{$^{+0.29}_{-0.39}$} &	{$^{+0.56}_{-0.74}$} &	$^{+0.51}_{-0.60}$ &	{$^{+0.33}_{-0.56}$} &	$^{+0.36}_{-0.43}$ \\
\rowcolor{Gray}
Fake lepton efficiency alternate CR [\%]	
&	$\pm$0.31 &	$\pm$0.36 &	$\pm$0.32 &	$\pm$0.40 &	$\pm$0.35 &	$\pm$0.30 &	$\pm$0.33 &	$\pm$0.29 &	$\pm$0.35 &	$\pm$0.39 &	$\pm$0.40 &	{$\pm$0.28} &	$\pm$0.29 &	$\pm$0.29 &	$\pm$0.35 &	$\pm$0.42 &	{\textrm -} &	{$\pm$0.35} \\
Fake overall normalisation [\%]	
&	$\pm$3.74 &	$\pm$3.68 &	$\pm$3.76 &	$\pm$3.37 &	$\pm$3.61 &	$\pm$3.62 &	$\pm$3.46 &	$\pm$3.61 &	$\pm$3.41 &	$\pm$3.54 &	$\pm$2.83 &	$\pm$3.12 &	$\pm$3.12 &	{$\pm$2.31} &	$\pm$2.68 &	$\pm$3.08 &	{$\pm$2.07} &	$\pm$2.16 \\
\rowcolor{Gray}
$W$+jets $CA_{4incl}$ stat error [\%]	
&	$\mp$0.12 &	$\mp$0.12 &	$\mp$0.11 &	$\mp$0.11 &	$\mp$0.12 &	$\mp$0.11 &	$\mp$0.12 &	$\mp$0.11 &	\textrm - &	$\mp$0.11 &	$\mp$0.10 &	$\mp$0.10 &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$W$+jets Fc stat error [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$W$+jets Fcc stat error [\%]	
&	\textrm - &	{\textrm -} &	{$^{-0.18}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$^{+0.19}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{\textrm -} &	{$^{+0.15}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	\textrm - &	{$^{+0.14}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} \\
$W$+jets Flight stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\hline
\end{tabular}}


==> tables/systematics/resolved/table_syst_particle_topH_absrap_RelativeDiffXs.tex <==
\resizebox*{\textwidth}{!}{
\begin{tabular}{l c c c c c c c c c c c c c c c c c c}
\hline
Bins  [ Unit $|y^{t}|$ ]
 & 0--0.10   & 0.10--0.20   & 0.20--0.30   & 0.30--0.40   & 0.40--0.50   & 0.50--0.60   & 0.60--0.70   & 0.70--0.80   & 0.80--0.90   & 0.90--1   & 1--1.10   & 1.10--1.20   & 1.20--1.30   & 1.30--1.40   & 1.40--1.50   & 1.50--1.70   & 1.70--1.90   & 1.90--2.50  \\
\hline
\hline
1/$\sigma$ $\cdot$ d$\sigma$ / d$|y^{t}|$	&	$7.94 \cdot 10^{-1}$ &	$7.69 \cdot 10^{-1}$ &	$7.69 \cdot 10^{-1}$ &	$7.54 \cdot 10^{-1}$ &	$7.26 \cdot 10^{-1}$ &	$7.05 \cdot 10^{-1}$ &	$6.59 \cdot 10^{-1}$ &	$6.16 \cdot 10^{-1}$ &	$6.14 \cdot 10^{-1}$ &	$5.42 \cdot 10^{-1}$ &	$4.94 \cdot 10^{-1}$ &	$4.64 \cdot 10^{-1}$ &	$4.14 \cdot 10^{-1}$ &	$3.65 \cdot 10^{-1}$ &	$3.14 \cdot 10^{-1}$ &	$2.39 \cdot 10^{-1}$ &	$1.55 \cdot 10^{-1}$ &	$3.50 \cdot 10^{-2}$ \\
\hline
\rowcolor{Gray}
Total uncertainty [\%]	
&	$^{+1.69}_{-2.41}$ &	$^{+1.99}_{-1.97}$ &	$^{+2.20}_{-1.77}$ &	$^{+2.46}_{-2.40}$ &	$^{+3.53}_{-3.65}$ &	$^{+1.93}_{-1.87}$ &	$^{+2.17}_{-2.27}$ &	$^{+2.08}_{-2.30}$ &	$^{+2.73}_{-2.08}$ &	$^{+1.86}_{-2.04}$ &	$^{+2.78}_{-2.81}$ &	$^{+1.98}_{-2.50}$ &	$^{+3.12}_{-3.19}$ &	$^{+3.32}_{-2.54}$ &	$^{+2.91}_{-2.93}$ &	$^{+2.58}_{-2.46}$ &	$^{+3.68}_{-3.34}$ &	$^{+5.12}_{-4.71}$ \\
Statistical uncertainty [\%]	
&	$\pm1.1$ &	$\pm1.2$ &	$\pm1.2$ &	$\pm1.2$ &	$\pm1.2$ &	$\pm1.3$ &	$\pm1.3$ &	$\pm1.4$ &	$\pm1.3$ &	$\pm1.5$ &	$\pm1.6$ &	$\pm1.6$ &	$\pm1.7$ &	$\pm1.8$ &	$\pm2.0$ &	$\pm1.5$ &	$\pm1.9$ &	$\pm2.1$ \\
\rowcolor{Gray}
Systematic uncertainty [\%]	
&	$^{+1.16}_{-2.07}$ &	$^{+1.47}_{-1.45}$ &	$^{+1.75}_{-1.18}$ &	$^{+2.06}_{-1.99}$ &	$^{+3.25}_{-3.37}$ &	$^{+1.34}_{-1.25}$ &	$^{+1.61}_{-1.75}$ &	$^{+1.42}_{-1.73}$ &	$^{+2.29}_{-1.46}$ &	$^{+0.86}_{-1.22}$ &	$^{+2.18}_{-2.23}$ &	$^{+0.94}_{-1.79}$ &	$^{+2.50}_{-2.58}$ &	$^{+2.65}_{-1.55}$ &	$^{+1.88}_{-1.91}$ &	$^{+2.02}_{-1.86}$ &	$^{+3.05}_{-2.63}$ &	$^{+4.55}_{-4.09}$ \\
\hline
\hline
$b$-Tagged jet energy scale (JES) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.23}$ &	\textrm - &	\textrm - &	{\textrm -} &	{$^{+0.19}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{$^{-0.11}_{+0.14}$} \\
\rowcolor{Gray}
Effective detector NP set 1 (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.23}$ &	$^{+0.28}_{\textrm{ \phantom{ai}-}}$ &	{$^{-0.15}_{+0.42}$} &	{$^{-0.19}_{\textrm{ \phantom{ai}-}}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.34}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.39}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.26}$ &	\textrm - &	{$^{+0.70}_{-0.26}$} &	{$^{+0.20}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{+0.59}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.41}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.32}$ &	{$^{+0.72}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{$^{+0.34}_{\textrm{ \phantom{ai}-}}$} &	$^{+0.34}_{\textrm{ \phantom{ai}-}}$ &	{$^{+0.59}_{\textrm{ \phantom{ai}-}}$} \\
Effective detector NP set 2 (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.27}$ &	\textrm - &	{$^{+0.28}_{-0.11}$} &	{\textrm -} &	{\textrm -} &	\textrm - &	{$^{+0.24}_{\textrm{ \phantom{ai}-}}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.26}$ &	$^{-0.16}_{+0.14}$ &	\textrm - &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.29}$ &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{+0.54}$} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.22}$} \\
\rowcolor{Gray}
Effective detector NP set 3 (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$^{+0.22}_{\textrm{ \phantom{ai}-}}$} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
Effective detector NP set 4 (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Effective detector NP set 5 (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
Effective detector NP set 6 restTerm (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$\eta$ intercalibration model (JES) [\%]	
&	$^{-0.91}_{+0.64}$ &	$^{-0.62}_{+0.66}$ &	$^{-0.61}_{+0.79}$ &	$^{-0.90}_{+0.91}$ &	{$^{-0.60}_{+0.45}$} &	$^{-0.49}_{+0.43}$ &	{$^{-0.21}_{+0.10}$} &	{$^{-0.40}_{+0.17}$} &	{$^{+0.28}_{\textrm{ \phantom{ai}-}}$} &	$^{+0.30}_{-0.31}$ &	$^{+0.39}_{-0.15}$ &	{$^{+0.56}_{-1.07}$} &	$^{+0.66}_{-0.67}$ &	{$^{+1.33}_{-0.46}$} &	{$^{+0.68}_{-1.15}$} &	{$^{+1.54}_{-1.50}$} &	$^{+1.90}_{-1.47}$ &	$^{+2.04}_{-1.62}$ \\
$\eta$ intercalibration total stat (JES) [\%]	
&	$^{-0.37}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	{$^{-0.14}_{+0.36}$} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.25}$ &	$^{+0.23}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.28}$ &	$^{+0.12}_{-0.18}$ &	{$^{+0.48}_{-0.12}$} &	{\textrm -} &	{$^{+0.22}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.37}_{-0.27}$} &	{$^{+0.27}_{-0.24}$} \\
\rowcolor{Gray}
Flavour composition (JES) [\%]	
&	$^{-0.41}_{\textrm{ \phantom{ai}-}}$ &	$^{+0.21}_{\textrm{ \phantom{ai}-}}$ &	{$^{-0.42}_{+0.58}$} &	{$^{+0.33}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.49}$} &	$^{-0.71}_{\textrm{ \phantom{ai}-}}$ &	$^{+0.17}_{-0.16}$ &	\textrm - &	{$^{+0.65}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.24}_{-0.34}$} &	$^{+0.28}_{\textrm{ \phantom{ai}-}}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.20}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.54}$ &	{$^{+0.79}_{-0.22}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.22}$} &	$^{+0.19}_{-0.28}$ &	{$^{+0.55}_{-0.20}$} &	{$^{+0.40}_{\textrm{ \phantom{ai}-}}$} \\
Flavour response (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.51}$ &	\textrm - &	{$^{+0.25}_{-0.13}$} &	$^{+0.28}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	$^{-0.20}_{\textrm{ \phantom{ai}-}}$ &	$^{+0.18}_{-0.24}$ &	$^{+0.19}_{-0.17}$ &	{$^{\textrm{ \phantom{ai}-}}_{+0.43}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.27}$} &	$^{+0.29}_{\textrm{ \phantom{ai}-}}$ &	$^{-0.41}_{\textrm{ \phantom{ai}-}}$ &	$^{-0.40}_{\textrm{ \phantom{ai}-}}$ &	{$^{+0.93}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.15}_{-0.29}$} &	{\textrm -} &	{$^{-0.22}_{+0.70}$} &	{$^{-0.26}_{+0.36}$} \\
\rowcolor{Gray}
Pile-up offset $\mu$ (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.23}$ &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{$^{-0.11}_{+0.24}$} &	{$^{-0.22}_{+0.16}$} \\
Pile-up offset $N_{\textrm PV}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.12}$ &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{+0.21}$} &	\textrm - &	{\textrm -} &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.21}$} \\
\rowcolor{Gray}
Pile-up offset $p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	$^{+0.15}_{-0.14}$ \\
Pile-up offset $\rho$ topology (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.35}$ &	$^{-0.11}_{+0.13}$ &	{$^{\textrm{ \phantom{ai}-}}_{+0.24}$} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{$^{+0.42}_{-0.18}$} &	{\textrm -} &	$^{+0.22}_{\textrm{ \phantom{ai}-}}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.33}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.34}$ &	{$^{+0.92}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.28}_{\textrm{ \phantom{ai}-}}$} &	$^{+0.25}_{\textrm{ \phantom{ai}-}}$ &	$^{+0.32}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} \\
\rowcolor{Gray}
Punch-through (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Single particle high-$p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Jet energy resolution [\%]	
&	$\mp$0.57 &	{$\mp$0.27} &	{\textrm -} &	{$\pm$1.48} &	$\mp$1.34 &	{$\mp$0.32} &	{$\pm$0.17} &	{$\mp$0.64} &	{$\pm$1.25} &	{$\pm$0.53} &	$\mp$0.58 &	{$\pm$0.18} &	{\textrm -} &	{$\pm$0.46} &	$\pm$0.54 &	{$\mp$0.15} &	$\mp$0.18 &	{$\pm$0.38} \\
Jet vertex fraction [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.11} &	{\textrm -} &	\textrm - &	{\textrm -} &	{$^{+0.10}_{-0.11}$} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{$\mp$0.11} &	{$\mp$0.43} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 0) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - \\
$b$-Quark tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - \\
$b$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$c$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$\mp$0.13 &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{$^{+0.17}_{-0.16}$} &	{$\pm$0.13} &	\textrm - &	{$\pm$0.21} &	{$\pm$0.33} \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$c$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 0) [\%]	
&	$^{+0.14}_{-0.20}$ &	{$^{-0.21}_{+0.28}$} &	$^{+0.20}_{-0.24}$ &	{$^{+0.12}_{-0.11}$} &	{$^{-0.10}_{+0.15}$} &	{$^{+0.24}_{-0.29}$} &	{\textrm -} &	{\textrm -} &	{$^{+0.24}_{-0.32}$} &	{\textrm -} &	{$^{-0.17}_{+0.22}$} &	$^{\textrm{ \phantom{ai}-}}_{+0.18}$ &	{$^{+0.16}_{-0.25}$} &	{\textrm -} &	{$^{-0.16}_{\textrm{ \phantom{ai}-}}$} &	\textrm - &	{$^{-0.64}_{+0.81}$} &	{$^{-0.57}_{+0.48}$} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{$\mp$0.12} &	$\mp$0.15 &	{$\mp$0.23} \\
Light-jet tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 5) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 6) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 7) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 8) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 9) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 10) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 11) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$b$-Quark tagging  extrapolation  [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$b$-Quark tagging extrapolation from $c$-Quark [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} \\
Electron energy resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Electron energy scale [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} \\
Electron trigger efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Electron reconstruction efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Electron identification efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Electron isolation efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon (MS) momentum resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon (ID) momentum resolution [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon trigger efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon trigger efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon identification stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon identification syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon isolation efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon isolation efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon TTVA efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon TTVA efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution para [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution perp [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Luminosity [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Single top cross-section [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - \\
$Z$+jets cross-section [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{$\pm$0.23} &	{\textrm -} &	{\textrm -} &	{$\mp$0.11} &	{$\mp$0.22} &	{$\pm$0.15} &	{$\mp$0.23} &	{\textrm -} &	{$\mp$0.18} \\
\rowcolor{Gray}
Diboson cross-section [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
$t\bar{t}V$ cross-section [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Monte Carlo sample statistics [\%]	
&	$\pm$0.44 &	$\pm$0.51 &	$\pm$0.49 &	$\pm$0.51 &	$\pm$0.53 &	$\pm$0.48 &	$\pm$0.53 &	$\pm$0.58 &	$\pm$0.52 &	$\pm$0.63 &	$\pm$0.63 &	$\pm$0.66 &	$\pm$0.65 &	$\pm$0.67 &	$\pm$0.75 &	{$\pm$0.53} &	{$\pm$0.79} &	$\pm$0.82 \\
ISR/FSR + scale [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-1.39}$ &	$^{+0.29}_{-0.44}$ &	{$^{+0.98}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.29}_{-0.10}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.55}$} &	{$^{+0.81}_{\textrm{ \phantom{ai}-}}$} &	$^{-0.67}_{+0.18}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.39}$ &	{$^{+1.35}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.74}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.98}$ &	{$^{+0.31}_{-0.60}$} &	{$^{+0.59}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.66}$} &	{$^{+0.92}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.47}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.70}$} &	{$^{+1.18}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Alternate hard-scattering model [\%]	
&	\textrm - &	{$\mp$1.06} &	{$\pm$0.54} &	{$\mp$0.86} &	{$\pm$2.69} &	{$\pm$0.44} &	{$\mp$1.50} &	{$\mp$0.90} &	{$\pm$0.37} &	{$\mp$0.14} &	{$\pm$1.79} &	{\textrm -} &	{$\mp$2.24} &	{$\mp$0.37} &	{$\pm$0.85} &	$\mp$0.67 &	$\mp$0.53 &	{$\pm$3.21} \\
Alternate parton-shower model [\%]	
&	$\mp$0.13 &	{\textrm -} &	{$\pm$0.12} &	{\textrm -} &	{$\mp$1.03} &	{$\pm$0.21} &	{\textrm -} &	{$\pm$0.61} &	{$\pm$0.16} &	{$\pm$0.11} &	{$\pm$0.24} &	{$\mp$0.54} &	$\pm$0.43 &	{$\pm$0.13} &	{$\pm$0.73} &	{$\mp$0.29} &	{$\mp$1.10} &	$\pm$1.07 \\
\rowcolor{Gray}
Inter PDF [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{$\pm$0.13} \\
Intra PDF [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{$\pm$0.11} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{$\pm$0.10} &	{$\pm$0.18} \\
\rowcolor{Gray}
Real lepton efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Fake lepton efficiency MC scale [\%]	
&	\textrm - &	$^{+0.18}_{-0.19}$ &	\textrm - &	$\pm$0.10 &	$^{+0.13}_{-0.10}$ &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	$^{-0.17}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{$^{-0.12}_{+0.17}$} &	{$^{-0.29}_{+0.34}$} &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{+0.13}$} &	{$^{-0.25}_{+0.17}$} &	{$^{-0.22}_{+0.30}$} \\
\rowcolor{Gray}
Fake lepton efficiency alternate CR [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{$\mp$0.33} &	{\textrm -} \\
Fake overall normalisation [\%]	
&	$\pm$0.39 &	$\pm$0.34 &	$\pm$0.41 &	{\textrm -} &	{$\pm$0.26} &	$\pm$0.27 &	{$\pm$0.12} &	{$\pm$0.26} &	{\textrm -} &	{$\pm$0.20} &	{$\mp$0.48} &	{$\mp$0.20} &	$\mp$0.20 &	{$\mp$0.99} &	{$\mp$0.63} &	{$\mp$0.24} &	{$\mp$1.22} &	$\mp$1.13 \\
\rowcolor{Gray}
$W$+jets $CA_{4incl}$ stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - \\
$W$+jets Fc stat error [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$W$+jets Fcc stat error [\%]	
&	\textrm - &	{\textrm -} &	{$^{-0.18}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$^{+0.18}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{\textrm -} &	{$^{+0.15}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	\textrm - &	{$^{+0.14}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} \\
$W$+jets Flight stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\hline
\end{tabular}}


==> tables/systematics/resolved/table_syst_particle_topH_pt_AbsoluteDiffXs.tex <==
\resizebox*{\textwidth}{!}{
\begin{tabular}{l c c c c c c c c c c c c c c c}
\hline
Bins  [GeV]
 & 0--25   & 25--50   & 50--75   & 75--105   & 105--135   & 135--165   & 165--195   & 195--230   & 230--265   & 265--300   & 300--350   & 350--400   & 400--450   & 450--500   & 500--1000.00  \\
\hline
\hline
d$\sigma$ / d$p_{\textrm T}^{t}$ [pb/GeV]	&	$1.35 \cdot 10^{-1}$ &	$3.91 \cdot 10^{-1}$ &	$5.80 \cdot 10^{-1}$ &	$6.42 \cdot 10^{-1}$ &	$5.74 \cdot 10^{-1}$ &	$4.11 \cdot 10^{-1}$ &	$2.80 \cdot 10^{-1}$ &	$1.84 \cdot 10^{-1}$ &	$1.13 \cdot 10^{-1}$ &	$7.69 \cdot 10^{-2}$ &	$4.08 \cdot 10^{-2}$ &	$2.23 \cdot 10^{-2}$ &	$1.10 \cdot 10^{-2}$ &	$5.24 \cdot 10^{-3}$ &	$7.30 \cdot 10^{-4}$ \\
\hline
\rowcolor{Gray}
Total uncertainty [\%]	
&	$^{+12.5}_{-14.0}$ &	$^{+12.3}_{-13.2}$ &	$^{+11.6}_{-12.7}$ &	$^{+11.1}_{-11.7}$ &	$^{+10.5}_{-11.5}$ &	$^{+10.4}_{-10.6}$ &	$^{+9.27}_{-10.3}$ &	$^{+9.24}_{-11.1}$ &	$^{+9.44}_{-9.53}$ &	$^{+10.0}_{-10.9}$ &	$^{+9.87}_{-10.4}$ &	$^{+11.8}_{-11.4}$ &	$^{+12.2}_{-13.6}$ &	$^{+22.2}_{-23.2}$ &	$^{+18.3}_{-18.6}$ \\
Statistical uncertainty [\%]	
&	$\pm2.0$ &	$\pm1.1$ &	$\pm0.9$ &	$\pm0.7$ &	$\pm0.8$ &	$\pm1.0$ &	$\pm1.2$ &	$\pm1.3$ &	$\pm1.7$ &	$\pm2.1$ &	$\pm2.5$ &	$\pm3.5$ &	$\pm5.2$ &	$\pm8.2$ &	$\pm7.3$ \\
\rowcolor{Gray}
Systematic uncertainty [\%]	
&	$^{+12.2}_{-13.8}$ &	$^{+12.2}_{-13.2}$ &	$^{+11.6}_{-12.7}$ &	$^{+11.1}_{-11.7}$ &	$^{+10.5}_{-11.5}$ &	$^{+10.3}_{-10.5}$ &	$^{+9.18}_{-10.3}$ &	$^{+9.12}_{-11.0}$ &	$^{+9.26}_{-9.34}$ &	$^{+9.78}_{-10.6}$ &	$^{+9.49}_{-10.0}$ &	$^{+11.2}_{-10.8}$ &	$^{+10.8}_{-12.3}$ &	$^{+20.5}_{-21.6}$ &	$^{+16.7}_{-17.0}$ \\
\hline
\hline
$b$-Tagged jet energy scale (JES) [\%]	
&	$^{-0.28}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{$^{+0.25}_{-0.22}$} &	{$^{+0.38}_{-0.33}$} &	{$^{+0.73}_{-0.85}$} &	$^{+0.83}_{-0.79}$ &	$^{+0.81}_{-0.62}$ &	$^{+0.79}_{-0.84}$ &	$^{+0.78}_{-0.69}$ &	$^{+0.72}_{-0.50}$ &	$^{+0.82}_{-0.91}$ &	$^{+0.68}_{-0.51}$ &	{$^{+0.42}_{-0.64}$} &	{$^{+0.99}_{-1.27}$} &	{$^{+0.64}_{-0.51}$} \\
\rowcolor{Gray}
Effective detector NP set 1 (JES) [\%]	
&	$^{+4.90}_{-6.46}$ &	$^{+5.00}_{-6.12}$ &	$^{+4.95}_{-6.28}$ &	$^{+5.31}_{-5.86}$ &	$^{+5.30}_{-6.00}$ &	$^{+5.06}_{-5.48}$ &	$^{+4.58}_{-5.23}$ &	$^{+3.59}_{-5.00}$ &	$^{+3.78}_{-3.80}$ &	{$^{+2.56}_{-3.94}$} &	$^{+3.15}_{-3.74}$ &	$^{+3.44}_{-3.00}$ &	{$^{+2.17}_{-4.00}$} &	{$^{+1.23}_{-4.20}$} &	{$^{+1.70}_{-4.40}$} \\
Effective detector NP set 2 (JES) [\%]	
&	$^{-1.80}_{+1.32}$ &	{$^{-2.02}_{+1.86}$} &	$^{-1.81}_{+1.77}$ &	$^{-1.35}_{+1.48}$ &	{$^{-1.00}_{+0.84}$} &	{$^{-0.27}_{+0.38}$} &	{\textrm -} &	$^{+0.18}_{-0.57}$ &	{$^{+1.19}_{-0.91}$} &	$^{+0.92}_{-1.44}$ &	{$^{+1.51}_{-1.50}$} &	{$^{+3.02}_{-2.76}$} &	{$^{+1.78}_{-2.55}$} &	{$^{+2.80}_{-3.14}$} &	{$^{+5.58}_{-5.07}$} \\
\rowcolor{Gray}
Effective detector NP set 3 (JES) [\%]	
&	$^{+0.52}_{-0.96}$ &	{$^{+0.87}_{-0.94}$} &	$\pm$0.73 &	$^{+0.62}_{-0.68}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.24}$} &	{\textrm -} &	{$^{-0.39}_{+0.31}$} &	$^{-0.75}_{+0.40}$ &	{$^{-0.66}_{+1.03}$} &	{$^{-1.12}_{+0.79}$} &	{$^{-1.03}_{+1.24}$} &	$^{-1.53}_{+1.60}$ &	{$^{-1.49}_{+0.95}$} &	{$^{-2.64}_{+1.91}$} &	{$^{-2.09}_{+2.56}$} \\
Effective detector NP set 4 (JES) [\%]	
&	$^{-0.71}_{+0.50}$ &	$^{-0.57}_{+0.49}$ &	{$^{-0.49}_{+0.35}$} &	$^{-0.39}_{+0.33}$ &	{\textrm -} &	$^{+0.10}_{-0.25}$ &	{$^{+0.35}_{-0.18}$} &	$^{+0.27}_{-0.46}$ &	$^{+0.33}_{-0.42}$ &	$^{+0.29}_{-0.44}$ &	$^{+0.33}_{-0.39}$ &	$^{+0.38}_{-0.14}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.29}$} &	{$^{+0.31}_{-0.23}$} &	{$^{-0.46}_{+0.48}$} \\
\rowcolor{Gray}
Effective detector NP set 5 (JES) [\%]	
&	$^{+0.23}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{\textrm -} &	{\textrm -} &	$^{-0.10}_{+0.11}$ &	$^{-0.14}_{+0.11}$ &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{$\pm$0.34} &	$^{+0.37}_{-0.18}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.51}$} &	{$^{+0.80}_{-0.73}$} &	{$^{+0.31}_{\textrm{ \phantom{ai}-}}$} \\
Effective detector NP set 6 restTerm (JES) [\%]	
&	$^{-0.15}_{\textrm{ \phantom{ai}-}}$ &	{$^{-0.11}_{+0.16}$} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{-0.17}$} &	{$^{+0.14}_{-0.11}$} &	{\textrm -} &	{$^{+0.22}_{-0.34}$} &	{$^{+0.35}_{-0.18}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.31}$} &	{$^{+0.71}_{-0.69}$} &	$^{+0.61}_{-0.52}$ \\
\rowcolor{Gray}
$\eta$ intercalibration model (JES) [\%]	
&	$^{+0.83}_{-1.51}$ &	$^{+1.04}_{-1.36}$ &	$^{+1.04}_{-1.73}$ &	$^{+1.27}_{-1.57}$ &	$^{+1.48}_{-1.86}$ &	$^{+1.70}_{-1.66}$ &	$^{+1.35}_{-1.88}$ &	$^{+1.12}_{-1.78}$ &	$^{+1.23}_{-1.09}$ &	{$^{+0.94}_{-1.78}$} &	$^{+1.08}_{-1.55}$ &	$^{+1.32}_{-1.13}$ &	{$^{+0.51}_{-1.65}$} &	{$^{+0.89}_{-1.38}$} &	{$^{+1.97}_{-2.18}$} \\
$\eta$ intercalibration total stat (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.39}$ &	{$^{+0.48}_{-0.62}$} &	{$^{+0.64}_{-0.67}$} &	$^{+0.59}_{-0.40}$ &	$^{+0.68}_{-0.97}$ &	$^{+0.79}_{-0.69}$ &	$^{+0.75}_{-0.71}$ &	$^{+0.71}_{-0.94}$ &	$^{+0.72}_{-0.43}$ &	{$^{+0.52}_{-1.05}$} &	{$^{+0.99}_{-0.77}$} &	$^{+0.88}_{-0.63}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.89}$} &	{$^{+1.05}_{-0.90}$} &	$^{+1.14}_{-0.79}$ \\
\rowcolor{Gray}
Flavour composition (JES) [\%]	
&	$^{+3.67}_{-5.10}$ &	$^{+3.44}_{-4.33}$ &	$^{+3.21}_{-4.23}$ &	$^{+3.35}_{-3.95}$ &	$^{+3.47}_{-4.19}$ &	$^{+3.53}_{-4.01}$ &	$^{+3.32}_{-3.78}$ &	{$^{+2.50}_{-3.69}$} &	$^{+2.75}_{-2.61}$ &	{$^{+1.60}_{-2.70}$} &	$^{+2.08}_{-2.73}$ &	{$^{+2.75}_{-2.13}$} &	{$^{+1.23}_{-2.40}$} &	{$^{+0.73}_{-2.70}$} &	{$^{+1.65}_{-3.19}$} \\
Flavour response (JES) [\%]	
&	$^{-1.47}_{+0.35}$ &	{$^{-0.97}_{+0.56}$} &	$^{-1.04}_{+0.51}$ &	$^{-0.79}_{+0.51}$ &	{$^{-1.34}_{+0.83}$} &	$^{-1.13}_{+0.92}$ &	$^{-1.38}_{+0.90}$ &	$^{-1.28}_{+0.75}$ &	$^{-0.71}_{+0.82}$ &	{$^{-1.39}_{+0.52}$} &	{$^{-1.16}_{+0.89}$} &	$^{-1.00}_{+0.86}$ &	$^{\textrm{ \phantom{ai}-}}_{-1.02}$ &	$^{-1.56}_{+0.70}$ &	{$^{-0.30}_{+0.11}$} \\
\rowcolor{Gray}
Pile-up offset $\mu$ (JES) [\%]	
&	\textrm - &	$^{-0.17}_{+0.20}$ &	$^{-0.28}_{+0.18}$ &	{$^{-0.12}_{+0.10}$} &	{$^{-0.29}_{+0.20}$} &	$\mp$0.20 &	$^{-0.17}_{+0.18}$ &	{$^{-0.27}_{+0.10}$} &	{\textrm -} &	{\textrm -} &	$^{-0.17}_{+0.13}$ &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.25}$ &	\textrm - &	{$^{+0.74}_{-0.49}$} \\
Pile-up offset $N_{\textrm PV}$ (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.20}$ &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	$^{+0.22}_{\textrm{ \phantom{ai}-}}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.47}$ &	$^{-0.24}_{\textrm{ \phantom{ai}-}}$ &	{$^{+0.81}_{-0.45}$} \\
\rowcolor{Gray}
Pile-up offset $p_{\textrm T}$ (JES) [\%]	
&	$^{-0.23}_{+0.43}$ &	{$^{-0.33}_{+0.29}$} &	$^{-0.20}_{+0.26}$ &	{$\mp$0.13} &	\textrm - &	\textrm - &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.23}$} &	{$^{+0.20}_{\textrm{ \phantom{ai}-}}$} &	$^{+0.18}_{-0.42}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.22}$} &	{$^{+0.34}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.10}_{-0.59}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.43}$ &	{$^{+0.32}_{\textrm{ \phantom{ai}-}}$} \\
Pile-up offset $\rho$ topology (JES) [\%]	
&	$^{+0.76}_{-2.30}$ &	{$^{+1.32}_{-1.97}$} &	$^{+1.32}_{-2.16}$ &	$^{+1.34}_{-1.76}$ &	$^{+1.62}_{-2.18}$ &	$^{+1.59}_{-1.99}$ &	$^{+1.25}_{-1.84}$ &	$^{+1.12}_{-1.77}$ &	$^{+0.89}_{-1.25}$ &	$^{+0.81}_{-1.65}$ &	$^{+1.02}_{-1.45}$ &	{$^{+0.75}_{-0.98}$} &	{$^{\textrm{ \phantom{ai}-}}_{-1.34}$} &	{$^{+0.48}_{-1.86}$} &	$^{+0.45}_{-1.20}$ \\
\rowcolor{Gray}
Punch-through (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.28}$ &	{$^{+0.17}_{\textrm{ \phantom{ai}-}}$} \\
Single particle high-$p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Jet energy resolution [\%]	
&	$\mp$2.08 &	$\mp$2.41 &	$\mp$2.16 &	$\mp$1.80 &	$\mp$1.55 &	{$\mp$0.91} &	$\mp$0.86 &	{$\mp$1.58} &	{$\mp$0.16} &	{$\mp$1.47} &	$\mp$1.23 &	{\textrm -} &	{$\mp$2.18} &	$\mp$2.71 &	$\mp$2.12 \\
Jet vertex fraction [\%]	
&	$^{+5.31}_{-5.11}$ &	$^{+5.34}_{-5.18}$ &	$^{+4.95}_{-4.82}$ &	$^{+4.18}_{-4.09}$ &	$^{+3.50}_{-3.46}$ &	$^{+2.75}_{-2.73}$ &	$^{+2.23}_{-2.20}$ &	$\pm$1.78 &	$^{+1.46}_{-1.45}$ &	$\pm$1.47 &	{$^{+1.05}_{-1.02}$} &	$\pm$0.83 &	{$^{+0.39}_{-0.35}$} &	{$^{+0.89}_{-0.86}$} &	{$^{+0.27}_{-0.19}$} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-4.72}_{+4.81}$ &	$^{-4.61}_{+4.69}$ &	$^{-4.38}_{+4.46}$ &	$^{-4.12}_{+4.19}$ &	$^{-3.96}_{+4.02}$ &	$^{-3.85}_{+3.92}$ &	$^{-3.80}_{+3.86}$ &	$^{-3.75}_{+3.80}$ &	$^{-3.72}_{+3.78}$ &	$^{-3.72}_{+3.78}$ &	$^{-3.74}_{+3.80}$ &	$^{-3.82}_{+3.88}$ &	$^{-3.66}_{+3.71}$ &	$^{-3.81}_{+3.86}$ &	$^{-4.10}_{+4.16}$ \\
$b$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$\mp$0.88 &	$\mp$0.93 &	$\mp$1.02 &	$^{-1.18}_{+1.19}$ &	$\mp$1.40 &	$^{-1.71}_{+1.73}$ &	$^{-2.10}_{+2.12}$ &	$^{-2.53}_{+2.56}$ &	$^{-3.05}_{+3.09}$ &	$^{-3.35}_{+3.40}$ &	$^{-3.71}_{+3.77}$ &	$^{-4.17}_{+4.25}$ &	$^{-4.27}_{+4.36}$ &	$^{-4.52}_{+4.60}$ &	$^{-5.15}_{+5.26}$ \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 2) [\%]	
&	$^{+1.47}_{-1.46}$ &	$^{+1.49}_{-1.48}$ &	$^{+1.46}_{-1.45}$ &	$^{+1.38}_{-1.37}$ &	$\pm$1.25 &	$^{+1.05}_{-1.04}$ &	$^{+0.81}_{-0.80}$ &	{$\pm$0.54} &	{$\pm$0.24} &	{\textrm -} &	{$\mp$0.14} &	{$\mp$0.39} &	{$\mp$0.54} &	$\mp$0.69 &	{$\mp$0.91} \\
$b$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$^{+0.16}_{-0.15}$} &	$\pm$0.19 &	$^{+0.19}_{-0.18}$ &	{$\pm$0.13} &	{\textrm -} &	{\textrm -} &	{$\mp$0.18} &	{$\mp$0.28} &	$\mp$0.35 &	$^{-0.42}_{+0.43}$ &	{$\mp$0.57} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{$\mp$0.10} &	{$\mp$0.14} &	$\mp$0.16 &	$\mp$0.19 &	$\mp$0.24 \\
$c$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-1.74}_{+1.76}$ &	$^{-1.74}_{+1.75}$ &	$^{-1.81}_{+1.82}$ &	$^{-1.67}_{+1.68}$ &	$^{-1.51}_{+1.52}$ &	$^{-1.41}_{+1.42}$ &	$^{-1.19}_{+1.20}$ &	$\mp$1.06 &	$^{-1.05}_{+1.06}$ &	$\mp$0.98 &	$^{-0.87}_{+0.88}$ &	$\mp$0.87 &	$^{-0.91}_{+0.92}$ &	$\mp$1.05 &	$^{-1.34}_{+1.36}$ \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$\pm$0.36 &	$\pm$0.34 &	$\pm$0.31 &	$\pm$0.24 &	{$\pm$0.16} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\mp$0.14} &	$\mp$0.18 &	$\mp$0.15 &	$\mp$0.14 &	{$\mp$0.21} &	$\mp$0.27 \\
$c$-Quark tagging efficiency (eigenvector 2) [\%]	
&	$\pm$0.16 &	$\pm$0.18 &	$\pm$0.21 &	$\pm$0.24 &	$\pm$0.23 &	$\pm$0.18 &	{$\pm$0.13} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 3) [\%]	
&	$\mp$0.11 &	$\mp$0.11 &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 0) [\%]	
&	$^{-2.05}_{+2.41}$ &	$^{-2.16}_{+2.30}$ &	{$^{-1.60}_{+1.67}$} &	$^{-1.43}_{+1.47}$ &	$^{-1.32}_{+1.36}$ &	$^{-1.35}_{+1.38}$ &	$^{-1.42}_{+1.54}$ &	$^{-1.25}_{+1.28}$ &	$^{-1.32}_{+1.35}$ &	$^{-1.58}_{+1.63}$ &	$^{-1.40}_{+1.39}$ &	$^{-1.15}_{+1.21}$ &	{$^{-2.54}_{+3.16}$} &	$\mp$2.71 &	{$^{-3.81}_{+4.06}$} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	$^{+0.20}_{-0.18}$ &	{\textrm -} &	{$\mp$0.11} \\
Light-jet tagging efficiency (eigenvector 2) [\%]	
&	$\pm$0.21 &	$^{+0.21}_{-0.22}$ &	{$\pm$0.13} &	$\pm$0.10 &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{$\mp$0.11} &	$\mp$0.10 &	{$\mp$0.14} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{$\mp$0.18} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 5) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 6) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 7) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 8) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 9) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 10) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 11) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$b$-Quark tagging  extrapolation  [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{$\pm$0.10} &	{$^{+0.20}_{-0.22}$} &	{$\pm$0.41} &	{$\pm$0.97} &	{$^{+1.58}_{-1.57}$} &	{$^{+2.41}_{-2.39}$} &	{$^{+3.44}_{-3.40}$} &	$^{+3.84}_{-3.76}$ &	$^{+4.55}_{-4.48}$ &	{$^{+7.08}_{-6.94}$} \\
\rowcolor{Gray}
$b$-Quark tagging extrapolation from $c$-Quark [\%]	
&	$\pm$0.12 &	$^{+0.12}_{-0.13}$ &	$\pm$0.14 &	$\pm$0.13 &	$\pm$0.11 &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - \\
Electron energy resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Electron energy scale [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
Electron trigger efficiency [\%]	
&	$\pm$0.25 &	$\pm$0.25 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.25 &	$\pm$0.26 &	$\pm$0.27 &	$\pm$0.29 &	$\pm$0.29 &	$\pm$0.30 &	$\pm$0.31 &	$\pm$0.31 &	$\pm$0.31 &	$\pm$0.34 &	$\pm$0.37 \\
\rowcolor{Gray}
Electron reconstruction efficiency [\%]	
&	$\pm$0.15 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.17 &	$\pm$0.19 &	$\pm$0.20 &	$\pm$0.21 &	$\pm$0.22 &	$\pm$0.23 &	$\pm$0.24 &	$\pm$0.25 &	$\pm$0.25 &	$\pm$0.27 &	$\pm$0.30 \\
Electron identification efficiency [\%]	
&	$\pm$0.39 &	$\pm$0.39 &	$\pm$0.39 &	$\pm$0.39 &	$\pm$0.41 &	$\pm$0.43 &	$\pm$0.46 &	$\pm$0.51 &	$\pm$0.55 &	$\pm$0.59 &	$\pm$0.65 &	$\pm$0.71 &	$\pm$0.75 &	$\pm$0.84 &	$\pm$0.99 \\
\rowcolor{Gray}
Electron isolation efficiency [\%]	
&	$\pm$0.12 &	$\pm$0.12 &	$\pm$0.12 &	$\pm$0.13 &	$\pm$0.14 &	$\pm$0.15 &	$\pm$0.18 &	$\pm$0.21 &	$\pm$0.25 &	$\pm$0.29 &	$\pm$0.35 &	$\pm$0.41 &	$\pm$0.47 &	$\pm$0.54 &	$\pm$0.69 \\
Muon energy scale [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon (MS) momentum resolution [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} \\
Muon (ID) momentum resolution [\%]	
&	$^{-0.21}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon trigger efficiency stat [\%]	
&	$^{+0.61}_{-0.63}$ &	$^{+0.59}_{-0.60}$ &	$^{+0.58}_{-0.60}$ &	$^{+0.57}_{-0.58}$ &	$^{+0.56}_{-0.58}$ &	$^{+0.56}_{-0.57}$ &	$^{+0.55}_{-0.57}$ &	$^{+0.55}_{-0.57}$ &	$^{+0.56}_{-0.57}$ &	$^{+0.55}_{-0.57}$ &	$^{+0.55}_{-0.56}$ &	$^{+0.55}_{-0.57}$ &	$^{+0.57}_{-0.59}$ &	$^{+0.57}_{-0.59}$ &	$^{+0.56}_{-0.58}$ \\
Muon trigger efficiency syst [\%]	
&	$^{+0.26}_{-0.25}$ &	$\pm$0.25 &	$\pm$0.25 &	$^{+0.25}_{-0.24}$ &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.24 &	$^{+0.24}_{-0.23}$ &	$^{+0.24}_{-0.23}$ &	$^{+0.24}_{-0.23}$ &	$\pm$0.25 &	$\pm$0.24 &	$^{+0.26}_{-0.25}$ \\
\rowcolor{Gray}
Muon identification stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon identification syst [\%]	
&	$\pm$0.17 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.17 &	$\pm$0.18 &	$\pm$0.20 &	$\pm$0.22 &	$\pm$0.24 &	$\pm$0.26 &	$\pm$0.29 &	$^{+0.34}_{-0.33}$ &	$\pm$0.36 &	$\pm$0.44 \\
\rowcolor{Gray}
Muon isolation efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - \\
Muon isolation efficiency syst [\%]	
&	$\pm$0.11 &	$\pm$0.11 &	$\pm$0.11 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.11 &	$\pm$0.10 &	{$\pm$0.16} \\
\rowcolor{Gray}
Muon TTVA efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon TTVA efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution para [\%]	
&	$\pm$0.12 &	$\pm$0.11 &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{$\pm$0.10} &	{$\pm$0.17} \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution perp [\%]	
&	\textrm - &	{$\mp$0.12} &	$\mp$0.13 &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\mp$0.11} &	{\textrm -} &	\textrm - &	{$\mp$0.19} \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Luminosity [\%]	
&	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 \\
\rowcolor{Gray}
Single top cross-section [\%]	
&	$\pm$0.26 &	$\pm$0.26 &	$\pm$0.25 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.25 &	$\pm$0.27 &	$\pm$0.27 &	$\pm$0.29 &	$\pm$0.30 &	$\pm$0.33 &	$\pm$0.36 &	$\pm$0.39 &	$\pm$0.44 &	{$\pm$0.69} \\
$Z$+jets cross-section [\%]	
&	$\pm$0.59 &	$\pm$0.70 &	$\pm$0.88 &	$\pm$0.68 &	$\pm$0.57 &	{$\pm$0.43} &	$\pm$0.45 &	$\pm$0.38 &	$\pm$0.39 &	$\pm$0.38 &	$\pm$0.33 &	$\pm$0.39 &	{$\pm$0.28} &	{$\pm$0.43} &	{$\pm$0.94} \\
\rowcolor{Gray}
Diboson cross-section [\%]	
&	$\pm$0.18 &	$\pm$0.14 &	$\pm$0.13 &	$\pm$0.12 &	$\pm$0.11 &	$\pm$0.12 &	$\pm$0.13 &	$\pm$0.14 &	$\pm$0.17 &	$\pm$0.17 &	{$\pm$0.24} &	$\pm$0.22 &	{$\pm$0.38} &	$\pm$0.46 &	{$\pm$0.83} \\
$t\bar{t}V$ cross-section [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{$\mp$0.10} &	\textrm - &	{$\mp$0.21} \\
\rowcolor{Gray}
Monte Carlo sample statistics [\%]	
&	$\pm$1.04 &	{$\pm$0.52} &	$\pm$0.41 &	$\pm$0.32 &	$\pm$0.33 &	$\pm$0.36 &	$\pm$0.44 &	$\pm$0.48 &	$\pm$0.55 &	{$\pm$0.78} &	$\pm$0.75 &	{$\pm$1.09} &	{$\pm$1.96} &	$\pm$2.26 &	$\pm$1.94 \\
ISR/FSR + scale [\%]	
&	$^{-3.28}_{+2.58}$ &	{$^{-2.54}_{+1.96}$} &	$^{-2.26}_{+2.33}$ &	{$^{-2.49}_{+1.65}$} &	{$^{-3.08}_{+2.33}$} &	{$^{-2.44}_{+3.21}$} &	{$^{-3.45}_{+1.86}$} &	$^{-3.85}_{+1.73}$ &	{$^{-3.52}_{+2.87}$} &	$^{-2.13}_{+2.93}$ &	{$^{-2.26}_{+1.55}$} &	$^{-1.77}_{+1.66}$ &	{$^{-4.67}_{+3.16}$} &	{$^{-4.00}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.67}_{+1.13}$} \\
\rowcolor{Gray}
Alternate hard-scattering model [\%]	
&	$\mp$0.90 &	{$\mp$0.33} &	$\pm$0.41 &	{\textrm -} &	\textrm - &	{$\mp$0.35} &	$\pm$0.32 &	{$\pm$2.49} &	{$\pm$1.38} &	{$\pm$4.87} &	{$\pm$2.82} &	{$\pm$1.57} &	{$\pm$3.04} &	{$\pm$14.7} &	{$\pm$1.95} \\
Alternate parton-shower model [\%]	
&	$\mp$2.52 &	{$\mp$1.77} &	$\mp$1.58 &	{$\mp$2.28} &	$\mp$2.24 &	$\mp$2.28 &	{$\mp$1.50} &	{$\mp$3.08} &	{$\mp$2.32} &	$\mp$2.03 &	$\mp$2.09 &	{$\mp$5.27} &	{$\mp$2.90} &	{$\mp$9.59} &	{$\mp$6.81} \\
\rowcolor{Gray}
Inter PDF [\%]	
&	\textrm - &	{$\pm$0.13} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{$\pm$0.11} &	{\textrm -} &	\textrm - &	{$\pm$0.14} &	$\pm$0.18 &	{\textrm -} &	{$\mp$0.17} &	{$\pm$1.93} \\
Intra PDF [\%]	
&	\textrm - &	{$\pm$0.15} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{$\pm$0.11} &	{\textrm -} &	\textrm - &	{$\pm$0.13} &	{$\pm$0.28} &	$\pm$0.31 &	{$\pm$1.52} \\
\rowcolor{Gray}
Real lepton efficiency stat [\%]	
&	$\mp$0.11 &	$\mp$0.12 &	$^{-0.13}_{+0.12}$ &	$^{-0.13}_{+0.12}$ &	$^{-0.15}_{+0.14}$ &	$^{-0.16}_{+0.15}$ &	$^{-0.19}_{+0.17}$ &	$^{-0.21}_{+0.19}$ &	$^{-0.25}_{+0.22}$ &	$^{-0.27}_{+0.24}$ &	$^{-0.32}_{+0.26}$ &	$^{-0.39}_{+0.32}$ &	$^{-0.38}_{+0.32}$ &	$^{-0.55}_{+0.37}$ &	{$^{-1.09}_{+0.63}$} \\
Fake lepton efficiency MC scale [\%]	
&	$^{+0.67}_{-0.74}$ &	$^{+0.80}_{-0.86}$ &	$^{+0.67}_{-0.77}$ &	$^{+0.71}_{-0.84}$ &	{$^{+0.53}_{-0.68}$} &	$^{+0.57}_{-0.75}$ &	$^{+0.46}_{-0.58}$ &	{$^{+0.34}_{-0.68}$} &	{$^{+0.51}_{-0.68}$} &	{$^{+0.32}_{-0.34}$} &	{$^{+0.56}_{-0.64}$} &	{$^{+0.26}_{-0.39}$} &	$^{+0.30}_{-1.11}$ &	{$^{+1.05}_{-1.19}$} &	{$^{+0.19}_{-1.23}$} \\
\rowcolor{Gray}
Fake lepton efficiency alternate CR [\%]	
&	$\pm$0.27 &	{$\pm$0.39} &	$\pm$0.40 &	$\pm$0.45 &	{$\pm$0.27} &	$\pm$0.30 &	{$\pm$0.20} &	{$\pm$0.34} &	{$\pm$0.17} &	$\pm$0.14 &	{$\pm$0.31} &	{$\pm$0.44} &	{$\pm$0.18} &	$\pm$0.20 &	{$\pm$0.15} \\
Fake overall normalisation [\%]	
&	$\pm$4.59 &	$\pm$4.88 &	$\pm$4.33 &	$\pm$3.96 &	{$\pm$2.83} &	$\pm$2.82 &	$\pm$2.26 &	$\pm$2.18 &	$\pm$2.31 &	$\pm$1.90 &	$\pm$2.41 &	{$\pm$1.70} &	{$\pm$3.00} &	$\pm$2.76 &	{$\pm$6.06} \\
\rowcolor{Gray}
$W$+jets $CA_{4incl}$ stat error [\%]	
&	$\mp$0.20 &	$\mp$0.18 &	$\mp$0.14 &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\mp$0.15} &	$\mp$0.12 &	{$\mp$0.18} \\
$W$+jets Fc stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$W$+jets Fcc stat error [\%]	
&	$^{+0.62}_{-0.30}$ &	{$^{+0.20}_{-0.10}$} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$^{-0.17}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{$^{+0.65}_{-0.31}$} &	{\textrm -} &	$^{-0.42}_{+0.20}$ \\
$W$+jets Flight stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\hline
\end{tabular}}


==> tables/systematics/resolved/table_syst_particle_topH_pt_RelativeDiffXs.tex <==
\resizebox*{\textwidth}{!}{
\begin{tabular}{l c c c c c c c c c c c c c c c}
\hline
Bins  [GeV]
 & 0--25   & 25--50   & 50--75   & 75--105   & 105--135   & 135--165   & 165--195   & 195--230   & 230--265   & 265--300   & 300--350   & 350--400   & 400--450   & 450--500   & 500--1000.00  \\
\hline
\hline
1/$\sigma$ $\cdot$ d$\sigma$ / d$p_{\textrm T}^{t}$	&	$1.32 \cdot 10^{-3}$ &	$3.82 \cdot 10^{-3}$ &	$5.68 \cdot 10^{-3}$ &	$6.28 \cdot 10^{-3}$ &	$5.61 \cdot 10^{-3}$ &	$4.02 \cdot 10^{-3}$ &	$2.74 \cdot 10^{-3}$ &	$1.79 \cdot 10^{-3}$ &	$1.10 \cdot 10^{-3}$ &	$7.52 \cdot 10^{-4}$ &	$3.99 \cdot 10^{-4}$ &	$2.18 \cdot 10^{-4}$ &	$1.08 \cdot 10^{-4}$ &	$5.13 \cdot 10^{-5}$ &	$7.14 \cdot 10^{-6}$ \\
\hline
\rowcolor{Gray}
Total uncertainty [\%]	
&	$^{+4.08}_{-4.58}$ &	$^{+3.67}_{-3.74}$ &	$^{+2.83}_{-2.97}$ &	$^{+2.00}_{-1.88}$ &	$^{+1.51}_{-1.57}$ &	$^{+2.29}_{-1.88}$ &	$^{+2.68}_{-2.71}$ &	$^{+3.78}_{-4.36}$ &	$^{+5.21}_{-4.42}$ &	$^{+6.75}_{-7.06}$ &	$^{+6.63}_{-6.36}$ &	$^{+9.38}_{-8.54}$ &	$^{+9.44}_{-10.1}$ &	$^{+19.9}_{-20.4}$ &	$^{+15.5}_{-15.0}$ \\
Statistical uncertainty [\%]	
&	$\pm2.0$ &	$\pm1.1$ &	$\pm0.9$ &	$\pm0.7$ &	$\pm0.8$ &	$\pm0.9$ &	$\pm1.1$ &	$\pm1.3$ &	$\pm1.7$ &	$\pm2.1$ &	$\pm2.5$ &	$\pm3.5$ &	$\pm5.2$ &	$\pm8.2$ &	$\pm7.3$ \\
\rowcolor{Gray}
Systematic uncertainty [\%]	
&	$^{+3.38}_{-3.97}$ &	$^{+3.46}_{-3.54}$ &	$^{+2.65}_{-2.80}$ &	$^{+1.84}_{-1.70}$ &	$^{+1.23}_{-1.31}$ &	$^{+2.04}_{-1.57}$ &	$^{+2.36}_{-2.40}$ &	$^{+3.51}_{-4.12}$ &	$^{+4.88}_{-4.03}$ &	$^{+6.35}_{-6.67}$ &	$^{+6.07}_{-5.77}$ &	$^{+8.61}_{-7.68}$ &	$^{+7.61}_{-8.47}$ &	$^{+18.0}_{-18.5}$ &	$^{+13.5}_{-13.0}$ \\
\hline
\hline
$b$-Tagged jet energy scale (JES) [\%]	
&	$^{-0.82}_{+0.61}$ &	$^{-0.42}_{+0.48}$ &	{$^{-0.28}_{+0.30}$} &	{$^{-0.15}_{+0.18}$} &	$^{+0.19}_{-0.33}$ &	{$^{+0.29}_{-0.27}$} &	$^{+0.27}_{-0.10}$ &	$^{+0.25}_{-0.32}$ &	$^{+0.24}_{-0.17}$ &	{\textrm -} &	{$^{+0.28}_{-0.39}$} &	{\textrm -} &	\textrm - &	{$^{+0.45}_{-0.75}$} &	{\textrm -} \\
\rowcolor{Gray}
Effective detector NP set 1 (JES) [\%]	
&	$^{+0.14}_{-0.93}$ &	{$^{+0.23}_{-0.57}$} &	$^{+0.18}_{-0.74}$ &	{$^{+0.53}_{-0.30}$} &	$^{+0.52}_{-0.44}$ &	{$^{+0.29}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.16}_{+0.37}$} &	{$^{-1.10}_{+0.61}$} &	{$^{-0.93}_{+1.88}$} &	$^{-2.09}_{+1.74}$ &	$^{-1.53}_{+1.95}$ &	{$^{-1.25}_{+2.73}$} &	{$^{-2.46}_{+1.68}$} &	$^{-3.36}_{+1.46}$ &	$^{-2.90}_{+1.25}$ \\
Effective detector NP set 2 (JES) [\%]	
&	$^{-1.08}_{+0.65}$ &	{$^{-1.30}_{+1.18}$} &	$\mp$1.09 &	{$^{-0.62}_{+0.81}$} &	{$^{-0.28}_{+0.17}$} &	{$^{+0.45}_{-0.28}$} &	{$^{+0.73}_{-0.74}$} &	$^{+0.92}_{-1.24}$ &	{$^{+1.93}_{-1.57}$} &	$^{+1.66}_{-2.09}$ &	{$^{+2.26}_{-2.16}$} &	{$^{+3.78}_{-3.40}$} &	{$^{+2.53}_{-3.19}$} &	{$^{+3.55}_{-3.78}$} &	{$^{+6.36}_{-5.70}$} \\
\rowcolor{Gray}
Effective detector NP set 3 (JES) [\%]	
&	$^{+0.41}_{-0.79}$ &	{$\pm$0.76} &	$^{+0.61}_{-0.56}$ &	$\pm$0.51 &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{+0.32}$} &	{$^{-0.50}_{+0.48}$} &	$^{-0.86}_{+0.57}$ &	{$^{-0.77}_{+1.21}$} &	$^{-1.22}_{+0.97}$ &	{$^{-1.14}_{+1.42}$} &	$^{-1.64}_{+1.77}$ &	{$^{-1.60}_{+1.12}$} &	{$^{-2.74}_{+2.09}$} &	{$^{-2.19}_{+2.74}$} \\
Effective detector NP set 4 (JES) [\%]	
&	$^{-0.59}_{+0.47}$ &	$^{-0.45}_{+0.46}$ &	{$^{-0.36}_{+0.32}$} &	$^{-0.27}_{+0.30}$ &	{$^{+0.11}_{-0.16}$} &	{$^{+0.22}_{-0.28}$} &	{$^{+0.48}_{-0.20}$} &	$^{+0.40}_{-0.49}$ &	$\pm$0.45 &	$^{+0.41}_{-0.47}$ &	$^{+0.46}_{-0.42}$ &	$^{+0.50}_{-0.17}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.32}$} &	{$^{+0.43}_{-0.26}$} &	{$^{-0.34}_{+0.45}$} \\
\rowcolor{Gray}
Effective detector NP set 5 (JES) [\%]	
&	$^{+0.21}_{-0.11}$ &	{\textrm -} &	{\textrm -} &	{\textrm -} &	$^{-0.12}_{\textrm{ \phantom{ai}-}}$ &	$^{-0.16}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{$^{+0.32}_{-0.36}$} &	$^{+0.35}_{-0.20}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.53}$} &	{$^{+0.78}_{-0.75}$} &	{$^{+0.29}_{\textrm{ \phantom{ai}-}}$} \\
Effective detector NP set 6 restTerm (JES) [\%]	
&	$^{-0.14}_{\textrm{ \phantom{ai}-}}$ &	{$^{-0.10}_{+0.17}$} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{-0.16}$} &	{$^{+0.14}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{$^{+0.23}_{-0.33}$} &	{$^{+0.35}_{-0.16}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.30}$} &	{$^{+0.71}_{-0.67}$} &	$^{+0.61}_{-0.50}$ \\
\rowcolor{Gray}
$\eta$ intercalibration model (JES) [\%]	
&	$^{-0.43}_{+0.14}$ &	{$^{-0.23}_{+0.29}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.22}$} &	\textrm - &	$^{+0.20}_{-0.21}$ &	{$^{+0.42}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.23}$} &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{+0.57}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.33}$} &	$^{-0.19}_{+0.10}$ &	{$^{+0.52}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.75}$} &	$^{-0.38}_{+0.27}$ &	{$^{+0.69}_{-0.53}$} \\
$\eta$ intercalibration total stat (JES) [\%]	
&	$^{-0.74}_{+0.29}$ &	{$^{-0.16}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{+0.28}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.29}$ &	{\textrm -} &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.25}$} &	{$^{+0.26}_{\textrm{ \phantom{ai}-}}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.36}$ &	{$^{+0.34}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.23}_{\textrm{ \phantom{ai}-}}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.58}$ &	{$^{+0.40}_{-0.22}$} &	$^{+0.49}_{-0.11}$ \\
\rowcolor{Gray}
Flavour composition (JES) [\%]	
&	$^{+0.46}_{-1.22}$ &	{$^{+0.23}_{-0.43}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.32}$} &	{\textrm -} &	{$^{+0.26}_{-0.28}$} &	$^{+0.32}_{-0.10}$ &	{\textrm -} &	$^{-0.67}_{+0.23}$ &	{$^{-0.43}_{+1.35}$} &	$^{-1.54}_{+1.26}$ &	$^{-1.07}_{+1.23}$ &	{$^{-0.42}_{+1.85}$} &	$^{-1.90}_{+1.58}$ &	$^{-2.38}_{+1.27}$ &	{$^{-1.49}_{+0.76}$} \\
Flavour response (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.37}$ &	$^{+0.13}_{-0.12}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.17}$} &	{$^{+0.31}_{-0.17}$} &	{$^{-0.23}_{+0.14}$} &	{$^{\textrm{ \phantom{ai}-}}_{+0.23}$} &	$^{-0.27}_{+0.21}$ &	{$^{-0.17}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.39}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.29}$} &	$^{\textrm{ \phantom{ai}-}}_{+0.20}$ &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.71}$} &	$^{-0.46}_{\textrm{ \phantom{ai}-}}$ &	{$^{+0.81}_{-0.57}$} \\
\rowcolor{Gray}
Pile-up offset $\mu$ (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.20}$ &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{+0.11}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	{\textrm -} &	{$^{+0.21}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.40}$} &	{\textrm -} &	{$^{+0.95}_{-0.63}$} \\
Pile-up offset $N_{\textrm PV}$ (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.24}$ &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.51}$ &	$^{-0.26}_{\textrm{ \phantom{ai}-}}$ &	{$^{+0.79}_{-0.48}$} \\
\rowcolor{Gray}
Pile-up offset $p_{\textrm T}$ (JES) [\%]	
&	$^{-0.16}_{+0.37}$ &	{$^{-0.26}_{+0.23}$} &	$^{-0.13}_{+0.20}$ &	{\textrm -} &	\textrm - &	$^{+0.16}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.29}$ &	{$^{+0.27}_{\textrm{ \phantom{ai}-}}$} &	$^{+0.25}_{-0.49}$ &	{$^{+0.15}_{-0.28}$} &	{$^{+0.41}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.17}_{-0.65}$} &	$^{+0.16}_{-0.50}$ &	{$^{+0.39}_{\textrm{ \phantom{ai}-}}$} \\
Pile-up offset $\rho$ topology (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.53}$ &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.25}$ &	\textrm - &	{$^{+0.31}_{-0.27}$} &	$^{+0.27}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{$^{-0.18}_{+0.14}$} &	{$^{-0.41}_{+0.67}$} &	{$^{-0.49}_{+0.26}$} &	{$^{-0.27}_{+0.46}$} &	{$^{-0.54}_{+0.95}$} &	{$^{-1.49}_{+0.57}$} &	{$^{-0.81}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.84}_{+0.72}$} \\
\rowcolor{Gray}
Punch-through (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.28}$ &	{$^{+0.17}_{\textrm{ \phantom{ai}-}}$} \\
Single particle high-$p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Jet energy resolution [\%]	
&	$\mp$0.53 &	{$\mp$0.85} &	{$\mp$0.60} &	{$\mp$0.24} &	{\textrm -} &	{$\pm$0.66} &	$\pm$0.71 &	{\textrm -} &	{$\pm$1.42} &	{\textrm -} &	{$\pm$0.33} &	{$\pm$1.62} &	{$\mp$0.63} &	{$\mp$1.17} &	{$\mp$0.57} \\
Jet vertex fraction [\%]	
&	$\pm$1.78 &	$^{+1.81}_{-1.85}$ &	$^{+1.43}_{-1.48}$ &	{$^{+0.69}_{-0.72}$} &	{\textrm -} &	{$\mp$0.68} &	{$^{-1.19}_{+1.23}$} &	{$^{-1.61}_{+1.67}$} &	$^{-1.93}_{+2.00}$ &	$^{-1.92}_{+1.98}$ &	$^{-2.33}_{+2.45}$ &	$^{-2.54}_{+2.64}$ &	$^{-2.96}_{+3.14}$ &	$^{-2.48}_{+2.61}$ &	$^{-3.07}_{+3.31}$ \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-0.68}_{+0.65}$ &	$^{-0.56}_{+0.53}$ &	{$^{-0.33}_{+0.31}$} &	{\textrm -} &	{$\pm$0.10} &	{$^{+0.21}_{-0.20}$} &	$^{+0.27}_{-0.25}$ &	$^{+0.33}_{-0.31}$ &	$^{+0.35}_{-0.33}$ &	$^{+0.35}_{-0.34}$ &	$^{+0.33}_{-0.31}$ &	{$^{+0.25}_{-0.23}$} &	{$^{+0.41}_{-0.40}$} &	{$^{+0.26}_{-0.25}$} &	{\textrm -} \\
$b$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$^{+0.80}_{-0.79}$ &	$^{+0.75}_{-0.74}$ &	$^{+0.66}_{-0.65}$ &	{$^{+0.50}_{-0.49}$} &	{$\pm$0.28} &	{\textrm -} &	{$^{-0.43}_{+0.42}$} &	{$^{-0.86}_{+0.85}$} &	{$^{-1.39}_{+1.37}$} &	$^{-1.69}_{+1.67}$ &	$^{-2.06}_{+2.04}$ &	$^{-2.54}_{+2.51}$ &	$^{-2.64}_{+2.62}$ &	$^{-2.88}_{+2.86}$ &	$^{-3.53}_{+3.50}$ \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 2) [\%]	
&	$^{+0.39}_{-0.40}$ &	$^{+0.41}_{-0.42}$ &	$^{+0.38}_{-0.39}$ &	$^{+0.30}_{-0.31}$ &	{$\pm$0.18} &	{\textrm -} &	{$^{-0.25}_{+0.26}$} &	{$\mp$0.52} &	{$^{-0.81}_{+0.82}$} &	$^{-0.99}_{+1.01}$ &	$^{-1.20}_{+1.22}$ &	$^{-1.44}_{+1.47}$ &	$^{-1.60}_{+1.63}$ &	$^{-1.74}_{+1.77}$ &	$^{-1.96}_{+2.00}$ \\
$b$-Quark tagging efficiency (eigenvector 3) [\%]	
&	$\mp$0.14 &	$\mp$0.12 &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.12} &	$\pm$0.11 &	{\textrm -} &	\textrm - &	{$\mp$0.14} &	{$\mp$0.25} &	{$^{-0.35}_{+0.36}$} &	$\mp$0.42 &	$\mp$0.50 &	$\mp$0.64 \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{$\mp$0.12} &	$\mp$0.13 &	$\mp$0.16 &	{$\mp$0.21} \\
$c$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-0.26}_{+0.27}$ &	$^{-0.26}_{+0.25}$ &	$^{-0.33}_{+0.32}$ &	{$\mp$0.19} &	{\textrm -} &	{\textrm -} &	{$\pm$0.28} &	{$^{+0.42}_{-0.41}$} &	$\pm$0.42 &	$^{+0.50}_{-0.49}$ &	$^{+0.61}_{-0.60}$ &	$^{+0.61}_{-0.60}$ &	$^{+0.57}_{-0.55}$ &	{$\pm$0.43} &	{$^{+0.13}_{-0.11}$} \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$\pm$0.20 &	$\pm$0.19 &	$\pm$0.16 &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\mp$0.13} &	{$\mp$0.18} &	$\mp$0.22 &	{$\mp$0.29} &	$\mp$0.33 &	$\mp$0.30 &	$^{-0.29}_{+0.30}$ &	$\mp$0.36 &	$^{-0.42}_{+0.43}$ \\
$c$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	$\mp$0.10 &	{$\mp$0.17} &	$\mp$0.20 &	$\mp$0.19 &	$\mp$0.19 &	$^{-0.22}_{+0.23}$ &	$\mp$0.25 \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 0) [\%]	
&	$^{-0.53}_{+0.80}$ &	$^{-0.65}_{+0.70}$ &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.11}$ &	{$^{+0.19}_{-0.22}$} &	$^{+0.16}_{-0.20}$ &	{\textrm -} &	{$^{+0.27}_{-0.30}$} &	{$^{+0.20}_{-0.23}$} &	{\textrm -} &	{$^{+0.12}_{-0.19}$} &	{$\pm$0.37} &	{$^{-1.03}_{+1.54}$} &	{$^{-1.20}_{+1.10}$} &	{$^{-2.33}_{+2.43}$} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{$^{+0.17}_{-0.15}$} &	{$\mp$0.12} &	$^{-0.14}_{+0.15}$ \\
Light-jet tagging efficiency (eigenvector 2) [\%]	
&	$^{+0.13}_{-0.12}$ &	$^{+0.12}_{-0.13}$ &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{$\mp$0.12} &	$\mp$0.10 &	{$\mp$0.16} &	$\mp$0.20 &	$^{-0.18}_{+0.19}$ &	$\mp$0.23 \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{$\mp$0.21} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 5) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 6) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 7) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 8) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 9) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 10) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 11) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$b$-Quark tagging  extrapolation  [\%]	
&	$\mp$0.31 &	$^{-0.31}_{+0.30}$ &	$\mp$0.31 &	$\mp$0.29 &	$\mp$0.28 &	$^{-0.23}_{+0.22}$ &	{$^{-0.13}_{+0.11}$} &	{\textrm -} &	{$\pm$0.63} &	{$\pm$1.24} &	{$^{+2.07}_{-2.06}$} &	{$^{+3.10}_{-3.07}$} &	$^{+3.49}_{-3.44}$ &	$^{+4.20}_{-4.15}$ &	{$^{+6.72}_{-6.62}$} \\
\rowcolor{Gray}
$b$-Quark tagging extrapolation from $c$-Quark [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - \\
Electron energy resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Electron energy scale [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{+0.13}$} \\
Electron trigger efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{$\pm$0.10} \\
\rowcolor{Gray}
Electron reconstruction efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\pm$0.12} \\
Electron identification efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{$\pm$0.10} &	{$\pm$0.15} &	{$\pm$0.21} &	$\pm$0.26 &	$\pm$0.31 &	$\pm$0.39 &	{$\pm$0.55} \\
\rowcolor{Gray}
Electron isolation efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{$\pm$0.12} &	{$\pm$0.18} &	{$\pm$0.24} &	$\pm$0.30 &	$\pm$0.37 &	{$^{+0.51}_{-0.52}$} \\
Muon energy scale [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon (MS) momentum resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon (ID) momentum resolution [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Muon trigger efficiency stat [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - \\
Muon trigger efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon identification stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon identification syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{$\pm$0.11} &	{$\pm$0.15} &	$\pm$0.18 &	{$^{+0.26}_{-0.25}$} \\
\rowcolor{Gray}
Muon isolation efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
Muon isolation efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon TTVA efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon TTVA efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution para [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution perp [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	$\mp$0.10 \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Luminosity [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Single top cross-section [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{$\pm$0.12} &	{$\pm$0.18} &	{$\pm$0.42} \\
$Z$+jets cross-section [\%]	
&	\textrm - &	$\pm$0.11 &	{$\pm$0.29} &	{\textrm -} &	{\textrm -} &	{$\mp$0.15} &	$\mp$0.13 &	{$\mp$0.20} &	$\mp$0.18 &	$\mp$0.20 &	$\mp$0.25 &	{$\mp$0.19} &	{$\mp$0.29} &	{$\mp$0.15} &	{$\pm$0.35} \\
\rowcolor{Gray}
Diboson cross-section [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\pm$0.10} &	{\textrm -} &	{$\pm$0.24} &	{$\pm$0.32} &	{$\pm$0.68} \\
$t\bar{t}V$ cross-section [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$\mp$0.13 \\
\rowcolor{Gray}
Monte Carlo sample statistics [\%]	
&	$\pm$1.02 &	{$\pm$0.50} &	$\pm$0.39 &	$\pm$0.30 &	$\pm$0.31 &	$\pm$0.35 &	$\pm$0.43 &	$\pm$0.47 &	$\pm$0.55 &	{$\pm$0.78} &	$\pm$0.75 &	{$\pm$1.08} &	{$\pm$1.95} &	$\pm$2.26 &	$\pm$1.94 \\
ISR/FSR + scale [\%]	
&	$^{-0.51}_{+0.36}$ &	{$^{+0.25}_{-0.24}$} &	{$^{+0.53}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.30}_{-0.54}$} &	$^{-0.31}_{+0.11}$ &	{$^{+0.97}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.69}$} &	$^{\textrm{ \phantom{ai}-}}_{-1.10}$ &	$^{-0.76}_{+0.64}$ &	{$^{+0.69}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.53}_{-0.64}$} &	{$^{+1.03}_{-0.53}$} &	{$^{-1.94}_{+0.92}$} &	$^{\textrm{ \phantom{ai}-}}_{-2.15}$ &	{$^{+2.17}_{-1.05}$} \\
\rowcolor{Gray}
Alternate hard-scattering model [\%]	
&	$\mp$1.39 &	{$\mp$0.83} &	{\textrm -} &	{$\mp$0.44} &	$\mp$0.54 &	{$\mp$0.84} &	{$\mp$0.17} &	{$\pm$1.98} &	{$\pm$0.88} &	{$\pm$4.35} &	{$\pm$2.31} &	{$\pm$1.06} &	{$\pm$2.53} &	{$\pm$14.1} &	{$\pm$1.44} \\
Alternate parton-shower model [\%]	
&	$\mp$0.31 &	{$\pm$0.44} &	{$\pm$0.64} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.72} &	$\mp$0.88 &	{$\mp$0.11} &	{$\pm$0.17} &	{$\pm$0.12} &	{$\mp$3.13} &	{$\mp$0.71} &	{$\mp$7.54} &	{$\mp$4.70} \\
\rowcolor{Gray}
Inter PDF [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{$\pm$0.11} &	$\mp$0.14 &	{$\mp$0.24} &	{$\pm$1.86} \\
Intra PDF [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.21} &	$\pm$0.24 &	{$\pm$1.45} \\
\rowcolor{Gray}
Real lepton efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	$^{-0.14}_{+0.10}$ &	{$^{-0.21}_{+0.16}$} &	$^{-0.20}_{+0.16}$ &	{$^{-0.38}_{+0.22}$} &	{$^{-0.92}_{+0.47}$} \\
Fake lepton efficiency MC scale [\%]	
&	\textrm - &	{$^{+0.21}_{-0.12}$} &	{\textrm -} &	{$^{+0.12}_{-0.10}$} &	{\textrm -} &	{\textrm -} &	{$^{-0.12}_{+0.15}$} &	{$^{-0.24}_{\textrm{ \phantom{ai}-}}$} &	\textrm - &	{$^{-0.26}_{+0.39}$} &	{\textrm -} &	{$^{-0.32}_{+0.34}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.37}$ &	{$\pm$0.45} &	{$^{\textrm{ \phantom{ai}-}}_{-0.50}$} \\
\rowcolor{Gray}
Fake lepton efficiency alternate CR [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{$\pm$0.11} &	{\textrm -} &	{\textrm -} &	{$\mp$0.12} &	{\textrm -} &	{$\mp$0.15} &	$\mp$0.18 &	{\textrm -} &	{$\pm$0.11} &	$\mp$0.14 &	$\mp$0.12 &	{$\mp$0.17} \\
Fake overall normalisation [\%]	
&	$\pm$1.21 &	$\pm$1.49 &	{$\pm$0.96} &	{$\pm$0.60} &	$\mp$0.49 &	$\mp$0.50 &	{$\mp$1.04} &	$\mp$1.12 &	$\mp$0.99 &	{$\mp$1.38} &	{$\mp$0.89} &	{$\mp$1.58} &	{$\mp$0.32} &	{$\mp$0.55} &	{$\pm$2.64} \\
\rowcolor{Gray}
$W$+jets $CA_{4incl}$ stat error [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
$W$+jets Fc stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$W$+jets Fcc stat error [\%]	
&	$^{+0.62}_{-0.30}$ &	{$^{+0.20}_{-0.10}$} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$^{-0.17}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{$^{+0.65}_{-0.31}$} &	{\textrm -} &	$^{-0.42}_{+0.20}$ \\
$W$+jets Flight stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\hline
\end{tabular}}


==> tables/systematics/resolved/table_syst_particle_tt_absrap_AbsoluteDiffXs.tex <==
\resizebox*{\textwidth}{!}{
\begin{tabular}{l c c c c c c c c c c c c c c c c c c}
\hline
Bins  [ Unit $|y^{t\bar{t}}|$ ]
 & 0--0.10   & 0.10--0.20   & 0.20--0.30   & 0.30--0.40   & 0.40--0.50   & 0.50--0.60   & 0.60--0.70   & 0.70--0.80   & 0.80--0.90   & 0.90--1   & 1--1.10   & 1.10--1.20   & 1.20--1.30   & 1.30--1.40   & 1.40--1.50   & 1.50--1.60   & 1.60--1.80   & 1.80--2.50  \\
\hline
\hline
d$\sigma$ / d$|y^{t\bar{t}}|$ [pb/ Unit $|y^{t\bar{t}}|$ ]	&	$1.04 \cdot 10^{2}$ &	$1.05 \cdot 10^{2}$ &	$1.02 \cdot 10^{2}$ &	$9.80 \cdot 10^{1}$ &	$9.56 \cdot 10^{1}$ &	$8.61 \cdot 10^{1}$ &	$7.71 \cdot 10^{1}$ &	$7.07 \cdot 10^{1}$ &	$6.13 \cdot 10^{1}$ &	$5.17 \cdot 10^{1}$ &	$4.27 \cdot 10^{1}$ &	$3.54 \cdot 10^{1}$ &	$2.78 \cdot 10^{1}$ &	$2.25 \cdot 10^{1}$ &	$1.53 \cdot 10^{1}$ &	$1.12 \cdot 10^{1}$ &	$6.20 \cdot 10^{0}$ &	$6.32 \cdot 10^{-1}$ \\
\hline
\rowcolor{Gray}
Total uncertainty [\%]	
&	$^{+10.2}_{-11.5}$ &	$^{+10.1}_{-11.0}$ &	$^{+10.7}_{-11.9}$ &	$^{+10.5}_{-11.3}$ &	$^{+10.6}_{-11.3}$ &	$^{+10.4}_{-10.9}$ &	$^{+10.3}_{-10.6}$ &	$^{+10.3}_{-11.4}$ &	$^{+10.3}_{-11.8}$ &	$^{+10.4}_{-11.5}$ &	$^{+10.2}_{-11.2}$ &	$^{+10.3}_{-10.6}$ &	$^{+10.6}_{-12.4}$ &	$^{+11.3}_{-11.5}$ &	$^{+12.5}_{-12.3}$ &	$^{+11.8}_{-11.2}$ &	$^{+10.8}_{-13.6}$ &	$^{+14.3}_{-14.1}$ \\
Statistical uncertainty [\%]	
&	$\pm1.0$ &	$\pm0.9$ &	$\pm1.0$ &	$\pm1.0$ &	$\pm1.0$ &	$\pm1.1$ &	$\pm1.1$ &	$\pm1.2$ &	$\pm1.2$ &	$\pm1.4$ &	$\pm1.5$ &	$\pm1.7$ &	$\pm1.9$ &	$\pm2.2$ &	$\pm2.7$ &	$\pm3.2$ &	$\pm3.3$ &	$\pm5.7$ \\
\rowcolor{Gray}
Systematic uncertainty [\%]	
&	$^{+10.1}_{-11.5}$ &	$^{+10.1}_{-10.9}$ &	$^{+10.6}_{-11.8}$ &	$^{+10.4}_{-11.2}$ &	$^{+10.5}_{-11.3}$ &	$^{+10.3}_{-10.8}$ &	$^{+10.2}_{-10.5}$ &	$^{+10.3}_{-11.4}$ &	$^{+10.2}_{-11.7}$ &	$^{+10.3}_{-11.4}$ &	$^{+10.0}_{-11.1}$ &	$^{+10.2}_{-10.5}$ &	$^{+10.3}_{-12.3}$ &	$^{+11.1}_{-11.2}$ &	$^{+12.1}_{-11.9}$ &	$^{+11.2}_{-10.6}$ &	$^{+10.2}_{-13.1}$ &	$^{+13.0}_{-12.7}$ \\
\hline
\hline
$b$-Tagged jet energy scale (JES) [\%]	
&	$\pm$0.48 &	$^{+0.56}_{-0.50}$ &	{$^{+0.38}_{-0.50}$} &	{$^{+0.58}_{-0.48}$} &	$^{+0.73}_{-0.55}$ &	{$^{+0.56}_{-0.46}$} &	$^{+0.50}_{-0.44}$ &	$^{+0.53}_{-0.51}$ &	$^{+0.45}_{-0.69}$ &	{$^{+0.59}_{-0.54}$} &	$^{+0.50}_{-0.60}$ &	{$^{+0.26}_{-0.38}$} &	{$^{+0.71}_{-0.59}$} &	$^{+0.79}_{-0.54}$ &	$^{+0.61}_{-0.60}$ &	$^{+0.55}_{-0.71}$ &	{$^{+0.24}_{-0.43}$} &	{$^{+0.52}_{-0.50}$} \\
\rowcolor{Gray}
Effective detector NP set 1 (JES) [\%]	
&	$^{+4.42}_{-5.54}$ &	$^{+4.72}_{-5.63}$ &	$^{+4.94}_{-5.53}$ &	$^{+5.17}_{-5.79}$ &	$^{+4.82}_{-5.84}$ &	$^{+4.65}_{-5.24}$ &	$^{+4.72}_{-5.03}$ &	$^{+4.69}_{-5.87}$ &	$^{+4.98}_{-6.25}$ &	$^{+4.75}_{-5.48}$ &	$^{+4.46}_{-5.50}$ &	$^{+4.43}_{-5.30}$ &	$^{+4.59}_{-6.08}$ &	$^{+5.16}_{-5.53}$ &	$^{+5.21}_{-5.23}$ &	$^{+5.62}_{-5.42}$ &	$^{+4.38}_{-6.10}$ &	$^{+5.27}_{-4.90}$ \\
Effective detector NP set 2 (JES) [\%]	
&	$^{-0.89}_{+0.71}$ &	$^{-0.62}_{+0.82}$ &	{$^{-0.66}_{+0.55}$} &	{$^{-0.87}_{+0.78}$} &	$^{-0.92}_{+0.65}$ &	$^{-0.70}_{+0.64}$ &	{$^{-0.71}_{+0.92}$} &	$^{-0.64}_{+0.79}$ &	{$^{-0.92}_{+0.59}$} &	$^{-0.85}_{+0.72}$ &	{$^{-0.77}_{+0.34}$} &	{$^{-0.42}_{+0.77}$} &	$^{-0.84}_{+0.70}$ &	$^{-0.58}_{+0.67}$ &	$^{-0.48}_{+0.67}$ &	{$^{-0.78}_{+1.46}$} &	$^{\textrm{ \phantom{ai}-}}_{-1.18}$ &	$^{-0.39}_{+0.51}$ \\
\rowcolor{Gray}
Effective detector NP set 3 (JES) [\%]	
&	$^{+0.11}_{-0.18}$ &	$^{+0.14}_{-0.16}$ &	$^{+0.15}_{-0.28}$ &	$\pm$0.19 &	{$^{\textrm{ \phantom{ai}-}}_{-0.21}$} &	{$^{+0.12}_{-0.20}$} &	{$^{+0.26}_{-0.23}$} &	$^{+0.21}_{\textrm{ \phantom{ai}-}}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.27}$ &	$^{+0.12}_{-0.23}$ &	\textrm - &	$^{+0.17}_{-0.19}$ &	{\textrm -} &	\textrm - &	{\textrm -} &	{$^{+0.93}_{-0.15}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.31}$} &	\textrm - \\
Effective detector NP set 4 (JES) [\%]	
&	\textrm - &	{\textrm -} &	{$^{-0.20}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.20}$ &	$^{-0.15}_{\textrm{ \phantom{ai}-}}$ &	{$^{-0.13}_{+0.10}$} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{+0.14}$} &	{$^{+0.32}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.26}$} &	$^{+0.13}_{-0.23}$ \\
\rowcolor{Gray}
Effective detector NP set 5 (JES) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{+0.26}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{$^{-0.29}_{\textrm{ \phantom{ai}-}}$} \\
Effective detector NP set 6 restTerm (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.18}$ &	{$^{+0.28}_{\textrm{ \phantom{ai}-}}$} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$\eta$ intercalibration model (JES) [\%]	
&	$^{+0.38}_{-1.39}$ &	{$^{+1.04}_{-1.12}$} &	$^{+1.05}_{-1.32}$ &	$^{+1.30}_{-1.28}$ &	$^{+1.01}_{-1.62}$ &	$^{+0.92}_{-1.26}$ &	{$^{+1.50}_{-1.40}$} &	$^{+1.27}_{-1.99}$ &	$^{+1.45}_{-2.25}$ &	$^{+1.60}_{-1.96}$ &	$^{+1.89}_{-1.85}$ &	$^{+1.67}_{-1.90}$ &	$^{+1.75}_{-3.07}$ &	{$^{+2.71}_{-2.69}$} &	$^{+3.10}_{-2.55}$ &	$^{+2.58}_{-2.80}$ &	$^{+2.93}_{-4.03}$ &	$^{+3.34}_{-3.21}$ \\
$\eta$ intercalibration total stat (JES) [\%]	
&	$^{+0.54}_{-0.63}$ &	$^{+0.70}_{-0.61}$ &	{$^{+0.52}_{-0.53}$} &	$^{+0.57}_{-0.64}$ &	$^{+0.57}_{-0.87}$ &	$\pm$0.60 &	$^{+0.78}_{-0.46}$ &	{$^{+0.54}_{-0.67}$} &	{$^{+0.72}_{-1.06}$} &	$^{+0.72}_{-0.65}$ &	{$^{+0.52}_{-0.84}$} &	{$^{+0.94}_{-0.56}$} &	{$^{+0.72}_{-0.77}$} &	{$^{+0.95}_{-1.00}$} &	$^{+1.00}_{-0.75}$ &	$^{+1.16}_{-0.53}$ &	{$^{+0.32}_{-1.40}$} &	{$^{+0.96}_{-0.80}$} \\
\rowcolor{Gray}
Flavour composition (JES) [\%]	
&	$^{+2.81}_{-3.70}$ &	$^{+3.27}_{-3.84}$ &	$^{+3.40}_{-3.96}$ &	$^{+3.30}_{-4.08}$ &	$^{+3.32}_{-4.04}$ &	$^{+2.99}_{-3.64}$ &	$^{+3.13}_{-3.63}$ &	$^{+3.21}_{-4.18}$ &	$^{+3.24}_{-4.36}$ &	$^{+3.15}_{-4.13}$ &	$^{+3.43}_{-3.33}$ &	$^{+3.13}_{-3.51}$ &	$^{+2.94}_{-4.90}$ &	$^{+3.65}_{-4.66}$ &	$^{+3.39}_{-3.51}$ &	$^{+3.99}_{-3.47}$ &	{$^{+2.88}_{-4.72}$} &	{$^{+4.21}_{-4.17}$} \\
Flavour response (JES) [\%]	
&	$^{-1.14}_{+0.61}$ &	$^{-1.00}_{+0.63}$ &	$^{-0.98}_{+0.59}$ &	{$^{-1.20}_{+0.83}$} &	{$^{-1.18}_{+0.61}$} &	$^{-0.99}_{+0.58}$ &	{$^{-0.99}_{+0.78}$} &	$^{-1.10}_{+0.65}$ &	$^{-1.37}_{+0.76}$ &	{$^{-1.05}_{+0.51}$} &	$^{-1.14}_{+0.62}$ &	{$^{-0.98}_{+1.06}$} &	{$^{-1.06}_{+0.69}$} &	$^{-1.14}_{+0.88}$ &	$^{-0.86}_{+1.10}$ &	$^{-1.18}_{+0.98}$ &	{$^{-2.21}_{+0.48}$} &	{$^{-1.18}_{+1.30}$} \\
\rowcolor{Gray}
Pile-up offset $\mu$ (JES) [\%]	
&	$^{-0.22}_{+0.10}$ &	{$^{-0.12}_{+0.16}$} &	{\textrm -} &	{$^{-0.19}_{+0.10}$} &	{$^{-0.24}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.23}_{+0.22}$} &	{$^{-0.19}_{+0.15}$} &	{\textrm -} &	{$^{-0.31}_{+0.23}$} &	$^{-0.23}_{+0.19}$ &	{$^{-0.31}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.17}_{+0.30}$} &	{$^{-0.18}_{+0.14}$} &	{$^{-0.33}_{+0.32}$} &	$^{-0.29}_{+0.37}$ &	{$^{\textrm{ \phantom{ai}-}}_{+0.56}$} &	{$^{-0.59}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.25}_{+0.15}$} \\
Pile-up offset $N_{\textrm PV}$ (JES) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{+0.21}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.26}$} &	{$^{+0.33}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.73}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.34}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.20}$ \\
\rowcolor{Gray}
Pile-up offset $p_{\textrm T}$ (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{+0.14}$ &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$^{-0.16}_{+0.11}$} &	{\textrm -} &	{$^{-0.15}_{+0.14}$} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.20}$ &	$^{+0.18}_{-0.14}$ &	{\textrm -} &	{$^{+0.49}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.23}$} &	$^{+0.19}_{-0.26}$ \\
Pile-up offset $\rho$ topology (JES) [\%]	
&	$^{+1.09}_{-1.99}$ &	$^{+1.31}_{-1.76}$ &	$^{+1.26}_{-1.82}$ &	$^{+1.53}_{-2.06}$ &	$^{+1.23}_{-2.15}$ &	$^{+1.33}_{-1.75}$ &	$^{+1.57}_{-1.78}$ &	{$^{+1.16}_{-1.93}$} &	$^{+1.28}_{-2.24}$ &	$^{+1.31}_{-1.89}$ &	$^{+1.14}_{-1.91}$ &	$^{+1.34}_{-1.71}$ &	$^{+1.29}_{-1.79}$ &	$^{+1.63}_{-1.86}$ &	$^{+1.82}_{-1.71}$ &	$^{+1.68}_{-1.96}$ &	{$^{+0.97}_{-2.47}$} &	{$^{+1.37}_{-1.56}$} \\
\rowcolor{Gray}
Punch-through (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Single particle high-$p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Jet energy resolution [\%]	
&	$\mp$1.77 &	$\mp$1.42 &	{$\mp$1.95} &	{$\mp$0.78} &	{$\mp$1.53} &	$\mp$1.53 &	{$\mp$0.75} &	{$\mp$1.79} &	$\mp$1.62 &	$\mp$1.75 &	$\mp$1.65 &	$\mp$1.46 &	{$\mp$2.72} &	$\mp$2.49 &	$\mp$2.21 &	{$\mp$1.46} &	{$\mp$2.20} &	{$\mp$3.22} \\
Jet vertex fraction [\%]	
&	$^{+3.50}_{-3.43}$ &	$^{+3.54}_{-3.48}$ &	$^{+3.49}_{-3.43}$ &	$^{+3.45}_{-3.39}$ &	$^{+3.49}_{-3.40}$ &	$^{+3.52}_{-3.44}$ &	$^{+3.52}_{-3.45}$ &	$^{+3.49}_{-3.43}$ &	$^{+3.43}_{-3.36}$ &	$^{+3.52}_{-3.45}$ &	$^{+3.41}_{-3.35}$ &	$^{+3.43}_{-3.35}$ &	$^{+3.57}_{-3.49}$ &	$^{+3.47}_{-3.40}$ &	$^{+3.57}_{-3.51}$ &	$^{+3.38}_{-3.32}$ &	$^{+3.28}_{-3.23}$ &	$^{+3.12}_{-3.06}$ \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-4.13}_{+4.20}$ &	$^{-4.09}_{+4.16}$ &	$^{-4.09}_{+4.16}$ &	$^{-4.06}_{+4.13}$ &	$^{-4.12}_{+4.19}$ &	$^{-4.08}_{+4.15}$ &	$^{-4.05}_{+4.12}$ &	$^{-4.05}_{+4.12}$ &	$^{-4.05}_{+4.12}$ &	$^{-4.03}_{+4.09}$ &	$^{-4.02}_{+4.09}$ &	$^{-4.00}_{+4.06}$ &	$^{-4.02}_{+4.08}$ &	$^{-3.94}_{+4.00}$ &	$^{-3.92}_{+3.98}$ &	$^{-3.92}_{+3.99}$ &	$^{-3.87}_{+3.94}$ &	$^{-4.03}_{+4.10}$ \\
$b$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$^{-1.63}_{+1.65}$ &	$^{-1.64}_{+1.65}$ &	$^{-1.65}_{+1.67}$ &	$^{-1.63}_{+1.64}$ &	$^{-1.65}_{+1.67}$ &	$^{-1.64}_{+1.66}$ &	$^{-1.66}_{+1.67}$ &	$^{-1.65}_{+1.66}$ &	$^{-1.65}_{+1.67}$ &	$^{-1.65}_{+1.67}$ &	$^{-1.66}_{+1.68}$ &	$^{-1.69}_{+1.71}$ &	$^{-1.69}_{+1.71}$ &	$^{-1.68}_{+1.69}$ &	$^{-1.70}_{+1.71}$ &	$^{-1.68}_{+1.70}$ &	$^{-1.73}_{+1.75}$ &	$^{-1.81}_{+1.83}$ \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 2) [\%]	
&	$^{+1.08}_{-1.07}$ &	$^{+1.09}_{-1.08}$ &	$^{+1.08}_{-1.07}$ &	$^{+1.08}_{-1.07}$ &	$^{+1.09}_{-1.08}$ &	$^{+1.08}_{-1.07}$ &	$^{+1.09}_{-1.08}$ &	$^{+1.09}_{-1.08}$ &	$^{+1.08}_{-1.07}$ &	$\pm$1.08 &	$^{+1.10}_{-1.09}$ &	$^{+1.07}_{-1.06}$ &	$^{+1.08}_{-1.07}$ &	$^{+1.07}_{-1.06}$ &	$\pm$1.06 &	$\pm$1.05 &	$\pm$1.04 &	$\pm$1.00 \\
$b$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$\pm$0.10 &	$\pm$0.11 &	$\pm$0.11 \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
$c$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-1.52}_{+1.53}$ &	$^{-1.53}_{+1.54}$ &	$^{-1.55}_{+1.56}$ &	$^{-1.53}_{+1.54}$ &	$^{-1.49}_{+1.50}$ &	$^{-1.44}_{+1.45}$ &	$^{-1.42}_{+1.43}$ &	$^{-1.50}_{+1.51}$ &	$^{-1.46}_{+1.47}$ &	$^{-1.44}_{+1.45}$ &	$\mp$1.43 &	$^{-1.45}_{+1.46}$ &	$^{-1.45}_{+1.46}$ &	$^{-1.45}_{+1.46}$ &	$\mp$1.49 &	$\mp$1.33 &	$^{-1.30}_{+1.31}$ &	$\mp$1.24 \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$\pm$0.16 &	$\pm$0.15 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.15 &	$\pm$0.13 &	$\pm$0.14 &	$\pm$0.17 &	$\pm$0.16 &	$\pm$0.14 &	$\pm$0.14 &	$\pm$0.15 &	$\pm$0.13 &	$\pm$0.14 &	$\pm$0.14 &	$\pm$0.18 &	$^{+0.17}_{-0.16}$ &	{$\pm$0.13} \\
$c$-Quark tagging efficiency (eigenvector 2) [\%]	
&	$\pm$0.17 &	$\pm$0.18 &	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.18 &	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.18 &	$\pm$0.17 &	$\pm$0.19 &	$\pm$0.18 &	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.15 \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 0) [\%]	
&	$^{-1.49}_{+1.53}$ &	$^{-1.38}_{+1.44}$ &	$^{-1.27}_{+1.23}$ &	$^{-1.30}_{+1.31}$ &	$^{-1.43}_{+1.52}$ &	$^{-1.54}_{+1.66}$ &	$^{-1.65}_{+1.81}$ &	$^{-1.61}_{+1.66}$ &	$^{-1.43}_{+1.49}$ &	$^{-1.59}_{+1.69}$ &	$\mp$1.45 &	{$^{-1.82}_{+1.95}$} &	$^{-2.13}_{+2.42}$ &	$^{-1.88}_{+1.96}$ &	$^{-2.29}_{+2.45}$ &	$^{-2.13}_{+2.33}$ &	{$^{-1.72}_{+1.77}$} &	{$^{-1.16}_{+1.13}$} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	$\mp$0.11 &	{$\mp$0.16} &	$\mp$0.17 &	$\mp$0.16 \\
Light-jet tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	$\pm$0.11 &	$\pm$0.11 &	{\textrm -} &	\textrm - &	\textrm - &	{$\pm$0.10} &	{$\pm$0.14} &	{\textrm -} &	{$\pm$0.12} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 5) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 6) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 7) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 8) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 9) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 10) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 11) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$b$-Quark tagging  extrapolation  [\%]	
&	$^{+0.31}_{-0.32}$ &	$^{+0.32}_{-0.31}$ &	$^{+0.31}_{-0.32}$ &	$^{+0.30}_{-0.31}$ &	$^{+0.32}_{-0.31}$ &	$^{+0.32}_{-0.31}$ &	$^{+0.31}_{-0.30}$ &	$^{+0.30}_{-0.29}$ &	$\pm$0.29 &	$^{+0.29}_{-0.28}$ &	$\pm$0.30 &	$\pm$0.31 &	$\pm$0.28 &	$\pm$0.27 &	$\pm$0.27 &	$\pm$0.29 &	$\pm$0.26 &	$\pm$0.29 \\
\rowcolor{Gray}
$b$-Quark tagging extrapolation from $c$-Quark [\%]	
&	$^{+0.10}_{-0.12}$ &	$^{+0.13}_{-0.12}$ &	$^{+0.11}_{-0.12}$ &	$^{+0.10}_{-0.11}$ &	$\pm$0.11 &	$\pm$0.11 &	$\pm$0.11 &	{\textrm -} &	\textrm - &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.12 &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
Electron energy resolution [\%]	
&	\textrm - &	\textrm - &	$^{-0.19}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.22}$ &	\textrm - &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{+0.23}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.35}$ &	$^{\textrm{ \phantom{ai}-}}_{+0.21}$ &	{\textrm -} &	{$^{+0.17}_{-0.16}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.50}$ &	{$^{+0.78}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Electron energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	$^{+0.19}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.34}$ &	{$^{+0.33}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.25}_{\textrm{ \phantom{ai}-}}$} &	$^{+0.28}_{-0.29}$ &	\textrm - &	{$^{+1.05}_{-0.14}$} \\
Electron trigger efficiency [\%]	
&	$\pm$0.22 &	$\pm$0.22 &	$\pm$0.22 &	$\pm$0.22 &	$\pm$0.23 &	$\pm$0.24 &	$\pm$0.25 &	$\pm$0.26 &	$\pm$0.27 &	$\pm$0.28 &	$\pm$0.30 &	$\pm$0.33 &	$\pm$0.35 &	$\pm$0.39 &	$\pm$0.45 &	$\pm$0.49 &	$\pm$0.55 &	$\pm$0.66 \\
\rowcolor{Gray}
Electron reconstruction efficiency [\%]	
&	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.17 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.19 &	$\pm$0.19 &	$\pm$0.20 &	$\pm$0.21 &	$\pm$0.21 &	$\pm$0.23 \\
Electron identification efficiency [\%]	
&	$\pm$0.43 &	$\pm$0.43 &	$\pm$0.43 &	$\pm$0.43 &	$\pm$0.43 &	$\pm$0.43 &	$\pm$0.43 &	$\pm$0.43 &	$\pm$0.43 &	$\pm$0.43 &	$\pm$0.44 &	$\pm$0.45 &	$\pm$0.46 &	$\pm$0.47 &	$\pm$0.52 &	$\pm$0.55 &	$\pm$0.58 &	$\pm$0.72 \\
\rowcolor{Gray}
Electron isolation efficiency [\%]	
&	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.17 &	$\pm$0.18 &	$\pm$0.19 &	$\pm$0.22 \\
Muon energy scale [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
Muon (MS) momentum resolution [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	$^{-0.23}_{\textrm{ \phantom{ai}-}}$ \\
Muon (ID) momentum resolution [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{+0.20}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.44}$ &	\textrm - &	{$^{+0.23}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.10}_{+0.12}$} &	{\textrm -} &	{$^{+0.25}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Muon trigger efficiency stat [\%]	
&	$^{+0.58}_{-0.59}$ &	$^{+0.58}_{-0.59}$ &	$^{+0.57}_{-0.59}$ &	$^{+0.57}_{-0.59}$ &	$^{+0.57}_{-0.59}$ &	$^{+0.57}_{-0.58}$ &	$^{+0.57}_{-0.59}$ &	$^{+0.56}_{-0.58}$ &	$^{+0.56}_{-0.58}$ &	$^{+0.57}_{-0.58}$ &	$^{+0.56}_{-0.58}$ &	$^{+0.56}_{-0.58}$ &	$^{+0.55}_{-0.57}$ &	$^{+0.53}_{-0.55}$ &	$^{+0.51}_{-0.53}$ &	$^{+0.49}_{-0.51}$ &	$^{+0.50}_{-0.52}$ &	$^{+0.58}_{-0.59}$ \\
Muon trigger efficiency syst [\%]	
&	$^{+0.26}_{-0.25}$ &	$\pm$0.25 &	$\pm$0.25 &	$\pm$0.25 &	$\pm$0.25 &	$^{+0.25}_{-0.24}$ &	$^{+0.25}_{-0.24}$ &	$\pm$0.24 &	$\pm$0.24 &	$^{+0.24}_{-0.23}$ &	$\pm$0.23 &	$\pm$0.23 &	$^{+0.23}_{-0.22}$ &	$^{+0.22}_{-0.21}$ &	$\pm$0.21 &	$^{+0.21}_{-0.20}$ &	$\pm$0.20 &	$\pm$0.20 \\
\rowcolor{Gray}
Muon identification stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon identification syst [\%]	
&	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.19 &	$^{+0.20}_{-0.19}$ &	$\pm$0.20 &	$\pm$0.21 &	$\pm$0.21 &	$\pm$0.22 &	$\pm$0.22 &	$\pm$0.22 &	$\pm$0.23 \\
\rowcolor{Gray}
Muon isolation efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon isolation efficiency syst [\%]	
&	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.11 &	$\pm$0.11 &	$\pm$0.11 &	$\pm$0.11 &	$\pm$0.11 &	$^{+0.12}_{-0.11}$ &	$\pm$0.12 &	$^{+0.12}_{-0.11}$ &	$\pm$0.11 &	$\pm$0.11 \\
\rowcolor{Gray}
Muon TTVA efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon TTVA efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution para [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{$\pm$0.10} &	{$\pm$0.20} &	{$\mp$0.11} &	{$\pm$0.20} &	{\textrm -} &	{$\mp$0.13} &	{$\pm$0.29} &	{$\pm$0.42} &	{\textrm -} &	{$\pm$0.43} &	$\pm$0.34 &	{$\pm$0.26} \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution perp [\%]	
&	\textrm - &	{$\mp$0.17} &	$\mp$0.17 &	$\mp$0.14 &	{\textrm -} &	{\textrm -} &	{$\mp$0.13} &	$\mp$0.11 &	{\textrm -} &	{\textrm -} &	{$\mp$0.17} &	{$\mp$0.12} &	$\mp$0.13 &	{$\pm$0.19} &	$\pm$0.21 &	{$\pm$0.28} &	{$\mp$0.12} &	{$\pm$0.45} \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet scale [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.27}$ &	{$^{+0.29}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.14}_{-0.12}$} &	{$^{+0.21}_{-0.52}$} &	{$^{+0.36}_{\textrm{ \phantom{ai}-}}$} \\
Luminosity [\%]	
&	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 \\
\rowcolor{Gray}
Single top cross-section [\%]	
&	$\pm$0.28 &	$\pm$0.28 &	$\pm$0.28 &	$\pm$0.28 &	$\pm$0.27 &	$\pm$0.27 &	$\pm$0.26 &	$\pm$0.25 &	$\pm$0.25 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.23 &	$\pm$0.22 &	$\pm$0.21 &	$\pm$0.21 &	$\pm$0.20 &	$\pm$0.18 &	$\pm$0.17 \\
$Z$+jets cross-section [\%]	
&	$\pm$0.58 &	$\pm$0.51 &	$\pm$0.58 &	$\pm$0.51 &	{$\pm$0.69} &	$\pm$0.67 &	$\pm$0.64 &	$\pm$0.63 &	$\pm$0.61 &	$\pm$0.51 &	$\pm$0.53 &	$\pm$0.60 &	$\pm$0.71 &	{$\pm$0.43} &	{$\pm$0.61} &	$\pm$0.57 &	{$\pm$0.42} &	{$\mp$0.11} \\
\rowcolor{Gray}
Diboson cross-section [\%]	
&	$\pm$0.12 &	$\pm$0.13 &	$\pm$0.12 &	$\pm$0.13 &	$\pm$0.14 &	$\pm$0.13 &	$\pm$0.13 &	$\pm$0.14 &	$\pm$0.15 &	$\pm$0.16 &	$\pm$0.15 &	$\pm$0.15 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.15 &	$\pm$0.17 &	$\pm$0.15 &	{$\pm$0.27} \\
$t\bar{t}V$ cross-section [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Monte Carlo sample statistics [\%]	
&	$\pm$0.41 &	$\pm$0.38 &	$\pm$0.41 &	$\pm$0.37 &	$\pm$0.42 &	$\pm$0.45 &	$\pm$0.47 &	$\pm$0.47 &	$\pm$0.54 &	$\pm$0.54 &	$\pm$0.55 &	{$\pm$0.73} &	$\pm$0.85 &	$\pm$0.77 &	{$\pm$1.26} &	$\pm$1.20 &	$\pm$1.09 &	{$\pm$1.79} \\
ISR/FSR + scale [\%]	
&	$^{-3.17}_{+1.86}$ &	{$^{-2.18}_{+1.34}$} &	$^{-4.14}_{+1.72}$ &	{$^{-2.90}_{+2.33}$} &	{$^{-2.24}_{+3.13}$} &	$^{-2.42}_{+2.63}$ &	$^{-2.53}_{+2.15}$ &	$^{-2.12}_{+2.02}$ &	$^{-2.90}_{+2.56}$ &	$^{-3.39}_{+2.55}$ &	{$^{-3.25}_{+1.59}$} &	{$^{-1.92}_{+2.64}$} &	$^{-3.40}_{+2.58}$ &	{$^{-2.57}_{+3.94}$} &	{$\mp$2.72} &	$^{-2.57}_{+3.31}$ &	{$^{-4.46}_{+2.31}$} &	{$^{-3.47}_{+3.41}$} \\
\rowcolor{Gray}
Alternate hard-scattering model [\%]	
&	\textrm - &	{$\pm$0.80} &	{$\pm$1.29} &	{\textrm -} &	{$\pm$1.16} &	{$\pm$1.97} &	{$\mp$0.17} &	{$\mp$1.61} &	{$\pm$0.48} &	$\mp$0.53 &	$\pm$0.46 &	{$\pm$1.46} &	{$\mp$0.27} &	{$\pm$0.63} &	{$\pm$4.31} &	{$\pm$0.56} &	{$\mp$2.70} &	{$\pm$6.22} \\
Alternate parton-shower model [\%]	
&	$\mp$2.61 &	{$\mp$1.40} &	{$\mp$2.82} &	{$\mp$2.02} &	$\mp$1.59 &	$\mp$1.46 &	$\mp$1.64 &	$\mp$2.04 &	$\mp$1.79 &	{$\mp$2.35} &	$\mp$2.41 &	{$\mp$1.80} &	$\mp$1.40 &	$\mp$1.18 &	{$\mp$2.14} &	{$\mp$1.07} &	{$\mp$2.38} &	{$\mp$1.05} \\
\rowcolor{Gray}
Inter PDF [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.31} &	{\textrm -} &	\textrm - &	{$\pm$0.16} &	{$\mp$0.47} \\
Intra PDF [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{$\pm$0.12} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{$\pm$0.29} &	{$\pm$0.14} &	{\textrm -} &	{$\pm$0.21} &	{$\pm$0.42} &	{$\pm$0.56} \\
\rowcolor{Gray}
Real lepton efficiency stat [\%]	
&	$^{-0.17}_{+0.15}$ &	$^{-0.16}_{+0.15}$ &	$^{-0.16}_{+0.15}$ &	$^{-0.16}_{+0.14}$ &	$^{-0.16}_{+0.15}$ &	$^{-0.16}_{+0.15}$ &	$^{-0.16}_{+0.15}$ &	$^{-0.17}_{+0.15}$ &	$^{-0.17}_{+0.15}$ &	$^{-0.17}_{+0.15}$ &	$^{-0.18}_{+0.16}$ &	$^{-0.18}_{+0.16}$ &	$^{-0.18}_{+0.17}$ &	$^{-0.19}_{+0.17}$ &	$^{-0.17}_{+0.16}$ &	$^{-0.20}_{+0.18}$ &	$^{-0.19}_{+0.18}$ &	$^{-0.23}_{+0.21}$ \\
Fake lepton efficiency MC scale [\%]	
&	$^{+0.65}_{-0.71}$ &	$^{+0.74}_{-0.90}$ &	$^{+0.69}_{-0.82}$ &	$^{+0.69}_{-0.79}$ &	$^{+0.61}_{-0.76}$ &	$^{+0.68}_{-0.81}$ &	$^{+0.69}_{-0.82}$ &	$^{+0.56}_{-0.70}$ &	$^{+0.47}_{-0.72}$ &	$^{+0.53}_{-0.63}$ &	$^{+0.60}_{-0.72}$ &	$^{+0.47}_{-0.57}$ &	{$^{+0.13}_{-0.41}$} &	{$^{+0.23}_{-0.26}$} &	{$^{+0.41}_{-0.59}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.57}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.61}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.57}$ \\
\rowcolor{Gray}
Fake lepton efficiency alternate CR [\%]	
&	$\pm$0.31 &	$\pm$0.39 &	$\pm$0.33 &	{$\pm$0.46} &	$\pm$0.40 &	{$\pm$0.30} &	$\pm$0.39 &	$\pm$0.31 &	{$\pm$0.18} &	{$\pm$0.31} &	{$\pm$0.42} &	{$\pm$0.30} &	{$\pm$0.11} &	{$\pm$0.19} &	{\textrm -} &	\textrm - &	$\pm$0.30 &	{$\pm$0.54} \\
Fake overall normalisation [\%]	
&	$\pm$3.90 &	$\pm$3.71 &	$\pm$3.64 &	$\pm$3.46 &	$\pm$3.54 &	$\pm$3.45 &	$\pm$3.53 &	$\pm$3.19 &	$\pm$2.91 &	$\pm$3.01 &	$\pm$3.12 &	$\pm$2.78 &	$\pm$2.68 &	{$\pm$1.61} &	{$\pm$3.03} &	{$\pm$1.85} &	$\pm$1.73 &	$\pm$1.57 \\
\rowcolor{Gray}
$W$+jets $CA_{4incl}$ stat error [\%]	
&	$\mp$0.12 &	$\mp$0.11 &	$\mp$0.11 &	$\mp$0.10 &	$\mp$0.11 &	\textrm - &	$\mp$0.11 &	$\mp$0.12 &	$\mp$0.10 &	$\mp$0.10 &	\textrm - &	$\mp$0.11 &	$\mp$0.13 &	$\mp$0.10 &	$\mp$0.11 &	{\textrm -} &	\textrm - &	\textrm - \\
$W$+jets Fc stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$W$+jets Fcc stat error [\%]	
&	\textrm - &	{\textrm -} &	{$^{-0.14}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$^{+0.41}_{-0.19}$} &	{$^{+0.16}_{\textrm{ \phantom{ai}-}}$} &	$^{-0.17}_{\textrm{ \phantom{ai}-}}$ &	\textrm - \\
$W$+jets Flight stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\hline
\end{tabular}}


==> tables/systematics/resolved/table_syst_particle_tt_absrap_RelativeDiffXs.tex <==
\resizebox*{\textwidth}{!}{
\begin{tabular}{l c c c c c c c c c c c c c c c c c c}
\hline
Bins  [ Unit $|y^{t\bar{t}}|$ ]
 & 0--0.10   & 0.10--0.20   & 0.20--0.30   & 0.30--0.40   & 0.40--0.50   & 0.50--0.60   & 0.60--0.70   & 0.70--0.80   & 0.80--0.90   & 0.90--1   & 1--1.10   & 1.10--1.20   & 1.20--1.30   & 1.30--1.40   & 1.40--1.50   & 1.50--1.60   & 1.60--1.80   & 1.80--2.50  \\
\hline
\hline
1/$\sigma$ $\cdot$ d$\sigma$ / d$|y^{t\bar{t}}|$	&	$1.02 \cdot 10^{0}$ &	$1.03 \cdot 10^{0}$ &	$9.97 \cdot 10^{-1}$ &	$9.58 \cdot 10^{-1}$ &	$9.34 \cdot 10^{-1}$ &	$8.41 \cdot 10^{-1}$ &	$7.53 \cdot 10^{-1}$ &	$6.91 \cdot 10^{-1}$ &	$5.99 \cdot 10^{-1}$ &	$5.05 \cdot 10^{-1}$ &	$4.17 \cdot 10^{-1}$ &	$3.46 \cdot 10^{-1}$ &	$2.71 \cdot 10^{-1}$ &	$2.19 \cdot 10^{-1}$ &	$1.50 \cdot 10^{-1}$ &	$1.09 \cdot 10^{-1}$ &	$6.05 \cdot 10^{-2}$ &	$6.17 \cdot 10^{-3}$ \\
\hline
\rowcolor{Gray}
Total uncertainty [\%]	
&	$^{+1.54}_{-1.88}$ &	$^{+1.59}_{-1.66}$ &	$^{+1.76}_{-2.26}$ &	$^{+1.68}_{-1.52}$ &	$^{+1.70}_{-1.47}$ &	$^{+2.10}_{-2.01}$ &	$^{+1.92}_{-1.70}$ &	$^{+2.62}_{-2.55}$ &	$^{+1.81}_{-1.94}$ &	$^{+1.98}_{-2.07}$ &	$^{+1.95}_{-2.07}$ &	$^{+2.59}_{-2.25}$ &	$^{+3.01}_{-3.56}$ &	$^{+4.00}_{-3.58}$ &	$^{+5.47}_{-5.19}$ &	$^{+4.82}_{-4.23}$ &	$^{+5.43}_{-6.44}$ &	$^{+9.34}_{-9.06}$ \\
Statistical uncertainty [\%]	
&	$\pm1.0$ &	$\pm0.9$ &	$\pm0.9$ &	$\pm0.9$ &	$\pm1.0$ &	$\pm1.0$ &	$\pm1.1$ &	$\pm1.1$ &	$\pm1.2$ &	$\pm1.3$ &	$\pm1.5$ &	$\pm1.7$ &	$\pm1.9$ &	$\pm2.1$ &	$\pm2.6$ &	$\pm3.2$ &	$\pm3.3$ &	$\pm5.7$ \\
\rowcolor{Gray}
Systematic uncertainty [\%]	
&	$^{+1.10}_{-1.53}$ &	$^{+1.22}_{-1.31}$ &	$^{+1.41}_{-2.00}$ &	$^{+1.30}_{-1.10}$ &	$^{+1.30}_{-0.99}$ &	$^{+1.76}_{-1.66}$ &	$^{+1.50}_{-1.19}$ &	$^{+2.29}_{-2.22}$ &	$^{+1.19}_{-1.39}$ &	$^{+1.30}_{-1.43}$ &	$^{+1.08}_{-1.28}$ &	$^{+1.82}_{-1.28}$ &	$^{+2.16}_{-2.87}$ &	$^{+3.27}_{-2.73}$ &	$^{+4.60}_{-4.26}$ &	$^{+3.32}_{-2.40}$ &	$^{+4.17}_{-5.43}$ &	$^{+7.13}_{-6.76}$ \\
\hline
\hline
$b$-Tagged jet energy scale (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$^{+0.19}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$^{-0.26}_{+0.13}$} &	{$^{+0.17}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.25}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.19}$} &	$^{-0.29}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} \\
\rowcolor{Gray}
Effective detector NP set 1 (JES) [\%]	
&	$^{-0.33}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	\textrm - &	{$^{+0.37}_{-0.20}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.25}$} &	{$^{-0.12}_{+0.38}$} &	{$^{\textrm{ \phantom{ai}-}}_{+0.60}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.28}$} &	$^{+0.20}_{-0.68}$ &	{\textrm -} &	$^{-0.29}_{+0.10}$ &	{$^{-0.32}_{+0.31}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.50}$ &	{$^{+0.36}_{\textrm{ \phantom{ai}-}}$} &	$^{+0.41}_{\textrm{ \phantom{ai}-}}$ &	{$^{+0.80}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.53}$} &	{$^{+0.73}_{\textrm{ \phantom{ai}-}}$} \\
Effective detector NP set 2 (JES) [\%]	
&	\textrm - &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{-0.14}$} &	\textrm - &	\textrm - &	\textrm - &	{$^{+0.21}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.35}$ &	{$^{+0.34}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{\textrm -} &	{$^{+0.28}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{+0.76}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.79}$ &	{$^{+0.37}_{-0.18}$} \\
\rowcolor{Gray}
Effective detector NP set 3 (JES) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$^{-0.15}_{+0.10}$} &	\textrm - &	\textrm - &	{$^{-0.20}_{+0.21}$} &	\textrm - &	{$^{+0.80}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.43}$} &	$^{-0.29}_{+0.18}$ \\
Effective detector NP set 4 (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.18}$ &	{\textrm -} &	{\textrm -} &	{$^{+0.28}_{\textrm{ \phantom{ai}-}}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.23}$ &	$^{+0.26}_{-0.27}$ \\
\rowcolor{Gray}
Effective detector NP set 5 (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{+0.24}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	$^{-0.31}_{\textrm{ \phantom{ai}-}}$ \\
Effective detector NP set 6 restTerm (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.16}$ &	{$^{+0.29}_{\textrm{ \phantom{ai}-}}$} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$\eta$ intercalibration model (JES) [\%]	
&	$^{-0.89}_{+0.28}$ &	{$^{-0.24}_{+0.55}$} &	{$^{-0.23}_{+0.35}$} &	{$^{+0.38}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.27}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.36}_{+0.41}$} &	{$^{+0.27}_{\textrm{ \phantom{ai}-}}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.32}$ &	$^{+0.15}_{-0.59}$ &	{$\pm$0.30} &	{$^{+0.59}_{-0.18}$} &	{$^{+0.37}_{-0.23}$} &	$^{+0.45}_{-1.42}$ &	{$^{+1.39}_{-1.04}$} &	$^{+1.78}_{-0.89}$ &	{$^{+1.27}_{-1.15}$} &	$^{+1.62}_{-2.40}$ &	$^{+2.02}_{-1.56}$ \\
$\eta$ intercalibration total stat (JES) [\%]	
&	\textrm - &	\textrm - &	$^{-0.12}_{+0.15}$ &	{\textrm -} &	\textrm - &	\textrm - &	{$^{+0.22}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.38}$ &	\textrm - &	\textrm - &	$^{+0.29}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{$^{+0.30}_{-0.31}$} &	$^{+0.35}_{\textrm{ \phantom{ai}-}}$ &	{$^{+0.51}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.72}$} &	{$^{+0.31}_{-0.11}$} \\
\rowcolor{Gray}
Flavour composition (JES) [\%]	
&	$^{-0.38}_{+0.23}$ &	\textrm - &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.15}$} &	$\pm$0.11 &	{$^{-0.20}_{+0.30}$} &	$^{\textrm{ \phantom{ai}-}}_{+0.31}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.25}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.44}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.20}$ &	{$^{+0.62}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{+0.43}$} &	$^{\textrm{ \phantom{ai}-}}_{-1.01}$ &	{$^{+0.42}_{-0.75}$} &	$^{+0.44}_{\textrm{ \phantom{ai}-}}$ &	{$^{+0.76}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.82}$} &	{$^{+0.97}_{-0.25}$} \\
Flavour response (JES) [\%]	
&	\textrm - &	\textrm - &	$^{+0.12}_{\textrm{ \phantom{ai}-}}$ &	{$^{\textrm{ \phantom{ai}-}}_{+0.13}$} &	{\textrm -} &	$^{+0.11}_{-0.10}$ &	\textrm - &	\textrm - &	{$^{-0.27}_{\textrm{ \phantom{ai}-}}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.17}$ &	\textrm - &	{$^{+0.36}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{+0.19}$} &	{$^{+0.41}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{+0.29}$} &	$^{\textrm{ \phantom{ai}-}}_{-1.12}$ &	$^{\textrm{ \phantom{ai}-}}_{+0.61}$ \\
\rowcolor{Gray}
Pile-up offset $\mu$ (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	$^{-0.13}_{+0.17}$ &	$^{\textrm{ \phantom{ai}-}}_{+0.22}$ &	{$^{+0.41}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.39}$} &	\textrm - \\
Pile-up offset $N_{\textrm PV}$ (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{+0.18}_{-0.12}$ &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.30}$ &	{$^{+0.30}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.69}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.37}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.23}$ \\
\rowcolor{Gray}
Pile-up offset $p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{+0.25}_{-0.20}$ &	{$^{+0.14}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.43}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.24}$} &	$^{+0.26}_{-0.33}$ \\
Pile-up offset $\rho$ topology (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.21}$ &	\textrm - &	{\textrm -} &	{$^{+0.21}_{-0.14}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.23}$ &	\textrm - &	{$^{+0.25}_{\textrm{ \phantom{ai}-}}$} &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.32}$ &	\textrm - &	\textrm - &	$^{+0.21}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{$^{+0.31}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.49}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.36}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.56}$} &	{$^{+0.35}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Punch-through (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Single particle high-$p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Jet energy resolution [\%]	
&	$\mp$0.20 &	{$\pm$0.15} &	{$\mp$0.38} &	{$\pm$0.80} &	{\textrm -} &	\textrm - &	{$\pm$0.83} &	{$\mp$0.22} &	{\textrm -} &	{$\mp$0.18} &	{\textrm -} &	{$\pm$0.11} &	{$\mp$1.16} &	$\mp$0.93 &	{$\mp$0.64} &	{$\pm$0.11} &	{$\mp$0.63} &	{$\mp$1.67} \\
Jet vertex fraction [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	$\mp$0.10 &	{$\mp$0.19} &	{$^{-0.35}_{+0.37}$} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 0) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.12} &	$^{+0.15}_{-0.14}$ &	$^{+0.14}_{-0.13}$ &	{$^{+0.20}_{-0.18}$} &	{\textrm -} \\
$b$-Quark tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\mp$0.15} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
$b$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$c$-Quark tagging efficiency (eigenvector 0) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	$\pm$0.15 &	$^{+0.18}_{-0.17}$ &	{$\pm$0.24} \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
$c$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 0) [\%]	
&	\textrm - &	{$^{+0.13}_{-0.14}$} &	{$^{+0.25}_{-0.35}$} &	$^{+0.22}_{-0.27}$ &	{\textrm -} &	{\textrm -} &	{$^{-0.13}_{+0.21}$} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{$^{-0.30}_{+0.36}$} &	{$^{-0.62}_{+0.82}$} &	{$\mp$0.36} &	{$^{-0.78}_{+0.84}$} &	$^{-0.62}_{+0.72}$ &	{$^{-0.20}_{+0.18}$} &	{$^{+0.35}_{-0.45}$} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{$\mp$0.12} &	$\mp$0.13 &	$\mp$0.14 &	{$\mp$0.19} &	$\mp$0.20 &	$\mp$0.19 \\
Light-jet tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 5) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 6) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 7) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 8) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 9) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 10) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 11) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$b$-Quark tagging  extrapolation  [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$b$-Quark tagging extrapolation from $c$-Quark [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
Electron energy resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{$^{+0.23}_{\textrm{ \phantom{ai}-}}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.25}$ &	$^{+0.21}_{\textrm{ \phantom{ai}-}}$ &	$^{+0.21}_{\textrm{ \phantom{ai}-}}$ &	$^{+0.26}_{-0.16}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.41}$ &	{$^{+0.87}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Electron energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.30}$ &	$^{+0.28}_{\textrm{ \phantom{ai}-}}$ &	{$^{+0.20}_{\textrm{ \phantom{ai}-}}$} &	$^{+0.23}_{-0.25}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.21}$ &	{$^{+1.00}_{-0.11}$} \\
Electron trigger efficiency [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{$\pm$0.12} &	{$\pm$0.18} &	$\pm$0.23 &	$\pm$0.28 &	{$\pm$0.39} \\
\rowcolor{Gray}
Electron reconstruction efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
Electron identification efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{$\pm$0.11} &	$\pm$0.14 &	{$\pm$0.27} \\
\rowcolor{Gray}
Electron isolation efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
Muon energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
Muon (MS) momentum resolution [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	$^{-0.24}_{\textrm{ \phantom{ai}-}}$ \\
Muon (ID) momentum resolution [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$^{+0.15}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	\textrm - &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-0.40}$ &	\textrm - &	{$^{+0.26}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	{\textrm -} &	$^{+0.29}_{\textrm{ \phantom{ai}-}}$ \\
\rowcolor{Gray}
Muon trigger efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - \\
Muon trigger efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
Muon identification stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon identification syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon isolation efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon isolation efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon TTVA efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
Muon TTVA efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution para [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{$\pm$0.12} &	{$\mp$0.19} &	{$\pm$0.12} &	{\textrm -} &	{$\mp$0.20} &	$\pm$0.21 &	{$\pm$0.34} &	{\textrm -} &	{$\pm$0.35} &	{$\pm$0.26} &	{$\pm$0.18} \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution perp [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{$\pm$0.15} &	{\textrm -} &	{\textrm -} &	\textrm - &	{$\pm$0.27} &	$\pm$0.30 &	$\pm$0.37 &	{\textrm -} &	{$\pm$0.54} \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{$^{+0.11}_{-0.26}$} &	{$^{+0.32}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.17}_{-0.11}$} &	{$^{+0.24}_{-0.51}$} &	{$^{+0.39}_{\textrm{ \phantom{ai}-}}$} \\
Luminosity [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Single top cross-section [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - \\
$Z$+jets cross-section [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\pm$0.10} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.12} &	$\mp$0.15 &	{\textrm -} &	{\textrm -} &	{$\mp$0.15} &	{$\mp$0.70} \\
\rowcolor{Gray}
Diboson cross-section [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{$\pm$0.13} \\
$t\bar{t}V$ cross-section [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Monte Carlo sample statistics [\%]	
&	$\pm$0.39 &	$\pm$0.36 &	$\pm$0.40 &	$\pm$0.36 &	$\pm$0.40 &	$\pm$0.43 &	$\pm$0.45 &	$\pm$0.46 &	$\pm$0.52 &	$\pm$0.53 &	$\pm$0.55 &	$\pm$0.71 &	$\pm$0.84 &	$\pm$0.77 &	{$\pm$1.25} &	$\pm$1.20 &	$\pm$1.09 &	{$\pm$1.78} \\
ISR/FSR + scale [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.38}$ &	{$^{+0.66}_{-0.88}$} &	{$^{\textrm{ \phantom{ai}-}}_{-1.35}$} &	\textrm - &	{$^{+0.86}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.41}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.30}_{-0.10}$} &	{$^{+0.73}_{-0.22}$} &	{$^{\textrm{ \phantom{ai}-}}_{+0.30}$} &	$^{-0.58}_{+0.29}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.64}$ &	{$^{+0.92}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.59}_{+0.31}$} &	{$^{+1.65}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.46}_{\textrm{ \phantom{ai}-}}$} &	{$^{+1.03}_{\textrm{ \phantom{ai}-}}$} &	$^{-1.68}_{\textrm{ \phantom{ai}-}}$ &	{$^{-0.66}_{+1.13}$} \\
\rowcolor{Gray}
Alternate hard-scattering model [\%]	
&	$\mp$0.44 &	{$\pm$0.29} &	{$\pm$0.78} &	{$\mp$0.55} &	$\pm$0.65 &	{$\pm$1.46} &	{$\mp$0.67} &	{$\mp$2.11} &	{\textrm -} &	{$\mp$1.03} &	{\textrm -} &	{$\pm$0.95} &	$\mp$0.77 &	{$\pm$0.13} &	{$\pm$3.79} &	{\textrm -} &	{$\mp$3.19} &	{$\pm$5.68} \\
Alternate parton-shower model [\%]	
&	$\mp$0.67 &	$\pm$0.56 &	{$\mp$0.88} &	{\textrm -} &	{$\pm$0.36} &	{$\pm$0.50} &	{$\pm$0.31} &	{\textrm -} &	{$\pm$0.16} &	{$\mp$0.40} &	$\mp$0.46 &	{$\pm$0.15} &	{$\pm$0.56} &	{$\pm$0.78} &	{$\mp$0.18} &	{$\pm$0.90} &	{$\mp$0.44} &	{$\pm$0.91} \\
\rowcolor{Gray}
Inter PDF [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	$\mp$0.12 &	{$\pm$0.27} &	\textrm - &	\textrm - &	$\pm$0.12 &	{$\mp$0.51} \\
Intra PDF [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{$\pm$0.23} &	{\textrm -} &	\textrm - &	$\pm$0.14 &	{$\pm$0.36} &	{$\pm$0.49} \\
\rowcolor{Gray}
Real lepton efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Fake lepton efficiency MC scale [\%]	
&	\textrm - &	{$^{+0.15}_{-0.16}$} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	$^{-0.11}_{+0.16}$ &	{$^{-0.44}_{+0.32}$} &	{$^{-0.35}_{+0.47}$} &	{$^{-0.17}_{+0.13}$} &	$^{-0.66}_{+0.16}$ &	{$^{-1.19}_{+0.55}$} &	{$^{-0.70}_{+0.16}$} \\
\rowcolor{Gray}
Fake lepton efficiency alternate CR [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	$\pm$0.13 &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\mp$0.15} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\mp$0.21} &	{$\mp$0.13} &	{$\mp$0.31} &	$\mp$0.32 &	{\textrm -} &	{$\pm$0.21} \\
Fake overall normalisation [\%]	
&	$\pm$0.55 &	{$\pm$0.36} &	$\pm$0.30 &	{$\pm$0.13} &	{$\pm$0.20} &	{$\pm$0.11} &	{$\pm$0.19} &	{$\mp$0.13} &	{$\mp$0.40} &	{$\mp$0.30} &	{$\mp$0.20} &	{$\mp$0.52} &	$\mp$0.62 &	{$\mp$1.66} &	{$\mp$0.28} &	{$\mp$1.42} &	$\mp$1.54 &	$\mp$1.70 \\
\rowcolor{Gray}
$W$+jets $CA_{4incl}$ stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - \\
$W$+jets Fc stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$W$+jets Fcc stat error [\%]	
&	\textrm - &	{\textrm -} &	{$^{-0.14}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{$^{+0.40}_{-0.19}$} &	{$^{+0.16}_{\textrm{ \phantom{ai}-}}$} &	$^{-0.17}_{\textrm{ \phantom{ai}-}}$ &	\textrm - \\
$W$+jets Flight stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\hline
\end{tabular}}


==> tables/systematics/resolved/table_syst_particle_tt_m_AbsoluteDiffXs.tex <==
\resizebox*{\textwidth}{!}{
\begin{tabular}{l c c c c c c c c c c c}
\hline
Bins  [GeV]
 & 225--345   & 345--420   & 420--500   & 500--590   & 590--685   & 685--790   & 790--910   & 910--1040   & 1040--1175   & 1175--1320   & 1320--3000  \\
\hline
\hline
d$\sigma$ / d$m^{t\bar{t}}$ [pb/GeV]	&	$4.95 \cdot 10^{-2}$ &	$2.89 \cdot 10^{-1}$ &	$2.90 \cdot 10^{-1}$ &	$2.12 \cdot 10^{-1}$ &	$1.29 \cdot 10^{-1}$ &	$7.80 \cdot 10^{-2}$ &	$4.33 \cdot 10^{-2}$ &	$2.34 \cdot 10^{-2}$ &	$1.19 \cdot 10^{-2}$ &	$6.60 \cdot 10^{-3}$ &	$7.33 \cdot 10^{-4}$ \\
\hline
\rowcolor{Gray}
Total uncertainty [\%]	
&	$^{+16.3}_{-16.6}$ &	$^{+11.0}_{-11.9}$ &	$^{+11.6}_{-12.2}$ &	$^{+11.1}_{-11.9}$ &	$^{+10.5}_{-11.3}$ &	$\pm$10.2 &	$^{+10.1}_{-11.0}$ &	$^{+10.8}_{-12.0}$ &	$^{+12.0}_{-13.9}$ &	$^{+12.2}_{-13.8}$ &	$^{+19.9}_{-20.3}$ \\
Statistical uncertainty [\%]	
&	$\pm1.6$ &	$\pm0.7$ &	$\pm0.7$ &	$\pm0.7$ &	$\pm0.9$ &	$\pm1.2$ &	$\pm1.5$ &	$\pm2.0$ &	$\pm2.7$ &	$\pm3.9$ &	$\pm3.4$ \\
\rowcolor{Gray}
Systematic uncertainty [\%]	
&	$^{+16.2}_{-16.5}$ &	$^{+11.0}_{-11.9}$ &	$^{+11.5}_{-12.2}$ &	$^{+11.0}_{-11.9}$ &	$^{+10.4}_{-11.2}$ &	$\pm$10.2 &	$^{+9.99}_{-10.8}$ &	$^{+10.6}_{-11.8}$ &	$^{+11.6}_{-13.6}$ &	$^{+11.4}_{-13.2}$ &	$^{+19.5}_{-19.9}$ \\
\hline
\hline
$b$-Tagged jet energy scale (JES) [\%]	
&	$^{-2.89}_{+2.93}$ &	{$^{-0.26}_{+0.13}$} &	{$^{+0.86}_{-0.79}$} &	$^{+1.03}_{-1.01}$ &	$^{+1.07}_{-1.11}$ &	$^{+1.31}_{-0.95}$ &	{$^{+0.80}_{-0.90}$} &	$^{+1.01}_{-0.89}$ &	$^{+0.79}_{-0.85}$ &	$^{+0.97}_{-0.77}$ &	$^{+0.85}_{-0.54}$ \\
\rowcolor{Gray}
Effective detector NP set 1 (JES) [\%]	
&	$^{-2.66}_{+0.12}$ &	{$^{+4.08}_{-5.02}$} &	{$^{+6.48}_{-6.88}$} &	$^{+6.39}_{-6.87}$ &	$^{+5.44}_{-6.00}$ &	$^{+4.55}_{-5.16}$ &	$^{+3.59}_{-4.41}$ &	$^{+2.91}_{-4.66}$ &	{$^{+1.96}_{-5.45}$} &	$^{+2.18}_{-3.74}$ &	{$^{\textrm{ \phantom{ai}-}}_{-2.46}$} \\
Effective detector NP set 2 (JES) [\%]	
&	$^{-3.50}_{+3.37}$ &	{$^{-2.30}_{+2.19}$} &	{$^{-1.19}_{+1.26}$} &	{$^{-0.67}_{+0.50}$} &	{$^{+0.22}_{-0.25}$} &	{$^{+0.97}_{-0.62}$} &	{$^{+0.41}_{-1.02}$} &	{$^{+2.06}_{-2.10}$} &	$^{+2.00}_{-2.17}$ &	$^{+2.43}_{-2.37}$ &	{$^{+3.68}_{-4.24}$} \\
\rowcolor{Gray}
Effective detector NP set 3 (JES) [\%]	
&	$\pm$2.37 &	{$^{+1.10}_{-1.16}$} &	{$^{+0.34}_{-0.36}$} &	{\textrm -} &	{$^{-0.55}_{+0.46}$} &	{$^{-0.69}_{+0.93}$} &	{$^{-0.88}_{+0.49}$} &	{$^{-1.23}_{+1.34}$} &	$^{-1.42}_{+1.44}$ &	$^{-1.53}_{+1.39}$ &	{$^{-2.09}_{+1.94}$} \\
Effective detector NP set 4 (JES) [\%]	
&	$^{-1.92}_{+1.80}$ &	{$^{-0.71}_{+0.64}$} &	{\textrm -} &	{$^{+0.11}_{-0.26}$} &	{$^{+0.35}_{-0.37}$} &	{$^{+0.46}_{-0.44}$} &	{$^{+0.14}_{-0.50}$} &	{$^{+0.38}_{-0.47}$} &	$^{+0.48}_{-0.64}$ &	{$^{+0.26}_{-0.56}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.39}$} \\
\rowcolor{Gray}
Effective detector NP set 5 (JES) [\%]	
&	$^{+0.78}_{-0.74}$ &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{+0.14}$} &	{\textrm -} &	{$^{-0.10}_{+0.16}$} &	\textrm - &	{\textrm -} &	{$^{+0.22}_{-0.10}$} &	{\textrm -} &	$^{+0.14}_{-0.17}$ &	{$^{+0.28}_{-0.10}$} \\
Effective detector NP set 6 restTerm (JES) [\%]	
&	$^{-0.52}_{+0.51}$ &	{$^{-0.15}_{+0.10}$} &	{\textrm -} &	{\textrm -} &	{$^{+0.13}_{-0.14}$} &	{$^{+0.18}_{-0.15}$} &	{\textrm -} &	{$^{+0.20}_{-0.24}$} &	{\textrm -} &	{$^{+0.21}_{-0.28}$} &	$^{+0.19}_{-0.26}$ \\
\rowcolor{Gray}
$\eta$ intercalibration model (JES) [\%]	
&	$^{-2.49}_{+2.14}$ &	{$^{+0.27}_{-0.75}$} &	{$^{+1.50}_{-1.84}$} &	{$^{+2.10}_{-2.19}$} &	$^{+1.99}_{-2.44}$ &	$^{+1.91}_{-2.27}$ &	$^{+1.65}_{-2.10}$ &	$^{+1.81}_{-2.76}$ &	$^{+1.79}_{-2.63}$ &	$^{+1.74}_{-2.14}$ &	{$^{+1.08}_{-2.08}$} \\
$\eta$ intercalibration total stat (JES) [\%]	
&	$^{-1.62}_{+1.14}$ &	{$^{+0.29}_{-0.41}$} &	{$^{+0.90}_{-0.82}$} &	$^{+1.04}_{-1.08}$ &	$^{+0.99}_{-0.96}$ &	$^{+1.11}_{-0.81}$ &	{$^{+0.35}_{-0.75}$} &	{$^{+0.71}_{-0.70}$} &	{$^{+0.31}_{-0.69}$} &	{$^{+0.72}_{-0.43}$} &	{$^{-0.43}_{+0.12}$} \\
\rowcolor{Gray}
Flavour composition (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-1.31}$ &	{$^{+3.05}_{-3.71}$} &	{$^{+4.19}_{-4.91}$} &	$^{+4.17}_{-4.87}$ &	$^{+3.66}_{-4.05}$ &	$^{+2.93}_{-3.22}$ &	$^{+2.44}_{-2.80}$ &	{$^{+1.79}_{-3.07}$} &	{$^{+0.73}_{-3.39}$} &	{$^{+1.87}_{-1.83}$} &	{$^{\textrm{ \phantom{ai}-}}_{-1.09}$} \\
Flavour response (JES) [\%]	
&	$^{+0.61}_{-1.11}$ &	$^{-0.82}_{+0.55}$ &	{$^{-1.29}_{+0.95}$} &	$^{-1.51}_{+1.13}$ &	$^{-1.37}_{+0.90}$ &	$^{-1.02}_{+0.98}$ &	{$^{-0.99}_{+0.15}$} &	{$^{-1.33}_{+0.36}$} &	$^{\textrm{ \phantom{ai}-}}_{-1.07}$ &	$^{-1.40}_{+0.44}$ &	$^{\textrm{ \phantom{ai}-}}_{-1.48}$ \\
\rowcolor{Gray}
Pile-up offset $\mu$ (JES) [\%]	
&	$^{+0.13}_{-0.33}$ &	$^{-0.16}_{+0.17}$ &	$^{-0.26}_{+0.21}$ &	$^{-0.33}_{+0.24}$ &	$^{-0.23}_{+0.21}$ &	$^{-0.16}_{+0.27}$ &	{\textrm -} &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.27}$ &	\textrm - &	{$^{+0.38}_{-0.66}$} \\
Pile-up offset $N_{\textrm PV}$ (JES) [\%]	
&	$^{+0.20}_{-0.41}$ &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{$^{+0.21}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.16}_{-0.20}$} &	{\textrm -} &	{$^{+0.23}_{-0.18}$} &	$^{+0.28}_{-0.19}$ &	{$^{+0.59}_{-0.47}$} \\
\rowcolor{Gray}
Pile-up offset $p_{\textrm T}$ (JES) [\%]	
&	$^{-0.78}_{+0.83}$ &	{$^{-0.30}_{+0.28}$} &	{\textrm -} &	\textrm - &	{$^{+0.11}_{-0.14}$} &	\textrm - &	{\textrm -} &	{$^{+0.20}_{-0.19}$} &	{$^{+0.27}_{\textrm{ \phantom{ai}-}}$} &	{$^{+0.13}_{-0.18}$} &	{\textrm -} \\
Pile-up offset $\rho$ topology (JES) [\%]	
&	$^{-1.29}_{+0.56}$ &	$^{+1.18}_{-1.74}$ &	{$^{+1.89}_{-2.27}$} &	$^{+2.01}_{-2.45}$ &	{$^{+1.44}_{-2.25}$} &	$^{+1.61}_{-1.67}$ &	{$^{+0.32}_{-1.55}$} &	{$^{+0.43}_{-1.71}$} &	{$^{\textrm{ \phantom{ai}-}}_{-1.73}$} &	{$^{+0.48}_{-1.69}$} &	{$^{\textrm{ \phantom{ai}-}}_{-1.75}$} \\
\rowcolor{Gray}
Punch-through (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Single particle high-$p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Jet energy resolution [\%]	
&	$\mp$4.57 &	$\mp$3.74 &	{$\mp$1.53} &	{$\mp$0.39} &	$\mp$0.49 &	$\pm$0.38 &	{$\mp$0.75} &	{$\mp$0.18} &	{$\mp$1.00} &	{$\mp$2.38} &	$\mp$2.35 \\
Jet vertex fraction [\%]	
&	$^{+7.71}_{-7.39}$ &	{$^{+5.38}_{-5.24}$} &	{$^{+3.82}_{-3.77}$} &	{$^{+2.93}_{-2.91}$} &	$^{+2.30}_{-2.29}$ &	$^{+1.82}_{-1.81}$ &	{$^{+1.35}_{-1.31}$} &	$^{+1.07}_{-1.05}$ &	{$^{+0.82}_{-0.72}$} &	$^{+0.69}_{-0.66}$ &	{$^{+0.18}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-6.09}_{+6.24}$ &	{$^{-4.51}_{+4.60}$} &	$^{-3.93}_{+4.00}$ &	$^{-3.79}_{+3.84}$ &	$^{-3.72}_{+3.78}$ &	$^{-3.67}_{+3.73}$ &	$^{-3.66}_{+3.71}$ &	$^{-3.76}_{+3.81}$ &	$^{-3.83}_{+3.88}$ &	$^{-3.78}_{+3.82}$ &	$^{-4.11}_{+4.17}$ \\
$b$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$\mp$0.17 &	{$\mp$0.81} &	{$\mp$1.27} &	{$^{-1.70}_{+1.72}$} &	$^{-2.15}_{+2.17}$ &	$^{-2.51}_{+2.54}$ &	$^{-2.91}_{+2.95}$ &	$^{-3.27}_{+3.31}$ &	$^{-3.60}_{+3.65}$ &	$^{-3.76}_{+3.81}$ &	$^{-4.40}_{+4.46}$ \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 2) [\%]	
&	$^{+1.49}_{-1.48}$ &	$^{+1.55}_{-1.54}$ &	$^{+1.37}_{-1.36}$ &	$\pm$1.08 &	{$\pm$0.81} &	{$\pm$0.58} &	{$\pm$0.36} &	{$\pm$0.18} &	\textrm - &	\textrm - &	{$\mp$0.37} \\
$b$-Quark tagging efficiency (eigenvector 3) [\%]	
&	$\mp$0.37 &	{\textrm -} &	{$\pm$0.16} &	{$\pm$0.21} &	{$\pm$0.16} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\mp$0.12} &	{$\mp$0.16} &	{$\mp$0.28} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	$\mp$0.11 &	{$\mp$0.15} \\
$c$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-2.04}_{+2.07}$ &	{$^{-1.39}_{+1.40}$} &	$\mp$1.28 &	$^{-1.39}_{+1.40}$ &	$^{-1.50}_{+1.51}$ &	$\mp$1.55 &	$^{-1.75}_{+1.77}$ &	$^{-1.82}_{+1.83}$ &	$^{-1.92}_{+1.93}$ &	$^{-1.96}_{+1.97}$ &	$^{-2.45}_{+2.48}$ \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$\pm$0.58 &	{$\pm$0.31} &	{$\pm$0.20} &	{$\pm$0.14} &	{\textrm -} &	\textrm - &	\textrm - &	{$\mp$0.17} &	{$\mp$0.27} &	$\mp$0.30 &	{$\mp$0.55} \\
$c$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	{$\pm$0.15} &	$\pm$0.19 &	$\pm$0.22 &	$\pm$0.21 &	$\pm$0.19 &	$\pm$0.17 &	$\pm$0.14 &	$\pm$0.12 &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 3) [\%]	
&	$\mp$0.22 &	{$\mp$0.11} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 0) [\%]	
&	$^{-1.95}_{+2.09}$ &	{$^{-0.99}_{+1.02}$} &	$^{-1.11}_{+1.15}$ &	$^{-1.18}_{+1.23}$ &	{$^{-1.63}_{+1.75}$} &	$^{-2.01}_{+2.15}$ &	$^{-2.20}_{+2.23}$ &	$^{-2.68}_{+2.71}$ &	{$^{-3.39}_{+3.53}$} &	$^{-3.41}_{+3.51}$ &	{$^{-6.94}_{+7.57}$} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{$\mp$0.11} &	{$^{-0.37}_{+0.38}$} \\
Light-jet tagging efficiency (eigenvector 2) [\%]	
&	$\pm$0.23 &	{$\pm$0.10} &	\textrm - &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.11}$ &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$\mp$0.10} &	{$\mp$0.29} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 3) [\%]	
&	$\mp$0.12 &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 5) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 6) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 7) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 8) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 9) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 10) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 11) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$b$-Quark tagging  extrapolation  [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{$^{+0.23}_{-0.25}$} &	{$^{+0.63}_{-0.62}$} &	{$^{+1.20}_{-1.19}$} &	{$^{+1.76}_{-1.75}$} &	$^{+2.27}_{-2.25}$ &	$^{+2.61}_{-2.59}$ &	{$^{+4.30}_{-4.24}$} \\
\rowcolor{Gray}
$b$-Quark tagging extrapolation from $c$-Quark [\%]	
&	$\pm$0.15 &	{\textrm -} &	\textrm - &	$\pm$0.10 &	$^{+0.11}_{-0.13}$ &	$^{+0.13}_{-0.12}$ &	$\pm$0.13 &	$^{+0.13}_{-0.14}$ &	$\pm$0.15 &	$\pm$0.14 &	{$\pm$0.21} \\
Electron energy resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$^{-0.12}_{+0.10}$ &	{$^{-0.25}_{+0.14}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.37}$ &	$^{-0.35}_{+0.10}$ \\
\rowcolor{Gray}
Electron energy scale [\%]	
&	$^{-0.19}_{+0.18}$ &	\textrm - &	\textrm - &	{\textrm -} &	{$\pm$0.11} &	{$^{+0.25}_{\textrm{ \phantom{ai}-}}$} &	\textrm - &	$^{+0.28}_{-0.15}$ &	{$^{+0.21}_{-0.12}$} &	{\textrm -} &	{$^{+0.28}_{-0.17}$} \\
Electron trigger efficiency [\%]	
&	$\pm$0.23 &	$\pm$0.22 &	$\pm$0.23 &	$\pm$0.25 &	$\pm$0.28 &	$\pm$0.30 &	$\pm$0.32 &	$\pm$0.36 &	$\pm$0.38 &	$\pm$0.40 &	$\pm$0.51 \\
\rowcolor{Gray}
Electron reconstruction efficiency [\%]	
&	$\pm$0.14 &	$\pm$0.15 &	$\pm$0.16 &	$\pm$0.18 &	$\pm$0.20 &	$\pm$0.21 &	$\pm$0.22 &	$\pm$0.24 &	$\pm$0.26 &	$\pm$0.27 &	$\pm$0.32 \\
Electron identification efficiency [\%]	
&	$\pm$0.36 &	$\pm$0.35 &	$\pm$0.38 &	$\pm$0.42 &	$\pm$0.47 &	$\pm$0.53 &	$\pm$0.58 &	$\pm$0.64 &	$\pm$0.71 &	$\pm$0.74 &	$\pm$0.92 \\
\rowcolor{Gray}
Electron isolation efficiency [\%]	
&	$\pm$0.11 &	$\pm$0.11 &	$\pm$0.12 &	$\pm$0.15 &	$\pm$0.18 &	$\pm$0.23 &	$\pm$0.27 &	$\pm$0.32 &	$\pm$0.37 &	$\pm$0.39 &	{$\pm$0.52} \\
Muon energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Muon (MS) momentum resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - \\
Muon (ID) momentum resolution [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	$^{-0.14}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
Muon trigger efficiency stat [\%]	
&	$^{+0.60}_{-0.62}$ &	$^{+0.56}_{-0.57}$ &	$^{+0.56}_{-0.58}$ &	$^{+0.56}_{-0.58}$ &	$^{+0.57}_{-0.58}$ &	$^{+0.57}_{-0.58}$ &	$^{+0.57}_{-0.59}$ &	$^{+0.59}_{-0.61}$ &	$^{+0.60}_{-0.61}$ &	$^{+0.59}_{-0.60}$ &	$^{+0.65}_{-0.68}$ \\
Muon trigger efficiency syst [\%]	
&	$\pm$0.26 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.25 &	$\pm$0.25 &	$\pm$0.25 &	$\pm$0.25 &	$^{+0.28}_{-0.27}$ \\
\rowcolor{Gray}
Muon identification stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon identification syst [\%]	
&	$\pm$0.15 &	$\pm$0.14 &	$\pm$0.15 &	$\pm$0.17 &	$\pm$0.19 &	$\pm$0.21 &	$\pm$0.24 &	$\pm$0.26 &	$\pm$0.29 &	$\pm$0.32 &	$\pm$0.41 \\
\rowcolor{Gray}
Muon isolation efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} \\
Muon isolation efficiency syst [\%]	
&	$\pm$0.11 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.11 &	$\pm$0.11 &	$\pm$0.11 &	$\pm$0.12 &	$\pm$0.12 &	$\pm$0.15 \\
\rowcolor{Gray}
Muon TTVA efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon TTVA efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution para [\%]	
&	$\pm$0.59 &	{$\pm$0.27} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	$\mp$0.10 &	{\textrm -} &	{$\pm$0.13} &	{$\mp$0.23} &	$\pm$0.26 \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution perp [\%]	
&	$\pm$0.43 &	{$\pm$0.13} &	{\textrm -} &	{$\mp$0.13} &	{$\mp$0.29} &	$\mp$0.27 &	{$\mp$0.38} &	{$\mp$0.25} &	$\mp$0.26 &	{$\mp$0.59} &	$\mp$0.57 \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet scale [\%]	
&	$^{+0.67}_{-0.49}$ &	{$^{+0.17}_{-0.26}$} &	\textrm - &	$^{-0.13}_{\textrm{ \phantom{ai}-}}$ &	{$^{-0.23}_{+0.16}$} &	{$^{-0.17}_{+0.24}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.27}$ &	$^{-0.16}_{+0.27}$ &	$^{-0.26}_{+0.22}$ &	{$^{-0.28}_{+0.11}$} &	{$^{-0.37}_{+0.16}$} \\
Luminosity [\%]	
&	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 \\
\rowcolor{Gray}
Single top cross-section [\%]	
&	$\pm$0.27 &	{$\pm$0.17} &	$\pm$0.19 &	$\pm$0.23 &	$\pm$0.29 &	$\pm$0.35 &	$\pm$0.42 &	$\pm$0.49 &	$\pm$0.57 &	$\pm$0.63 &	{$\pm$0.83} \\
$Z$+jets cross-section [\%]	
&	$\pm$1.40 &	{$\pm$0.48} &	$\pm$0.44 &	$\pm$0.48 &	$\pm$0.62 &	{$\pm$0.46} &	$\pm$0.51 &	{$\pm$0.93} &	$\pm$1.16 &	$\pm$0.92 &	{$\pm$2.32} \\
\rowcolor{Gray}
Diboson cross-section [\%]	
&	$\pm$0.19 &	{\textrm -} &	\textrm - &	$\pm$0.10 &	$\pm$0.13 &	{$\pm$0.19} &	$\pm$0.24 &	$\pm$0.30 &	$\pm$0.39 &	$\pm$0.44 &	{$\pm$0.65} \\
$t\bar{t}V$ cross-section [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$\mp$0.12} &	{$\mp$0.18} &	$\mp$0.20 &	$\mp$0.21 &	$\mp$0.25 \\
\rowcolor{Gray}
Monte Carlo sample statistics [\%]	
&	$\pm$0.76 &	{$\pm$0.29} &	$\pm$0.27 &	$\pm$0.29 &	{$\pm$0.39} &	$\pm$0.47 &	$\pm$0.54 &	{$\pm$0.75} &	{$\pm$1.38} &	$\pm$1.39 &	$\pm$1.70 \\
ISR/FSR + scale [\%]	
&	$^{-2.26}_{+1.69}$ &	{$^{-2.31}_{+0.86}$} &	{$^{-3.07}_{+2.75}$} &	$^{-3.17}_{+2.52}$ &	$^{-2.80}_{+2.22}$ &	{$^{-2.03}_{+3.22}$} &	$^{-3.09}_{+2.50}$ &	$^{-2.42}_{+2.52}$ &	$^{-2.80}_{+2.24}$ &	{$^{-5.25}_{+0.56}$} &	{$^{-2.00}_{+1.66}$} \\
\rowcolor{Gray}
Alternate hard-scattering model [\%]	
&	$\mp$1.35 &	$\mp$1.33 &	{$\pm$0.12} &	{$\mp$0.37} &	{$\pm$0.75} &	{$\mp$1.14} &	{$\pm$3.30} &	$\pm$3.29 &	$\pm$4.23 &	{$\pm$2.34} &	{$\pm$9.04} \\
Alternate parton-shower model [\%]	
&	\textrm - &	{$\pm$0.13} &	{$\mp$2.55} &	{$\mp$1.71} &	$\mp$1.93 &	{$\mp$1.00} &	{$\mp$1.76} &	{$\mp$0.74} &	{$\mp$1.49} &	{$\mp$2.48} &	{$\mp$3.77} \\
\rowcolor{Gray}
Inter PDF [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{$\pm$0.12} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.11} &	{$\pm$0.42} \\
Intra PDF [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{$\pm$0.14} &	{$\pm$0.30} \\
\rowcolor{Gray}
Real lepton efficiency stat [\%]	
&	$\mp$0.10 &	$^{-0.11}_{+0.10}$ &	$\mp$0.12 &	$^{-0.15}_{+0.14}$ &	$^{-0.18}_{+0.17}$ &	$^{-0.23}_{+0.20}$ &	$^{-0.25}_{+0.23}$ &	$^{-0.34}_{+0.28}$ &	$^{-0.39}_{+0.31}$ &	$^{-0.48}_{+0.36}$ &	$^{-0.64}_{+0.44}$ \\
Fake lepton efficiency MC scale [\%]	
&	$^{+1.70}_{-1.85}$ &	{$^{+0.53}_{-0.57}$} &	$^{+0.43}_{-0.48}$ &	$^{+0.39}_{-0.50}$ &	{$^{+0.56}_{-0.74}$} &	$^{+0.65}_{-0.89}$ &	$^{+0.67}_{-0.86}$ &	{$^{+0.89}_{-1.42}$} &	$^{+0.70}_{-1.78}$ &	{$^{+0.17}_{-1.29}$} &	{$^{+1.89}_{-2.07}$} \\
\rowcolor{Gray}
Fake lepton efficiency alternate CR [\%]	
&	$\pm$0.83 &	{$\pm$0.28} &	{$\pm$0.21} &	{$\pm$0.28} &	$\pm$0.36 &	{$\pm$0.52} &	{$\pm$0.26} &	{$\pm$0.54} &	$\pm$0.55 &	$\pm$0.65 &	{\textrm -} \\
Fake overall normalisation [\%]	
&	$\pm$8.86 &	{$\pm$2.97} &	$\pm$2.30 &	$\pm$2.46 &	{$\pm$3.23} &	$\pm$3.35 &	$\pm$3.88 &	$\pm$4.84 &	$\pm$5.87 &	$\pm$5.60 &	{$\pm$10.5} \\
\rowcolor{Gray}
$W$+jets $CA_{4incl}$ stat error [\%]	
&	$\mp$0.17 &	{\textrm -} &	\textrm - &	{\textrm -} &	{$\mp$0.12} &	$\mp$0.13 &	{$\mp$0.17} &	$\mp$0.20 &	$\mp$0.23 &	$\mp$0.27 &	{$\mp$0.41} \\
$W$+jets Fc stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{$^{+0.16}_{-0.15}$} \\
\rowcolor{Gray}
$W$+jets Fcc stat error [\%]	
&	$^{+0.20}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{$^{-0.16}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.43}_{+0.21}$} &	$^{-0.41}_{+0.20}$ &	{\textrm -} \\
$W$+jets Flight stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\hline
\end{tabular}}


==> tables/systematics/resolved/table_syst_particle_tt_m_RelativeDiffXs.tex <==
\resizebox*{\textwidth}{!}{
\begin{tabular}{l c c c c c c c c c c c}
\hline
Bins  [GeV]
 & 225--345   & 345--420   & 420--500   & 500--590   & 590--685   & 685--790   & 790--910   & 910--1040   & 1040--1175   & 1175--1320   & 1320--3000  \\
\hline
\hline
1/$\sigma$ $\cdot$ d$\sigma$ / d$m^{t\bar{t}}$	&	$4.83 \cdot 10^{-4}$ &	$2.82 \cdot 10^{-3}$ &	$2.83 \cdot 10^{-3}$ &	$2.07 \cdot 10^{-3}$ &	$1.26 \cdot 10^{-3}$ &	$7.62 \cdot 10^{-4}$ &	$4.23 \cdot 10^{-4}$ &	$2.28 \cdot 10^{-4}$ &	$1.17 \cdot 10^{-4}$ &	$6.44 \cdot 10^{-5}$ &	$7.16 \cdot 10^{-6}$ \\
\hline
\rowcolor{Gray}
Total uncertainty [\%]	
&	$^{+13.2}_{-14.0}$ &	$^{+4.45}_{-4.73}$ &	$^{+3.02}_{-2.77}$ &	$^{+3.18}_{-2.98}$ &	$^{+3.01}_{-2.95}$ &	$^{+4.59}_{-3.95}$ &	$^{+5.35}_{-5.56}$ &	$^{+6.90}_{-7.15}$ &	$^{+8.25}_{-9.22}$ &	$^{+8.74}_{-9.07}$ &	$^{+16.9}_{-17.9}$ \\
Statistical uncertainty [\%]	
&	$\pm1.6$ &	$\pm0.6$ &	$\pm0.6$ &	$\pm0.7$ &	$\pm0.9$ &	$\pm1.1$ &	$\pm1.5$ &	$\pm1.9$ &	$\pm2.7$ &	$\pm3.9$ &	$\pm3.4$ \\
\rowcolor{Gray}
Systematic uncertainty [\%]	
&	$^{+13.1}_{-13.9}$ &	$^{+4.39}_{-4.68}$ &	$^{+2.93}_{-2.67}$ &	$^{+3.08}_{-2.88}$ &	$^{+2.83}_{-2.77}$ &	$^{+4.41}_{-3.75}$ &	$^{+5.11}_{-5.32}$ &	$^{+6.57}_{-6.83}$ &	$^{+7.64}_{-8.68}$ &	$^{+7.70}_{-8.07}$ &	$^{+16.5}_{-17.5}$ \\
\hline
\hline
$b$-Tagged jet energy scale (JES) [\%]	
&	$^{-3.38}_{+3.43}$ &	{$^{-0.76}_{+0.62}$} &	{$^{+0.36}_{-0.32}$} &	{$^{+0.53}_{-0.54}$} &	$^{+0.57}_{-0.63}$ &	{$^{+0.80}_{-0.48}$} &	{$^{+0.30}_{-0.42}$} &	{$^{+0.51}_{-0.41}$} &	{$^{+0.29}_{-0.37}$} &	{$^{+0.46}_{-0.29}$} &	{$^{+0.35}_{\textrm{ \phantom{ai}-}}$} \\
\rowcolor{Gray}
Effective detector NP set 1 (JES) [\%]	
&	$^{-7.03}_{+6.00}$ &	{$^{-0.59}_{+0.55}$} &	{$^{+1.70}_{-1.41}$} &	$^{+1.61}_{-1.40}$ &	{$^{+0.70}_{-0.48}$} &	{$^{-0.14}_{+0.40}$} &	{$^{-1.05}_{+1.20}$} &	$^{-1.71}_{+0.93}$ &	{$^{-2.61}_{\textrm{ \phantom{ai}-}}$} &	{$^{-2.40}_{+1.90}$} &	{$^{-4.98}_{+3.26}$} \\
Effective detector NP set 2 (JES) [\%]	
&	$^{-2.72}_{+2.61}$ &	{$^{-1.51}_{+1.44}$} &	{$^{-0.39}_{+0.52}$} &	{$^{+0.13}_{-0.24}$} &	{$^{+1.03}_{-0.98}$} &	{$^{+1.79}_{-1.35}$} &	{$^{+1.23}_{-1.75}$} &	{$^{+2.88}_{-2.83}$} &	$^{+2.83}_{-2.89}$ &	$^{+3.26}_{-3.09}$ &	{$^{+4.52}_{-4.95}$} \\
\rowcolor{Gray}
Effective detector NP set 3 (JES) [\%]	
&	$^{+2.21}_{-2.16}$ &	{$\pm$0.94} &	{$^{+0.18}_{-0.14}$} &	$^{-0.30}_{+0.18}$ &	{$^{-0.71}_{+0.69}$} &	{$^{-0.85}_{+1.15}$} &	{$^{-1.03}_{+0.71}$} &	{$^{-1.39}_{+1.57}$} &	$^{-1.58}_{+1.66}$ &	$^{-1.69}_{+1.62}$ &	{$^{-2.25}_{+2.16}$} \\
Effective detector NP set 4 (JES) [\%]	
&	$^{-1.77}_{+1.74}$ &	{$^{-0.56}_{+0.58}$} &	{\textrm -} &	{$^{+0.26}_{-0.31}$} &	{$^{+0.50}_{-0.43}$} &	$^{+0.61}_{-0.50}$ &	{$^{+0.29}_{-0.56}$} &	{$^{+0.53}_{-0.52}$} &	$^{+0.63}_{-0.70}$ &	{$^{+0.42}_{-0.62}$} &	{$^{+0.18}_{-0.45}$} \\
\rowcolor{Gray}
Effective detector NP set 5 (JES) [\%]	
&	$\pm$0.76 &	{\textrm -} &	{$^{-0.11}_{+0.12}$} &	{\textrm -} &	{$^{-0.12}_{+0.14}$} &	\textrm - &	\textrm - &	$^{+0.20}_{-0.11}$ &	{\textrm -} &	$^{+0.11}_{-0.19}$ &	{$^{+0.25}_{-0.11}$} \\
Effective detector NP set 6 restTerm (JES) [\%]	
&	$^{-0.50}_{+0.51}$ &	{$^{-0.14}_{+0.10}$} &	{\textrm -} &	\textrm - &	{$^{+0.14}_{-0.13}$} &	{$^{+0.19}_{-0.14}$} &	{\textrm -} &	{$^{+0.21}_{-0.23}$} &	{\textrm -} &	{$^{+0.22}_{-0.28}$} &	$^{+0.20}_{-0.25}$ \\
\rowcolor{Gray}
$\eta$ intercalibration model (JES) [\%]	
&	$^{-3.67}_{+3.82}$ &	{$^{-0.94}_{+0.87}$} &	{$^{+0.27}_{-0.23}$} &	{$^{+0.85}_{-0.59}$} &	$^{+0.75}_{-0.84}$ &	$\pm$0.67 &	{$^{+0.42}_{-0.50}$} &	{$^{+0.58}_{-1.17}$} &	$^{+0.55}_{-1.03}$ &	$^{+0.51}_{-0.54}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.48}$} \\
$\eta$ intercalibration total stat (JES) [\%]	
&	$^{-2.22}_{+1.81}$ &	{$^{-0.32}_{+0.25}$} &	{$^{+0.28}_{-0.16}$} &	{$\pm$0.42} &	$^{+0.37}_{-0.29}$ &	{$^{+0.49}_{-0.15}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.26}$} &	\textrm - &	$^{\textrm{ \phantom{ai}-}}_{-0.30}$ &	$^{+0.23}_{\textrm{ \phantom{ai}-}}$ &	{$^{-1.04}_{+0.79}$} \\
\rowcolor{Gray}
Flavour composition (JES) [\%]	
&	$^{-4.34}_{+3.46}$ &	{$^{-0.10}_{+0.19}$} &	{$^{+0.99}_{-1.05}$} &	$^{+0.97}_{-1.00}$ &	{$^{+0.47}_{-0.16}$} &	{$^{-0.23}_{+0.70}$} &	{$^{-0.70}_{+1.14}$} &	{$^{-1.33}_{+0.86}$} &	{$^{-2.35}_{+0.52}$} &	{$^{-1.25}_{+2.15}$} &	{$^{-4.12}_{+3.14}$} \\
Flavour response (JES) [\%]	
&	$^{+1.72}_{-1.77}$ &	{$^{+0.26}_{-0.11}$} &	{$^{-0.21}_{+0.27}$} &	{$^{-0.43}_{+0.46}$} &	{$^{-0.29}_{+0.23}$} &	$^{+0.31}_{\textrm{ \phantom{ai}-}}$ &	{$^{\textrm{ \phantom{ai}-}}_{-0.51}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.30}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.73}$ &	$^{\textrm{ \phantom{ai}-}}_{-0.32}$ &	{$^{+0.71}_{-2.14}$} \\
\rowcolor{Gray}
Pile-up offset $\mu$ (JES) [\%]	
&	$^{+0.33}_{-0.47}$ &	{\textrm -} &	\textrm - &	{$^{-0.14}_{+0.10}$} &	{\textrm -} &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.22}$} &	{$^{+0.24}_{\textrm{ \phantom{ai}-}}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.42}$} &	{$^{+0.12}_{-0.17}$} &	{$^{+0.57}_{-0.80}$} \\
Pile-up offset $N_{\textrm PV}$ (JES) [\%]	
&	$^{+0.17}_{-0.44}$ &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$^{+0.13}_{-0.23}$} &	{\textrm -} &	{$\pm$0.21} &	$^{+0.26}_{-0.22}$ &	{$^{+0.57}_{-0.50}$} \\
\rowcolor{Gray}
Pile-up offset $p_{\textrm T}$ (JES) [\%]	
&	$^{-0.69}_{+0.75}$ &	{$^{-0.22}_{+0.20}$} &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{-0.15}$} &	{$^{+0.20}_{-0.21}$} &	$^{+0.20}_{\textrm{ \phantom{ai}-}}$ &	{$^{+0.13}_{-0.20}$} &	{$^{+0.28}_{-0.27}$} &	$^{+0.35}_{-0.16}$ &	{$^{+0.21}_{-0.26}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.18}$} \\
Pile-up offset $\rho$ topology (JES) [\%]	
&	$^{-2.55}_{+2.51}$ &	{$^{-0.10}_{+0.15}$} &	{$^{+0.60}_{-0.38}$} &	$^{+0.71}_{-0.57}$ &	{$^{+0.15}_{-0.36}$} &	{$^{+0.31}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.94}_{+0.34}$} &	{$^{-0.84}_{+0.18}$} &	$^{-1.61}_{+0.16}$ &	$^{-0.79}_{+0.20}$ &	{$^{-3.01}_{+1.18}$} \\
\rowcolor{Gray}
Punch-through (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Single particle high-$p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Jet energy resolution [\%]	
&	$\mp$2.99 &	{$\mp$2.15} &	{\textrm -} &	{$\pm$1.25} &	$\pm$1.15 &	{$\pm$2.05} &	{$\pm$0.88} &	{$\pm$1.47} &	{$\pm$0.63} &	$\mp$0.76 &	$\mp$0.74 \\
Jet vertex fraction [\%]	
&	$^{+4.02}_{-4.05}$ &	{$^{+1.77}_{-1.83}$} &	{$^{+0.26}_{-0.30}$} &	{$^{-0.59}_{+0.58}$} &	{$^{-1.20}_{+1.22}$} &	{$^{-1.67}_{+1.72}$} &	{$^{-2.12}_{+2.24}$} &	$^{-2.39}_{+2.51}$ &	$^{-2.63}_{+2.85}$ &	$^{-2.76}_{+2.91}$ &	$^{-3.25}_{+3.51}$ \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-2.08}_{+1.99}$ &	{$^{-0.44}_{+0.42}$} &	{$^{+0.16}_{-0.15}$} &	{$^{+0.31}_{-0.30}$} &	$^{+0.38}_{-0.36}$ &	$^{+0.43}_{-0.41}$ &	$^{+0.44}_{-0.42}$ &	$^{+0.34}_{-0.33}$ &	$^{+0.27}_{-0.26}$ &	$\pm$0.32 &	{\textrm -} \\
$b$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$^{+1.48}_{-1.44}$ &	{$^{+0.83}_{-0.82}$} &	{$^{+0.37}_{-0.36}$} &	{\textrm -} &	{$^{-0.52}_{+0.51}$} &	{$^{-0.89}_{+0.88}$} &	{$^{-1.30}_{+1.28}$} &	$^{-1.66}_{+1.64}$ &	$^{-1.99}_{+1.97}$ &	$^{-2.16}_{+2.13}$ &	{$^{-2.81}_{+2.77}$} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 2) [\%]	
&	$\pm$0.39 &	$^{+0.45}_{-0.46}$ &	{$\pm$0.27} &	\textrm - &	$\mp$0.27 &	{$\mp$0.50} &	{$^{-0.72}_{+0.73}$} &	$^{-0.90}_{+0.91}$ &	$^{-1.08}_{+1.10}$ &	$^{-1.17}_{+1.19}$ &	$^{-1.45}_{+1.48}$ \\
$b$-Quark tagging efficiency (eigenvector 3) [\%]	
&	$\mp$0.44 &	{\textrm -} &	\textrm - &	{$\pm$0.14} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\mp$0.11} &	{$\mp$0.19} &	$\mp$0.23 &	{$\mp$0.35} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{$\mp$0.13} \\
$c$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$\mp$0.56 &	{\textrm -} &	{$\pm$0.21} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\mp$0.27} &	$^{-0.34}_{+0.33}$ &	$^{-0.43}_{+0.42}$ &	$\mp$0.47 &	{$^{-0.98}_{+0.97}$} \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$\pm$0.42 &	{$\pm$0.15} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\mp$0.16} &	{$\mp$0.24} &	{$\mp$0.33} &	{$\mp$0.43} &	$\mp$0.46 &	{$\mp$0.71} \\
$c$-Quark tagging efficiency (eigenvector 2) [\%]	
&	$\mp$0.11 &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{$\mp$0.10} &	{$\mp$0.20} \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 3) [\%]	
&	$\mp$0.17 &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 0) [\%]	
&	$^{-0.44}_{+0.50}$ &	$^{+0.53}_{-0.55}$ &	{$^{+0.40}_{-0.42}$} &	$^{+0.33}_{-0.34}$ &	{$^{-0.12}_{+0.16}$} &	{$^{-0.50}_{+0.55}$} &	$^{-0.69}_{+0.63}$ &	{$^{-1.18}_{+1.11}$} &	{$^{-1.90}_{+1.91}$} &	$^{-1.92}_{+1.89}$ &	{$^{-5.50}_{+5.89}$} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$\mp$0.14 &	{$^{-0.41}_{+0.42}$} \\
Light-jet tagging efficiency (eigenvector 2) [\%]	
&	$\pm$0.14 &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	$^{-0.11}_{+0.10}$ &	{$\mp$0.19} &	{$\mp$0.38} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 3) [\%]	
&	$\mp$0.10 &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{$^{+0.12}_{-0.11}$} &	{\textrm -} &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 5) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - \\
Light-jet tagging efficiency (eigenvector 6) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 7) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 8) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 9) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 10) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 11) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$b$-Quark tagging  extrapolation  [\%]	
&	$^{-0.31}_{+0.32}$ &	$\mp$0.31 &	$\mp$0.31 &	$\mp$0.27 &	{\textrm -} &	{$^{+0.33}_{-0.32}$} &	{$^{+0.89}_{-0.88}$} &	{$\pm$1.45} &	{$^{+1.96}_{-1.95}$} &	$^{+2.30}_{-2.29}$ &	{$^{+3.98}_{-3.95}$} \\
\rowcolor{Gray}
$b$-Quark tagging extrapolation from $c$-Quark [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{$\pm$0.10} \\
Electron energy resolution [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$^{-0.16}_{+0.14}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.32}$ &	$^{-0.26}_{+0.10}$ \\
\rowcolor{Gray}
Electron energy scale [\%]	
&	$^{-0.24}_{+0.22}$ &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{$^{+0.20}_{\textrm{ \phantom{ai}-}}$} &	\textrm - &	$^{+0.23}_{-0.11}$ &	{$^{+0.16}_{\textrm{ \phantom{ai}-}}$} &	\textrm - &	$^{+0.23}_{-0.13}$ \\
Electron trigger efficiency [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.12} &	$\pm$0.14 &	{$\pm$0.25} \\
\rowcolor{Gray}
Electron reconstruction efficiency [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{$^{+0.13}_{-0.14}$} \\
Electron identification efficiency [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.14} &	{$\pm$0.20} &	{$\pm$0.27} &	$\pm$0.30 &	{$\pm$0.48} \\
\rowcolor{Gray}
Electron isolation efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.11} &	{$\pm$0.15} &	{$\pm$0.20} &	$\pm$0.23 &	{$\pm$0.35} \\
Muon energy scale [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Muon (MS) momentum resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - \\
Muon (ID) momentum resolution [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon trigger efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
Muon trigger efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Muon identification stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon identification syst [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\pm$0.11} &	$\pm$0.14 &	{$\pm$0.23} \\
\rowcolor{Gray}
Muon isolation efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Muon isolation efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Muon TTVA efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
Muon TTVA efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution para [\%]	
&	$\pm$0.50 &	{$\pm$0.18} &	{\textrm -} &	{$\mp$0.15} &	{$\mp$0.10} &	{$\mp$0.17} &	$\mp$0.18 &	{\textrm -} &	{\textrm -} &	{$\mp$0.31} &	{$\pm$0.17} \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution perp [\%]	
&	$\pm$0.51 &	{$\pm$0.21} &	{\textrm -} &	\textrm - &	{$\mp$0.21} &	$\mp$0.18 &	{$\mp$0.30} &	{$\mp$0.17} &	$\mp$0.18 &	{$\mp$0.51} &	$\mp$0.49 \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet scale [\%]	
&	$^{+0.70}_{-0.47}$ &	{$^{+0.19}_{-0.24}$} &	{\textrm -} &	\textrm - &	{$^{-0.21}_{+0.18}$} &	{$^{-0.15}_{+0.25}$} &	{$^{-0.25}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.14}_{+0.29}$} &	$^{-0.23}_{+0.24}$ &	{$^{-0.26}_{+0.13}$} &	{$^{-0.35}_{+0.17}$} \\
Luminosity [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Single top cross-section [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{$\pm$0.15} &	{$\pm$0.23} &	{$\pm$0.31} &	$\pm$0.36 &	{$\pm$0.56} \\
$Z$+jets cross-section [\%]	
&	$\pm$0.79 &	{$\mp$0.11} &	{$\mp$0.15} &	{$\mp$0.11} &	{\textrm -} &	{$\mp$0.13} &	{\textrm -} &	{$\pm$0.33} &	{$\pm$0.56} &	{$\pm$0.32} &	{$\pm$1.71} \\
\rowcolor{Gray}
Diboson cross-section [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{$\pm$0.10} &	{$\pm$0.16} &	{$\pm$0.25} &	$\pm$0.30 &	{$\pm$0.51} \\
$t\bar{t}V$ cross-section [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{$\mp$0.10} &	$\mp$0.12 &	$\mp$0.13 &	{$\mp$0.17} \\
\rowcolor{Gray}
Monte Carlo sample statistics [\%]	
&	$\pm$0.74 &	{$\pm$0.26} &	$\pm$0.25 &	$\pm$0.28 &	{$\pm$0.37} &	$\pm$0.46 &	$\pm$0.54 &	{$\pm$0.74} &	{$\pm$1.37} &	$\pm$1.38 &	$\pm$1.68 \\
ISR/FSR + scale [\%]	
&	$^{+0.50}_{-0.45}$ &	$^{+0.45}_{-1.26}$ &	{$^{-0.33}_{+0.57}$} &	{$^{-0.42}_{+0.35}$} &	{\textrm -} &	{$^{+1.04}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.34}_{+0.33}$} &	{$^{+0.35}_{\textrm{ \phantom{ai}-}}$} &	{\textrm -} &	$^{\textrm{ \phantom{ai}-}}_{-2.57}$ &	{$^{+0.76}_{-0.48}$} \\
\rowcolor{Gray}
Alternate hard-scattering model [\%]	
&	$\mp$1.41 &	$\mp$1.40 &	{\textrm -} &	{$\mp$0.44} &	{$\pm$0.68} &	{$\mp$1.20} &	{$\pm$3.23} &	$\pm$3.22 &	$\pm$4.16 &	{$\pm$2.27} &	{$\pm$8.97} \\
Alternate parton-shower model [\%]	
&	$\pm$1.36 &	$\pm$1.55 &	{$\mp$1.18} &	{$\mp$0.32} &	{$\mp$0.54} &	{$\pm$0.39} &	$\mp$0.37 &	{$\pm$0.66} &	{\textrm -} &	{$\mp$1.10} &	{$\mp$2.41} \\
\rowcolor{Gray}
Inter PDF [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{$\pm$0.34} \\
Intra PDF [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{$\pm$0.24} \\
\rowcolor{Gray}
Real lepton efficiency stat [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{$^{-0.17}_{+0.12}$} &	$^{-0.22}_{+0.15}$ &	{$^{-0.31}_{+0.21}$} &	{$^{-0.47}_{+0.29}$} \\
Fake lepton efficiency MC scale [\%]	
&	$^{+1.10}_{-1.11}$ &	{$^{\textrm{ \phantom{ai}-}}_{+0.16}$} &	{$^{-0.16}_{+0.26}$} &	$^{-0.20}_{+0.24}$ &	\textrm - &	{\textrm -} &	{\textrm -} &	{$^{+0.29}_{-0.67}$} &	{$^{+0.10}_{-1.04}$} &	$^{\textrm{ \phantom{ai}-}}_{-0.55}$ &	{$^{+1.28}_{-1.34}$} \\
\rowcolor{Gray}
Fake lepton efficiency alternate CR [\%]	
&	$\pm$0.50 &	{\textrm -} &	{$\mp$0.12} &	{\textrm -} &	{\textrm -} &	{$\pm$0.18} &	{\textrm -} &	{$\pm$0.20} &	$\pm$0.21 &	{$\pm$0.32} &	$\mp$0.34 \\
Fake overall normalisation [\%]	
&	$\pm$5.28 &	{$\mp$0.40} &	{$\mp$1.05} &	$\mp$0.90 &	{$\mp$0.15} &	{\textrm -} &	{$\pm$0.47} &	{$\pm$1.40} &	{$\pm$2.40} &	$\pm$2.14 &	{$\pm$6.96} \\
\rowcolor{Gray}
$W$+jets $CA_{4incl}$ stat error [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{$\mp$0.12} &	{$\mp$0.16} &	{$\mp$0.30} \\
$W$+jets Fc stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{$^{+0.16}_{-0.15}$} \\
\rowcolor{Gray}
$W$+jets Fcc stat error [\%]	
&	$^{+0.20}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	{$^{-0.16}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.44}_{+0.21}$} &	$^{-0.41}_{+0.20}$ &	{\textrm -} \\
$W$+jets Flight stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\hline
\end{tabular}}


==> tables/systematics/resolved/table_syst_particle_tt_pt_AbsoluteDiffXs.tex <==
\resizebox*{!}{\textheight}{
\begin{tabular}{l c c c c c c}
\hline
Bins  [GeV]
 & 0--35   & 35--75   & 75--125   & 125--170   & 170--225   & 225--800  \\
\hline
\hline
d$\sigma$ / d$p_{\textrm T}^{t\bar{t}}$ [pb/GeV]	&	$1.03 \cdot 10^{0}$ &	$8.08 \cdot 10^{-1}$ &	$3.42 \cdot 10^{-1}$ &	$1.67 \cdot 10^{-1}$ &	$8.33 \cdot 10^{-2}$ &	$8.56 \cdot 10^{-3}$ \\
\hline
\rowcolor{Gray}
Total uncertainty [\%]	
&	$^{+11.2}_{-11.7}$ &	$^{+12.3}_{-13.3}$ &	$^{+17.8}_{-17.6}$ &	$^{+15.3}_{-15.2}$ &	$^{+13.0}_{-14.2}$ &	$^{+11.0}_{-12.2}$ \\
Statistical uncertainty [\%]	
&	$\pm0.5$ &	$\pm0.5$ &	$\pm0.8$ &	$\pm1.2$ &	$\pm1.6$ &	$\pm1.5$ \\
\rowcolor{Gray}
Systematic uncertainty [\%]	
&	$^{+11.2}_{-11.7}$ &	$^{+12.3}_{-13.3}$ &	$^{+17.8}_{-17.6}$ &	$^{+15.3}_{-15.1}$ &	$^{+12.9}_{-14.0}$ &	$^{+10.9}_{-12.1}$ \\
\hline
\hline
$b$-Tagged jet energy scale (JES) [\%]	
&	$^{+0.51}_{-0.46}$ &	$^{+0.55}_{-0.52}$ &	$^{+0.58}_{-0.63}$ &	$^{+0.56}_{-0.57}$ &	$^{+0.63}_{-0.71}$ &	{$^{+0.34}_{-0.25}$} \\
\rowcolor{Gray}
Effective detector NP set 1 (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-1.29}$ &	{$^{+6.38}_{-7.33}$} &	{$^{+10.2}_{-10.0}$} &	$^{+8.22}_{-8.13}$ &	$^{+6.64}_{-7.46}$ &	{$^{+5.00}_{-6.28}$} \\
Effective detector NP set 2 (JES) [\%]	
&	\textrm - &	{$^{-1.55}_{+1.48}$} &	$^{-1.62}_{+1.52}$ &	{$^{-0.62}_{+0.47}$} &	{$^{-0.35}_{\textrm{ \phantom{ai}-}}$} &	{$^{+1.04}_{-1.07}$} \\
\rowcolor{Gray}
Effective detector NP set 3 (JES) [\%]	
&	\textrm - &	{$^{+0.50}_{-0.56}$} &	{$^{+0.34}_{-0.40}$} &	$^{-0.27}_{+0.17}$ &	$^{-0.42}_{+0.20}$ &	{$\mp$0.86} \\
Effective detector NP set 4 (JES) [\%]	
&	\textrm - &	{$^{-0.30}_{+0.23}$} &	{\textrm -} &	$^{+0.14}_{-0.26}$ &	$^{+0.16}_{-0.30}$ &	\textrm - \\
\rowcolor{Gray}
Effective detector NP set 5 (JES) [\%]	
&	\textrm - &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{+0.13}$} &	{\textrm -} &	{$^{+0.12}_{-0.20}$} &	{$^{+0.30}_{-0.19}$} \\
Effective detector NP set 6 restTerm (JES) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{$^{+0.11}_{-0.14}$} &	{$^{+0.19}_{-0.20}$} \\
\rowcolor{Gray}
$\eta$ intercalibration model (JES) [\%]	
&	$^{-1.54}_{+0.98}$ &	{$^{+2.35}_{-2.71}$} &	{$^{+4.17}_{-4.21}$} &	{$^{+2.98}_{-3.08}$} &	$^{+2.51}_{-3.13}$ &	$^{+2.04}_{-2.54}$ \\
$\eta$ intercalibration total stat (JES) [\%]	
&	$^{-0.25}_{+0.28}$ &	{$^{+0.98}_{-1.05}$} &	{$^{+1.46}_{-1.63}$} &	$^{+1.24}_{-1.13}$ &	$^{+1.29}_{-1.50}$ &	$^{+1.00}_{-1.03}$ \\
\rowcolor{Gray}
Flavour composition (JES) [\%]	
&	$^{-1.94}_{+0.89}$ &	{$^{+4.36}_{-5.33}$} &	{$^{+9.12}_{-9.04}$} &	$^{+8.00}_{-7.90}$ &	$^{+6.60}_{-6.98}$ &	{$^{+4.69}_{-5.42}$} \\
Flavour response (JES) [\%]	
&	$^{+0.42}_{-0.90}$ &	$^{-1.46}_{+1.13}$ &	{$^{-2.66}_{+2.30}$} &	$^{-2.38}_{+2.09}$ &	$^{-2.65}_{+1.72}$ &	$^{-1.90}_{+1.41}$ \\
\rowcolor{Gray}
Pile-up offset $\mu$ (JES) [\%]	
&	$^{+0.18}_{-0.21}$ &	{$^{-0.36}_{+0.28}$} &	{$^{-0.58}_{+0.56}$} &	{$^{-0.37}_{+0.29}$} &	$^{-0.48}_{+0.32}$ &	{$^{-0.15}_{+0.13}$} \\
Pile-up offset $N_{\textrm PV}$ (JES) [\%]	
&	$^{+0.20}_{\textrm{ \phantom{ai}-}}$ &	{\textrm -} &	{$^{-0.16}_{+0.17}$} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Pile-up offset $p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	{$^{-0.20}_{+0.19}$} &	\textrm - &	{$^{+0.10}_{-0.14}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.22}$} &	{\textrm -} \\
Pile-up offset $\rho$ topology (JES) [\%]	
&	$^{\textrm{ \phantom{ai}-}}_{-0.46}$ &	{$^{+2.03}_{-2.46}$} &	{$^{+2.96}_{-3.39}$} &	$^{+2.52}_{-2.81}$ &	{$^{+1.87}_{-3.12}$} &	{$^{+1.09}_{-1.99}$} \\
\rowcolor{Gray}
Punch-through (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Single particle high-$p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Jet energy resolution [\%]	
&	$\mp$3.09 &	{$\mp$1.28} &	{$\pm$0.12} &	$\pm$0.14 &	{\textrm -} &	{$\mp$1.59} \\
Jet vertex fraction [\%]	
&	$^{+3.28}_{-3.24}$ &	$^{+3.65}_{-3.58}$ &	$^{+3.85}_{-3.73}$ &	$^{+3.65}_{-3.59}$ &	$^{+3.38}_{-3.31}$ &	$^{+2.62}_{-2.54}$ \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-4.30}_{+4.38}$ &	$^{-4.09}_{+4.16}$ &	$^{-3.85}_{+3.90}$ &	$^{-3.74}_{+3.80}$ &	$^{-3.69}_{+3.74}$ &	$^{-3.62}_{+3.67}$ \\
$b$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$^{-1.62}_{+1.63}$ &	$^{-1.62}_{+1.64}$ &	$^{-1.61}_{+1.63}$ &	$^{-1.59}_{+1.60}$ &	$\mp$1.60 &	{$^{-2.38}_{+2.40}$} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 2) [\%]	
&	$^{+1.23}_{-1.22}$ &	$^{+1.13}_{-1.12}$ &	$\pm$0.95 &	$^{+0.90}_{-0.89}$ &	$\pm$0.91 &	{$\pm$0.48} \\
$b$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
$c$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-1.50}_{+1.51}$ &	$^{-1.49}_{+1.50}$ &	$\mp$1.50 &	$^{-1.48}_{+1.49}$ &	$\mp$1.41 &	$\mp$1.34 \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 1) [\%]	
&	$\pm$0.17 &	$\pm$0.14 &	$\pm$0.13 &	$\pm$0.16 &	$\pm$0.16 &	$\pm$0.13 \\
$c$-Quark tagging efficiency (eigenvector 2) [\%]	
&	$\pm$0.19 &	$\pm$0.18 &	$\pm$0.14 &	$\pm$0.15 &	$\pm$0.18 &	$\pm$0.18 \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 0) [\%]	
&	$^{-1.32}_{+1.40}$ &	$^{-1.60}_{+1.69}$ &	$^{-1.77}_{+1.83}$ &	$\mp$1.59 &	$\mp$1.48 &	$^{-1.42}_{+1.46}$ \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	$\pm$0.10 \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 5) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 6) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 7) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 8) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 9) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 10) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 11) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$b$-Quark tagging  extrapolation  [\%]	
&	$\pm$0.22 &	$\pm$0.25 &	{$^{+0.34}_{-0.33}$} &	$^{+0.42}_{-0.43}$ &	$\pm$0.38 &	{$^{+0.92}_{-0.93}$} \\
\rowcolor{Gray}
$b$-Quark tagging extrapolation from $c$-Quark [\%]	
&	$\pm$0.12 &	$\pm$0.10 &	\textrm - &	\textrm - &	\textrm - &	$\pm$0.11 \\
Electron energy resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Electron energy scale [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
Electron trigger efficiency [\%]	
&	$\pm$0.26 &	$\pm$0.25 &	$\pm$0.26 &	$\pm$0.27 &	$\pm$0.28 &	$\pm$0.30 \\
\rowcolor{Gray}
Electron reconstruction efficiency [\%]	
&	$\pm$0.18 &	$\pm$0.17 &	$\pm$0.18 &	$\pm$0.19 &	$\pm$0.20 &	$\pm$0.23 \\
Electron identification efficiency [\%]	
&	$\pm$0.43 &	$\pm$0.42 &	$\pm$0.43 &	$\pm$0.46 &	$\pm$0.49 &	$\pm$0.60 \\
\rowcolor{Gray}
Electron isolation efficiency [\%]	
&	$\pm$0.15 &	$\pm$0.15 &	$\pm$0.16 &	$\pm$0.18 &	$\pm$0.20 &	{$\pm$0.31} \\
Muon energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon (MS) momentum resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Muon (ID) momentum resolution [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon trigger efficiency stat [\%]	
&	$^{+0.56}_{-0.58}$ &	$^{+0.57}_{-0.59}$ &	$^{+0.57}_{-0.58}$ &	$^{+0.56}_{-0.58}$ &	$^{+0.56}_{-0.58}$ &	$^{+0.56}_{-0.57}$ \\
Muon trigger efficiency syst [\%]	
&	$\pm$0.24 &	$^{+0.25}_{-0.24}$ &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.24 &	$\pm$0.24 \\
\rowcolor{Gray}
Muon identification stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon identification syst [\%]	
&	$\pm$0.17 &	$\pm$0.17 &	$\pm$0.18 &	$\pm$0.18 &	$\pm$0.19 &	$\pm$0.24 \\
\rowcolor{Gray}
Muon isolation efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Muon isolation efficiency syst [\%]	
&	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$\pm$0.10 &	$^{+0.11}_{-0.10}$ \\
\rowcolor{Gray}
Muon TTVA efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon TTVA efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution para [\%]	
&	$\mp$0.12 &	{$\pm$0.23} &	$\pm$0.28 &	{$\mp$0.10} &	$\pm$0.12 &	$\pm$0.13 \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution perp [\%]	
&	$\mp$0.36 &	{$\pm$0.14} &	$\pm$0.11 &	{$\mp$0.15} &	$\mp$0.15 &	$\mp$0.12 \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Luminosity [\%]	
&	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 &	$\mp$2.06 \\
\rowcolor{Gray}
Single top cross-section [\%]	
&	$\pm$0.29 &	$\pm$0.25 &	$\pm$0.23 &	$\pm$0.24 &	$\pm$0.25 &	$\pm$0.26 \\
$Z$+jets cross-section [\%]	
&	$\pm$0.67 &	$\pm$0.54 &	$\pm$0.54 &	$\pm$0.52 &	$\pm$0.48 &	$\pm$0.56 \\
\rowcolor{Gray}
Diboson cross-section [\%]	
&	$\pm$0.11 &	$\pm$0.10 &	{$\pm$0.14} &	{$\pm$0.19} &	$\pm$0.24 &	{$\pm$0.47} \\
$t\bar{t}V$ cross-section [\%]	
&	$\mp$0.10 &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Monte Carlo sample statistics [\%]	
&	$\pm$0.22 &	$\pm$0.20 &	{$\pm$0.31} &	{$\pm$0.44} &	{$\pm$0.58} &	$\pm$0.49 \\
ISR/FSR + scale [\%]	
&	$^{-1.84}_{\textrm{ \phantom{ai}-}}$ &	{$^{-3.27}_{+3.37}$} &	$^{-2.36}_{+3.47}$ &	$^{-3.01}_{+3.59}$ &	$^{-3.50}_{+3.55}$ &	$^{-2.80}_{+2.78}$ \\
\rowcolor{Gray}
Alternate hard-scattering model [\%]	
&	$\mp$0.64 &	$\pm$0.55 &	{$\pm$0.82} &	{$\pm$3.99} &	{$\pm$2.17} &	{$\pm$1.26} \\
Alternate parton-shower model [\%]	
&	$\mp$7.92 &	{$\pm$0.59} &	{$\pm$4.22} &	{$\mp$0.66} &	{\textrm -} &	{$\mp$1.34} \\
\rowcolor{Gray}
Inter PDF [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	$\pm$0.10 &	{\textrm -} &	{$\pm$0.16} \\
Intra PDF [\%]	
&	\textrm - &	{\textrm -} &	{$\pm$0.11} &	{\textrm -} &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Real lepton efficiency stat [\%]	
&	$^{-0.15}_{+0.14}$ &	$^{-0.15}_{+0.14}$ &	$^{-0.16}_{+0.15}$ &	$^{-0.20}_{+0.18}$ &	$^{-0.21}_{+0.19}$ &	{$^{-0.36}_{+0.28}$} \\
Fake lepton efficiency MC scale [\%]	
&	$^{+0.20}_{-0.24}$ &	{$^{+0.91}_{-1.14}$} &	$^{+0.94}_{-1.22}$ &	{$^{+0.46}_{-0.58}$} &	$^{+0.46}_{-0.57}$ &	$^{+0.43}_{-0.48}$ \\
\rowcolor{Gray}
Fake lepton efficiency alternate CR [\%]	
&	$\pm$0.24 &	{$\pm$0.45} &	$\pm$0.41 &	{$\pm$0.29} &	{$\pm$0.13} &	{$\pm$0.17} \\
Fake overall normalisation [\%]	
&	$\pm$2.58 &	{$\pm$4.04} &	$\pm$3.98 &	{$\pm$2.95} &	$\pm$2.89 &	$\pm$3.25 \\
\rowcolor{Gray}
$W$+jets $CA_{4incl}$ stat error [\%]	
&	$\mp$0.13 &	{\textrm -} &	\textrm - &	{$\mp$0.10} &	$\mp$0.11 &	$\mp$0.13 \\
$W$+jets Fc stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
$W$+jets Fcc stat error [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	$^{-0.16}_{\textrm{ \phantom{ai}-}}$ &	{$^{-0.23}_{+0.11}$} &	$^{-0.28}_{+0.13}$ \\
$W$+jets Flight stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\hline
\end{tabular}}


==> tables/systematics/resolved/table_syst_particle_tt_pt_RelativeDiffXs.tex <==
\resizebox*{!}{\textheight}{
\begin{tabular}{l c c c c c c}
\hline
Bins  [GeV]
 & 0--35   & 35--75   & 75--125   & 125--170   & 170--225   & 225--800  \\
\hline
\hline
1/$\sigma$ $\cdot$ d$\sigma$ / d$p_{\textrm T}^{t\bar{t}}$	&	$1.00 \cdot 10^{-2}$ &	$7.89 \cdot 10^{-3}$ &	$3.34 \cdot 10^{-3}$ &	$1.63 \cdot 10^{-3}$ &	$8.14 \cdot 10^{-4}$ &	$8.37 \cdot 10^{-5}$ \\
\hline
\rowcolor{Gray}
Total uncertainty [\%]	
&	$^{+10.1}_{-10.4}$ &	$^{+3.94}_{-4.03}$ &	$^{+11.0}_{-10.3}$ &	$^{+7.73}_{-6.90}$ &	$^{+5.67}_{-5.94}$ &	$^{+3.78}_{-3.82}$ \\
Statistical uncertainty [\%]	
&	$\pm0.4$ &	$\pm0.4$ &	$\pm0.7$ &	$\pm1.1$ &	$\pm1.6$ &	$\pm1.4$ \\
\rowcolor{Gray}
Systematic uncertainty [\%]	
&	$^{+10.1}_{-10.4}$ &	$^{+3.91}_{-4.00}$ &	$^{+10.9}_{-10.3}$ &	$^{+7.62}_{-6.79}$ &	$^{+5.40}_{-5.68}$ &	$^{+3.43}_{-3.48}$ \\
\hline
\hline
$b$-Tagged jet energy scale (JES) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{$^{\textrm{ \phantom{ai}-}}_{-0.19}$} &	{$^{-0.19}_{+0.26}$} \\
\rowcolor{Gray}
Effective detector NP set 1 (JES) [\%]	
&	$^{-4.61}_{+4.62}$ &	{$^{+1.47}_{-1.77}$} &	{$^{+5.17}_{-4.65}$} &	{$^{+3.23}_{-2.62}$} &	{$^{+1.72}_{-1.91}$} &	{$^{+0.16}_{-0.66}$} \\
Effective detector NP set 2 (JES) [\%]	
&	$^{+0.78}_{-0.71}$ &	$^{-0.78}_{+0.77}$ &	$^{-0.86}_{+0.80}$ &	{$^{+0.14}_{-0.22}$} &	{$^{+0.42}_{-0.64}$} &	{$^{+1.83}_{-1.77}$} \\
\rowcolor{Gray}
Effective detector NP set 3 (JES) [\%]	
&	$^{-0.16}_{+0.17}$ &	{$\pm$0.37} &	{$\pm$0.21} &	{$^{-0.40}_{+0.36}$} &	$^{-0.54}_{+0.39}$ &	{$^{-0.99}_{+1.06}$} \\
Effective detector NP set 4 (JES) [\%]	
&	\textrm - &	{$^{-0.17}_{+0.20}$} &	{\textrm -} &	{$^{+0.27}_{-0.29}$} &	$^{+0.29}_{-0.33}$ &	\textrm - \\
\rowcolor{Gray}
Effective detector NP set 5 (JES) [\%]	
&	\textrm - &	{\textrm -} &	{$^{-0.11}_{+0.10}$} &	{\textrm -} &	{$^{+0.10}_{-0.22}$} &	{$^{+0.28}_{-0.21}$} \\
Effective detector NP set 6 restTerm (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{$^{+0.12}_{-0.13}$} &	{$^{+0.20}_{-0.19}$} \\
\rowcolor{Gray}
$\eta$ intercalibration model (JES) [\%]	
&	$^{-2.82}_{+2.72}$ &	{$^{+1.02}_{-1.04}$} &	{$^{+2.82}_{-2.56}$} &	{$^{+1.65}_{-1.42}$} &	{$^{+1.18}_{-1.46}$} &	{$^{+0.72}_{-0.86}$} \\
$\eta$ intercalibration total stat (JES) [\%]	
&	$^{-0.90}_{+0.99}$ &	{$^{+0.32}_{-0.35}$} &	{$^{+0.80}_{-0.94}$} &	{$^{+0.58}_{-0.44}$} &	$^{+0.63}_{-0.80}$ &	{$^{+0.34}_{-0.33}$} \\
\rowcolor{Gray}
Flavour composition (JES) [\%]	
&	$^{-5.06}_{+5.09}$ &	{$^{+1.04}_{-1.39}$} &	{$^{+5.66}_{-5.25}$} &	$^{+4.58}_{-4.07}$ &	{$^{+3.22}_{-3.10}$} &	{$^{+1.37}_{-1.48}$} \\
Flavour response (JES) [\%]	
&	$^{+1.57}_{-1.60}$ &	{$^{-0.34}_{+0.41}$} &	{$^{-1.55}_{+1.57}$} &	$^{-1.27}_{+1.37}$ &	{$^{-1.54}_{+1.00}$} &	{$^{-0.78}_{+0.70}$} \\
\rowcolor{Gray}
Pile-up offset $\mu$ (JES) [\%]	
&	$^{+0.38}_{-0.36}$ &	{$^{-0.16}_{+0.13}$} &	{$^{-0.37}_{+0.40}$} &	{$^{-0.17}_{+0.14}$} &	$^{-0.28}_{+0.17}$ &	{\textrm -} \\
Pile-up offset $N_{\textrm PV}$ (JES) [\%]	
&	$^{+0.18}_{\textrm{ \phantom{ai}-}}$ &	\textrm - &	{$^{-0.19}_{+0.14}$} &	{\textrm -} &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
Pile-up offset $p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	{$^{-0.13}_{+0.12}$} &	{\textrm -} &	{$^{+0.17}_{-0.21}$} &	{$^{+0.13}_{-0.29}$} &	{$^{+0.18}_{-0.10}$} \\
Pile-up offset $\rho$ topology (JES) [\%]	
&	$^{-1.63}_{+1.50}$ &	{$^{+0.69}_{-0.53}$} &	{$^{+1.60}_{-1.47}$} &	{$^{+1.17}_{-0.88}$} &	{$^{+0.53}_{-1.20}$} &	{$^{\textrm{ \phantom{ai}-}}_{-0.23}$} \\
\rowcolor{Gray}
Punch-through (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Single particle high-$p_{\textrm T}$ (JES) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Jet energy resolution [\%]	
&	$\mp$1.56 &	{$\pm$0.27} &	{$\pm$1.70} &	$\pm$1.72 &	$\pm$1.66 &	{\textrm -} \\
Jet vertex fraction [\%]	
&	$^{-0.20}_{+0.19}$ &	$^{+0.15}_{-0.16}$ &	{$^{+0.34}_{-0.32}$} &	{$^{+0.15}_{-0.17}$} &	{$^{-0.10}_{+0.11}$} &	{$^{-0.83}_{+0.90}$} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 0) [\%]	
&	$^{-0.25}_{+0.24}$ &	{\textrm -} &	{$^{+0.22}_{-0.21}$} &	{$^{+0.33}_{-0.32}$} &	$^{+0.38}_{-0.37}$ &	$^{+0.45}_{-0.44}$ \\
$b$-Quark tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{$^{-0.74}_{+0.71}$} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 2) [\%]	
&	$\pm$0.15 &	{\textrm -} &	{$\mp$0.12} &	{$^{-0.17}_{+0.18}$} &	$\mp$0.16 &	{$\mp$0.59} \\
$b$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
$b$-Quark tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$c$-Quark tagging efficiency (eigenvector 0) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$^{+0.14}_{-0.15}$} \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} \\
$c$-Quark tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$c$-Quark tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 0) [\%]	
&	$^{+0.19}_{-0.17}$ &	{\textrm -} &	{$^{-0.26}_{+0.24}$} &	\textrm - &	\textrm - &	{$^{\textrm{ \phantom{ai}-}}_{-0.12}$} \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 1) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Light-jet tagging efficiency (eigenvector 2) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 3) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 4) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 5) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 6) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 7) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 8) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 9) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Light-jet tagging efficiency (eigenvector 10) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Light-jet tagging efficiency (eigenvector 11) [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
$b$-Quark tagging  extrapolation  [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{$^{+0.11}_{-0.12}$} &	{\textrm -} &	{$^{+0.61}_{-0.63}$} \\
\rowcolor{Gray}
$b$-Quark tagging extrapolation from $c$-Quark [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Electron energy resolution [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Electron energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Electron trigger efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Electron reconstruction efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
Electron identification efficiency [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{$\pm$0.16} \\
\rowcolor{Gray}
Electron isolation efficiency [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{$\pm$0.14} \\
Muon energy scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon (MS) momentum resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon (ID) momentum resolution [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Muon trigger efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon trigger efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon identification stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon identification syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Muon isolation efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon isolation efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Muon TTVA efficiency stat [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
Muon TTVA efficiency syst [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution para [\%]	
&	$\mp$0.20 &	{$\pm$0.14} &	{$\pm$0.20} &	$\mp$0.18 &	{\textrm -} &	\textrm - \\
$E_{\textrm T}^{\textrm{miss}}$ Soft jet resolution perp [\%]	
&	$\mp$0.28 &	$\pm$0.23 &	$\pm$0.20 &	{\textrm -} &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
$E_{\textrm T}^{\textrm{miss}}$ Soft jet scale [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
Luminosity [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\rowcolor{Gray}
Single top cross-section [\%]	
&	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - &	\textrm - \\
$Z$+jets cross-section [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	{\textrm -} &	{$\mp$0.10} &	{\textrm -} \\
\rowcolor{Gray}
Diboson cross-section [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{$\pm$0.10} &	{$\pm$0.33} \\
$t\bar{t}V$ cross-section [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} \\
\rowcolor{Gray}
Monte Carlo sample statistics [\%]	
&	$\pm$0.18 &	$\pm$0.17 &	{$\pm$0.29} &	{$\pm$0.44} &	$\pm$0.57 &	$\pm$0.48 \\
ISR/FSR + scale [\%]	
&	$^{+0.75}_{-2.11}$ &	$^{-0.70}_{+1.13}$ &	{$^{+1.23}_{\textrm{ \phantom{ai}-}}$} &	{$^{-0.43}_{+1.35}$} &	$^{-0.94}_{+1.31}$ &	{$^{-0.22}_{+0.56}$} \\
\rowcolor{Gray}
Alternate hard-scattering model [\%]	
&	$\mp$1.14 &	{\textrm -} &	{$\pm$0.30} &	{$\pm$3.46} &	{$\pm$1.65} &	{$\pm$0.75} \\
Alternate parton-shower model [\%]	
&	$\mp$6.03 &	{$\pm$2.66} &	{$\pm$6.37} &	{$\pm$1.37} &	{$\pm$2.06} &	{$\pm$0.69} \\
\rowcolor{Gray}
Inter PDF [\%]	
&	\textrm - &	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	{\textrm -} \\
Intra PDF [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} &	{\textrm -} \\
\rowcolor{Gray}
Real lepton efficiency stat [\%]	
&	\textrm - &	{\textrm -} &	\textrm - &	\textrm - &	{\textrm -} &	{$^{-0.19}_{+0.12}$} \\
Fake lepton efficiency MC scale [\%]	
&	$^{-0.38}_{+0.50}$ &	$^{+0.31}_{-0.40}$ &	$^{+0.34}_{-0.48}$ &	{$^{-0.13}_{+0.16}$} &	$^{-0.13}_{+0.17}$ &	{$^{-0.16}_{+0.26}$} \\
\rowcolor{Gray}
Fake lepton efficiency alternate CR [\%]	
&	\textrm - &	{$\pm$0.12} &	{\textrm -} &	{\textrm -} &	{$\mp$0.19} &	$\mp$0.15 \\
Fake overall normalisation [\%]	
&	$\mp$0.75 &	$\pm$0.66 &	$\pm$0.61 &	{$\mp$0.39} &	$\mp$0.44 &	{\textrm -} \\
\rowcolor{Gray}
$W$+jets $CA_{4incl}$ stat error [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	\textrm - &	\textrm - &	\textrm - \\
$W$+jets Fc stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	{\textrm -} &	\textrm - \\
\rowcolor{Gray}
$W$+jets Fcc stat error [\%]	
&	\textrm - &	{\textrm -} &	{\textrm -} &	$^{-0.16}_{\textrm{ \phantom{ai}-}}$ &	{$^{-0.23}_{+0.11}$} &	$^{-0.28}_{+0.13}$ \\
$W$+jets Flight stat error [\%]	
&	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - &	\textrm - \\
\hline
\end{tabular}}


==> tables/systematics/systematics.tex <==





\begin{table}
  \input{tables/systematics/resolved/table_syst_particle_topH_pt_AbsoluteDiffXs}
\caption{Table of systematic uncertainties for the absolute differential cross-section at particle level for the top quark transverse momentum in the resolved regime. Note that the values shown here are obtained by propagating the individual uncertainties to the measured cross-sections, while the covariance matrices are evaluated using pseudo-experiments as described in the text.}
\label{tab:syst:topH_pt_abs}
\end{table}
\begin{table}
  \input{tables/systematics/resolved/table_syst_particle_topH_pt_RelativeDiffXs}
\caption{Table of systematic uncertainties for the relative differential cross-section at particle level for the top quark transverse momentum in the resolved regime. Note that the values shown here are obtained by propagating the individual uncertainties to the measured cross-sections, while the covariance matrices are evaluated using pseudo-experiments as described in the text.}
\label{tab:syst:topH_pt_rel}
\end{table}

\begin{table}
  \input{tables/systematics/resolved/table_syst_particle_topH_absrap_AbsoluteDiffXs}
\caption{Table of systematic uncertainties for the absolute differential cross-section at particle level for the absolute value of the top quark rapidity in the resolved regime. Note that the values shown here are obtained by propagating the individual uncertainties to the measured cross-sections, while the covariance matrices are evaluated using pseudo-experiments as described in the text.}
\label{tab:syst:topH_absrap_abs}
\end{table}
\begin{table}
  \input{tables/systematics/resolved/table_syst_particle_topH_absrap_RelativeDiffXs}
\caption{Table of systematic uncertainties for the relative differential cross-section at particle level for the absolute value of the top quark rapidity in the resolved regime. Note that the values shown here are obtained by propagating the individual uncertainties to the measured cross-sections, while the covariance matrices are evaluated using pseudo-experiments as described in the text.}
\label{tab:syst:topH_absrap_rel}
\end{table}



\begin{table}
{\tiny   \input{tables/systematics/resolved/table_syst_particle_tt_pt_AbsoluteDiffXs}}
\caption{Table of systematic uncertainties for the absolute differential cross-section at particle level for the \ttbar{} system transverse momentum in the resolved regime. Note that the values shown here are obtained by propagating the individual uncertainties to the measured cross-sections, while the covariance matrices are evaluated using pseudo-experiments as described in the text.}
\label{tab:syst:tt_pt_abs}
\end{table}
\begin{table}
{\tiny    \input{tables/systematics/resolved/table_syst_particle_tt_pt_RelativeDiffXs}}
\caption{Table of systematic uncertainties for the relative differential cross-section at particle level for the \ttbar{} system transverse momentum in the resolved regime. Note that the values shown here are obtained by propagating the individual uncertainties to the measured cross-sections, while the covariance matrices are evaluated using pseudo-experiments as described in the text.}
\label{tab:syst:tt_pt_rel}
\end{table}


\begin{table}
  \input{tables/systematics/resolved/table_syst_particle_tt_absrap_AbsoluteDiffXs}
\caption{Table of systematic uncertainties for the absolute differential cross-section at particle level for the absolute value of the \ttbar{} system rapidity in the resolved regime. Note that the values shown here are obtained by propagating the individual uncertainties to the measured cross-sections, while the covariance matrices are evaluated using pseudo-experiments as described in the text.}
\label{tab:syst:tt_absrap_abs}
\end{table}
\begin{table}
  \input{tables/systematics/resolved/table_syst_particle_tt_absrap_RelativeDiffXs}
\caption{Table of systematic uncertainties for the relative differential cross-section at particle level for the absolute value of the \ttbar{} system rapidity in the resolved regime. Note that the values shown here are obtained by propagating the individual uncertainties to the measured cross-sections, while the covariance matrices are evaluated using pseudo-experiments as described in the text.}
\label{tab:syst:tt_absrap_rel}
\end{table}


\begin{table}
  \input{tables/systematics/resolved/table_syst_particle_tt_m_AbsoluteDiffXs}
\caption{Table of systematic uncertainties for the absolute differential cross-section at particle level for the mass of the \ttbar{} system in the resolved regime. Note that the values shown here are obtained by propagating the individual uncertainties to the measured cross-sections, while the covariance matrices are evaluated using pseudo-experiments as described in the text.}
\label{tab:syst:tt_m_abs}
\end{table}
\begin{table}
  \input{tables/systematics/resolved/table_syst_particle_tt_m_RelativeDiffXs}
\caption{Table of systematic uncertainties for the relative differential cross-section at particle level for the mass of the \ttbar{} system in the resolved regime. Note that the values shown here are obtained by propagating the individual uncertainties to the measured cross-sections, while the covariance matrices are evaluated using pseudo-experiments as described in the text.}
\label{tab:syst:tt_m_rel}
\end{table}





\begin{table}
{\tiny   \input{tables/systematics/boosted/table_syst_particle_topH_pt_AbsoluteDiffXs}}
\caption{Table of systematic uncertainties for the absolute differential cross-section at particle level for the top quark transverse momentum in the boosted regime. Note that the values shown here are obtained by propagating the individual uncertainties to the measured cross-sections, while the covariance matrices are evaluated using pseudo-experiments as described in the text.}
\label{tab:syst:topH_pt_abs}
\end{table}

\begin{table}
 {\tiny  \input{tables/systematics/boosted/table_syst_particle_topH_pt_RelativeDiffXs}}
\caption{Table of systematic uncertainties for the relative differential cross-section at particle level for the top quark transverse momentum in the boosted regime. Note that the values shown here are obtained by propagating the individual uncertainties to the measured cross-sections, while the covariance matrices are evaluated using pseudo-experiments as described in the text.}
\label{tab:syst:topH_pt_rel}
\end{table}

\begin{table}
{\tiny   \input{tables/systematics/boosted/table_syst_particle_topH_absrap_AbsoluteDiffXs}}
\caption{Table of systematic uncertainties for the absolute differential cross-section at particle level for the absolute value of the top quark rapidity in the boosted regime. Note that the values shown here are obtained by propagating the individual uncertainties to the measured cross-sections, while the covariance matrices are evaluated using pseudo-experiments as described in the text.}
\label{tab:syst:topH_absrap_abs}
\end{table}

\begin{table}
{\tiny   \input{tables/systematics/boosted/table_syst_particle_topH_absrap_RelativeDiffXs}}
\caption{Table of systematic uncertainties for the relative differential cross-section at particle level for the absolute value of the top quark rapidity in the boosted regime. Note that the values shown here are obtained by propagating the individual uncertainties to the measured cross-sections, while the covariance matrices are evaluated using pseudo-experiments as described in the text.}
\label{tab:syst:topH_absy_rel}
\end{table}




==> tables/table_MC.tex <==
\begin{table*} 
\scriptsize
\centering
\begin{tabular}{|l|l|c|c|c|c|} \hline
Physics process & Event generator & Cross-section & PDF set for & Parton shower & Tune \\
& & normalisation & hard process & & \\ \hline
$\ttbar$ Nominal & \PowHegBox v2 & \NNLO{}+\NNLL & CT10 &  \Pythia 6.428 & Perugia2012 \\ 
$\ttbar$ PS syst. & \PowHegBox v2 & \NNLO{}+\NNLL & CT10 & \herwigpp v2.7.1 & UE-EE-5 \\
$\ttbar$ ME syst. & \textsc{MadGraph5}\_ & \NNLO{}+\NNLL & CT10 & \herwigpp v2.7.1 & UE-EE-5 \\
                            & a\textsc{MC@NLO} & & & & \\
$\ttbar$ rad. syst. & \PowHegBox v2 & \NNLO{}+\NNLL & CT10 &  \Pythia 6.428 & `radHi/Lo'  \\ 
Extra $\ttbar$ model & \PowHegBox v2 & \NNLO{}+\NNLL &  NNPDF3.0NLO &  \Pythia 8.210 & A14 \\ 
Extra $\ttbar$ model & \PowHegBox v2 & \NNLO{}+\NNLL &  NNPDF3.0NLO &  \Herwig v7.0.1 & H7-UE-MMHT \\
Extra $\ttbar$ model &  \textsc{MadGraph5}\_  & \NNLO{}+\NNLL &  NNPDF3.0NLO &  \Pythia 8.210 & A14 \\  
                            & a\textsc{MC@NLO} & & & & \\

Single top  $t$-channel &\PowHegBox v1 & \NLO{} & CT10f4 &  \Pythia 6.428 & Perugia2012 \\ 
Single top  $s$-channel & \PowHegBox v2 & \NLO{} & CT10 &  \Pythia 6.428 & Perugia2012 \\ 
Single top $Wt$-channel & \PowHegBox v2 & \NLO{}+\NNLL & CT10 &  \Pythia 6.428 & Perugia2012 \\ 
$\ttbar$+$W/Z/WW$ &  \textsc{MadGraph5}\_ & \NLO{} & NNPDF2.3LO & \Pythia 8.186 & A14 \\ 
                            & a\textsc{MC@NLO} & & & & \\
$W(\to \ell \nu) $+ jets & \Sherpa v2.1.1 & \NNLO{} & CT10 & \Sherpa & \Sherpa  \\ 
$Z(\to \ell {\bar \ell}) $+ jets & \Sherpa v2.1.1 & \NNLO{} & CT10 & \Sherpa & \Sherpa  \\ 
$WW, WZ, ZZ$ & \Sherpa v2.1.1 & \NLO{} & CT10 & \Sherpa & \Sherpa  \\ \hline
\end{tabular}
\caption{Summary of MC samples, showing the event generator for the hard-scattering process, cross-section normalisation precision, PDF choice as well as the parton shower and the corresponding tune used in the analysis. The \PythiaSix{} and \herwigpp{} parton-shower models use the CTEQ6L1 PDF set, while \PythiaEight{} uses the NNPDF2.3LO PDF set and \HerwigSeven{} uses the MMHT2014lo68cl PDF set.}
\label{tab:MC}
\end{table*}



==> tables/table_chi2_particle_abs.tex <==

\footnotesize
\centering
\noindent\makebox[\textwidth]{
\begin{tabular}{|c | r @{/} l c  | r @{/} l c  | r @{/} l c  | r @{/} l c  | r @{/} l c  | r @{/} l c |}
\hline
Variable  & \multicolumn{3}{|c|}{\textsf{PWG+PY6}}  & \multicolumn{3}{|c|}{\textsf{PWG+PY6}(radHi)} & \multicolumn{3}{|c|}{\textsf{PWG+PY6}(radLo)} & \multicolumn{3}{|c|}{\textsf{PWG+PY8}} & \multicolumn{3}{|c|}{\textsf{PWG+HW++}} & \multicolumn{3}{|c|}{\textsf{\mgamcatnlo}}  \\
& \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-value  & \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-value  & \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-value  & \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-value  & \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-value  & \multicolumn{2}{|c}{$\chi^{2}$/NDF} &  ~$p$-value  \\
\hline
\hline
 \ptthad{} &
 {\ } 8.8 & 15 & 0.89  & {\ } 8.7 & 15 & 0.89  &  {\ } 11.0 & 15 & 0.75  &  {\ } 8.6 & 15 & 0.90  &  {\ } 26.7 & 15 & 0.03  &  {\ } 13.5 & 15 & 0.56  
\\
\absythad &  {\ } 9.2 & 18 & 0.95 &
{\ } 10.0 & 18 & 0.93  &  {\ } 8.7 & 18 & 0.97  &  {\ } 11.8 & 18 & 0.86  &  {\ } 9.2 & 18 & 0.95  &  {\ } 12.9 & 18 & 0.80    \\
\mttbar{}  & {\ } 8.6 & 11 & 0.66 &
{\ } 8.2 & 11 & 0.70  &  {\ } 9.6 & 11 & 0.57  &  {\ } 7.6 & 11 & 0.75  &  {\ } 47.1 & 11 & $<$0.01  &  {\ } 21.6 & 11 & 0.03     \\
\ptttbar{} &  {\ } 7.8 & 6 & 0.25 &
{\ } 6.2 & 6 & 0.40  &  {\ } 6.5 & 6 & 0.37  &  {\ } 3.9 & 6 & 0.69  &  {\ } 17.0 & 6 & $<$0.01  &  {\ } 2.0 & 6 & 0.92    \\
 \absyttbar{} & {\ } 21.4 & 18 & 0.26 &
{\ } 19.4 & 18 & 0.37  &  {\ } 27.2 & 18 & 0.07  &  {\ } 15.6 & 18 & 0.62  &  {\ } 30.6 & 18 & 0.03  &  {\ } 27.3 & 18 & 0.07    \\
\hline
\end{tabular}}



==> tables/table_fiducial_xsections.tex <==
\begin{table}[!h]
  \centering
\begin{tabular}{l|ll}
  \hline\hline


Sample  &  \multicolumn{2}{l}{Fiducial cross-section $[\textrm{pb}]$} \\ \hline
          &   Resolved           & Boosted \\ \hline
\Powheg{}+\PythiaSix{}  &  92.0       &  2.96    \\ 
\Powheg{}+\Pythia{} radHi  &  90.9       &    3.10  \\ 
\Powheg{}+\Pythia{} radLo  &  94.2       &     2.89 \\ 
\aMCatNLO{}+\Herwig{}++  &  94.9       &      3.19 \\ 
\Powheg{}+\Herwig{}++  &  93.5       &   2.84   \\ 
\Powheg{}+\PythiaEight{}  & 97.5   & 3.07 \\
\Powheg{}+\HerwigSeven{} & 97.2 & 2.84 \\
\aMCatNLO{}+\PythiaEight{} & 98.5 & 2.88 
\\ \hline
Data & $110 {}^{+13}_{-14} $ (stat+syst)   &  $2.54 \pm 0.54$ (stat+syst)   \\ \hline\hline

\end{tabular}
\caption{Fiducial cross-sections in the resolved and boosted topologies for data and different models. Each model's cross-section is scaled to the NNLO+NNLL value from Refs.~\cite{Cacciari:2011hy,Beneke:2011mq,Baernreuther:2012ws,Czakon:2012zr,Czakon:2012pz,Czakon:2013goa}, hence the quoted fiducial cross-sections result from different kinematic regions and thus acceptance from each model.}
\label{tab:fid_xsects}
\end{table}



==> tables/table_fiducial_xsections_boosted.tex <==
\begin{table}[!h]
\begin{tabular}{l|lr}
\hline\hline
Powheg+Pythia6           & 2.959 & \\
aMC@NLO+Herwig++  & 3.185 & \\
Powheg+Herwig++      & 2.838 & \\
Powheg+Pythia8           & 3.010 & \\
Powheg+Pythia6 radHi & 3.102 & \\
Powheg+Pythia6 radLo & 2.889 & \\ \hline
Data & $2.62\,\textrm{pb}$ &  $\pm 18\%$ (stat+syst) \\ \hline\hline
\end{tabular}
\caption{Fiducial cross sections in the boosted regime for different models and in data extracted from the single bin contructed from the hadronic top quark $\pt$. Each model is scaled to the NNLO+NNLL inclusive cross section~\cite{Cacciari:2011hy,Beneke:2011mq,Baernreuther:2012ws,Czakon:2012zr,Czakon:2012pz,Czakon:2013goa} and the quoted fiducial cross-sections result from different kinematics and thus acceptance from each model.}
\label{tab:fid_xsects_boosted}
\end{table}


==> tables/table_fiducial_xsections_resolved.tex <==
\begin{table}[!h]
\begin{tabular}{l|l}
\hline\hline
Sample  &  cross-section  pb \\ 
\Powheg{}+\Pythia{}  &  91.95  pb \\ 
\Powheg{}+\Pythia{} radHi  &  90.85  pb \\ 
\Powheg{}+\Pythia{} radLo  &  94.22  pb \\ 
\aMCatNLO{}+\Herwig{}++  &  94.86  pb \\ 
\Powheg{}+\Herwig{}++  &  93.48  pb \\ 
\Powheg{}+\Pythia{}8  &  96.37  pb \\ \hline
Data & $105\,\textrm{pb} {}^{+12\%}_{-13\%} $ (stat+syst) \\ \hline\hline
\end{tabular}
\caption{Fiducial cross sections in the resolved regime for different models and in data extracted from the single bin contructed from the hadronic top quark $\pt$. Each model is scaled to the NNLO+NNLL inclusive cross section~\cite{Cacciari:2011hy,Beneke:2011mq,Baernreuther:2012ws,Czakon:2012zr,Czakon:2012pz,Czakon:2013goa} and the quoted fiducial cross-sections result from different kinematics and thus acceptance from each model.}
\label{tab:fid_xsects_resolved}
\end{table}


==> tables/table_selections.tex <==
\resizebox{\textwidth}{!}{
 \begin{tabular}{|l|c|c|l|}
  \hline
  Level & \multicolumn{2}{c|}{Detector} & Particle \\
  \hline
   Topology         & Resolved & Boosted & \\
  \hline\hline
  Leptons &  \multicolumn{2}{c|}{\parbox[c][3em][c]{8.5cm}{ $|d_0|/\sigma(d_0)<5$ and $|z_0 \sin\theta | <$ 0.5 mm \\ Track and calorimeter isolation\\ 
 $|\eta|<1.37$ or $1.52<|\eta|<2.47$ {($e$)},  $|\eta|<2.5$ {($\mu$)} \\ $E_{\mathrm{T}} $ {($e$)}, $p_{\mathrm{T}}$ {($\mu$)} $>$ 25 \GeV{} }}  & \parbox[c][7em][c]{2.0cm}{ $|\eta|<2.5$\\ \mbox{$p_{\mathrm T} >$ 25~\GeV{}}  } \\
  \hline
  Small-$R$ jets &
  \multicolumn{2}{c|}{\parbox[c][4em][c]{8.5cm}{  $|\eta|<2.5$ \\$p_{\mathrm{T}} > $ 25~\GeV{}   \\ JVT cut (if $p_{\mathrm{T}}<$ 60~\GeV{} and $|\eta| < 2.4$)}} & \parbox[c][4em][c]{2.0cm}{$|\eta|<2.5$\\ \mbox{$p_{\mathrm T} >$ 25~\GeV{}}}\\ \hline
Num. of  small-$R$ jets &  $\geq 4$ jets &  $\geq 1$ jet & Same as detector level
\\   \hline
\parbox[l][2.5em][c]{2cm}{  \met, \mtw} & & \met $>$ 20~\GeV{}, $\met+\mtw >$ 60~\GeV{} & Same as detector level  \\
  \hline
  Leptonic top  &  \parbox[c][6em][c]{3.5cm}{ Kinematic top-quark \\ reconstruction \\ for detector \\ and particle level} & \parbox[c][4em][c]{7.5cm}{ At least one small-$R$ jet \\with $\Delta R$($\ell$, small-$R$ jet) $< 2.0$ }& \\ 
  \hline
  Hadronic top &  \parbox[c][6em][c]{3.5cm}{ Kinematic top-quark \\ reconstruction \\ for detector \\ and particle level} &
 \parbox[c][4em][c]{7.0cm}{ The
      leading-$p_{\mathrm T}$ trimmed large-$R$ jet has: \\  $|\eta|<2.0$, \\ 300~\GeV{} $< p_{\mathrm{T}}<$ 1500~\GeV{}, $m > 50$~\GeV{}, \\Top-tagging at 80\% efficiency \\ $\Delta R$(large-$R$ jet, small-$R$ jet associated with lepton) $>1.5$, \\ $\Delta \phi$($\ell$, large-$R$ jet) $ > 1.0$}
      &  \parbox[c][8.5em][c]{3.7cm}{  {\textbf{Boosted:}} \\ $|\eta|<2.0$\\ 300 $< p_{\mathrm{T}}<$ 1500~\GeV{} \\ Top-tagging:\\  $m>$ 100~\GeV{}, \\ $\tau_{32} <$ 0.75} \\
  \hline
  $b$-tagging & At least 2 $b$-tagged jets & 
   \parbox[c][4em][c]{7.5cm}{At least
      one of: \\1) the leading-$p_{\mathrm T}$ small-$R$ jet with \\ $\Delta R$($\ell$, small-$R$ jet) $ < 2.0$ is $b$-tagged \\  2) at least one small-$R$ jet with \\ $\Delta R$(large-$R$ jet, small-$R$ jet) $ < 1.0$ is $b$-tagged 
     } 
     &\parbox[c][7em][c]{3.2cm}{ Ghost-matched \\ $b$-hadron}\\
  \hline
  \end{tabular}
}


==> tables/table_xsecvalues.tex <==
\begin{table}[t]
\centering
\begin{tabular}{r|r}
\hline 
\hline
 \multicolumn{1}{l|}{Resolved} &  \multicolumn{1}{l}{$\sigma$ in resolved}       \\
 \multicolumn{1}{l|}{particle-level \ptthad{} [\GeV{}]} & \multicolumn{1}{l}{fiducial phase-space [pb]}      \\
\hline
  0--25  &	$3.37 \pm 0.07 \pm 0.44$ \\
  25--50  &	$9.77 \pm 0.11 \pm 1.22$ \\
  50--75  &	$14.51 \pm 0.14 \pm 1.73$ \\
  75--105  &	$19.26 \pm 0.15 \pm 2.17$ \\
  105--135  &	$17.21 \pm 0.15 \pm 1.88$ \\
  135--165  &	$12.34 \pm 0.12 \pm 1.28$ \\
  165--195  &	$8.40 \pm 0.10 \pm 0.81$ \\
  195--230  &	$6.42 \pm 0.09 \pm 0.65$ \\
  230--265  &	$3.95 \pm 0.07 \pm 0.37$ \\
  265--300  &	$2.69 \pm 0.06 \pm 0.28$ \\
  300--350  &	$2.04 \pm 0.05 \pm 0.21$ \\
  350--400  &	$1.11 \pm 0.04 \pm 0.13$ \\
  400--450  &	$0.55 \pm 0.03 \pm 0.07$ \\
  450--500  &	$0.26 \pm 0.02 \pm 0.06$ \\
  500--1000  &	$0.36 \pm 0.03 \pm 0.07$ \\
\hline
\multicolumn{1}{l|}{Boosted} & \multicolumn{1}{l}{$\sigma$ in boosted}       \\
 \multicolumn{1}{l|}{particle-level \ptthad{} [\GeV{}]} & \multicolumn{1}{l}{fiducial phase-space [pb]}      \\
\hline
  300--350  &	$0.95 \pm 0.02 \pm 0.19$ \\
  350--400  &	$0.61 \pm 0.02 \pm 0.12$ \\
  400--450  &	$0.35 \pm 0.02 \pm 0.07$ \\
  450--500  &	$0.20 \pm 0.01 \pm 0.05$ \\
  500--550  &	$0.14 \pm 0.01 \pm 0.04$ \\
  550--650  &	$0.17 \pm 0.01 \pm 0.05$ \\
  650--750  &	$0.042 \pm 0.009 \pm 0.016$ \\
  750--1500  &	$0.043 \pm 0.010 \pm 0.023$ \\
\hline
\hline
\end{tabular}
\caption{Unfolded fiducial phase-space differential cross-section values in bins of hadronic top-quark transverse momentum for the resolved (top) and boosted (bottom) topologies. The first uncertainty is statistical and the second one is systematic. }
\label{Tab:XsecValues}
\end{table}



==> tables/table_yields.tex <==
\begin{table}[!ht]
\centering
\begin{tabular}{				l
                S[separate-uncertainty=true,table-figures-uncertainty=1]
                S[separate-uncertainty=true,table-figures-uncertainty=1]
                S
}
                
 \hline \hline Sample & Yield  \\ \hline
\input{tables/Yields_el}\hline
\end{tabular}

\begin{tabular}{ll}
 \hline \hline Sample & Yield  \\ \hline
\input{tables/Yields_mu}\hline
\end{tabular}
\begin{tabular}{ll}
 \hline \hline Sample & Yield  \\ \hline
\input{tables/Yields_co}\hline
\end{tabular}

\caption{Observed and expected number of events in the individual \ejets{} (top left), \mujets{} (top right) as well as the combined $e$ and $\mu$+jets channel (bottom) after the full event selection. The systematic uncertainties do not include the signal modelling ones.}

\label{Tab:EventYield}
\end{table}


==> tables/table_yields_boosted.tex <==

\begin{table}[t]
\centering
\input{tables/EventYield_boosted}
\caption{Event yields 

after the boosted selection. The signal model, denoted $t\bar{t}$ in the table, is generated using \PowHeg{}+\Pythia{}, normalised to NNLO calculations.  The systematic uncertainties include the combined statistical and systematic uncertainties, excluding the systematic uncertainties related to the modelling of the \ttbar{} system, as described in Section~\ref{sec:Uncertainties}.}
\label{Tab:EventYieldBoosted}
\end{table}


